Resource Sharing in the Edge: A Distributed Bargaining-Theoretic Approach

The growing demand for edge computing resources, particularly due to increasing popularity of Internet of Things (IoT), and distributed machine/deep learning applications poses a significant challenge. On the one hand, certain edge service providers (ESPs) may not have sufficient resources to satisfy their applications according to the associated service-level agreements. On the other hand, some ESPs may have additional unused resources. In this paper, we propose a resource-sharing framework that allows different ESPs to optimally utilize their resources and improve the satisfaction level of applications subject to constraints such as communication cost for sharing resources across ESPs. Our framework considers that different ESPs have their own objectives for utilizing their resources, thus resulting in a multi-objective optimization problem. We present an $N$-person \emph{Nash Bargaining Solution} (NBS) for resource allocation and sharing among ESPs with \emph{Pareto} optimality guarantee. Furthermore, we propose a \emph{distributed}, primal-dual algorithm to obtain the NBS by proving that the strong-duality property holds for the resultant resource sharing optimization problem. Using synthetic and real-world data traces, we show numerically that the proposed NBS based framework not only enhances the ability to satisfy applications' resource demands, but also improves utilities of different ESPs.

==> 02-sysmodel.tex <==
Any entity or service provider  that has specific resources such as CPU, storage and communication links can serve as the building block of our system as shown in Figure~\ref{fig:system_model}. We call this basic building block  a \emph{domain}\footnote{Throughout the paper, we will use domain, service provider and player interchangeably.}. The domain can be as small as a sensor and as large as data centers.  Each domain has a \emph{domain controller} that is aware of all resources available within the domain. The domain controller only shares an abstraction of this resource information and does not share the entire information\footnote{This can be due to a number of reasons including security and privacy. For example, Amazon and Dropbox may share limited information to satisfy their user's needs. However, they will not provide the entire information to each other.}. Different domains share resources with  the presence of a \emph{coalition controller}. The coalition controller can be either a separate controller or chosen among  the domain controllers. %Figure \ref{fig:system_model} the model used in this paper.   
Table \ref{tab:notationTable} provides  notation used in this paper. Below, we model our resource allocation and sharing problem from a  game theoretic perspective.   
 \begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{figures/domain}
	\caption{Our system model with domain and coalition controllers}
	\protect\label{fig:system_model}
	\vspace{-0.1in}
\end{figure}

\begin{table}[]
	\caption{List of notations (Not.) used in the paper}
	\begin{tabular}{|p{0.44cm}|p{2.7cm}||p{0.44cm}|p{3.2cm}|}
		\hline
		\textbf{NOT.} & \textbf{Description} & \textbf{NOT.} & \textbf{Description} \\ \hline
	$\mathcal{N}$	& Set of game players                     &        $n$           &Player from set   $\mathcal{N}$  \\ \hline
	$\mathcal{M}$	& Set of applications                     &      $\mathcal{M}_n$             & Set of native applications of player $n$                     \\ \hline
	$\mathcal{K}$	& Set of resource types                     &     $k$              &  Resource from set $\mathcal{K}$                    \\ \hline
	$C^{(n)}$	&  Capacity of player $n$                    &    $C_k^{(n)}$	&  Capacity of $k^{th}$ resource at player $n$           \\ \hline
	$x_{ik}^{(n)}$	&  Resource $k$ allocated to application $i$ by player $n$      &   $r_{ik}^{(n)}$      &     Request for  resource $k$ from application $i$ of player $n$                 \\ \hline
%		&                      &                   &                      \\ \hline
%		&                      &                   &                      \\ \hline
	\end{tabular}
\label{tab:notationTable}
%\vspace{-0.2in}
\end{table}

Let $\mathcal{N}=\{1,2, \cdots, N\}$ be the set of all domains (or service providers) that act as players in our game. We assume that each player has a set of $\mathcal{K}=\{1,2,\cdots, K\}$ different types of resources such as communication, computation and storage resources.  The $n$-th domain reports its available resources $C^n = \{ C_1^{(n)},\cdots, C_K^{(n)}\}$ to a central entity, the coalition controller. Here $C_k^{(n)}$ is the amount of type $k$ resources available to domain $n$.  
%All edge clouds can report their available resources  to any central entity, coalition controller \footnote{Coalition controller can be chosen from the edge clouds.},  where ${C}^{(n)}=\{ {C}_{1}^{(n)}, \cdots, {C}_{K}^{(n)}\}$ represents the available resources $k \in \mathcal{K}$ for the player $n \in \mathcal{N}$. 
Vector $C=\{\sum_{n \in \mathcal{N}}C_{1}^{(n)}, \sum_{n \in \mathcal{N}}C_{2}^{(n)}, \cdots ,\sum_{n \in \mathcal{N}}C_{K}^{(n)}\}$ represents  all available resources in different domains.  Each domain $n$ has a set of  native applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$ that ask for resources. Furthermore, the set of all applications that ask for resources from the set of domains (coalition of domains) is given by $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where $|\mathcal{M}|=M$,  and $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset, \; \forall i \neq j,$ i.e., each application originally asks only  one domain for resources. 
%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
The coalition controller receives a request (requirement) matrix $R^{(n)}$ from every player (domain) $n \in \mathcal{N}$.% \vspace{-0.1in}
\begin{equation}
\label{eq:R_Req}
R^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{r^{(n)}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{(n)}_{{M}_n}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r^{(n)}_{11} & \cdots  &\cdots   & r^{(n)}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{(n)}_{M_{n}1}&\cdots  &\cdots   & r^{(n)}_{{M}_n{K}}
\end{smallmatrix}\Biggr].
\end{equation}
%\vspace{-0.01in}
\noindent where the $i^{th}$ row corresponds to the $i^{th}$ application while  columns represent different resources, i.e., $r_{ij}^{(n)}$ is the amount of $j^{th}$ resource that application $i \in \mathcal{M}_n$ requests.
%The vector ${C}^{(n)}$ received by coalition controller shows different available resources at edge cloud $n$. 
The coalition request matrix $R$ is a combination of all the request matrices (from all the domains)  as given below. 
\begin{equation}
\label{eq:R_Reqco}
R^{}=\Biggl[\begin{smallmatrix}
\mathbf{r^{}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{}_{{M}}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r^{}_{11} & \cdots  &\cdots   & r^{}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{}_{M1}&\cdots  &\cdots   & r^{}_{{M}{K}}
\end{smallmatrix}\Biggr].
\end{equation}
\noindent where $r_{ij}$ is the amount of $j^{th}$ resource that application $i \in \mathcal{M}$ requests.
The coalition, based on $R$ and  $C$, has to make an allocation decision $\mathcal{X}$ that optimizes the utilities of all the domains  $n \in \mathcal{N}$.  The allocation decision for the entire coalition $\mathcal{X}$ consists of all the  allocation decisions $X^{(n)}$ in every domain $n \in \mathcal{N}$ i.e.,  $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$.  
%The allocation decision $\mathcal{X}$ is  given by $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$ indicating how much of each resource $k \in \mathcal{K}$ is allocated to application $i$ at domain $n \in \mathcal{N}$. The matrix $X^{(n)}$ is a combination of different matrices $\{X_{i\in \mathcal{M}_1}^{(n)}, \cdots,X_{i\in \mathcal{M}_n}^{(n)},\cdots, X_{i\in \mathcal{M}_N}^{(n)} \}$, where $X_{i\in \mathcal{M}_n}^{(n)}$ is the allocation decision  at domain $n$ for the applications $i$ originally belonging to domain $n \in \mathcal{N}$ i.e., the original applications of the domain $n$. Furthermore,  $X_{i\in \mathcal{M}_j}^{(n)}$, $\forall j \in \mathcal{N},$ where $j \neq n$, is the allocation decision at domain $n$ for applications $i$ belonging to domain $j$.  
Mathematically,  $X^{(n)}$ is represented by % \eqref{eq:A_n}, where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$.  %Table \ref{tab:notationTable} provides some of the notations used in the paper. 
\begin{equation}
\label{eq:A_n}
X^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{{M}}}^{(n)}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{{M}}1}^{(n)}&\cdots  &\cdots   & x_{{{M}}{K}}^{(n)}
\end{smallmatrix}\Biggr].
\end{equation}
where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$.
% \subsection{Assumptions}



\begin{comment}
Let $\mathcal{N}=\{1,2, \cdots, N\}$ be the set of all the domains that act as players in our game. % For simplicity, we drop the $P$ in $P_n$ and represent the players only with the subscript $n$. 
Each player has a utility function $u_n(\mathcal{X})$ that depends on the allocation decision $X$ (details for $X$ will be given later). We assume that each player has set of $\mathcal{K}=\{1,2,\cdots, K\}$ different resources such as communication, computation and storage resources. %Each player $n \in \mathcal{N}$ has complete information about its own resources $k \in \mathcal{K}$, however it reports only abstract information to a coalition controller 
All domains report their available resources  to the coalition controller where $C^{(n)}$ represent the available resources for the domain/player $n \in \mathcal{N}$. Each domain $n$ has a set of users or applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$ that ask for resources. Also $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset \; \forall i \neq j$ represents the set of all users that ask for resources from the coalition. 

%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
The coalition controller receives a matrix $R^{(n)}$ for every player $n \in \mathcal{N}$ 
	\begin{equation}
\label{eq:R_Req}
R^{(n)}=\Biggl(\begin{smallmatrix}
\mathbf{r^{(n)}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{(n)}_{{M}_n}}
\end{smallmatrix}\Biggr) = \Biggl(\begin{smallmatrix}
r^{(n)}_{11} & \cdots  &\cdots   & r^{(n)}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{(n)}_{M_{n}1}&\cdots  &\cdots   & r^{(n)}_{{M}_n{K}}
\end{smallmatrix}\Biggr)
\end{equation}
where the $i^{th}$ row corresponds to the $i^{th}$ user while  the columns represent different resources i.e., $r_{ij}$ is the amount of $j^{th}$ resource user $i \in \mathcal{M}$ requests.

The vector ${C}^{(n)}=\{ {C}_{1}^{(n)}, \cdots, {C}_{K}^{(n)}\}$ received by coalition controller shows different available resources at domain $n$. 
The vector $C=\{\sum_{n \in \mathcal{N}}C_{1}^{(n)}, \sum_{n \in \mathcal{N}}C_{2}^{(n)}, \cdots ,\sum_{n \in \mathcal{N}}C_{K}^{(n)}\}$ consists of all the available resources at different domains. The coalition, based on $R$ and  $C$, has to make an allocation decision $\mathcal{X}$ that optimizes the utilities $u_n(\mathcal{X})$ of the domains.  The allocation decision $\mathcal{X}$ is  a vector $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$ that shows how much of each resource $k$ is allocated to user $i$ at domains $n \in \mathcal{N}$.

\begin{equation}
\label{eq:A_n}
X^{(n)}=\Biggl(\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{|\mathcal{M}|}}^{(n)}}
\end{smallmatrix}\Biggr) = \Biggl(\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{|\mathcal{M}|}1}^{(n)}&\cdots  &\cdots   & x_{{|\mathcal{M}|}{K}}^{(n)}
\end{smallmatrix}\Biggr)
\end{equation}
where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ allocated  to user $i$ at player $n$

 Since the utilities of different domains might be different (can be conflicting as well), this leads us to a multi-objective optimization (MOO) problem. Some of the assumptions in our model are given below
\subsection{Assumptions}
The assumptions made in our model are 
\begin{enumerate}
	\item The negotiation cost among different domains is negligible
	\item All the domains communicate their information to the coalition controller
	\item The coalition controller already exists% and do not discuss the selection of the coalition controller (can be explored in the future work)
	\item Resources across different domains are additive in nature i.e., if domain $X$ and $Y$ have $2$ GB RAM each, the coalition would have $4$ GB of RAM. 
	\item Each player has a single objective
	\item The objective of the coalition is a sum of the utilities of all the players with equal weight
%	\item Any new player/domain added into the coalition will have resources available
	\item All players or domains have the same number of users or jobs
\end{enumerate}
\end{comment}








==> 03-opt-problem.tex <==
%In this section, we first present the resource allocation problem for a single domain (no resource sharing with other domains). Then we present MOO resource sharing and allocation problem for the coalition. 
For a single domain $n \in \mathcal{N}$ (not  part of a coalition), the allocation decision matrix $X_{SO}^{(n)}$, where $SO$ stands for single objective,  is given by 

\begin{equation}
\label{eq:X_n}
X_{SO}^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{{M}_n}}^{(n)}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{{M}_n}1}^{(n)}&\cdots  &\cdots   & x_{{{M}_n}{K}}^{(n)}
\end{smallmatrix}\Biggr].
\end{equation}
%where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$. 



The optimization problem is: %given in Equation~\eqref{eq:opt_single}
\begin{subequations}\label{eq:opt_single}
	\begin{align}
	\max_{{X}_{SO}^{(n)}}\quad& u_n({X}_{SO}^{(n)}) \label{eq:objsingle}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall i \in \mathcal{M}_n, \label{eq:singlefirst} \displaybreak[0]\\
	& x_{ik}^{(n)} \leq r^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecond} \displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}. \label{eq:singlethird} \displaybreak[2]
	\end{align}
\end{subequations}
The goal of this single objective optimization problem is for every domain  to  maximize its utility by allocating available resources only to its own applications. %The first constraint \eqref{eq:singlefirst} indicates that the allocated resources to all the users $i \in \mathcal{M}_n$ cannot be more than the capacity. The second constraint \eqref{eq:singlesecond} indicates that the allocated resources cannot be more than the required resources, while the final constraint \eqref{eq:singlethird} indicates that the allocation cannot be negative.  
\par Next, we present the resource allocation problem for different domains that share their resources with each other. In the resource sharing case,  each domain aims to  maximize sum of utilities obtained by a) allocating resources to its native applications i.e., $u_n({X}_{i \in \mathcal{M}_n}^{(n)})$ where ${X}_{i \in \mathcal{M}_n}^{(n)}$ represents the allocation decision at domain $n$ for applications $i \in \mathcal{M}_n$, and b) allocating resources to  applications of other domains i.e.,  $u_j^n({X}_{i \in \mathcal{M}_j}^{(n)}),\; \forall j\in \mathcal{N}\backslash n$, where ${X}_{i \in \mathcal{M}_j}^{(n)}$ represents the allocation of resources to applications $i \in \mathcal{M}_j, \; \forall j \in \mathcal{N}\backslash n$  at domain $n$. This leads to: 
% in Equation~\eqref{eq:opt_higher}.  
\begin{subequations}\label{eq:opt_higher}
	\begin{align}
	\max_{\mathcal{X}}\quad&  \bigg(u_n({X}_{i \in \mathcal{M}_n}^{(n)})+ \sum_{j \in \mathcal{N}\backslash n}  u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})\bigg) \quad \forall n \in \mathcal{N} \label{eq:obj}\\%\{u_1(\mathcal{A}),u_2(\mathcal{A}),\cdots,u_N(\mathcal{A})\} \label{eq:obj}\\%U(A)\label{eq:obj}\\
	\text{s.t.}\quad & \sum_{i \in \mathcal{M}} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall n \in \mathcal{N},  \label{eq:obj1} \displaybreak[0]\\
	& \sum_{n \in \mathcal{N}}x_{ik}^{(n)} \leq r^{}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K},  \label{eq:obj2}\displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}. \label{eq:obj3} \displaybreak[2]
	\end{align}
\end{subequations}
%\begin{itemize}
% so that each enclaves first facilitates its own users and then assign the remaining resource to the users of other enclaves. $w_n +w'_{n}=1$  where $w_n > w'_{n}$. E.g., $w_n=0.8$ and $w'_{n}=0.2$ would mean that each enclave has an incentive to first satisfy its own users (higher utility) and then share the excess resources for other users $j \in \mathcal{N}\backslash n $
%	\item 
The first constraint in both optimization problems, \eqref{eq:opt_single}  and \eqref{eq:opt_higher}, indicates that the allocated resources cannot be more than the capacity. The second constraint  in \eqref{eq:singlesecond} and \eqref{eq:obj2} indicates, that the allocated resources should not be more than the required resources.  The last constraint, \eqref{eq:singlethird} and \eqref{eq:obj3},  indicates that allocation decision cannot be negative. 

The utility $u_n({X}_{i \in \mathcal{M}_n}^{(n)})$ given in \eqref{eq:obj}, that each player receives, is a payment that all users $i \in \mathcal{M}_n$  who use the resources pay the player. %Users of other domains $j \in \mathcal{N}\backslash n $ that use resources of domain $n$  will be charged at a rate that player $j$ would have charged the user $i \in \mathcal{M}_j$, had the request been fulfilled by player $j$. Hence, 
 $u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})$ is the utility that domain $n$ receives for sharing its resources with domain $j$. %There are different ways to capture this profit. However, for now, we can say that it would be equivalent to whatever domain $j$ would have earned had it satisfied the requests itself (however it can't as it does not have resources, so it borrows resources from domain $n$ and assigns all the profit it gains from the users to player $n$). 
 %We also assume that th
%\vspace{-0.02in}
\subsection{Assumptions}\label{sec:assumption}
 In our model, we assume that  utilities are  concave injective functions  for which the inverse of first derivative exists, such as $(1-e^{-x})$. While our centralized NBS framework requires only concave injective utility function, the existence of first derivative's inverse is required for the distributed NBS (details in Section \ref{sec:nbs}).  
 We also assume that  resources required by different applications are more than the capacity of domains. Hence, all resources are fully utilized at the optimal solution.   The single objective optimization problem in \eqref{eq:opt_single} is feasible for all the players $n \in \mathcal{N}$. Furthermore, we assume that  there exists solutions that are better than the disagreement point for all the players. 
% that retain the concavity and $1-1$ property after taking the first derivative as well. 
%	\item  $w_n$ is the weight assigned to the utility of player $n$. $\zeta_n$ is the weight assigned to the utility $u^{n}_j(\mathcal{X})$. 
%\end{itemize}
%The optimization problem in Equation~\eqref{eq:opt_higher} is a modified scalarized MOO problem \cite{cho2017survey}. 
\begin{comment}
Before we get into the details of solving the problem, we present an example to understand this
\begin{example}
Let's say we have two different data centers owned by service provider $A$ and $B$ respectively ($A$ and $B$ are game players). Resources available at domain $A$ and $B$ are represented by  $C^{A}$ and $C^{B}$ respectively.  Users in sets $\mathcal{M}_{A}$ and $\mathcal{M}_{B}$ ask for resources and pay a certain price (profit for data centers)  $u_A(\mathcal{X})$ and $u_B(\mathcal{X})$. However, let's say $A$ has scarce resources while $B$ has excess resources. So by forming a coalition, users in $\mathcal{M}_s \subset\mathcal{M}_{A}$ that can't be satisfied by $A$ will be provided resources by $B$ without the users realizing who are providing the resources (since the coalition will make everything appear as one to the user). The profit that $B$ will earn for providing its resources will be equivalent to the profit $A$ would have earned (as $A$ has agreed upon a certain contract with its users $\mathcal{M}_{A}$) had it satisfied the user's request itself. So for $B$, it will earn utility $u_B(X)$ for satisfying its own users plus $u_A^B(X^{\mathcal{M}_s})$ (slight abuse of notation where $X^{\mathcal{M}_s}$ represents the allocation decision for users ${\mathcal{M}_s}$ in domain $B$) for satisfying the users $\mathcal{M}_s \subset\mathcal{M}_{A}$. So this added utility $u_A^B(X^{\mathcal{M}_s})$ is the pay-off for $B$ to share resources. This coalition clearly helps both. $A$ increases its customer satisfaction (as per the contract $A$ had agreed to provide resources to all the users $\mathcal{M}_{A}$), while $B$ earns extra using its excess resources. So it is a stable coalition.
\end{example}

\begin{example}[Utility Example]
For any two players \{1,2\},  $u_1 (\mathcal{X})$ will be given by 
\begin{equation}
u_1(\mathcal{X})=\sum_{i \in \mathcal{M}_1}\bigg(\prod_{k=1}^{{K}}\frac{1}{1+e^{-m(x_{ik}^{(1)}-R^{(1)}_{req,ik})}}\bigg)
\end{equation}
$u_2 (\mathcal{X})$ will be given by 
\begin{equation}
u_2(\mathcal{X})=\sum_{i \in \mathcal{M}_2}\bigg(\prod_{k=1}^{|\mathcal{K}|}(1-e^{-(\frac{1}{R^{(2)}_{req,ik}})x_{ik}^{(2)}})\bigg)
\end{equation}
 $u_2^{\mathcal{X}} (\mathcal{X})$ will be given by 
 \begin{equation}
 u_2^{1}(\mathcal{X})=\sum_{i \in \mathcal{M}_2}\bigg(\prod_{k=1}^{|\mathcal{K}|}(1-e^{-(\frac{1}{R^{(2)}_{req,ik}})x_{ik}^{(1)}})\bigg)
 \end{equation}
  $u_1^{\mathcal{X}} (\mathcal{X})$ will be given by 
  \begin{equation}
  u_1^{2}(\mathcal{X})=\sum_{i \in \mathcal{M}_1}\bigg(\prod_{k=1}^{{K}}\frac{1}{1+e^{-m(x_{ik}^{(2)}-R^{(1)}_{req,ik})}}\bigg)
  \end{equation}
\end{example}
\end{comment}


%\subsection{Choice of Utility Function for Resource Allocation Problem}
%The resource allocation problem can be represented using a \emph{monotone non-decreasing utility function}. This is because in the systems that we consider, such as a cloud service provider or a cellular communication system etc.,  the more the resources provided, the higher is the gain or utility for the service provider. It is highly unlikely that the utility of any service provider will decrease with increase in the amount of resources allocated.  


%satisfying user requests increases the gain or utility for the service provider.  increases with increase in the amount of resources allocated to the user. It is highly unlikely for any r
\begin{comment}
\subsection{Game Theoretic Solution}

We first define the characteristic function $v$ for our game that can solve  problem in~\eqref{eq:opt_higher} 
\begin{align} \label{eq:payoff_function}
v(\mathcal{N})=\sum_{\substack{\text{$n \in \mathcal{N}$} \\ \text{$C_{k}= \sum_{n \in \mathcal{N}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in \mathcal{N}$}\\ \text{$\sum_{j \in \mathcal{N}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}$}}}\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in \mathcal{N},j\neq n} u^{n}_j(\mathcal{X})\bigg)
\end{align}
\begin{remark}
	The characteristic function in Equation~\eqref{eq:payoff_function} is for the grand coalition $\mathcal{N}$. For any $S \subseteq \mathcal{N}$, the characteristic function will be 
\end{remark}
\begin{align} \label{eq:payoff_s_function}
v({S})=\sum_{\substack{\text{$n \in {S}$} \\ \text{$C_{k}= \sum_{n \in {S}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {S}$}\\ \text{$\sum_{j \in {S}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S}$}}} \bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in S,j\neq n} u^{n}_j(\mathcal{X})\bigg)
\end{align}
\begin{theorem}
%	A Cooperative game $(\mathcal{N}, v)$ of $\mathcal{N}$ players and $v$ payoff function that can be used to solve the multi-objective optimization problem given in \eqref{eq:opt_higher}, is canonical\footnote{for monotonically non-decreasing utilities/pay-off function} with Transferable utility
Resource allocation and sharing problem (with multiple objectives) in aforementioned settings can be modeled as a canonical cooperative game with TU. 
\end{theorem}
\begin{proof}
To prove this, we need to show that the characteristic function of resource sharing and allocation problem satisfies the following two conditions
%	For a game to be canonical, we need to prove that the game  is superadditive and the payoff function is of characteristic form. 
	\begin{itemize}
		\item \textbf{Characteristic form of payoff:} As the utility function in a resource sharing and allocation problem  only relies on the domains that are part of the coalition, the game or payoff function is of characteristic form
		\item \textbf{Superadditivity:} Super-additivity for TU games requires $v(S_1 \cup S_2 )\geq v(S_1)+V(S_2) \; \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, s.t. S_1\cap S_2 =\emptyset$ i.e. we have to prove that the pay-off or utility for a domain in the coalition is as good as domain working alone or in a smaller coalition. Due to monotonicity property of the utility functions used,  for all  players/domains $n \in \mathcal{N}$,  $u_n(X_n^{NC})\leq u_n(X_n^{C})$ as $X_n^{NC}\subset {X_n^{C}}$ \footnote{because $X_n^{C}$ can contain much more elements due to the increase in $C$ in the coalition} where $X_n^{C}$ and $X_n^{NC}$ are the allocation decisions in  a cooperative game  and independent setting respectively for domain $n$. 
	\end{itemize}
\end{proof}
\begin{lemma}\label{lemma:MOOGame}
A canonical cooperative game $(\mathcal{N}, v)$ with TU can be used to obtain the Pareto-optimal solutions for the multi-objective optimization problem given in \eqref{eq:opt_higher}
\end{lemma}

%Given that the game is canonical, we are going to explore potential solution approaches for such a game. We start with the \emph{Core} \cite{han2012game}. 

To prove Lemma \ref{lemma:MOOGame}, we must show that the core is non-empty for  our canonical game. To do this, we first show that our game is convex. 

\begin{definition}[Convex Games]
	A coalition game is said to be convex if and only if for every player $n \in \mathcal{N}$, the marginal contribution of the player is non-decreasing W.R.T set inclusion. Mathematically, for $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash \{n\}$ 
	\begin{equation}\label{eq:convexgames}
	v(S_1 \cup \{n\})-v(S_1) \leq v(S_2 \cup \{n\})-v(S_2)
	\end{equation} 
\end{definition}
\begin{theorem}
	Our canonical game is convex
\end{theorem}
\begin{proof}
Let us consider two coalition $S_1$ and $S_2$, where $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash\{j\}$ where $j \in \mathcal{N}$. Then we first calculate $v(S_2 \cup \{j\})-v(S_1 \cup \{j\})$
\begin{align}\label{eq:convexityProof}
& \sum_{\substack{\text{$n \in {S_2}$},\; \text{$C_{k}= \sum_{n \in {S_2}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}$}\\ \text{$\sum_{j \in {S_2}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {S_2}, k\neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) - \nonumber \\
& \Bigg(\sum_{\substack{\text{$n \in {S_1}$},\; \text{$C_{k}= \sum_{n \in {S_1}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {S_1}$} \\ \text{$\sum_{j \in {S_1}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_1}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {S_1}, k \neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_1)}(\mathcal{X}) + \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\nonumber \Bigg)\\ 
&= \sum_{\substack{\text{$n \in {S_2}\backslash S_1$}, \text{$C_{k}= \sum_{n \in {S_2}\backslash S_1}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}\backslash S_1$} \\ \text{$\sum_{j \in {S_2 \backslash S_1}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2 \backslash S_1}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {\{S_2 \backslash S_1\}}, k \neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) \nonumber \\
&   + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) - w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X}) \nonumber \\
& = v(S_2)- v(S_1)+ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})  \nonumber \\
& \geq v(S_2)- v(S_1)
\end{align}
	where the last inequality follows from the fact that $ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\geq 0$ (monotonicity of the utility)
\end{proof}
\end{comment}

%Related to the core, there are certain questions that we must answer
\begin{comment}
\begin{enumerate}
	\item Is the core non-empty?
	\item If the core is non-empty and consists of different pay-off allocations, how do we choose any particular pay-off allocation vector? 
\end{enumerate}
Below we attempt to answer these questions



\begin{definition}[Balanced Collection] Let $\Omega$ be a collection of different coalitions. $\Omega$ is considered to be a \emph{balanced collection} if we can find non-negative weights $w_S$ for each $S \in \Omega$ such that for every player $n$ 
	\begin{align}\label{eq:balancedcollection}
	\sum_{S \in \Omega, S \ni n}w_S =1 
	\end{align}
\end{definition}

\begin{definition}[Balanced Game] A game is called balanced if for every balanced collection $\Omega$, the payoff vector $\mathbf{x}$ will be in $V_{\mathcal{N}}$ if $\mathbf{x}_S \in V_S\; \forall S \in \Omega$ 
	%Let $\Omega$ be a collection of different coalitions. $\Omega$ is considered to be a \emph{balanced collection} if we can find non-negative weights $w_S$ for each $S \in \Omega$ such that for every player $n$ 
\end{definition}
\begin{theorem}[Bondareva-Shapley Theorem]\label{thm:BST}
	The core of a game is non-empty if and only if the game is balanced
\end{theorem}


\begin{theorem}
The core for canonical game with our characteristic function(in Equation~\eqref{eq:payoff_function}) is non-empty
\end{theorem}

\begin{proof}
From the definition of characteristic functions for TU games (see \cite{han2012game} for details), $v: 2^{\mathcal{N}}$ \textrightarrow $\mathbb{R}$ with $v(\emptyset)=\emptyset$. This means that the total number of coalitions possible for $\mathcal{N}$ players is $2^{|\mathcal{N}|}-1$ (we ignore the empty set). For $\Omega$, the non-negative weights $w_S$ which satisfy the condition for  balanced collection in Equation~\eqref{eq:balancedcollection} are given by $\frac{1}{2^{|\mathcal{N}|-1}}$. Hence $\Omega$ is a balanced collection. We also know that $v(S)\subseteq v(\mathcal{N})$ as $v(\mathcal{N})$ is defined over a larger feasible set due to increased amount of available resources. Leveraging the monotonicity property of the utility functions used, we know that any payoff vector  $\mathbf{x}$ will be in $V_{\mathcal{N}}$ if $\mathbf{x}_S$\footnote{$\mathbf{x}_S$ is the projection of $\mathbf{x}$ onto the vector space $\mathbb{R}^{|S|}$} $\in V_S\; \forall S \in \Omega$. Hence our canonical game with characteristic function $v$ in Equation~\eqref{eq:payoff_function} is balanced and its core is non-empty (from Theorem \ref{thm:BST})

\end{proof}
\end{comment}


%For our problem, does the Shapley value lie in the core? To do so we first define \emph{convex games}
\begin{comment}
\begin{theorem}
	The core of any convex game $(\mathcal{N},v)$ is non-empty and large. 
\end{theorem}
\begin{proof}
	Available in \cite{sharkey1982cooperative}
\end{proof}
While the existence of core i.e., core being non-empty, guarantees the grand coalition is stable, finding a suitable allocation from the core is challenging particularly when the core is large (our game). Furthermore, as mentioned earlier, fairness is also a shortcoming of core based solutions.  Shapley value can be  used to obtain a fair allocation, however, we first need to show that the Shapley value lies in the core to guarantee that the Shapley value based allocation is stable for the grand coalition. 
\begin{theorem}
	The Shapley value in Equation~\eqref{eq:shapleyvalue} lies in the core of our canonical game
\end{theorem}
\begin{proof}
	Since our canonical game is convex, the Shapley value lies in the core \cite{han2012game} (see \cite{roger1991game} for details)
\end{proof}
We summarize this in the remark below. 
\begin{remark}
If a TU game $(\mathcal{N}, v)$ is convex, then the core is non-empty and the Shapley Value lies in the core \cite{garg2013novel}.	
\end{remark}
Calculation of Shapley value given in Equation~\eqref{eq:shapleyvalue} is challenging \cite{han2012game}. Since our game is convex, calculating its Shapley value is slightly easier as given below. 

%Now that we have proved that the game is convex, we divert our attention to the calculation of Shapley value for a convex game. 


\subsubsection{Shapley Value for a Convex Game}
Let $\pi$ denote the permutation of players in our game.  Then for any permutation $p$ from the total possible permutations $|\mathcal{N}|!$, one can obtain the initial segments of ordering by \cite{garg2013novel}
\begin{equation}\label{eq:initialsegment}
O_{\pi, r}=\{ n \in \mathcal{N} : \pi(n) \leq r \}, \; r \in \{1, \cdots, N\}
\end{equation}
where $O_{\pi, 0}=\{\}$ and $O_{\pi, |\mathcal{N}|} =\mathcal{N}$. $\pi(n)$ refers to the position of the player $n$ in the permutation $\pi$. The core of any particular ordering $\pi$ can be obtained by solving  equations
\begin{equation}
\label{eq:x_i_pi_sol}
x_n^{\pi}(O_{\pi, r}) = v(O_{\pi, r}), \; r \in \{ 1, \cdots, N\}
\end{equation}
The solution to  above Equations~\eqref{eq:x_i_pi_sol} will result in a payoff vector $x^{\pi}$ where the elements of the vector are given by 
\begin{equation}
\label{eq:vectorelements}
x_n^{\pi}=v(O_{\pi, \pi(n)})- v(O_{\pi, \pi(n)-1}), \quad \forall n \in \mathcal{N} 
\end{equation}
The payoff vectors $x^{\pi}$ represent the extreme points of the core in convex games \cite{garg2013novel}. So if $\prod$ represents the set of all possible permutations of $\mathcal{N}$, the Shapley value of any player $n$ can be calculated as 
\begin{equation}
\label{eq:shapleyconvex}
\phi_n=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} x_n^{\pi}
\end{equation}
\begin{comment}
So for our coalition game $(\mathcal{N},v)$, the Shapley value is 
\begin{align}
\label{eq:ourshapleyconvex}
\phi_n&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} \bigg( \sum_{\substack{\text{$n \in {O_{\pi, \pi(n)}}$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)}}$} \\ \text{$$}\text{$\sum_{j \in {O_{\pi, \pi(n)}}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in O_{\pi, \pi(n)}$}}}\bigg(w_n u_n^{(\pi)}(\mathcal{A})+ w'_{n}\sum_{j \in {O_{\pi, \pi(n)}}, j \neq  n} u^{n,(\pi)}_j(\mathcal{A})\bigg)- \nonumber \\
&\Bigg(\sum_{\substack{\text{$n \in {O_{\pi, \pi(n)-1}}$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)-1}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)-1}}$}}}\bigg(w_n u^{(\pi)}_n(\mathcal{A})+ w'_{n}\sum_{j \in {O_{\pi, \pi(n)-1}}, j \neq n} u^{n,(\pi)}_j(\mathcal{A})\bigg)\Bigg) \nonumber \\
&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} \bigg( \sum_{\substack{\text{$n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1} }$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}$} \\ \text{$\sum_{j \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}$} }}\bigg(w_n u^{(\pi)}_n(\mathcal{A})+  \nonumber \\ 
& w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{n,(\pi)}_j(\mathcal{A}) +  w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{j,(\pi)}_n(\mathcal{A})  \bigg)\bigg) \nonumber \\
&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod}\bigg(w_nu^{(\pi)}_n(\mathcal{A})+ w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{n,(\pi)}_j(\mathcal{A}) +w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{j,(\pi)}_n(\mathcal{A}) \bigg) 
\end{align}
where Equation~\eqref{eq:ourshapleyconvex} provides the Shapley value for our convex game. It is evident that our Shapley value depends on the utility of the player $n$, the utility  player $n$ achieves by allocating resources to players in $j \in O_{\pi, \pi(n)}, j \neq n $ and the utility player $j \neq n, j \in O_{\pi, \pi(n)}$ achieves by allocating resources to player $n$  in every possible permutation. 

\begin{comment}
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $tt$ 
		\State \textbf{Output}: The optimal hit probabilities
		\State \textbf{Step $1$:}  $t \leftarrow$0, $\boldsymbol{\lambda^{(t)}\leftarrow\lambda_0}$, $\boldsymbol{\mu^{(t)}\leftarrow\mu_0}$
		\While{Equation \eqref{eq:gradient1} $\neq$ 0}%$\partial L(\boldsymbol{h,\lambda,\mu})/\partial \lambda_{l} \neq0$ $\&\& $ $\partial L(\boldsymbol{h,\lambda,\mu})/\partial \mu_{ip} \neq0$}
		\State \textbf{Step $2$}:$\boldsymbol{h_{il}^{(p)}[t]} \leftarrow \frac{w_i\beta^{|p|-l}}{\lambda_{l}[t-1]\Bigg(\prod_{\substack{q \neq p,\\ q:l\in\{1,\cdots,|q|\}}}(1-h_{il}^{(q)}[t-1])\Bigg)+\mu_{ip}[t-1]}. $ %Algorithm 2($\boldsymbol{\lambda^{(t)},\mu^{(t)}}$) %\Comment{The node id and file content to Algorithm \ref{algo:alg1} for calculating the price function using~(\ref{eq:gradient2}) }
		\State \textbf{Step $3$:} Update $\lambda$ and $\mu$ using  \eqref{eq:update},  t $\leftarrow t+1$
		%	\State \textbf{Step $4$}: $\boldsymbol \tau_{\chi} \longleftarrow \text{Convex}(\text{slave},\boldsymbol u_{\chi})$ \Comment{Solve the slave optimization problem for $\boldsymbol \tau_{\chi}$  }
		%	\State \textbf{Step $5$}: $(\boldsymbol b_{\chi}, \boldsymbol{\delta_{\chi}}, \text{obj}_{\chi})  \longleftarrow \text{Rounding}(\boldsymbol u_{\chi},\boldsymbol \tau_{\chi})$ \Comment{Round the values of $\boldsymbol u_{\chi}$, remap $\boldsymbol u_{\chi}, \boldsymbol \tau_{\chi}$ to $\boldsymbol{b}_{\chi}$ and $ \boldsymbol{\delta}_{\chi}$ and obtain the new objective function value  }
		\EndWhile
	\end{algorithmic}
	\caption{Iterative Distributed Algorithm}
	\label{algo:alg}
\end{algorithm}
\end{comment}
\begin{comment}
\begin{remark}
	Shapley value calculation for our convex game requires solving at least $2^{N}-1$ optimization problems
\end{remark}
Algorithm \ref{algo:alg1} provides an overview of our proposed approach. We obtain $R, C$ and the utility of all players as $\mathbf{u}$. We initialize each player's utility value ($\mathbf{u}(R,\mathcal{X})$), Shapley value ($\boldsymbol{\phi} $) and resource allocation decision $\mathcal{X}$ to $0$. Then we calculate the Shapley value for the players and assign it to $\mathbf{u}(R,\mathcal{X})$. Finally to obtain $\mathcal{X}$, we take the inverse function of $\mathbf{u}$. As we are using monotone utilities, we know that the inverse of the utilities exist.

\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0, $ \boldsymbol{\phi} \leftarrow$0,  
		\State \textbf{Step $1$:}  Calculate Shapley Value $\phi_n$ using Equation \eqref{eq:shapleyconvex} $\forall n \in \mathcal{N}$
		\State \textbf{Step $2$:} $ \mathbf{u}(R,\mathcal{X}) \leftarrow \boldsymbol{\phi}$
		\State \textbf{Step $3$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{Shapley Value based Resource Allocation}
	\label{algo:alg1}
\end{algorithm}
%It is worth mentioning here that the Shapley value will only provide us the utility each player is going to receive that lies in the core (as a result of cooperation). The allocation decision can be obtained by taking the inverse of utilities.  \par 
\subsubsection{Reducing the Computational Complexity}
As mentioned earlier, that the calculation of Shapley value for our convex game requires at solving at least $2^{N}-1$ optimization problems that is computationally expensive. To reduce the complexity, we propose a computationally efficient approach in Algorithm 2 that requires solving $2N$ optimization problems i.e. $\mathcal{O}(N)$.  The input into the algorithm consists of available resources/capacities, user requirements and the utilities of all game players. The output of the algorithm is $\mathcal{X}$. In Step 1, the utility values of the players, the allocation decision,  and two vectors $\boldsymbol{O_1}$ and $\boldsymbol{O_2}$. In Step 2, every player's utility is calculated without any resource sharing i.e. single optimization and the values are stored in the vector $\boldsymbol{O_1}$. Then $C, R$ are updated and we move to Step 4, where we calculated the utilities $u_j^n$'s for all the players with updated $C, R$ and store them in $\boldsymbol{O_2}$. 

\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0, $ \boldsymbol{\phi} \leftarrow$0,  $ \boldsymbol{O_1} \leftarrow$0, $ \boldsymbol{O_2} \leftarrow$0, 
		\State \textbf{Step $2$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_1^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single}}
		\EndFor
		\State \textbf{Step $3$:} Update $C$ and $R$ based on Step 2
		\State \textbf{Step $4$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_2^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single_j}}
		\State Update $C$ and $R$
		\EndFor
		\State \textbf{Step $5$:} $u_n(R,\mathcal{X})\leftarrow O_1^n+O_2^n$ $\forall n \in \mathcal{N}$ 
		\State \textbf{Step $6$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{$\mathcal{O}$($N$) algorithm for obtaining Core's allocation}
	\label{algo:alg2}
\end{algorithm}
\begin{subequations}\label{eq:opt_single_j}
	\begin{align}
	\max_{\mathcal{X}}\quad& \sum_{j\neq n}u_j^n(\mathcal{X}) \quad  \forall n \in \mathcal{N} \label{eq:objsinglej}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall i \in \mathcal{M}\backslash\mathcal{M}_n, \label{eq:singlefirstj} \displaybreak[0]\\
	& x_{ik}^{(n)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecondj} \displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlethirdj} \displaybreak[2]
	\end{align}
\end{subequations}
\begin{theorem}
	The solution obtained from Algorithm \ref{algo:alg2} lies in the \emph{core}
\end{theorem}
\begin{proof}
	To prove the theorem, we need to show that the utilities obtained in Step $5$ of Algorithm \ref{algo:alg2}; a) are individually rational; b) are group rational and c) no players  have the incentive to leave the grand coalition and form another another coalition $S \subset \mathcal{N}$. 
	\paragraph{Individual Rationality} For each player $n \in \mathcal{N}$, the solution $O_1^n$ obtained by solving the optimization problem in Equation \eqref{eq:opt_single} is the utility a player will obtain by working alone i.e. it is $v\{n\}$. The value $O_2^n$ in Step 4 is either zero or positive but cannot be negative due to the nature of utility used i.e. 
	\begin{align}
u_n(R,\mathcal{X})&=O_1^n+O_2^n \quad \forall n \in \mathcal{N} \nonumber \\
u_n(R,\mathcal{X})&\geq O_1^n \quad \forall n \in \mathcal{N}\nonumber 
	\end{align}
	
	
	 Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is individually rational.
	\paragraph{Group Rationality} The value of the grand coalition $v\{\mathcal{N}\}$ as per Equation \eqref{eq:payoff_function} is the sum of utilities $u_n$'s and $u_j^n$'s. Steps 2, 4 and 5 of Algorithm \ref{algo:alg2} obtain the sum of the utilities as well. Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is group rational rational. 
	\par Furthermore, due to super-additivity of the game and monotonic non-decreasing nature of the utilities, no players have the incentive to form a smaller coalition. Hence Algorithm \ref{algo:alg2} provides a solution from the core.  
\end{proof}
\end{comment}
%\vspace{-0.1in}

==> arxiv version/01-intro.tex <==
\subsection{Motivation}
Edge computing has received much attention recently as it enables on-demand provisioning of computing resources for different applications and tasks at the network edge \cite{shi2014online,shi2016edge,satyanarayanan2017emergence}. One of the fundamental advantages of edge computing is that it can provide resources % to resource constrained applications 
with low latencies when compared with traditional cloud computing architecture \cite{shi2016edge}. The demand for edge computing has further increased due to the advent of Internet of Things (IoT) \cite{atzori2010internet} and wide-scale use of machine and deep learning \cite{li2018learning} in different industries as  these learning-based models can  be trained and run using edge computing nodes with adequate storage and computing power \cite{wang2018edge}. 

\par A typical edge computing system consists of a large number of edge nodes  that have different types of resources. Edge service provider (ESP) earns a \emph{utility} for allocating resources to different applications and guarantees to provide  resources according to a \emph{Service Level Agreement} (SLA). However, when compared with cloud computing systems and data centers, resources in an edge setting are limited. Therefore, optimal use and allocation of these limited resources has been an active area of research. 
Even when resources are available, allocating  them to  applications with the goal of maximizing overall ESP \emph{utility} is a difficult problem. Furthermore, the aforementioned resource intensive paradigms such as deep learning, and data analytics  exacerbate the problem by challenging the scalability of traditional resource allocation techniques. \par 

ESPs typically provide enough resources to different applications at their edge nodes to  meet the peak demand. However, it is highly likely that  resources of one ESP will be over-utilized, while other ESP's resources will be under-utilized.  
For example, an ESP provisions resources to an application at an edge node that is physically closest to the requesting application. However, if the closest edge node has a resource deficit or is overloaded, the request can be satisfied through ESP's next closest edge node that  may physically  be at a distant location or deep in the network such as at the data center. This incurs high cost and  causes high latency that may not be acceptable for delay constrained applications. One possible solution is  to create a shared  resource pool with other ESPs that are  physically closer  \cite{he2018s,openedge,openfog,etsi}. Such a resource pool allows  ESPs to share and use  resources whenever needed to meet their dynamic demands. This cooperation and resource sharing among ESPs seem beneficial for them, because it is unlikely that resources of different ESPs will be   simultaneously over-utilized.
\par  %While we use edge computing paradigm as an illustrative example, 
Our work has also been  motivated by military settings in which two or more  \emph{coalition partners}\footnote{Each coalition partner can be considered an ESP. } are jointly conducting a military operation using different resources from the partners. As military settings usually have strict  latency and reliability requirements, resources are placed at the edge to fulfill the aforementioned requirements. 
Hence, coalition settings can be considered a practical scenario for edge computing. In contrast with commercial edge computing settings, military settings require a higher reliability and robustness to ensure timely availability of resources. 
As seen in Figure \ref{fig:system_model}, both coalition partners $2$ and $3$ satisfy all their applications and have resource surpluses whereas partner $1$ has resource deficits when working alone. However, through cooperation among these coalition partner, $1$ satisfies its applications by using resources of other coalition partners resulting in  an improved utility for all partners. It is evident that if  different coalition partners do not share resources, different application requests cannot be satisfied. Therefore, there is a need for a framework that allows resource sharing among these coalition partners (i.e., ESPs). 
Furthermore, the framework needs to be distributed as a centralized solution may not be acceptable to the different coalition partners or ESPs because:
\begin{itemize}
	\item An adversary can target the central system  causing the entire military operation to fail.
	\item Coalition partners need to reach a consensus  for choosing the \emph{central} node that runs the resource sharing algorithm. 
	\item A centralized framework requires  a large amount of information to be transmitted to the central node. This may not be feasible or preferred by the coalition partners as certain information may be private.  
\end{itemize} 
Such a distributed resource sharing gives rise to a number of questions such as: 
 \begin{enumerate}
 	\item \emph{Should an ESP help another ESP by sharing resources?}
 	\item \emph{How should  resources be allocated to applications across different ESPs, while considering issues such as  communication cost and resource fragmentation? }
 	\item \emph{How can  ESPs share the profits of resource sharing?}
 \end{enumerate}
We  answer these questions in this paper. 
\subsection{Methodology and contributions}
In this paper, we consider a number of ESPs that share their resources and form a  resource pool to satisfy resource requests of different applications as shown in Figure \ref{fig:system_model}.
We formulate such resource sharing and allocation among ESPs as a   multi-objective optimization (MOO) problem, for which our goal is to achieve a Pareto optimal solution.  Furthermore, since Pareto solutions are spread over the \emph{Pareto frontier} \cite{cho2017survey}, choosing a single solution among them is challenging. As the \emph{Nash Bargaining Solution}  (NBS)\cite{nash1950bargaining} guarantees the provision of  a fair and Pareto optimal solution to such a MOO problem,  we develop a distributed NBS-based framework for  resource allocation and sharing here.  \emph{To the best of our knowledge, this is the first generic NBS-based framework for resource sharing and allocation among ESPs. } 

 \begin{figure}
	\centering
	\includegraphics[width=0.49\textwidth]{figures/pool_new2.jpg}
	\vspace{0.05in}
	\caption{Cooperation among ESPs}
	\protect\label{fig:system_model}
	%\vspace{-0.2in}
\end{figure}
The main contributions of this paper are: 
\begin{enumerate}
  
	\item We present an NBS based  resource  sharing framework for ESPs with different objectives in allocating resources to meet the dynamic demands. Our framework also considers practical engineering constraints such as communication costs and resource fragmentation. 
\item We show that ESPs can benefit from sharing resources  with other ESPs as they can earn a higher profit and improve the average application satisfaction.    
\item We  show that  \emph{strong-duality} property holds for the formulated problem, which enables us to propose a distributed  algorithm to obtain the NBS.   
\item 	We evaluate the performance of our algorithms using  synthetic and real world traces.  Results show that resource sharing improves the utilities of ESPs, increases resource utilization and enhances average user (application) satisfaction. Furthermore, our results show that the profit sharing among  ESPs is also fair. 
\end{enumerate}
The rest of this paper is structured as follows. We present the system model in Section~\ref{sec:sysmodel}. 
In Section~\ref{sec:nbs}, we first present a primer on NBS. We then describe our proposed  NBS framework  for resource sharing and allocation. In Section~\ref{sec:dist}, we present a distributed algorithm for obtaining the NBS. In Section~\ref{sec:exp_results}, we present simulation results of the proposed framework for different settings. We describe the related work in Section \ref{sec:related},  
and conclude the paper in Section~\ref{sec:conclusion}. 







==> arxiv version/02-sysmodel.tex <==
Any entity or service provider  that has specific resources such as CPU, storage and communication links can serve as the building block of our system as shown in Figure~\ref{fig:system_model}. We call this basic building block  a \emph{domain}\footnote{Throughout the paper, we will use domain, service provider and player interchangeably.}. The domain can be as small as a sensor and as large as data centers.  Each domain has a \emph{domain controller} that is aware of all resources available within the domain. The domain controller only shares an abstraction of this resource information and does not share the entire information\footnote{This can be due to a number of reasons including security and privacy. For example, Amazon and Dropbox may share limited information to satisfy their user's needs. However, they will not provide the entire information to each other.}. Different domains share resources with  the presence of a \emph{coalition controller}. The coalition controller can be either a separate controller or chosen among  the domain controllers. %Figure \ref{fig:system_model} the model used in this paper.   
Table \ref{tab:notationTable} provides  notation used in this paper. Below, we model our resource allocation and sharing problem from a  game theoretic perspective.   
 \begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{figures/domain}
	\caption{Our system model with domain and coalition controllers}
	\protect\label{fig:system_model}
	\vspace{-0.1in}
\end{figure}

\begin{table}[]
	\caption{List of notations (Not.) used in the paper}
	\begin{tabular}{|p{0.44cm}|p{2.7cm}||p{0.44cm}|p{3.2cm}|}
		\hline
		\textbf{NOT.} & \textbf{Description} & \textbf{NOT.} & \textbf{Description} \\ \hline
	$\mathcal{N}$	& Set of game players                     &        $n$           &Player from set   $\mathcal{N}$  \\ \hline
	$\mathcal{M}$	& Set of applications                     &      $\mathcal{M}_n$             & Set of native applications of player $n$                     \\ \hline
	$\mathcal{K}$	& Set of resource types                     &     $k$              &  Resource from set $\mathcal{K}$                    \\ \hline
	$C^{(n)}$	&  Capacity of player $n$                    &    $C_k^{(n)}$	&  Capacity of $k^{th}$ resource at player $n$           \\ \hline
	$x_{ik}^{(n)}$	&  Resource $k$ allocated to application $i$ by player $n$      &   $r_{ik}^{(n)}$      &     Request for  resource $k$ from application $i$ of player $n$                 \\ \hline
%		&                      &                   &                      \\ \hline
%		&                      &                   &                      \\ \hline
	\end{tabular}
\label{tab:notationTable}
%\vspace{-0.2in}
\end{table}

Let $\mathcal{N}=\{1,2, \cdots, N\}$ be the set of all domains (or service providers) that act as players in our game. We assume that each player has a set of $\mathcal{K}=\{1,2,\cdots, K\}$ different types of resources such as communication, computation and storage resources.  The $n$-th domain reports its available resources $C^n = \{ C_1^{(n)},\cdots, C_K^{(n)}\}$ to a central entity, the coalition controller. Here $C_k^{(n)}$ is the amount of type $k$ resources available to domain $n$.  
%All edge clouds can report their available resources  to any central entity, coalition controller \footnote{Coalition controller can be chosen from the edge clouds.},  where ${C}^{(n)}=\{ {C}_{1}^{(n)}, \cdots, {C}_{K}^{(n)}\}$ represents the available resources $k \in \mathcal{K}$ for the player $n \in \mathcal{N}$. 
Vector $C=\{\sum_{n \in \mathcal{N}}C_{1}^{(n)}, \sum_{n \in \mathcal{N}}C_{2}^{(n)}, \cdots ,\sum_{n \in \mathcal{N}}C_{K}^{(n)}\}$ represents  all available resources in different domains.  Each domain $n$ has a set of  native applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$ that ask for resources. Furthermore, the set of all applications that ask for resources from the set of domains (coalition of domains) is given by $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where $|\mathcal{M}|=M$,  and $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset, \; \forall i \neq j,$ i.e., each application originally asks only  one domain for resources. 
%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
The coalition controller receives a request (requirement) matrix $R^{(n)}$ from every player (domain) $n \in \mathcal{N}$.% \vspace{-0.1in}
\begin{equation}
\label{eq:R_Req}
R^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{r^{(n)}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{(n)}_{{M}_n}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r^{(n)}_{11} & \cdots  &\cdots   & r^{(n)}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{(n)}_{M_{n}1}&\cdots  &\cdots   & r^{(n)}_{{M}_n{K}}
\end{smallmatrix}\Biggr].
\end{equation}
%\vspace{-0.01in}
\noindent where the $i^{th}$ row corresponds to the $i^{th}$ application while  columns represent different resources, i.e., $r_{ij}^{(n)}$ is the amount of $j^{th}$ resource that application $i \in \mathcal{M}_n$ requests.
%The vector ${C}^{(n)}$ received by coalition controller shows different available resources at edge cloud $n$. 
The coalition request matrix $R$ is a combination of all the request matrices (from all the domains)  as given below. 
\begin{equation}
\label{eq:R_Reqco}
R^{}=\Biggl[\begin{smallmatrix}
\mathbf{r^{}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{}_{{M}}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r^{}_{11} & \cdots  &\cdots   & r^{}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{}_{M1}&\cdots  &\cdots   & r^{}_{{M}{K}}
\end{smallmatrix}\Biggr].
\end{equation}
\noindent where $r_{ij}$ is the amount of $j^{th}$ resource that application $i \in \mathcal{M}$ requests.
The coalition, based on $R$ and  $C$, has to make an allocation decision $\mathcal{X}$ that optimizes the utilities of all the domains  $n \in \mathcal{N}$.  The allocation decision for the entire coalition $\mathcal{X}$ consists of all the  allocation decisions $X^{(n)}$ in every domain $n \in \mathcal{N}$ i.e.,  $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$.  
%The allocation decision $\mathcal{X}$ is  given by $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$ indicating how much of each resource $k \in \mathcal{K}$ is allocated to application $i$ at domain $n \in \mathcal{N}$. The matrix $X^{(n)}$ is a combination of different matrices $\{X_{i\in \mathcal{M}_1}^{(n)}, \cdots,X_{i\in \mathcal{M}_n}^{(n)},\cdots, X_{i\in \mathcal{M}_N}^{(n)} \}$, where $X_{i\in \mathcal{M}_n}^{(n)}$ is the allocation decision  at domain $n$ for the applications $i$ originally belonging to domain $n \in \mathcal{N}$ i.e., the original applications of the domain $n$. Furthermore,  $X_{i\in \mathcal{M}_j}^{(n)}$, $\forall j \in \mathcal{N},$ where $j \neq n$, is the allocation decision at domain $n$ for applications $i$ belonging to domain $j$.  
Mathematically,  $X^{(n)}$ is represented by % \eqref{eq:A_n}, where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$.  %Table \ref{tab:notationTable} provides some of the notations used in the paper. 
\begin{equation}
\label{eq:A_n}
X^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{{M}}}^{(n)}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{{M}}1}^{(n)}&\cdots  &\cdots   & x_{{{M}}{K}}^{(n)}
\end{smallmatrix}\Biggr].
\end{equation}
where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$.
% \subsection{Assumptions}



\begin{comment}
Let $\mathcal{N}=\{1,2, \cdots, N\}$ be the set of all the domains that act as players in our game. % For simplicity, we drop the $P$ in $P_n$ and represent the players only with the subscript $n$. 
Each player has a utility function $u_n(\mathcal{X})$ that depends on the allocation decision $X$ (details for $X$ will be given later). We assume that each player has set of $\mathcal{K}=\{1,2,\cdots, K\}$ different resources such as communication, computation and storage resources. %Each player $n \in \mathcal{N}$ has complete information about its own resources $k \in \mathcal{K}$, however it reports only abstract information to a coalition controller 
All domains report their available resources  to the coalition controller where $C^{(n)}$ represent the available resources for the domain/player $n \in \mathcal{N}$. Each domain $n$ has a set of users or applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$ that ask for resources. Also $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset \; \forall i \neq j$ represents the set of all users that ask for resources from the coalition. 

%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
The coalition controller receives a matrix $R^{(n)}$ for every player $n \in \mathcal{N}$ 
	\begin{equation}
\label{eq:R_Req}
R^{(n)}=\Biggl(\begin{smallmatrix}
\mathbf{r^{(n)}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{(n)}_{{M}_n}}
\end{smallmatrix}\Biggr) = \Biggl(\begin{smallmatrix}
r^{(n)}_{11} & \cdots  &\cdots   & r^{(n)}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{(n)}_{M_{n}1}&\cdots  &\cdots   & r^{(n)}_{{M}_n{K}}
\end{smallmatrix}\Biggr)
\end{equation}
where the $i^{th}$ row corresponds to the $i^{th}$ user while  the columns represent different resources i.e., $r_{ij}$ is the amount of $j^{th}$ resource user $i \in \mathcal{M}$ requests.

The vector ${C}^{(n)}=\{ {C}_{1}^{(n)}, \cdots, {C}_{K}^{(n)}\}$ received by coalition controller shows different available resources at domain $n$. 
The vector $C=\{\sum_{n \in \mathcal{N}}C_{1}^{(n)}, \sum_{n \in \mathcal{N}}C_{2}^{(n)}, \cdots ,\sum_{n \in \mathcal{N}}C_{K}^{(n)}\}$ consists of all the available resources at different domains. The coalition, based on $R$ and  $C$, has to make an allocation decision $\mathcal{X}$ that optimizes the utilities $u_n(\mathcal{X})$ of the domains.  The allocation decision $\mathcal{X}$ is  a vector $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$ that shows how much of each resource $k$ is allocated to user $i$ at domains $n \in \mathcal{N}$.

\begin{equation}
\label{eq:A_n}
X^{(n)}=\Biggl(\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{|\mathcal{M}|}}^{(n)}}
\end{smallmatrix}\Biggr) = \Biggl(\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{|\mathcal{M}|}1}^{(n)}&\cdots  &\cdots   & x_{{|\mathcal{M}|}{K}}^{(n)}
\end{smallmatrix}\Biggr)
\end{equation}
where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ allocated  to user $i$ at player $n$

 Since the utilities of different domains might be different (can be conflicting as well), this leads us to a multi-objective optimization (MOO) problem. Some of the assumptions in our model are given below
\subsection{Assumptions}
The assumptions made in our model are 
\begin{enumerate}
	\item The negotiation cost among different domains is negligible
	\item All the domains communicate their information to the coalition controller
	\item The coalition controller already exists% and do not discuss the selection of the coalition controller (can be explored in the future work)
	\item Resources across different domains are additive in nature i.e., if domain $X$ and $Y$ have $2$ GB RAM each, the coalition would have $4$ GB of RAM. 
	\item Each player has a single objective
	\item The objective of the coalition is a sum of the utilities of all the players with equal weight
%	\item Any new player/domain added into the coalition will have resources available
	\item All players or domains have the same number of users or jobs
\end{enumerate}
\end{comment}








==> arxiv version/02-sysmodel2.tex <==
Let $\mathcal{N}=\{1,2, \cdots, N\}$ be the set of all ESPs. 
We assume that each  provider has a set of $\mathcal{K}=\{1,2,\cdots, K\}$  types of resources such as communication, computation and storage resources.  %Service provider  $n$ represents its  available resources as 
$C_{n} = \{ C_{n,1},\cdots, C_{n,K}\}$, with  $C_{n,k}$ denoting the amount of type $k$ resources available at service provider $n$. 

  Each service provider $n$ has a set of  native applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$. 
The set of all applications that request resources from all service providers  is given by $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where we assume  $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset, \; \forall i \neq j,$ i.e., each application initially  demands resources from only  its native service provider. We also define $\overline{\mathcal{M}}$ to represent  $\mathcal{{M}}\backslash \mathcal{{M}}_n$ and $\overline{\mathcal{N}}$ to represent $\mathcal{{N}}\backslash n $.  
%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
Every ESP  $n \in \mathcal{N}$ has a request (requirement) matrix $R_{n}$,% from every player $n \in \mathcal{N}$ 
\begin{equation}
\label{eq:R_Req}
R_{n}=\Biggl[\begin{smallmatrix}
\mathbf{r_{n}^1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r_{n}^{{M}_n}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r_{n,1}^{1} & \cdots  &\cdots   & r^{1}_{n,{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r_{n,1}^{{M}_n}&\cdots  &\cdots   & r_{n,K}^{{M}_n}
\end{smallmatrix}\Biggr],
\end{equation}
%where the $j^{th}$ row corresponds to  application $j$, while  columns represent different resources. That is,
Here  $r_{n,k}^{j}$ is the amount of resource $k$ that application $j \in \mathcal{M}_n$ requires. When an ESP is working alone (no sharing of  its resources with any other service provider),  its objective is to maximize its utility by allocating  resources to its native applications. % and improving application satisfaction.
 A service provider $n$ earns a  utility $u^j (x_{n,k}^j)$ by allocating $x_{n,k}^j$ amount of resource $k$ to application $j\in \mathcal{M}_n$, where the vector $\mathbf{x}_n^j= [x_{n,1}^j, x_{n,2}^j,\cdots, x_{n,K}^j]^T$. 
 Table \ref{tab:not} contains notations used throughout the paper. We present the optimization formulation for a single service provider in Section \ref{sec:prob}, followed by a formulation for the multiple service provider problem in Section \ref{sec:multP}.  %Below we present the optimization formulation for a single service provider. 

%\textbf{Add notation table here}


\begin{table}[]
	\centering
	\caption{List of notations used throughout the paper}
	\begin{tabular}{|p{1cm}|p{6.9cm}|}
		\hline
		\textbf{Notation}	& \textbf{Description} \\ \hline
		$\mathcal{{N}}, N, n$	& Set, number and index of ESPs  \\ \hline
		$\mathcal{K}, K, k$	& Set, number and index of resources \\ \hline
		$\mathcal{M}, M, j$	& Set, number and index of applications \\ \hline
		$\mathcal{M}_{n}$	& Set of native applications at ESP $n$  \\ \hline
	%	$\overline{\mathcal{M}}$	& Set of native applications at ESP $n$  \\ \hline
	%	${S}$	& A coalition of game players, where $S \subseteq \mathcal{{N}}$  \\ \hline
		%$\mathcal{M}_{n}$	& Set of native applications at player $n$  \\ \hline
%		$\mathcal{V}$	& Set of payoff vectors    \\ \hline
%		${v}(S)$	& Value of coalition $S$    \\ \hline
%		$\mathcal{G}_1$	& Set of players with resource deficit    \\ \hline
%		$\mathcal{G}_2$	& Set of players with resource surplus   \\ \hline
		$C$	& Capacity vector of all ESPs \\ \hline
		$C_n$	& Capacity vector of ESP $n$ \\ \hline
		$C_{n,k}$	& Capacity of resource $k$ at ESP $n$ \\ \hline
	%	$R$	& Request matrix of all game players \\ \hline
		$R_{n}$	& Request matrix at ESP $n$ \\ \hline
		$r_{n,k}^{j}$	& Request of application $j$ for resource $k$ from ESP $n$ \\ \hline
	%	${X}_{i \in \mathcal{M}_n}^{(n)}$	& Allocation decision matrix at player $n$ for its native applications \\ \hline
	%	${X}_{i \in \mathcal{M}_j}^{(n)}$	& Allocation decision matrix at player $n$ for applications of other players \\ \hline
	%	${X}^{(n)}$	& Allocation decision matrix at player $n$ for all applications (native and applications of other service providers)\\ \hline
	%	$\mathcal{X}_n$	& Allocation decision for all game players  \\ \hline
%		$X_{SO}^{(n)}$	& Single objective allocation decision at $n$  \\ \hline
		$x_{n,k}^{j}$	& Allocation decision of resource $k$ for application $j$ at ESP $n$ \\ \hline
	$\mathbf{x}_{n}^{j}$	& Allocation decision vector for application $j$ at ESP $n$ when working alone, i.e., $\mathbf{x}_{n}^{j}=[x_{n,1}^j, \cdots, x_{n,K}^j]^T$  \\ \hline

	%	$u_{j}^n$	& Utility player $n$ earns by allocating resources to applications of player $j$\\ \hline
	$\mathbf{X}_n$ & Allocation decision for ESP $n$ in the  resource sharing case \\ \hline 
	$\mathbf{X}$ & Allocation decision for the entire set of ESPs  \\ \hline 
	%	$\mathcal{X}_n$ & Allocation decision for player $n$ in the  coalition excluding its native applications \\ \hline	
			$u_{}^j({x}_{n,k}^j)$	& Utility ESP $n$ earns  by allocating resource $k$ to application $j$ \\ \hline
		$u_{}^j(\mathbf{x}_{n}^j)$	& Utility ESP  $n$ earns  by allocating vector of  resources to application $j$ \\ \hline
	%	$GC$	& Grand coalition\\ \hline
	%	$RS$ & Request satisfiability\\ \hline
	%	$TU$ & Transferable utility\\ \hline
	%	$NTU$ & Non-transferable utility\\ \hline
	%	$CGT$ & Cooperative game theory\\ \hline
	%	$MOO$ & Multi-objective optimization\\ \hline
	%	$SOO$ & Single-objective optimization\\ \hline
	%	$MEC$ & Mobile edge cloud\\ \hline
	\end{tabular}
	\label{tab:not}
\end{table}


\subsection{Problem Formulation for Single Service Provider } \label{sec:prob}
 We  first present the resource allocation problem for a stand-alone single service provider (i.e., no resource sharing with other service providers). 
For a single ESP $n \in \mathcal{N}$, the allocation decision  consists of  vectors $\mathbf{x}_n^1, \cdots, \mathbf{x}_n^{M_n}$. The optimization problem is: 
\begin{subequations}\label{eq:opt_single}
	\begin{align}
	\centering
%	\max_{\mathbf{x}_n^1, \cdots, \mathbf{x}_n^{M_n}}\quad& \sum_{j \in \mathcal{M}_n}\Big(u_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}} \frac{x_{n,k}^{j}}{r_{k}^{j}}\Big), \label{eq:objsingle}\\
\max_{\mathbf{x}_n^1, \cdots, \mathbf{x}_n^{M_n}}\quad& \sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}u^j({x}_{n,k}^j), \label{eq:objsingle}\\
	\text{s.t.}\quad & \sum_{j} x_{n,k}^{j}\leq C_{n,k}, \quad \forall k \in \mathcal{K}, \label{eq:singlefirst} \displaybreak[0]\\
	& x_{n,k}^{j} \leq r^{j}_{n,k}, \quad \forall\; j\in \mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecond} \displaybreak[1]\\
	&  x_{n,k}^{j} \geq 0, \quad \forall\; j\in \mathcal{M}_n, k \in \mathcal{K}. \label{eq:singlethird} \displaybreak[2]
	\end{align}
\end{subequations}
The goal of a single service provider in solving this single objective optimization (SOO) problem, as mentioned earlier,  is   to  maximize its utility by appropriately allocating  resources. %$ \sum_{j \in \mathcal{M}_n}\sum_{k \in \mathcal{K}} \frac{x_{n,k}^{j}}{r_{k}^{j}}$ captures the satisfaction of resource requests by applications. 
The first constraint  \eqref{eq:singlefirst} indicates that  allocated resources cannot exceed capacity. The second constraint   \eqref{eq:singlesecond} reflects that allocated resources should not exceed the requested amounts.  The last constraint, \eqref{eq:singlethird}  says the allocation  cannot be negative. However, it is possible that a service provider $n$ may 
earn a larger utility by providing its resources to applications of other service providers or it may not have sufficient resources to satisfy  requests of all its native applications. On the other hand, there may be another service provider $m\in \mathcal{{N}}\backslash n$ that may have a surplus of resources, which can be ``rented" by service provider $n$. %In this work, we focus on the strategy where each service provider has to allocate resources to its native applications and then share the remaining (if any) resources with other service providers who are not able to satisfy their native applications. 
Below, we discuss  resource sharing among these service providers. 


\subsection{Multiple Service Providers Problem Formulation}\label{sec:multP}
%We assume that a service provider $n$ does not have sufficient resources to satisfy all its native applications, while another service provider $m$ may have resource surpluses, which can be shared with provider $n$. Therefore, 
Allowing resource sharing among  service providers, while considering their objectives, could improve resource utilization and  application satisfaction. 
Let $D^j(x_{n,k}^j)$ denote the communication cost of serving application $j \in  \mathcal{{M}}_m$ at service provider $n$ rather than at its native service provider $m$. 
By sharing its resources, ESP $n$ earns a utility,
\begin{equation}\label{eq:util}
u^j (\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+x_{n,k}^j)-u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j)-D^j(x_{n,k}^j),
\end{equation}
after allocating  $x_{n,k}^j$ for application $j\in \mathcal{{M}}_m$, i.e., the net utility ESP $n$ earns is calculated as the \emph{differential utility} ($u^j (\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+x_{n,k}^j)-u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j)$) earned due to providing  $x_{n,k}^k$ amount of resources minus the communication cost between the native and non-native ESP. 
% the difference of total utility earned considering   resources provided to application $j$ by all ESPs ($u^j (\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+x_{n,k}^j)$), utility  $u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j)$ earned due to resource provided by all ESPs other than ESP $m$\footnote{$ u^j (\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+x_{n,k}^j)-u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j)$ is the \emph{differential utility}, i.e., the increase in  utility by providing  $x_{n,k}^j$ resources.} and the  communication cost $D^j(x_{n,k}^j)$. 
  We assume that  $ u^j (x_{n,k}^j)=u^j (x_{m,k}^j)$ when $x_{n,k}^j=x_{m,k}^j$. %In \eqref{eq:util}, the utility an ESP $m$ earns by allocating 
% \textbf{(This assumption may no longer be needed and we can relax it)}.
% and $d_m^j$ is the distance between service provider $m$ and the native service provider of application $j$.
   We also let
   \begin{equation*}
 \mathbf{x}^j= [\sum_{n \in \mathcal{{N}}}x_{n,1}^j, \sum_{n \in \mathcal{{N}}}x_{n,2}^j,\cdots, \sum_{n \in \mathcal{{N}}}x_{n,K}^j]^T,
   \end{equation*}
 i.e., the total resource allocated to any application $j \in \mathcal{M}$ is the sum of resources allocated to application $j$ from all service providers.  The resource sharing and allocation algorithm, based on resource requests and  capacities of service providers, has to make an allocation that optimizes  utilities of all  service providers $n \in \mathcal{N}$ and satisfy user requests as well.  The allocation decision is given by
%$\mathbf{x}_n^1, \cdots, \mathbf{x}_n^{|\mathcal{M}|}$
 $\mathbf{X}=\{\mathbf{X}_1, \mathbf{X}_2, \cdots, \mathbf{X}_N\}$, where $\mathbf{X}_n,\; \forall n \in \mathcal{N}$ is given by: 

\begin{equation}
\label{eq:X}
\mathbf{X}_{n}=\Biggl[\begin{smallmatrix}
\mathbf{x}^{1}_n\\ 
.\\ 
.\\ 
.\\
\mathbf{x}^{|\mathcal{{M}}|}_n
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{n,1}^{1} & \cdots  &\cdots   & x^{1}_{n,{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{n,1}^{|\mathcal{{M}}|}&\cdots  &\cdots   & x_{n,K}^{|\mathcal{{M}}|}
\end{smallmatrix}\Biggr].
\end{equation}
%In  the case of resource sharing among service providers,  
Each service provider aims to  maximize the sum of utilities by  allocating its resources to its native applications, and  allocating resources  to  applications belonging to other service providers. %; and c) improving its applications' satisfaction by using its own resources or borrowing from other service providers (if needed).  
Each provider $n \in \mathcal{{N}}$ solves the following multi-objective optimization problem.  
 
 


\begin{subequations}\label{eq:opt_higher}
	\begin{align}
	\max_{\mathbf{X}_n}\quad& \sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)- u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big) \nonumber \\
	&+\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)\nonumber\\
	&- D^l({x}_{n,k}^l)\big)\Big), \label{eq:obj}\\ 
	\text{s.t.}\quad 
& \sum_{j} x_{n,k}^{j}\leq C_{n,k}, \quad \forall\;  k \in \mathcal{K}, n \in \mathcal{N}, \label{eq:obj1} \displaybreak[0]\\
	& \sum_{m \in \mathcal{N}}x_{m,k}^{j} \leq r_{n,k}^{j}, \quad \forall\; j\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N},  \label{eq:obj2}\displaybreak[1]\\
	&  x_{n,k}^{j} \geq 0, \quad \forall\; j\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}, \label{eq:obj3} \displaybreak[2]\\
	& u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-
	u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)- \nonumber \\
	& D^l({x}_{n,k}^l)\geq0, \forall l \in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, n \in \mathcal{N}\label{eq:obj4} .
	\end{align}
\end{subequations}
The first summation term in \eqref{eq:obj} represents the utility earned by an ESP providing resources to the native applications, whereas the second summation term describes the utility earned by providing resources to non-native applications. 
 Note that constraint \eqref{eq:obj1} indicates that the total allocated resources cannot exceed the resource capacity of the service providers. \eqref{eq:obj2} states that the total amount of resources allocated to any application using the resource-sharing framework cannot exceed the amount of  requested resources. \eqref{eq:obj3}  says that the resource allocation cannot be negative  whereas \eqref{eq:obj4} indicates that the incremental increase in utility earned by providing resources to non-native applications should be non-negative. 
 
 \subsection{Assumptions}\label{sec:assumption}
 In our model, we assume that  each utility is a  concave injective function  for which the inverse of the first derivative exists, such as $(1-e^{-x})$. % or $\ln(x)$.
Strictly speaking,  our centralized NBS framework requires only concave injective utility functions\cite{yaiche2000game}. However,  the existence of the inverse of the first derivative is required for the distributed NBS (see details in Section \ref{sec:nbs}).  The communication cost is a convex function, hence the objective function in \eqref{eq:opt_higher} is  concave. 
% We also assume that all of the applications collectively demand more resources than the resource capacity of ESPs.  Hence, 
All resources are fully utilized in the  optimal solution.  However, there are enough resources to provide a positive utility to all  service providers when sharing resources.  This is a realistic assumption as the demand for resources is usually more than the supply.  %The single objective optimization problem in \eqref{eq:opt_single} is feasible for all the CSPs $n \in \mathcal{N}$. 
 Furthermore, we assume that when ESPs share resources,  there exist solutions that are better than when they are all  working alone. This assumption can be relaxed, that is, if certain ESPs cannot improve their utility using the bargaining solution, they will not  participate in the resource sharing framework. However, the framework can still be used for the remaining  ESPs. 
 
 
 \subsection{Choice of  utility function}
  While our framework works with any utility that satisfies the conditions in Section \ref{sec:assumption}, choosing a suitable utility function along with the communication cost can minimize \emph{resource fragmentation}\footnote{We define resource fragmentation as the process in which  resources provided to an application $j$ are split across multiple ESPs rather than a single ESP. }. %We use the term resource fragmentation for the case, where any application $j$ that needs $b$ units of  resource $k$ obtains the required $b$ amount from different ESPs rather than one ESP.} 
 Generally, a concave utility has a steeper slope at start that becomes flatter as more resources are allocated, i.e., the rate of increase in the payoff for allocating  resources reduces with increase in the amount of allocated resources.  This results in  an ESP providing a fraction of originally requested resources to an application and keeping the remaining resources for other applications. Hence, the application  does not get all the resources it needed, and has to ask another ESP for more resources, resulting in resource fragmentation. 
 For example, assume that two applications require $4$ units of a particular resource  from ESP $n$ that only has $3$ units available. Due to the nature of many concave utilities, ESP $n$ for maximizing its utility will provide part of its resources to one application and the remaining resources to the other application rather than providing all $3$ available units to one application and borrowing resources for the other application. This causes resource fragmentation, i.e., both  applications received only a part of the required resources and they will need to obtain the remaining amount from other ESP(s). To avoid such problems, we propose that the utility function should consider:
  \begin{itemize}
  	\item Minimum acceptable amount of resources: The ESPs should earn either zero utility or a negative utility if the resources provided are not within $\delta$ units of the  requested resource $r_{n,k}^j$. Rather than using a utility function such as  $1-e^{-(x_{n,k}^j)}$ that pays  the ESP even when a small amount of resources are provided, it is better to use $1-e^{-(x_{n,k}^j-r_{n,k}^j +\delta)}$  that becomes positive only when the allocation $x_{n,k}^j$ is within $\delta_t$ units of the requested resource $r_{n,k}^j$. Such a utility along  with the communication cost helps minimize the aforementioned fragmentation problem. 
  	%\item Total resources allocated across all ESPs: Each ESP should consider resources allocated at other ESPs  to avoid over-estimating its profit, since  the pay-off for many concave utilities increases drastically at start and rate of increase in utility decreases as more resources are allocated.   ESPs should share information about the amount of resources they allocated to a particular application $j$ to satisfy SLA and then divide the utility on the basis of  resources allocated to application $j$ by each ESP. 
  \end{itemize} 
  


==> arxiv version/03-opt-problem.tex <==
%In this section, we first present the resource allocation problem for a single domain (no resource sharing with other domains). Then we present MOO resource sharing and allocation problem for the coalition. 
For a single domain $n \in \mathcal{N}$ (not  part of a coalition), the allocation decision matrix $X_{SO}^{(n)}$, where $SO$ stands for single objective,  is given by 

\begin{equation}
\label{eq:X_n}
X_{SO}^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{{M}_n}}^{(n)}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{{M}_n}1}^{(n)}&\cdots  &\cdots   & x_{{{M}_n}{K}}^{(n)}
\end{smallmatrix}\Biggr].
\end{equation}
%where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$. 



The optimization problem is: %given in Equation~\eqref{eq:opt_single}
\begin{subequations}\label{eq:opt_single}
	\begin{align}
	\max_{{X}_{SO}^{(n)}}\quad& u_n({X}_{SO}^{(n)}) \label{eq:objsingle}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall i \in \mathcal{M}_n, \label{eq:singlefirst} \displaybreak[0]\\
	& x_{ik}^{(n)} \leq r^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecond} \displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}. \label{eq:singlethird} \displaybreak[2]
	\end{align}
\end{subequations}
The goal of this single objective optimization problem is for every domain  to  maximize its utility by allocating available resources only to its own applications. %The first constraint \eqref{eq:singlefirst} indicates that the allocated resources to all the users $i \in \mathcal{M}_n$ cannot be more than the capacity. The second constraint \eqref{eq:singlesecond} indicates that the allocated resources cannot be more than the required resources, while the final constraint \eqref{eq:singlethird} indicates that the allocation cannot be negative.  
\par Next, we present the resource allocation problem for different domains that share their resources with each other. In the resource sharing case,  each domain aims to  maximize sum of utilities obtained by a) allocating resources to its native applications i.e., $u_n({X}_{i \in \mathcal{M}_n}^{(n)})$ where ${X}_{i \in \mathcal{M}_n}^{(n)}$ represents the allocation decision at domain $n$ for applications $i \in \mathcal{M}_n$, and b) allocating resources to  applications of other domains i.e.,  $u_j^n({X}_{i \in \mathcal{M}_j}^{(n)}),\; \forall j\in \mathcal{N}\backslash n$, where ${X}_{i \in \mathcal{M}_j}^{(n)}$ represents the allocation of resources to applications $i \in \mathcal{M}_j, \; \forall j \in \mathcal{N}\backslash n$  at domain $n$. This leads to: 
% in Equation~\eqref{eq:opt_higher}.  
\begin{subequations}\label{eq:opt_higher}
	\begin{align}
	\max_{\mathcal{X}}\quad&  \bigg(u_n({X}_{i \in \mathcal{M}_n}^{(n)})+ \sum_{j \in \mathcal{N}\backslash n}  u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})\bigg) \quad \forall n \in \mathcal{N} \label{eq:obj}\\%\{u_1(\mathcal{A}),u_2(\mathcal{A}),\cdots,u_N(\mathcal{A})\} \label{eq:obj}\\%U(A)\label{eq:obj}\\
	\text{s.t.}\quad & \sum_{i \in \mathcal{M}} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall n \in \mathcal{N},  \label{eq:obj1} \displaybreak[0]\\
	& \sum_{n \in \mathcal{N}}x_{ik}^{(n)} \leq r^{}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K},  \label{eq:obj2}\displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}. \label{eq:obj3} \displaybreak[2]
	\end{align}
\end{subequations}
%\begin{itemize}
% so that each enclaves first facilitates its own users and then assign the remaining resource to the users of other enclaves. $w_n +w'_{n}=1$  where $w_n > w'_{n}$. E.g., $w_n=0.8$ and $w'_{n}=0.2$ would mean that each enclave has an incentive to first satisfy its own users (higher utility) and then share the excess resources for other users $j \in \mathcal{N}\backslash n $
%	\item 
The first constraint in both optimization problems, \eqref{eq:opt_single}  and \eqref{eq:opt_higher}, indicates that the allocated resources cannot be more than the capacity. The second constraint  in \eqref{eq:singlesecond} and \eqref{eq:obj2} indicates, that the allocated resources should not be more than the required resources.  The last constraint, \eqref{eq:singlethird} and \eqref{eq:obj3},  indicates that allocation decision cannot be negative. 

The utility $u_n({X}_{i \in \mathcal{M}_n}^{(n)})$ given in \eqref{eq:obj}, that each player receives, is a payment that all users $i \in \mathcal{M}_n$  who use the resources pay the player. %Users of other domains $j \in \mathcal{N}\backslash n $ that use resources of domain $n$  will be charged at a rate that player $j$ would have charged the user $i \in \mathcal{M}_j$, had the request been fulfilled by player $j$. Hence, 
 $u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})$ is the utility that domain $n$ receives for sharing its resources with domain $j$. %There are different ways to capture this profit. However, for now, we can say that it would be equivalent to whatever domain $j$ would have earned had it satisfied the requests itself (however it can't as it does not have resources, so it borrows resources from domain $n$ and assigns all the profit it gains from the users to player $n$). 
 %We also assume that th
%\vspace{-0.02in}
\subsection{Assumptions}\label{sec:assumption}
 In our model, we assume that  utilities are  concave injective functions  for which the inverse of first derivative exists, such as $(1-e^{-x})$. While our centralized NBS framework requires only concave injective utility function, the existence of first derivative's inverse is required for the distributed NBS (details in Section \ref{sec:nbs}).  
 We also assume that  resources required by different applications are more than the capacity of domains. Hence, all resources are fully utilized at the optimal solution.   The single objective optimization problem in \eqref{eq:opt_single} is feasible for all the players $n \in \mathcal{N}$. Furthermore, we assume that  there exists solutions that are better than the disagreement point for all the players. 
% that retain the concavity and $1-1$ property after taking the first derivative as well. 
%	\item  $w_n$ is the weight assigned to the utility of player $n$. $\zeta_n$ is the weight assigned to the utility $u^{n}_j(\mathcal{X})$. 
%\end{itemize}
%The optimization problem in Equation~\eqref{eq:opt_higher} is a modified scalarized MOO problem \cite{cho2017survey}. 
\begin{comment}
Before we get into the details of solving the problem, we present an example to understand this
\begin{example}
Let's say we have two different data centers owned by service provider $A$ and $B$ respectively ($A$ and $B$ are game players). Resources available at domain $A$ and $B$ are represented by  $C^{A}$ and $C^{B}$ respectively.  Users in sets $\mathcal{M}_{A}$ and $\mathcal{M}_{B}$ ask for resources and pay a certain price (profit for data centers)  $u_A(\mathcal{X})$ and $u_B(\mathcal{X})$. However, let's say $A$ has scarce resources while $B$ has excess resources. So by forming a coalition, users in $\mathcal{M}_s \subset\mathcal{M}_{A}$ that can't be satisfied by $A$ will be provided resources by $B$ without the users realizing who are providing the resources (since the coalition will make everything appear as one to the user). The profit that $B$ will earn for providing its resources will be equivalent to the profit $A$ would have earned (as $A$ has agreed upon a certain contract with its users $\mathcal{M}_{A}$) had it satisfied the user's request itself. So for $B$, it will earn utility $u_B(X)$ for satisfying its own users plus $u_A^B(X^{\mathcal{M}_s})$ (slight abuse of notation where $X^{\mathcal{M}_s}$ represents the allocation decision for users ${\mathcal{M}_s}$ in domain $B$) for satisfying the users $\mathcal{M}_s \subset\mathcal{M}_{A}$. So this added utility $u_A^B(X^{\mathcal{M}_s})$ is the pay-off for $B$ to share resources. This coalition clearly helps both. $A$ increases its customer satisfaction (as per the contract $A$ had agreed to provide resources to all the users $\mathcal{M}_{A}$), while $B$ earns extra using its excess resources. So it is a stable coalition.
\end{example}

\begin{example}[Utility Example]
For any two players \{1,2\},  $u_1 (\mathcal{X})$ will be given by 
\begin{equation}
u_1(\mathcal{X})=\sum_{i \in \mathcal{M}_1}\bigg(\prod_{k=1}^{{K}}\frac{1}{1+e^{-m(x_{ik}^{(1)}-R^{(1)}_{req,ik})}}\bigg)
\end{equation}
$u_2 (\mathcal{X})$ will be given by 
\begin{equation}
u_2(\mathcal{X})=\sum_{i \in \mathcal{M}_2}\bigg(\prod_{k=1}^{|\mathcal{K}|}(1-e^{-(\frac{1}{R^{(2)}_{req,ik}})x_{ik}^{(2)}})\bigg)
\end{equation}
 $u_2^{\mathcal{X}} (\mathcal{X})$ will be given by 
 \begin{equation}
 u_2^{1}(\mathcal{X})=\sum_{i \in \mathcal{M}_2}\bigg(\prod_{k=1}^{|\mathcal{K}|}(1-e^{-(\frac{1}{R^{(2)}_{req,ik}})x_{ik}^{(1)}})\bigg)
 \end{equation}
  $u_1^{\mathcal{X}} (\mathcal{X})$ will be given by 
  \begin{equation}
  u_1^{2}(\mathcal{X})=\sum_{i \in \mathcal{M}_1}\bigg(\prod_{k=1}^{{K}}\frac{1}{1+e^{-m(x_{ik}^{(2)}-R^{(1)}_{req,ik})}}\bigg)
  \end{equation}
\end{example}
\end{comment}


%\subsection{Choice of Utility Function for Resource Allocation Problem}
%The resource allocation problem can be represented using a \emph{monotone non-decreasing utility function}. This is because in the systems that we consider, such as a cloud service provider or a cellular communication system etc.,  the more the resources provided, the higher is the gain or utility for the service provider. It is highly unlikely that the utility of any service provider will decrease with increase in the amount of resources allocated.  


%satisfying user requests increases the gain or utility for the service provider.  increases with increase in the amount of resources allocated to the user. It is highly unlikely for any r
\begin{comment}
\subsection{Game Theoretic Solution}

We first define the characteristic function $v$ for our game that can solve  problem in~\eqref{eq:opt_higher} 
\begin{align} \label{eq:payoff_function}
v(\mathcal{N})=\sum_{\substack{\text{$n \in \mathcal{N}$} \\ \text{$C_{k}= \sum_{n \in \mathcal{N}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in \mathcal{N}$}\\ \text{$\sum_{j \in \mathcal{N}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}$}}}\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in \mathcal{N},j\neq n} u^{n}_j(\mathcal{X})\bigg)
\end{align}
\begin{remark}
	The characteristic function in Equation~\eqref{eq:payoff_function} is for the grand coalition $\mathcal{N}$. For any $S \subseteq \mathcal{N}$, the characteristic function will be 
\end{remark}
\begin{align} \label{eq:payoff_s_function}
v({S})=\sum_{\substack{\text{$n \in {S}$} \\ \text{$C_{k}= \sum_{n \in {S}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {S}$}\\ \text{$\sum_{j \in {S}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S}$}}} \bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in S,j\neq n} u^{n}_j(\mathcal{X})\bigg)
\end{align}
\begin{theorem}
%	A Cooperative game $(\mathcal{N}, v)$ of $\mathcal{N}$ players and $v$ payoff function that can be used to solve the multi-objective optimization problem given in \eqref{eq:opt_higher}, is canonical\footnote{for monotonically non-decreasing utilities/pay-off function} with Transferable utility
Resource allocation and sharing problem (with multiple objectives) in aforementioned settings can be modeled as a canonical cooperative game with TU. 
\end{theorem}
\begin{proof}
To prove this, we need to show that the characteristic function of resource sharing and allocation problem satisfies the following two conditions
%	For a game to be canonical, we need to prove that the game  is superadditive and the payoff function is of characteristic form. 
	\begin{itemize}
		\item \textbf{Characteristic form of payoff:} As the utility function in a resource sharing and allocation problem  only relies on the domains that are part of the coalition, the game or payoff function is of characteristic form
		\item \textbf{Superadditivity:} Super-additivity for TU games requires $v(S_1 \cup S_2 )\geq v(S_1)+V(S_2) \; \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, s.t. S_1\cap S_2 =\emptyset$ i.e. we have to prove that the pay-off or utility for a domain in the coalition is as good as domain working alone or in a smaller coalition. Due to monotonicity property of the utility functions used,  for all  players/domains $n \in \mathcal{N}$,  $u_n(X_n^{NC})\leq u_n(X_n^{C})$ as $X_n^{NC}\subset {X_n^{C}}$ \footnote{because $X_n^{C}$ can contain much more elements due to the increase in $C$ in the coalition} where $X_n^{C}$ and $X_n^{NC}$ are the allocation decisions in  a cooperative game  and independent setting respectively for domain $n$. 
	\end{itemize}
\end{proof}
\begin{lemma}\label{lemma:MOOGame}
A canonical cooperative game $(\mathcal{N}, v)$ with TU can be used to obtain the Pareto-optimal solutions for the multi-objective optimization problem given in \eqref{eq:opt_higher}
\end{lemma}

%Given that the game is canonical, we are going to explore potential solution approaches for such a game. We start with the \emph{Core} \cite{han2012game}. 

To prove Lemma \ref{lemma:MOOGame}, we must show that the core is non-empty for  our canonical game. To do this, we first show that our game is convex. 

\begin{definition}[Convex Games]
	A coalition game is said to be convex if and only if for every player $n \in \mathcal{N}$, the marginal contribution of the player is non-decreasing W.R.T set inclusion. Mathematically, for $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash \{n\}$ 
	\begin{equation}\label{eq:convexgames}
	v(S_1 \cup \{n\})-v(S_1) \leq v(S_2 \cup \{n\})-v(S_2)
	\end{equation} 
\end{definition}
\begin{theorem}
	Our canonical game is convex
\end{theorem}
\begin{proof}
Let us consider two coalition $S_1$ and $S_2$, where $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash\{j\}$ where $j \in \mathcal{N}$. Then we first calculate $v(S_2 \cup \{j\})-v(S_1 \cup \{j\})$
\begin{align}\label{eq:convexityProof}
& \sum_{\substack{\text{$n \in {S_2}$},\; \text{$C_{k}= \sum_{n \in {S_2}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}$}\\ \text{$\sum_{j \in {S_2}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {S_2}, k\neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) - \nonumber \\
& \Bigg(\sum_{\substack{\text{$n \in {S_1}$},\; \text{$C_{k}= \sum_{n \in {S_1}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {S_1}$} \\ \text{$\sum_{j \in {S_1}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_1}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {S_1}, k \neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_1)}(\mathcal{X}) + \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\nonumber \Bigg)\\ 
&= \sum_{\substack{\text{$n \in {S_2}\backslash S_1$}, \text{$C_{k}= \sum_{n \in {S_2}\backslash S_1}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}\backslash S_1$} \\ \text{$\sum_{j \in {S_2 \backslash S_1}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2 \backslash S_1}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {\{S_2 \backslash S_1\}}, k \neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) \nonumber \\
&   + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) - w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X}) \nonumber \\
& = v(S_2)- v(S_1)+ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})  \nonumber \\
& \geq v(S_2)- v(S_1)
\end{align}
	where the last inequality follows from the fact that $ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\geq 0$ (monotonicity of the utility)
\end{proof}
\end{comment}

%Related to the core, there are certain questions that we must answer
\begin{comment}
\begin{enumerate}
	\item Is the core non-empty?
	\item If the core is non-empty and consists of different pay-off allocations, how do we choose any particular pay-off allocation vector? 
\end{enumerate}
Below we attempt to answer these questions



\begin{definition}[Balanced Collection] Let $\Omega$ be a collection of different coalitions. $\Omega$ is considered to be a \emph{balanced collection} if we can find non-negative weights $w_S$ for each $S \in \Omega$ such that for every player $n$ 
	\begin{align}\label{eq:balancedcollection}
	\sum_{S \in \Omega, S \ni n}w_S =1 
	\end{align}
\end{definition}

\begin{definition}[Balanced Game] A game is called balanced if for every balanced collection $\Omega$, the payoff vector $\mathbf{x}$ will be in $V_{\mathcal{N}}$ if $\mathbf{x}_S \in V_S\; \forall S \in \Omega$ 
	%Let $\Omega$ be a collection of different coalitions. $\Omega$ is considered to be a \emph{balanced collection} if we can find non-negative weights $w_S$ for each $S \in \Omega$ such that for every player $n$ 
\end{definition}
\begin{theorem}[Bondareva-Shapley Theorem]\label{thm:BST}
	The core of a game is non-empty if and only if the game is balanced
\end{theorem}


\begin{theorem}
The core for canonical game with our characteristic function(in Equation~\eqref{eq:payoff_function}) is non-empty
\end{theorem}

\begin{proof}
From the definition of characteristic functions for TU games (see \cite{han2012game} for details), $v: 2^{\mathcal{N}}$ \textrightarrow $\mathbb{R}$ with $v(\emptyset)=\emptyset$. This means that the total number of coalitions possible for $\mathcal{N}$ players is $2^{|\mathcal{N}|}-1$ (we ignore the empty set). For $\Omega$, the non-negative weights $w_S$ which satisfy the condition for  balanced collection in Equation~\eqref{eq:balancedcollection} are given by $\frac{1}{2^{|\mathcal{N}|-1}}$. Hence $\Omega$ is a balanced collection. We also know that $v(S)\subseteq v(\mathcal{N})$ as $v(\mathcal{N})$ is defined over a larger feasible set due to increased amount of available resources. Leveraging the monotonicity property of the utility functions used, we know that any payoff vector  $\mathbf{x}$ will be in $V_{\mathcal{N}}$ if $\mathbf{x}_S$\footnote{$\mathbf{x}_S$ is the projection of $\mathbf{x}$ onto the vector space $\mathbb{R}^{|S|}$} $\in V_S\; \forall S \in \Omega$. Hence our canonical game with characteristic function $v$ in Equation~\eqref{eq:payoff_function} is balanced and its core is non-empty (from Theorem \ref{thm:BST})

\end{proof}
\end{comment}


%For our problem, does the Shapley value lie in the core? To do so we first define \emph{convex games}
\begin{comment}
\begin{theorem}
	The core of any convex game $(\mathcal{N},v)$ is non-empty and large. 
\end{theorem}
\begin{proof}
	Available in \cite{sharkey1982cooperative}
\end{proof}
While the existence of core i.e., core being non-empty, guarantees the grand coalition is stable, finding a suitable allocation from the core is challenging particularly when the core is large (our game). Furthermore, as mentioned earlier, fairness is also a shortcoming of core based solutions.  Shapley value can be  used to obtain a fair allocation, however, we first need to show that the Shapley value lies in the core to guarantee that the Shapley value based allocation is stable for the grand coalition. 
\begin{theorem}
	The Shapley value in Equation~\eqref{eq:shapleyvalue} lies in the core of our canonical game
\end{theorem}
\begin{proof}
	Since our canonical game is convex, the Shapley value lies in the core \cite{han2012game} (see \cite{roger1991game} for details)
\end{proof}
We summarize this in the remark below. 
\begin{remark}
If a TU game $(\mathcal{N}, v)$ is convex, then the core is non-empty and the Shapley Value lies in the core \cite{garg2013novel}.	
\end{remark}
Calculation of Shapley value given in Equation~\eqref{eq:shapleyvalue} is challenging \cite{han2012game}. Since our game is convex, calculating its Shapley value is slightly easier as given below. 

%Now that we have proved that the game is convex, we divert our attention to the calculation of Shapley value for a convex game. 


\subsubsection{Shapley Value for a Convex Game}
Let $\pi$ denote the permutation of players in our game.  Then for any permutation $p$ from the total possible permutations $|\mathcal{N}|!$, one can obtain the initial segments of ordering by \cite{garg2013novel}
\begin{equation}\label{eq:initialsegment}
O_{\pi, r}=\{ n \in \mathcal{N} : \pi(n) \leq r \}, \; r \in \{1, \cdots, N\}
\end{equation}
where $O_{\pi, 0}=\{\}$ and $O_{\pi, |\mathcal{N}|} =\mathcal{N}$. $\pi(n)$ refers to the position of the player $n$ in the permutation $\pi$. The core of any particular ordering $\pi$ can be obtained by solving  equations
\begin{equation}
\label{eq:x_i_pi_sol}
x_n^{\pi}(O_{\pi, r}) = v(O_{\pi, r}), \; r \in \{ 1, \cdots, N\}
\end{equation}
The solution to  above Equations~\eqref{eq:x_i_pi_sol} will result in a payoff vector $x^{\pi}$ where the elements of the vector are given by 
\begin{equation}
\label{eq:vectorelements}
x_n^{\pi}=v(O_{\pi, \pi(n)})- v(O_{\pi, \pi(n)-1}), \quad \forall n \in \mathcal{N} 
\end{equation}
The payoff vectors $x^{\pi}$ represent the extreme points of the core in convex games \cite{garg2013novel}. So if $\prod$ represents the set of all possible permutations of $\mathcal{N}$, the Shapley value of any player $n$ can be calculated as 
\begin{equation}
\label{eq:shapleyconvex}
\phi_n=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} x_n^{\pi}
\end{equation}
\begin{comment}
So for our coalition game $(\mathcal{N},v)$, the Shapley value is 
\begin{align}
\label{eq:ourshapleyconvex}
\phi_n&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} \bigg( \sum_{\substack{\text{$n \in {O_{\pi, \pi(n)}}$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)}}$} \\ \text{$$}\text{$\sum_{j \in {O_{\pi, \pi(n)}}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in O_{\pi, \pi(n)}$}}}\bigg(w_n u_n^{(\pi)}(\mathcal{A})+ w'_{n}\sum_{j \in {O_{\pi, \pi(n)}}, j \neq  n} u^{n,(\pi)}_j(\mathcal{A})\bigg)- \nonumber \\
&\Bigg(\sum_{\substack{\text{$n \in {O_{\pi, \pi(n)-1}}$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)-1}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)-1}}$}}}\bigg(w_n u^{(\pi)}_n(\mathcal{A})+ w'_{n}\sum_{j \in {O_{\pi, \pi(n)-1}}, j \neq n} u^{n,(\pi)}_j(\mathcal{A})\bigg)\Bigg) \nonumber \\
&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} \bigg( \sum_{\substack{\text{$n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1} }$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}$} \\ \text{$\sum_{j \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}$} }}\bigg(w_n u^{(\pi)}_n(\mathcal{A})+  \nonumber \\ 
& w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{n,(\pi)}_j(\mathcal{A}) +  w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{j,(\pi)}_n(\mathcal{A})  \bigg)\bigg) \nonumber \\
&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod}\bigg(w_nu^{(\pi)}_n(\mathcal{A})+ w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{n,(\pi)}_j(\mathcal{A}) +w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{j,(\pi)}_n(\mathcal{A}) \bigg) 
\end{align}
where Equation~\eqref{eq:ourshapleyconvex} provides the Shapley value for our convex game. It is evident that our Shapley value depends on the utility of the player $n$, the utility  player $n$ achieves by allocating resources to players in $j \in O_{\pi, \pi(n)}, j \neq n $ and the utility player $j \neq n, j \in O_{\pi, \pi(n)}$ achieves by allocating resources to player $n$  in every possible permutation. 

\begin{comment}
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $tt$ 
		\State \textbf{Output}: The optimal hit probabilities
		\State \textbf{Step $1$:}  $t \leftarrow$0, $\boldsymbol{\lambda^{(t)}\leftarrow\lambda_0}$, $\boldsymbol{\mu^{(t)}\leftarrow\mu_0}$
		\While{Equation \eqref{eq:gradient1} $\neq$ 0}%$\partial L(\boldsymbol{h,\lambda,\mu})/\partial \lambda_{l} \neq0$ $\&\& $ $\partial L(\boldsymbol{h,\lambda,\mu})/\partial \mu_{ip} \neq0$}
		\State \textbf{Step $2$}:$\boldsymbol{h_{il}^{(p)}[t]} \leftarrow \frac{w_i\beta^{|p|-l}}{\lambda_{l}[t-1]\Bigg(\prod_{\substack{q \neq p,\\ q:l\in\{1,\cdots,|q|\}}}(1-h_{il}^{(q)}[t-1])\Bigg)+\mu_{ip}[t-1]}. $ %Algorithm 2($\boldsymbol{\lambda^{(t)},\mu^{(t)}}$) %\Comment{The node id and file content to Algorithm \ref{algo:alg1} for calculating the price function using~(\ref{eq:gradient2}) }
		\State \textbf{Step $3$:} Update $\lambda$ and $\mu$ using  \eqref{eq:update},  t $\leftarrow t+1$
		%	\State \textbf{Step $4$}: $\boldsymbol \tau_{\chi} \longleftarrow \text{Convex}(\text{slave},\boldsymbol u_{\chi})$ \Comment{Solve the slave optimization problem for $\boldsymbol \tau_{\chi}$  }
		%	\State \textbf{Step $5$}: $(\boldsymbol b_{\chi}, \boldsymbol{\delta_{\chi}}, \text{obj}_{\chi})  \longleftarrow \text{Rounding}(\boldsymbol u_{\chi},\boldsymbol \tau_{\chi})$ \Comment{Round the values of $\boldsymbol u_{\chi}$, remap $\boldsymbol u_{\chi}, \boldsymbol \tau_{\chi}$ to $\boldsymbol{b}_{\chi}$ and $ \boldsymbol{\delta}_{\chi}$ and obtain the new objective function value  }
		\EndWhile
	\end{algorithmic}
	\caption{Iterative Distributed Algorithm}
	\label{algo:alg}
\end{algorithm}
\end{comment}
\begin{comment}
\begin{remark}
	Shapley value calculation for our convex game requires solving at least $2^{N}-1$ optimization problems
\end{remark}
Algorithm \ref{algo:alg1} provides an overview of our proposed approach. We obtain $R, C$ and the utility of all players as $\mathbf{u}$. We initialize each player's utility value ($\mathbf{u}(R,\mathcal{X})$), Shapley value ($\boldsymbol{\phi} $) and resource allocation decision $\mathcal{X}$ to $0$. Then we calculate the Shapley value for the players and assign it to $\mathbf{u}(R,\mathcal{X})$. Finally to obtain $\mathcal{X}$, we take the inverse function of $\mathbf{u}$. As we are using monotone utilities, we know that the inverse of the utilities exist.

\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0, $ \boldsymbol{\phi} \leftarrow$0,  
		\State \textbf{Step $1$:}  Calculate Shapley Value $\phi_n$ using Equation \eqref{eq:shapleyconvex} $\forall n \in \mathcal{N}$
		\State \textbf{Step $2$:} $ \mathbf{u}(R,\mathcal{X}) \leftarrow \boldsymbol{\phi}$
		\State \textbf{Step $3$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{Shapley Value based Resource Allocation}
	\label{algo:alg1}
\end{algorithm}
%It is worth mentioning here that the Shapley value will only provide us the utility each player is going to receive that lies in the core (as a result of cooperation). The allocation decision can be obtained by taking the inverse of utilities.  \par 
\subsubsection{Reducing the Computational Complexity}
As mentioned earlier, that the calculation of Shapley value for our convex game requires at solving at least $2^{N}-1$ optimization problems that is computationally expensive. To reduce the complexity, we propose a computationally efficient approach in Algorithm 2 that requires solving $2N$ optimization problems i.e. $\mathcal{O}(N)$.  The input into the algorithm consists of available resources/capacities, user requirements and the utilities of all game players. The output of the algorithm is $\mathcal{X}$. In Step 1, the utility values of the players, the allocation decision,  and two vectors $\boldsymbol{O_1}$ and $\boldsymbol{O_2}$. In Step 2, every player's utility is calculated without any resource sharing i.e. single optimization and the values are stored in the vector $\boldsymbol{O_1}$. Then $C, R$ are updated and we move to Step 4, where we calculated the utilities $u_j^n$'s for all the players with updated $C, R$ and store them in $\boldsymbol{O_2}$. 

\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0, $ \boldsymbol{\phi} \leftarrow$0,  $ \boldsymbol{O_1} \leftarrow$0, $ \boldsymbol{O_2} \leftarrow$0, 
		\State \textbf{Step $2$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_1^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single}}
		\EndFor
		\State \textbf{Step $3$:} Update $C$ and $R$ based on Step 2
		\State \textbf{Step $4$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_2^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single_j}}
		\State Update $C$ and $R$
		\EndFor
		\State \textbf{Step $5$:} $u_n(R,\mathcal{X})\leftarrow O_1^n+O_2^n$ $\forall n \in \mathcal{N}$ 
		\State \textbf{Step $6$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{$\mathcal{O}$($N$) algorithm for obtaining Core's allocation}
	\label{algo:alg2}
\end{algorithm}
\begin{subequations}\label{eq:opt_single_j}
	\begin{align}
	\max_{\mathcal{X}}\quad& \sum_{j\neq n}u_j^n(\mathcal{X}) \quad  \forall n \in \mathcal{N} \label{eq:objsinglej}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall i \in \mathcal{M}\backslash\mathcal{M}_n, \label{eq:singlefirstj} \displaybreak[0]\\
	& x_{ik}^{(n)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecondj} \displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlethirdj} \displaybreak[2]
	\end{align}
\end{subequations}
\begin{theorem}
	The solution obtained from Algorithm \ref{algo:alg2} lies in the \emph{core}
\end{theorem}
\begin{proof}
	To prove the theorem, we need to show that the utilities obtained in Step $5$ of Algorithm \ref{algo:alg2}; a) are individually rational; b) are group rational and c) no players  have the incentive to leave the grand coalition and form another another coalition $S \subset \mathcal{N}$. 
	\paragraph{Individual Rationality} For each player $n \in \mathcal{N}$, the solution $O_1^n$ obtained by solving the optimization problem in Equation \eqref{eq:opt_single} is the utility a player will obtain by working alone i.e. it is $v\{n\}$. The value $O_2^n$ in Step 4 is either zero or positive but cannot be negative due to the nature of utility used i.e. 
	\begin{align}
u_n(R,\mathcal{X})&=O_1^n+O_2^n \quad \forall n \in \mathcal{N} \nonumber \\
u_n(R,\mathcal{X})&\geq O_1^n \quad \forall n \in \mathcal{N}\nonumber 
	\end{align}
	
	
	 Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is individually rational.
	\paragraph{Group Rationality} The value of the grand coalition $v\{\mathcal{N}\}$ as per Equation \eqref{eq:payoff_function} is the sum of utilities $u_n$'s and $u_j^n$'s. Steps 2, 4 and 5 of Algorithm \ref{algo:alg2} obtain the sum of the utilities as well. Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is group rational rational. 
	\par Furthermore, due to super-additivity of the game and monotonic non-decreasing nature of the utilities, no players have the incentive to form a smaller coalition. Hence Algorithm \ref{algo:alg2} provides a solution from the core.  
\end{proof}
\end{comment}
%\vspace{-0.1in}

==> arxiv version/04-exp-results.tex <==




We evaluate the performance of the proposed NBS framework for resource sharing and allocation across several  settings  in Table \ref{tab:settings} where the communication cost between ESPs $1$ and $3$ is higher than the cost between ESP $1$ and $2$, and ESP $2$ and $3$. Each ESP has three different  resources, i.e., storage, communication and computation. The model can be extended to include other  resources/parameters. %We present the results in four different settings as given in Table \ref{tab:settings}. 
We study the proposed framework using both synthetic and real-world data traces \cite{shen2015statistical,kohne2014federatedcloudsim,kohne2016evaluation}. 
For the study with synthetic and real-world data traces,  request matrices and capacity vectors, $\forall n \in \mathcal{N}$ are randomly generated for each setting. % within a pre-specified range\footnote{The larger the number of applications in our simulation settings, the larger is the range for random number generation.}. 
To show the advantage of resource sharing for both synthetic and   data trace,  we set large resource capacities at certain ESPs so that they can improve their utilities by sharing  available resources with other ESPs for meeting the demand of  latter ESPs. 
% ESPs so that they can improve their utilities by  shar the available resources with other CSPs and assist them in meeting demand.   

% While our framework can work with any concave and injective utility function for which the inverse of first derivative exists, the utilities assigned to players in simulation for illustrative purpose are %\vspace{-0.1in}
%\begin{align}\label{eq:utilityPlayers}
%u_n(\mathcal{X})=\sum_{i\in \mathcal{M}_n}\sum_{k=1}^{K}\big(1-e^{-{x_{ik}^{(n)}}}\big),\quad  \forall n \in \mathcal{N}.
%\end{align}
\begin{figure}[h!]
	%	\centering
	\includegraphics[width=0.53\textwidth]{figures/dist2}%withNBS_mod3}
	%	\vspace{-0.1in}
	\caption{Comparison of centralized and distributed algorithms.}
	\protect\label{fig:dist}
	%	\vspace{-0.2in}
\end{figure}


Simulations were run in \texttt{Matlab R2019a} on a \texttt{Core-i7} processor with \texttt{16 GB RAM}. To solve the optimization problems in \eqref{eq:opt_single} and \eqref{eq:objmain2}, we use the \texttt{OPTI-toolbox}\cite{currie2012opti}. %Below, we provide detailed experimental results.
 We  evaluate our proposed algorithms from the perspective of  service providers that are interested in maximizing their utilities and  evaluate the impact of our framework on the applications.	%\vspace{-0.2in} 
 We define  application \emph{request satisfaction} (RS)  as the ratio of  allocated  resources to   requested resources. %, i.e., $x_{n,k}^{j}/r_{n,k}^{j}$. % We define RS as the percentage to which the requests of different applications are satisfied.
% The RS for a single application is $x_{ik}^{(n)}/r_{ik}^{(n)}$. 
 Mathematically, average RS for an ESP $n$ in the resource sharing case  is defined as: %\vspace{-0.1in}
 \begin{align}\label{eq:requestsatisfaction}
 \centering 
 RS_{n}= \frac{\sum_{j \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\big(\frac{\sum_{m \in \mathcal{{N}}}x_{m,k}^{j}}{r_{n,k}^{j}}\big)}{M_nK} \times 100, %\bigg(\big(100-\frac{(r_{ik}^{(n)}-x_{ik}^{(n)})}{r_{ik}^{(n)}}\big)\times 100\bigg)}{M_nK} 
\end{align} 
The utility  and communication cost functions used in simulation are given in \eqref{eq:utility}.

\begin{align}\label{eq:utility}
\centering
u^j(x_{n,k}^j) & = 1-e^{-(x_{n,k}^j-r_{n,k}^j+\delta)}, \nonumber \\
D^j(x_{n,k}^j) &= \frac{x_{n,k}^j}{w},
\end{align}
Here $\delta$ is set to $1$ and weight $w$ is randomly chosen.

 \begin{comment}
Furthermore, the utility each CSP earned by satisfying requests for resources by application $j$ in the simulations is given in \eqref{eq:util}. 

 \begin{align}\label{eq:util}
\centering 
u_n^j(x_{n,k}^j+\sum_{m \in \mathcal{{N}}\backslash n}x_{m,k}^j)= 1-e^{-(x_{n,k}^j+\sum_{m \in \mathcal{{N}}\backslash n}x_{m,k}^j-r_{n,k}^j +\delta t)}
\end{align} 
where $\delta_t$ was set to be $1$ and the communication cost $C_n^l(\boldsymbol{.})$ was  a weighted linear function of the resource allocated at the remote CSP. 
\end{comment}


\begin{table}[]
	\centering
	\caption{Simulation network settings.}
	\begin{tabular}{|l|l|}
		\hline
		\textbf{Setting}   & \textbf{Parameters} \\ \hline
		\textbf{1} & $N=3, M_n=3,\forall n \in \mathcal{N}, K=3$                    \\ \hline
		\textbf{2} & $N=3, M_n=20,\forall n \in \mathcal{N}, K=3$                    \\ \hline
		\textbf{3 (data traces)} & $N=3, M_n=20,\forall n \in \mathcal{N}, K=3$                    \\ \hline
		%	\textbf{3} & $N=3, M_n=100,\forall n \in \mathcal{N}$                    \\ \hline
		%	\textbf{4} & $N=6, M_n=3,\forall n \in \mathcal{N}$                   \\ \hline
	\end{tabular}
	\vspace{-0.2in}
	\label{tab:settings}
\end{table}
%\begin{comment}

%\end{comment}
\begin{figure*}

	%	\centering
	\includegraphics[width=1.02\textwidth]{figures/three3}%withNBS_mod3}
	%	\vspace{-0.1in}
	\caption{Utility, average request satisfaction and average resource utilization for Setting $1$ when ESPs are working alone and using our proposed NBS framework.}
	\protect\label{fig:withNBS1}
%\vspace{0.15in}
\end{figure*}
\begin{figure*}
	%	\centering
	\includegraphics[width=1.02\textwidth]{figures/three20}%withNBS_mod3}
	%	\vspace{-0.1in}
	\caption{Utility, average request satisfaction and average resource utilization for Setting $2$ when ESPs are working alone and using our proposed NBS framework.}
	\protect\label{fig:withNBS2}
	%	\vspace{0.1in}
\end{figure*}
\subsection{Simulations results for synthetic data}
%The efficacy of our distributed algorithm is evaluated using simulations for a $3$ ESP - $3$ application setting  as shown in Figure \ref{fig:dist}.
\subsubsection{{Evaluation of the distributed algorithm}}
%\textbf{\red{[To be added]}}
To validate our results related to strong duality and our proposed distributed algorithm, we obtain the solution for Setting $1$ in Table \ref{tab:settings} using both the central and distributed algorithm as shown in Figure \ref{fig:dist}. It is evident that both the algorithms converge to the same solution, hence the duality gap is zero and our proposed distributed algorithm converges to the global optimal. 

\subsubsection{Utility, resource utilization, request satisfaction and fairness}

To highlight the efficacy of our framework, we compare its performance with a setting where ESPs  work alone (i.e., no resource sharing among ESPs). 
  In particular, we compare ESP utility, the average resource utilization (averaged across all $k$ resources) and the average request satisfaction (averaged across requests of all ESPs applications) in Figures \ref{fig:withNBS1} and \ref{fig:withNBS2} for $3$ and $20$ applications per ESP, respectively. 
%\paragraph{ESP Utility}
%In both Figures \ref{fig:withNBS1} and \ref{fig:withNBS2},  it is evident that the utility of all CSPs improves with resource sharing. 
When ESP $1$  works alone, it has a resource deficit (evident from $100\%$ average resource utilization and  average request satisfaction of less than 60\%  and 80\% in Figures \ref{fig:withNBS1} and \ref{fig:withNBS2}, respectively) whereas ESPs $2$ and $3$ have  resource surpluses as indicated by less than $100\%$ resource utilization and $100\%$ request satisfaction. The resource deficit results in a lower utility and request satisfaction for ESP $1$. 

%When working alone, CSP $1$ has  lower utility due to resource deficit resulting in a lower application satisfaction. 
%is penalized with a negative utility (customer dissatisfaction) due to its resource deficit, hence it has a lower utility.
 On the other hand,  both ESPs $2$ and $3$   achieve  higher utilities by satisfying all their applications when working alone. However, by using our resource sharing framework, the utilities of all ESPs improve as the framework provides optimal resource sharing.  %Utilities of ESPs $2$ and $3$ improve as they  share their resources with ESP $1$, whereas ESP $1$'s utility improves due to improved request satisfaction. 
 For the case with  three applications,  average request satisfaction improves from $86.11\%$ (working alone) to $94.5\%$ (resource sharing) whereas it improves from  $90.9\%$ to $99\%$ for the $20$ application case. It is worth noting  that request satisfaction for native applications of ESPs $2$ and $3$ reduce as these ESPs allocate their resources to applications of ESP $1$ for a higher utility. 
Furthermore,   resource utilizations also increase for the ESPs with resource surpluses as they share their resources with the ESP with a resource deficit. To measure the degree of fairness of the proposed sharing framework, we calculate  \emph{Jain}'s index\footnote{$\frac{1}{|N|}\leq$Jain's index$\leq 1$ where $1$ is the highest value of fairness.} \cite{jain1999throughput,jain1984aquantitative} that is $0.95$ and $0.99$ for the cases with $3$ and $20$ applications. % indicating that our framework has a higher notion of fairness as it is based on NBS. 
Especially for scenarios with a large number of applications, these results reveal  that our framework enables  fair sharing and allocation of resources among ESPs, as one would expect from the product-based fairness as offered by the NBS. 
%\vspace{-0.2in}
\subsection{Results for the data traces}
We use trace files from \emph{fastStorage}, \emph{Rnd} \cite{shen2015statistical}, and \emph{materna} \cite{kohne2014federatedcloudsim,kohne2016evaluation}. 
%The trace files from \cite{shen2015statistical} have two different traces, i.e., \emph{fastStorage} and \emph{Rnd} whereas the trace files from \emph{materna} \cite{kohne2014federatedcloudsim,kohne2016evaluation} contain three datasets of different numbers of VMs.
 We simulate a setting with three different ESPs and randomly extract the normalized resource request information related to the number of CPU cores, the amount of CPU and memory (RAM) for 20 different resource requests  from  \emph{fastStorage}, \emph{Rnd} and \emph{materna} dataset. Since the datasets do not provide the capacities of these service providers, we assign capacities in such a way that fastStorage serves as the ESP with resource deficit while the other two have resource surplus. Figure \ref{fig:withNBS6} shows ESP utilities,  request satisfaction and resource utilization based on  the  data traces. It is evident that ESP utilities  improve  and resource utilizations  increase to satisfy more applications by use of the proposed NBS framework. The average request satisfaction also increases from $83.3\%$ to $92.05\%$ whereas the Jain index is  $0.98$. 
\begin{figure*}
	%	\centering
	\includegraphics[width=1.00\textwidth]{figures/tr1}%withNBS_mod3}
	%	\vspace{-0.1in}
	\caption{Utility, average request satisfaction and average resource utilization for Setting $3$ when ESPs are working alone and using our proposed NBS framework.}
	\protect\label{fig:withNBS6}
	%	\vspace{-0.1in}
\end{figure*}
\begin{comment}
\begin{figure}
%	\centering
	\includegraphics[width=0.4\textwidth]{figures/three20tr.eps}%withNBS_mod3}
	\vspace{-0.1in}
	\caption{Utility of CSPs with trace files.}

		\vspace{-0.2in}
\end{figure}

\begin{figure}
	%\centering
	\subfloat[Utility function\label{fig:withNBS3}]{\includegraphics[width=0.255\textwidth]{figures/three20tr_1.eps}}
	%	\qquad
	\hspace{-0.2in}
	\subfloat[Resource utilization \label{fig:withNBS4}]{\includegraphics[width=0.255\textwidth]{figures/three20tr2_1.eps}}
	\caption{Utility and resource utilization for the trace files (Setting $3$) using our proposed framework. }%
	%\label{fig:example}%
	\protect\label{fig:withNBS6}
	\vspace{-0.25in}
\end{figure}

\end{comment}

\begin{table*}[]
	\centering
	\caption{Comparison of our NBS based resource sharing and allocation framework with other NBS based solutions.}
	\begin{tabular}{|c|p{1.0cm}|p{2.0cm}|c|p{5.5cm}|}
		\hline
		\multirow{2}{*}{\textbf{Reference}} & \multirow{2}{*}{\textbf{Objective}} & \multirow{2}{*}{\textbf{Resource Sharing}} & \multicolumn{2}{c|}{\textbf{Distributed Algorithm}}             \\ \cline{4-5} 
		&                                     &                                            & \textbf{Proposed?}      & \multicolumn{1}{c|}{\textbf{Technique}} \\ \hline
		\multicolumn{1}{|l|}{\cite{yaiche2000game}}              & \multicolumn{1}{l|}{Fair Bandwidth allocation}               & \multicolumn{1}{c|}{$\times$}                      & \multicolumn{1}{c|}{$\checkmark$} & Gradient Projection                                   \\ \hline		
		
		\multicolumn{1}{|l|}{\cite{xu2012general}}              & \multicolumn{1}{l|}{Fairness}               & \multicolumn{1}{c|}{$\times$}                      & \multicolumn{1}{c|}{$\checkmark$} & Dual decomposition and sub-gradient method are used. %The authors consider generic concave utility.                                      
		\\ \hline
		
		\multicolumn{1}{|l|}{\cite{hassan2014virtual}}              & \multicolumn{1}{l|}{Cost and Resource Utilization}               & \multicolumn{1}{c|}{$\times$}                      & \multicolumn{1}{c|}{$\times$} & N/A                                     \\ \hline
		
		\multicolumn{1}{|l|}{\cite{he2013toward}}              & \multicolumn{1}{l|}{Cost and User Experience}               & \multicolumn{1}{c|}{$\times$}                      & \multicolumn{1}{c|}{$\times$} & N/A                                     \\ \hline
		
		\multicolumn{1}{|l|}{\cite{feng2012bargaining}}              & \multicolumn{1}{l|}{Resource utilization}               & \multicolumn{1}{c|}{$\times$}                      & \multicolumn{1}{c|}{$\times$} & N/A                                  \\ \hline		
		
		
		
		
		\multicolumn{1}{|l|}{\cite{guo2013cooperative}}              & \multicolumn{1}{l|}{Bandwidth allocation}               & \multicolumn{1}{c|}{$\times$}                      & \multicolumn{1}{c|}{$\checkmark$} & Gradient Projection                                   \\ \hline		
		
		\multicolumn{1}{|l|}{Our Approach}              & \multicolumn{1}{l|}{Service provider utility and user satisfaction}               & \multicolumn{1}{c|}{$\checkmark$}                      & \multicolumn{1}{c|}{$\checkmark$} & Gradient descent based algorithm that works for the class of utilities described in \ref{sec:assumption}.                                   \\ \hline			
		
	\end{tabular}
	\label{tab:comparison}
\end{table*}



==> arxiv version/05-conclusions.tex <==
The focus in this paper is to optimally utilize available resources for satisfying a larger number of edge applications and improving the utility of edge service providers. We have shown that although ESPs may have different utilities, they should share
resources to improve their utilities and enhance application request satisfaction. Resource sharing among ESPs has been formulated as a bargaining problem and a resource-sharing framework using Nash Bargaining Solution (NBS) has been proposed, which has also been shown to be beneficial for the ESPs. Since a centralized solution for obtaining the NBS may not always be desirable, the strong duality property has been proved, which has enabled us to develop a distributed algorithm for the NBS. Using synthetic and real-world  data traces, we have demonstrated the effectiveness of the proposed framework.  In particular, our results confirm that ESPs with resource
deficits and surpluses can improve their utilities as well as application satisfaction by sharing resources.




==> arxiv version/arxiv version/01-intro.tex <==
\subsection{Motivation}
Edge computing has received much attention recently as it enables on-demand provisioning of computing resources for different applications and tasks at the network edge \cite{shi2014online,shi2016edge,satyanarayanan2017emergence}. One of the fundamental advantages of edge computing is that it can provide resources % to resource constrained applications 
with low latencies when compared with traditional cloud computing architecture \cite{shi2016edge}. The demand for edge computing has further increased due to the advent of Internet of Things (IoT) \cite{atzori2010internet} and wide-scale use of machine and deep learning \cite{li2018learning} in different industries as  these learning-based models can  be trained and run using edge computing nodes with adequate storage and computing power \cite{wang2018edge}. 

\par A typical edge computing system consists of a large number of edge nodes  that have different types of resources. Edge service provider (ESP) earns a \emph{utility} for allocating resources to different applications and guarantees to provide  resources according to a \emph{Service Level Agreement} (SLA). However, when compared with cloud computing systems and data centers, resources in an edge setting are limited. Therefore, optimal use and allocation of these limited resources has been an active area of research. 
Even when resources are available, allocating  them to  applications with the goal of maximizing overall ESP \emph{utility} is a difficult problem. Furthermore, the aforementioned resource intensive paradigms such as deep learning, and data analytics  exacerbate the problem by challenging the scalability of traditional resource allocation techniques. \par 

ESPs typically provide enough resources to different applications at their edge nodes to  meet the peak demand. However, it is highly likely that  resources of one ESP will be over-utilized, while other ESP's resources will be under-utilized.  
For example, an ESP provisions resources to an application at an edge node that is physically closest to the requesting application. However, if the closest edge node has a resource deficit or is overloaded, the request can be satisfied through ESP's next closest edge node that  may physically  be at a distant location or deep in the network such as at the data center. This incurs high cost and  causes high latency that may not be acceptable for delay constrained applications. One possible solution is  to create a shared  resource pool with other ESPs that are  physically closer  \cite{he2018s,openedge,openfog,etsi}. Such a resource pool allows  ESPs to share and use  resources whenever needed to meet their dynamic demands. This cooperation and resource sharing among ESPs seem beneficial for them, because it is unlikely that resources of different ESPs will be   simultaneously over-utilized.
\par  %While we use edge computing paradigm as an illustrative example, 
Our work has also been  motivated by military settings in which two or more  \emph{coalition partners}\footnote{Each coalition partner can be considered an ESP. } are jointly conducting a military operation using different resources from the partners. As military settings usually have strict  latency and reliability requirements, resources are placed at the edge to fulfill the aforementioned requirements. 
Hence, coalition settings can be considered a practical scenario for edge computing. In contrast with commercial edge computing settings, military settings require a higher reliability and robustness to ensure timely availability of resources. 
As seen in Figure \ref{fig:system_model}, both coalition partners $2$ and $3$ satisfy all their applications and have resource surpluses whereas partner $1$ has resource deficits when working alone. However, through cooperation among these coalition partner, $1$ satisfies its applications by using resources of other coalition partners resulting in  an improved utility for all partners. It is evident that if  different coalition partners do not share resources, different application requests cannot be satisfied. Therefore, there is a need for a framework that allows resource sharing among these coalition partners (i.e., ESPs). 
Furthermore, the framework needs to be distributed as a centralized solution may not be acceptable to the different coalition partners or ESPs because:
\begin{itemize}
	\item An adversary can target the central system  causing the entire military operation to fail.
	\item Coalition partners need to reach a consensus  for choosing the \emph{central} node that runs the resource sharing algorithm. 
	\item A centralized framework requires  a large amount of information to be transmitted to the central node. This may not be feasible or preferred by the coalition partners as certain information may be private.  
\end{itemize} 
Such a distributed resource sharing gives rise to a number of questions such as: 
 \begin{enumerate}
 	\item \emph{Should an ESP help another ESP by sharing resources?}
 	\item \emph{How should  resources be allocated to applications across different ESPs, while considering issues such as  communication cost and resource fragmentation? }
 	\item \emph{How can  ESPs share the profits of resource sharing?}
 \end{enumerate}
We  answer these questions in this paper. 
\subsection{Methodology and contributions}
In this paper, we consider a number of ESPs that share their resources and form a  resource pool to satisfy resource requests of different applications as shown in Figure \ref{fig:system_model}.
We formulate such resource sharing and allocation among ESPs as a   multi-objective optimization (MOO) problem, for which our goal is to achieve a Pareto optimal solution.  Furthermore, since Pareto solutions are spread over the \emph{Pareto frontier} \cite{cho2017survey}, choosing a single solution among them is challenging. As the \emph{Nash Bargaining Solution}  (NBS)\cite{nash1950bargaining} guarantees the provision of  a fair and Pareto optimal solution to such a MOO problem,  we develop a distributed NBS-based framework for  resource allocation and sharing here.  \emph{To the best of our knowledge, this is the first generic NBS-based framework for resource sharing and allocation among ESPs. } 

 \begin{figure}
	\centering
	\includegraphics[width=0.49\textwidth]{figures/pool_new2.jpg}
	\vspace{0.05in}
	\caption{Cooperation among ESPs}
	\protect\label{fig:system_model}
	%\vspace{-0.2in}
\end{figure}
The main contributions of this paper are: 
\begin{enumerate}
  
	\item We present an NBS based  resource  sharing framework for ESPs with different objectives in allocating resources to meet the dynamic demands. Our framework also considers practical engineering constraints such as communication costs and resource fragmentation. 
\item We show that ESPs can benefit from sharing resources  with other ESPs as they can earn a higher profit and improve the average application satisfaction.    
\item We  show that  \emph{strong-duality} property holds for the formulated problem, which enables us to propose a distributed  algorithm to obtain the NBS.   
\item 	We evaluate the performance of our algorithms using  synthetic and real world traces.  Results show that resource sharing improves the utilities of ESPs, increases resource utilization and enhances average user (application) satisfaction. Furthermore, our results show that the profit sharing among  ESPs is also fair. 
\end{enumerate}
The rest of this paper is structured as follows. We present the system model in Section~\ref{sec:sysmodel}. 
In Section~\ref{sec:nbs}, we first present a primer on NBS. We then describe our proposed  NBS framework  for resource sharing and allocation. In Section~\ref{sec:dist}, we present a distributed algorithm for obtaining the NBS. In Section~\ref{sec:exp_results}, we present simulation results of the proposed framework for different settings. We describe the related work in Section \ref{sec:related},  
and conclude the paper in Section~\ref{sec:conclusion}. 







==> arxiv version/arxiv version/02-sysmodel.tex <==
Any entity or service provider  that has specific resources such as CPU, storage and communication links can serve as the building block of our system as shown in Figure~\ref{fig:system_model}. We call this basic building block  a \emph{domain}\footnote{Throughout the paper, we will use domain, service provider and player interchangeably.}. The domain can be as small as a sensor and as large as data centers.  Each domain has a \emph{domain controller} that is aware of all resources available within the domain. The domain controller only shares an abstraction of this resource information and does not share the entire information\footnote{This can be due to a number of reasons including security and privacy. For example, Amazon and Dropbox may share limited information to satisfy their user's needs. However, they will not provide the entire information to each other.}. Different domains share resources with  the presence of a \emph{coalition controller}. The coalition controller can be either a separate controller or chosen among  the domain controllers. %Figure \ref{fig:system_model} the model used in this paper.   
Table \ref{tab:notationTable} provides  notation used in this paper. Below, we model our resource allocation and sharing problem from a  game theoretic perspective.   
 \begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{figures/domain}
	\caption{Our system model with domain and coalition controllers}
	\protect\label{fig:system_model}
	\vspace{-0.1in}
\end{figure}

\begin{table}[]
	\caption{List of notations (Not.) used in the paper}
	\begin{tabular}{|p{0.44cm}|p{2.7cm}||p{0.44cm}|p{3.2cm}|}
		\hline
		\textbf{NOT.} & \textbf{Description} & \textbf{NOT.} & \textbf{Description} \\ \hline
	$\mathcal{N}$	& Set of game players                     &        $n$           &Player from set   $\mathcal{N}$  \\ \hline
	$\mathcal{M}$	& Set of applications                     &      $\mathcal{M}_n$             & Set of native applications of player $n$                     \\ \hline
	$\mathcal{K}$	& Set of resource types                     &     $k$              &  Resource from set $\mathcal{K}$                    \\ \hline
	$C^{(n)}$	&  Capacity of player $n$                    &    $C_k^{(n)}$	&  Capacity of $k^{th}$ resource at player $n$           \\ \hline
	$x_{ik}^{(n)}$	&  Resource $k$ allocated to application $i$ by player $n$      &   $r_{ik}^{(n)}$      &     Request for  resource $k$ from application $i$ of player $n$                 \\ \hline
%		&                      &                   &                      \\ \hline
%		&                      &                   &                      \\ \hline
	\end{tabular}
\label{tab:notationTable}
%\vspace{-0.2in}
\end{table}

Let $\mathcal{N}=\{1,2, \cdots, N\}$ be the set of all domains (or service providers) that act as players in our game. We assume that each player has a set of $\mathcal{K}=\{1,2,\cdots, K\}$ different types of resources such as communication, computation and storage resources.  The $n$-th domain reports its available resources $C^n = \{ C_1^{(n)},\cdots, C_K^{(n)}\}$ to a central entity, the coalition controller. Here $C_k^{(n)}$ is the amount of type $k$ resources available to domain $n$.  
%All edge clouds can report their available resources  to any central entity, coalition controller \footnote{Coalition controller can be chosen from the edge clouds.},  where ${C}^{(n)}=\{ {C}_{1}^{(n)}, \cdots, {C}_{K}^{(n)}\}$ represents the available resources $k \in \mathcal{K}$ for the player $n \in \mathcal{N}$. 
Vector $C=\{\sum_{n \in \mathcal{N}}C_{1}^{(n)}, \sum_{n \in \mathcal{N}}C_{2}^{(n)}, \cdots ,\sum_{n \in \mathcal{N}}C_{K}^{(n)}\}$ represents  all available resources in different domains.  Each domain $n$ has a set of  native applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$ that ask for resources. Furthermore, the set of all applications that ask for resources from the set of domains (coalition of domains) is given by $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where $|\mathcal{M}|=M$,  and $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset, \; \forall i \neq j,$ i.e., each application originally asks only  one domain for resources. 
%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
The coalition controller receives a request (requirement) matrix $R^{(n)}$ from every player (domain) $n \in \mathcal{N}$.% \vspace{-0.1in}
\begin{equation}
\label{eq:R_Req}
R^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{r^{(n)}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{(n)}_{{M}_n}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r^{(n)}_{11} & \cdots  &\cdots   & r^{(n)}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{(n)}_{M_{n}1}&\cdots  &\cdots   & r^{(n)}_{{M}_n{K}}
\end{smallmatrix}\Biggr].
\end{equation}
%\vspace{-0.01in}
\noindent where the $i^{th}$ row corresponds to the $i^{th}$ application while  columns represent different resources, i.e., $r_{ij}^{(n)}$ is the amount of $j^{th}$ resource that application $i \in \mathcal{M}_n$ requests.
%The vector ${C}^{(n)}$ received by coalition controller shows different available resources at edge cloud $n$. 
The coalition request matrix $R$ is a combination of all the request matrices (from all the domains)  as given below. 
\begin{equation}
\label{eq:R_Reqco}
R^{}=\Biggl[\begin{smallmatrix}
\mathbf{r^{}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{}_{{M}}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r^{}_{11} & \cdots  &\cdots   & r^{}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{}_{M1}&\cdots  &\cdots   & r^{}_{{M}{K}}
\end{smallmatrix}\Biggr].
\end{equation}
\noindent where $r_{ij}$ is the amount of $j^{th}$ resource that application $i \in \mathcal{M}$ requests.
The coalition, based on $R$ and  $C$, has to make an allocation decision $\mathcal{X}$ that optimizes the utilities of all the domains  $n \in \mathcal{N}$.  The allocation decision for the entire coalition $\mathcal{X}$ consists of all the  allocation decisions $X^{(n)}$ in every domain $n \in \mathcal{N}$ i.e.,  $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$.  
%The allocation decision $\mathcal{X}$ is  given by $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$ indicating how much of each resource $k \in \mathcal{K}$ is allocated to application $i$ at domain $n \in \mathcal{N}$. The matrix $X^{(n)}$ is a combination of different matrices $\{X_{i\in \mathcal{M}_1}^{(n)}, \cdots,X_{i\in \mathcal{M}_n}^{(n)},\cdots, X_{i\in \mathcal{M}_N}^{(n)} \}$, where $X_{i\in \mathcal{M}_n}^{(n)}$ is the allocation decision  at domain $n$ for the applications $i$ originally belonging to domain $n \in \mathcal{N}$ i.e., the original applications of the domain $n$. Furthermore,  $X_{i\in \mathcal{M}_j}^{(n)}$, $\forall j \in \mathcal{N},$ where $j \neq n$, is the allocation decision at domain $n$ for applications $i$ belonging to domain $j$.  
Mathematically,  $X^{(n)}$ is represented by % \eqref{eq:A_n}, where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$.  %Table \ref{tab:notationTable} provides some of the notations used in the paper. 
\begin{equation}
\label{eq:A_n}
X^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{{M}}}^{(n)}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{{M}}1}^{(n)}&\cdots  &\cdots   & x_{{{M}}{K}}^{(n)}
\end{smallmatrix}\Biggr].
\end{equation}
where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$.
% \subsection{Assumptions}



\begin{comment}
Let $\mathcal{N}=\{1,2, \cdots, N\}$ be the set of all the domains that act as players in our game. % For simplicity, we drop the $P$ in $P_n$ and represent the players only with the subscript $n$. 
Each player has a utility function $u_n(\mathcal{X})$ that depends on the allocation decision $X$ (details for $X$ will be given later). We assume that each player has set of $\mathcal{K}=\{1,2,\cdots, K\}$ different resources such as communication, computation and storage resources. %Each player $n \in \mathcal{N}$ has complete information about its own resources $k \in \mathcal{K}$, however it reports only abstract information to a coalition controller 
All domains report their available resources  to the coalition controller where $C^{(n)}$ represent the available resources for the domain/player $n \in \mathcal{N}$. Each domain $n$ has a set of users or applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$ that ask for resources. Also $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset \; \forall i \neq j$ represents the set of all users that ask for resources from the coalition. 

%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
The coalition controller receives a matrix $R^{(n)}$ for every player $n \in \mathcal{N}$ 
	\begin{equation}
\label{eq:R_Req}
R^{(n)}=\Biggl(\begin{smallmatrix}
\mathbf{r^{(n)}_1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r^{(n)}_{{M}_n}}
\end{smallmatrix}\Biggr) = \Biggl(\begin{smallmatrix}
r^{(n)}_{11} & \cdots  &\cdots   & r^{(n)}_{1{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r^{(n)}_{M_{n}1}&\cdots  &\cdots   & r^{(n)}_{{M}_n{K}}
\end{smallmatrix}\Biggr)
\end{equation}
where the $i^{th}$ row corresponds to the $i^{th}$ user while  the columns represent different resources i.e., $r_{ij}$ is the amount of $j^{th}$ resource user $i \in \mathcal{M}$ requests.

The vector ${C}^{(n)}=\{ {C}_{1}^{(n)}, \cdots, {C}_{K}^{(n)}\}$ received by coalition controller shows different available resources at domain $n$. 
The vector $C=\{\sum_{n \in \mathcal{N}}C_{1}^{(n)}, \sum_{n \in \mathcal{N}}C_{2}^{(n)}, \cdots ,\sum_{n \in \mathcal{N}}C_{K}^{(n)}\}$ consists of all the available resources at different domains. The coalition, based on $R$ and  $C$, has to make an allocation decision $\mathcal{X}$ that optimizes the utilities $u_n(\mathcal{X})$ of the domains.  The allocation decision $\mathcal{X}$ is  a vector $\mathcal{X}=\{X^{(1)},X^{(2)},\cdots, X^{(N)}\}$ that shows how much of each resource $k$ is allocated to user $i$ at domains $n \in \mathcal{N}$.

\begin{equation}
\label{eq:A_n}
X^{(n)}=\Biggl(\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{|\mathcal{M}|}}^{(n)}}
\end{smallmatrix}\Biggr) = \Biggl(\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{|\mathcal{M}|}1}^{(n)}&\cdots  &\cdots   & x_{{|\mathcal{M}|}{K}}^{(n)}
\end{smallmatrix}\Biggr)
\end{equation}
where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ allocated  to user $i$ at player $n$

 Since the utilities of different domains might be different (can be conflicting as well), this leads us to a multi-objective optimization (MOO) problem. Some of the assumptions in our model are given below
\subsection{Assumptions}
The assumptions made in our model are 
\begin{enumerate}
	\item The negotiation cost among different domains is negligible
	\item All the domains communicate their information to the coalition controller
	\item The coalition controller already exists% and do not discuss the selection of the coalition controller (can be explored in the future work)
	\item Resources across different domains are additive in nature i.e., if domain $X$ and $Y$ have $2$ GB RAM each, the coalition would have $4$ GB of RAM. 
	\item Each player has a single objective
	\item The objective of the coalition is a sum of the utilities of all the players with equal weight
%	\item Any new player/domain added into the coalition will have resources available
	\item All players or domains have the same number of users or jobs
\end{enumerate}
\end{comment}








==> arxiv version/arxiv version/02-sysmodel2.tex <==
Let $\mathcal{N}=\{1,2, \cdots, N\}$ be the set of all ESPs. 
We assume that each  provider has a set of $\mathcal{K}=\{1,2,\cdots, K\}$  types of resources such as communication, computation and storage resources.  %Service provider  $n$ represents its  available resources as 
$C_{n} = \{ C_{n,1},\cdots, C_{n,K}\}$, with  $C_{n,k}$ denoting the amount of type $k$ resources available at service provider $n$. 

  Each service provider $n$ has a set of  native applications $\mathcal{M}_n= \{1,2,\cdots, M_n\}$. 
The set of all applications that request resources from all service providers  is given by $\mathcal{M}=\mathcal{M}_1\cup\mathcal{M}_2\cdots\cup \mathcal{M}_N , \;$ where we assume  $\mathcal{M}_i \cap \mathcal{M}_j=\emptyset, \; \forall i \neq j,$ i.e., each application initially  demands resources from only  its native service provider. We also define $\overline{\mathcal{M}}$ to represent  $\mathcal{{M}}\backslash \mathcal{{M}}_n$ and $\overline{\mathcal{N}}$ to represent $\mathcal{{N}}\backslash n $.  
%We have $\mathcal{M}=\{1,2,\cdots, M\}$ users that ask for a set of resources to perform any particular task. 
Every ESP  $n \in \mathcal{N}$ has a request (requirement) matrix $R_{n}$,% from every player $n \in \mathcal{N}$ 
\begin{equation}
\label{eq:R_Req}
R_{n}=\Biggl[\begin{smallmatrix}
\mathbf{r_{n}^1}\\ 
.\\ 
.\\ 
.\\
\mathbf{r_{n}^{{M}_n}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
r_{n,1}^{1} & \cdots  &\cdots   & r^{1}_{n,{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
r_{n,1}^{{M}_n}&\cdots  &\cdots   & r_{n,K}^{{M}_n}
\end{smallmatrix}\Biggr],
\end{equation}
%where the $j^{th}$ row corresponds to  application $j$, while  columns represent different resources. That is,
Here  $r_{n,k}^{j}$ is the amount of resource $k$ that application $j \in \mathcal{M}_n$ requires. When an ESP is working alone (no sharing of  its resources with any other service provider),  its objective is to maximize its utility by allocating  resources to its native applications. % and improving application satisfaction.
 A service provider $n$ earns a  utility $u^j (x_{n,k}^j)$ by allocating $x_{n,k}^j$ amount of resource $k$ to application $j\in \mathcal{M}_n$, where the vector $\mathbf{x}_n^j= [x_{n,1}^j, x_{n,2}^j,\cdots, x_{n,K}^j]^T$. 
 Table \ref{tab:not} contains notations used throughout the paper. We present the optimization formulation for a single service provider in Section \ref{sec:prob}, followed by a formulation for the multiple service provider problem in Section \ref{sec:multP}.  %Below we present the optimization formulation for a single service provider. 

%\textbf{Add notation table here}


\begin{table}[]
	\centering
	\caption{List of notations used throughout the paper}
	\begin{tabular}{|p{1cm}|p{6.9cm}|}
		\hline
		\textbf{Notation}	& \textbf{Description} \\ \hline
		$\mathcal{{N}}, N, n$	& Set, number and index of ESPs  \\ \hline
		$\mathcal{K}, K, k$	& Set, number and index of resources \\ \hline
		$\mathcal{M}, M, j$	& Set, number and index of applications \\ \hline
		$\mathcal{M}_{n}$	& Set of native applications at ESP $n$  \\ \hline
	%	$\overline{\mathcal{M}}$	& Set of native applications at ESP $n$  \\ \hline
	%	${S}$	& A coalition of game players, where $S \subseteq \mathcal{{N}}$  \\ \hline
		%$\mathcal{M}_{n}$	& Set of native applications at player $n$  \\ \hline
%		$\mathcal{V}$	& Set of payoff vectors    \\ \hline
%		${v}(S)$	& Value of coalition $S$    \\ \hline
%		$\mathcal{G}_1$	& Set of players with resource deficit    \\ \hline
%		$\mathcal{G}_2$	& Set of players with resource surplus   \\ \hline
		$C$	& Capacity vector of all ESPs \\ \hline
		$C_n$	& Capacity vector of ESP $n$ \\ \hline
		$C_{n,k}$	& Capacity of resource $k$ at ESP $n$ \\ \hline
	%	$R$	& Request matrix of all game players \\ \hline
		$R_{n}$	& Request matrix at ESP $n$ \\ \hline
		$r_{n,k}^{j}$	& Request of application $j$ for resource $k$ from ESP $n$ \\ \hline
	%	${X}_{i \in \mathcal{M}_n}^{(n)}$	& Allocation decision matrix at player $n$ for its native applications \\ \hline
	%	${X}_{i \in \mathcal{M}_j}^{(n)}$	& Allocation decision matrix at player $n$ for applications of other players \\ \hline
	%	${X}^{(n)}$	& Allocation decision matrix at player $n$ for all applications (native and applications of other service providers)\\ \hline
	%	$\mathcal{X}_n$	& Allocation decision for all game players  \\ \hline
%		$X_{SO}^{(n)}$	& Single objective allocation decision at $n$  \\ \hline
		$x_{n,k}^{j}$	& Allocation decision of resource $k$ for application $j$ at ESP $n$ \\ \hline
	$\mathbf{x}_{n}^{j}$	& Allocation decision vector for application $j$ at ESP $n$ when working alone, i.e., $\mathbf{x}_{n}^{j}=[x_{n,1}^j, \cdots, x_{n,K}^j]^T$  \\ \hline

	%	$u_{j}^n$	& Utility player $n$ earns by allocating resources to applications of player $j$\\ \hline
	$\mathbf{X}_n$ & Allocation decision for ESP $n$ in the  resource sharing case \\ \hline 
	$\mathbf{X}$ & Allocation decision for the entire set of ESPs  \\ \hline 
	%	$\mathcal{X}_n$ & Allocation decision for player $n$ in the  coalition excluding its native applications \\ \hline	
			$u_{}^j({x}_{n,k}^j)$	& Utility ESP $n$ earns  by allocating resource $k$ to application $j$ \\ \hline
		$u_{}^j(\mathbf{x}_{n}^j)$	& Utility ESP  $n$ earns  by allocating vector of  resources to application $j$ \\ \hline
	%	$GC$	& Grand coalition\\ \hline
	%	$RS$ & Request satisfiability\\ \hline
	%	$TU$ & Transferable utility\\ \hline
	%	$NTU$ & Non-transferable utility\\ \hline
	%	$CGT$ & Cooperative game theory\\ \hline
	%	$MOO$ & Multi-objective optimization\\ \hline
	%	$SOO$ & Single-objective optimization\\ \hline
	%	$MEC$ & Mobile edge cloud\\ \hline
	\end{tabular}
	\label{tab:not}
\end{table}


\subsection{Problem Formulation for Single Service Provider } \label{sec:prob}
 We  first present the resource allocation problem for a stand-alone single service provider (i.e., no resource sharing with other service providers). 
For a single ESP $n \in \mathcal{N}$, the allocation decision  consists of  vectors $\mathbf{x}_n^1, \cdots, \mathbf{x}_n^{M_n}$. The optimization problem is: 
\begin{subequations}\label{eq:opt_single}
	\begin{align}
	\centering
%	\max_{\mathbf{x}_n^1, \cdots, \mathbf{x}_n^{M_n}}\quad& \sum_{j \in \mathcal{M}_n}\Big(u_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}} \frac{x_{n,k}^{j}}{r_{k}^{j}}\Big), \label{eq:objsingle}\\
\max_{\mathbf{x}_n^1, \cdots, \mathbf{x}_n^{M_n}}\quad& \sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}u^j({x}_{n,k}^j), \label{eq:objsingle}\\
	\text{s.t.}\quad & \sum_{j} x_{n,k}^{j}\leq C_{n,k}, \quad \forall k \in \mathcal{K}, \label{eq:singlefirst} \displaybreak[0]\\
	& x_{n,k}^{j} \leq r^{j}_{n,k}, \quad \forall\; j\in \mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecond} \displaybreak[1]\\
	&  x_{n,k}^{j} \geq 0, \quad \forall\; j\in \mathcal{M}_n, k \in \mathcal{K}. \label{eq:singlethird} \displaybreak[2]
	\end{align}
\end{subequations}
The goal of a single service provider in solving this single objective optimization (SOO) problem, as mentioned earlier,  is   to  maximize its utility by appropriately allocating  resources. %$ \sum_{j \in \mathcal{M}_n}\sum_{k \in \mathcal{K}} \frac{x_{n,k}^{j}}{r_{k}^{j}}$ captures the satisfaction of resource requests by applications. 
The first constraint  \eqref{eq:singlefirst} indicates that  allocated resources cannot exceed capacity. The second constraint   \eqref{eq:singlesecond} reflects that allocated resources should not exceed the requested amounts.  The last constraint, \eqref{eq:singlethird}  says the allocation  cannot be negative. However, it is possible that a service provider $n$ may 
earn a larger utility by providing its resources to applications of other service providers or it may not have sufficient resources to satisfy  requests of all its native applications. On the other hand, there may be another service provider $m\in \mathcal{{N}}\backslash n$ that may have a surplus of resources, which can be ``rented" by service provider $n$. %In this work, we focus on the strategy where each service provider has to allocate resources to its native applications and then share the remaining (if any) resources with other service providers who are not able to satisfy their native applications. 
Below, we discuss  resource sharing among these service providers. 


\subsection{Multiple Service Providers Problem Formulation}\label{sec:multP}
%We assume that a service provider $n$ does not have sufficient resources to satisfy all its native applications, while another service provider $m$ may have resource surpluses, which can be shared with provider $n$. Therefore, 
Allowing resource sharing among  service providers, while considering their objectives, could improve resource utilization and  application satisfaction. 
Let $D^j(x_{n,k}^j)$ denote the communication cost of serving application $j \in  \mathcal{{M}}_m$ at service provider $n$ rather than at its native service provider $m$. 
By sharing its resources, ESP $n$ earns a utility,
\begin{equation}\label{eq:util}
u^j (\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+x_{n,k}^j)-u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j)-D^j(x_{n,k}^j),
\end{equation}
after allocating  $x_{n,k}^j$ for application $j\in \mathcal{{M}}_m$, i.e., the net utility ESP $n$ earns is calculated as the \emph{differential utility} ($u^j (\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+x_{n,k}^j)-u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j)$) earned due to providing  $x_{n,k}^k$ amount of resources minus the communication cost between the native and non-native ESP. 
% the difference of total utility earned considering   resources provided to application $j$ by all ESPs ($u^j (\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+x_{n,k}^j)$), utility  $u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j)$ earned due to resource provided by all ESPs other than ESP $m$\footnote{$ u^j (\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+x_{n,k}^j)-u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j)$ is the \emph{differential utility}, i.e., the increase in  utility by providing  $x_{n,k}^j$ resources.} and the  communication cost $D^j(x_{n,k}^j)$. 
  We assume that  $ u^j (x_{n,k}^j)=u^j (x_{m,k}^j)$ when $x_{n,k}^j=x_{m,k}^j$. %In \eqref{eq:util}, the utility an ESP $m$ earns by allocating 
% \textbf{(This assumption may no longer be needed and we can relax it)}.
% and $d_m^j$ is the distance between service provider $m$ and the native service provider of application $j$.
   We also let
   \begin{equation*}
 \mathbf{x}^j= [\sum_{n \in \mathcal{{N}}}x_{n,1}^j, \sum_{n \in \mathcal{{N}}}x_{n,2}^j,\cdots, \sum_{n \in \mathcal{{N}}}x_{n,K}^j]^T,
   \end{equation*}
 i.e., the total resource allocated to any application $j \in \mathcal{M}$ is the sum of resources allocated to application $j$ from all service providers.  The resource sharing and allocation algorithm, based on resource requests and  capacities of service providers, has to make an allocation that optimizes  utilities of all  service providers $n \in \mathcal{N}$ and satisfy user requests as well.  The allocation decision is given by
%$\mathbf{x}_n^1, \cdots, \mathbf{x}_n^{|\mathcal{M}|}$
 $\mathbf{X}=\{\mathbf{X}_1, \mathbf{X}_2, \cdots, \mathbf{X}_N\}$, where $\mathbf{X}_n,\; \forall n \in \mathcal{N}$ is given by: 

\begin{equation}
\label{eq:X}
\mathbf{X}_{n}=\Biggl[\begin{smallmatrix}
\mathbf{x}^{1}_n\\ 
.\\ 
.\\ 
.\\
\mathbf{x}^{|\mathcal{{M}}|}_n
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{n,1}^{1} & \cdots  &\cdots   & x^{1}_{n,{K}} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{n,1}^{|\mathcal{{M}}|}&\cdots  &\cdots   & x_{n,K}^{|\mathcal{{M}}|}
\end{smallmatrix}\Biggr].
\end{equation}
%In  the case of resource sharing among service providers,  
Each service provider aims to  maximize the sum of utilities by  allocating its resources to its native applications, and  allocating resources  to  applications belonging to other service providers. %; and c) improving its applications' satisfaction by using its own resources or borrowing from other service providers (if needed).  
Each provider $n \in \mathcal{{N}}$ solves the following multi-objective optimization problem.  
 
 


\begin{subequations}\label{eq:opt_higher}
	\begin{align}
	\max_{\mathbf{X}_n}\quad& \sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)- u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big) \nonumber \\
	&+\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)\nonumber\\
	&- D^l({x}_{n,k}^l)\big)\Big), \label{eq:obj}\\ 
	\text{s.t.}\quad 
& \sum_{j} x_{n,k}^{j}\leq C_{n,k}, \quad \forall\;  k \in \mathcal{K}, n \in \mathcal{N}, \label{eq:obj1} \displaybreak[0]\\
	& \sum_{m \in \mathcal{N}}x_{m,k}^{j} \leq r_{n,k}^{j}, \quad \forall\; j\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N},  \label{eq:obj2}\displaybreak[1]\\
	&  x_{n,k}^{j} \geq 0, \quad \forall\; j\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}, \label{eq:obj3} \displaybreak[2]\\
	& u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-
	u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)- \nonumber \\
	& D^l({x}_{n,k}^l)\geq0, \forall l \in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, n \in \mathcal{N}\label{eq:obj4} .
	\end{align}
\end{subequations}
The first summation term in \eqref{eq:obj} represents the utility earned by an ESP providing resources to the native applications, whereas the second summation term describes the utility earned by providing resources to non-native applications. 
 Note that constraint \eqref{eq:obj1} indicates that the total allocated resources cannot exceed the resource capacity of the service providers. \eqref{eq:obj2} states that the total amount of resources allocated to any application using the resource-sharing framework cannot exceed the amount of  requested resources. \eqref{eq:obj3}  says that the resource allocation cannot be negative  whereas \eqref{eq:obj4} indicates that the incremental increase in utility earned by providing resources to non-native applications should be non-negative. 
 
 \subsection{Assumptions}\label{sec:assumption}
 In our model, we assume that  each utility is a  concave injective function  for which the inverse of the first derivative exists, such as $(1-e^{-x})$. % or $\ln(x)$.
Strictly speaking,  our centralized NBS framework requires only concave injective utility functions\cite{yaiche2000game}. However,  the existence of the inverse of the first derivative is required for the distributed NBS (see details in Section \ref{sec:nbs}).  The communication cost is a convex function, hence the objective function in \eqref{eq:opt_higher} is  concave. 
% We also assume that all of the applications collectively demand more resources than the resource capacity of ESPs.  Hence, 
All resources are fully utilized in the  optimal solution.  However, there are enough resources to provide a positive utility to all  service providers when sharing resources.  This is a realistic assumption as the demand for resources is usually more than the supply.  %The single objective optimization problem in \eqref{eq:opt_single} is feasible for all the CSPs $n \in \mathcal{N}$. 
 Furthermore, we assume that when ESPs share resources,  there exist solutions that are better than when they are all  working alone. This assumption can be relaxed, that is, if certain ESPs cannot improve their utility using the bargaining solution, they will not  participate in the resource sharing framework. However, the framework can still be used for the remaining  ESPs. 
 
 
 \subsection{Choice of  utility function}
  While our framework works with any utility that satisfies the conditions in Section \ref{sec:assumption}, choosing a suitable utility function along with the communication cost can minimize \emph{resource fragmentation}\footnote{We define resource fragmentation as the process in which  resources provided to an application $j$ are split across multiple ESPs rather than a single ESP. }. %We use the term resource fragmentation for the case, where any application $j$ that needs $b$ units of  resource $k$ obtains the required $b$ amount from different ESPs rather than one ESP.} 
 Generally, a concave utility has a steeper slope at start that becomes flatter as more resources are allocated, i.e., the rate of increase in the payoff for allocating  resources reduces with increase in the amount of allocated resources.  This results in  an ESP providing a fraction of originally requested resources to an application and keeping the remaining resources for other applications. Hence, the application  does not get all the resources it needed, and has to ask another ESP for more resources, resulting in resource fragmentation. 
 For example, assume that two applications require $4$ units of a particular resource  from ESP $n$ that only has $3$ units available. Due to the nature of many concave utilities, ESP $n$ for maximizing its utility will provide part of its resources to one application and the remaining resources to the other application rather than providing all $3$ available units to one application and borrowing resources for the other application. This causes resource fragmentation, i.e., both  applications received only a part of the required resources and they will need to obtain the remaining amount from other ESP(s). To avoid such problems, we propose that the utility function should consider:
  \begin{itemize}
  	\item Minimum acceptable amount of resources: The ESPs should earn either zero utility or a negative utility if the resources provided are not within $\delta$ units of the  requested resource $r_{n,k}^j$. Rather than using a utility function such as  $1-e^{-(x_{n,k}^j)}$ that pays  the ESP even when a small amount of resources are provided, it is better to use $1-e^{-(x_{n,k}^j-r_{n,k}^j +\delta)}$  that becomes positive only when the allocation $x_{n,k}^j$ is within $\delta_t$ units of the requested resource $r_{n,k}^j$. Such a utility along  with the communication cost helps minimize the aforementioned fragmentation problem. 
  	%\item Total resources allocated across all ESPs: Each ESP should consider resources allocated at other ESPs  to avoid over-estimating its profit, since  the pay-off for many concave utilities increases drastically at start and rate of increase in utility decreases as more resources are allocated.   ESPs should share information about the amount of resources they allocated to a particular application $j$ to satisfy SLA and then divide the utility on the basis of  resources allocated to application $j$ by each ESP. 
  \end{itemize} 
  


==> arxiv version/arxiv version/03-opt-problem.tex <==
%In this section, we first present the resource allocation problem for a single domain (no resource sharing with other domains). Then we present MOO resource sharing and allocation problem for the coalition. 
For a single domain $n \in \mathcal{N}$ (not  part of a coalition), the allocation decision matrix $X_{SO}^{(n)}$, where $SO$ stands for single objective,  is given by 

\begin{equation}
\label{eq:X_n}
X_{SO}^{(n)}=\Biggl[\begin{smallmatrix}
\mathbf{x_1^{(n)}}\\ 
.\\ 
.\\ 
.\\
\mathbf{x_{{{M}_n}}^{(n)}}
\end{smallmatrix}\Biggr] = \Biggl[\begin{smallmatrix}
x_{11}^{(n)} & \cdots  &\cdots   & x_{1{K}}^{(n)} \\ 
. & . &.  &. \\ 
. & . &.  &. \\
. & . &.  &. \\
x_{{{M}_n}1}^{(n)}&\cdots  &\cdots   & x_{{{M}_n}{K}}^{(n)}
\end{smallmatrix}\Biggr].
\end{equation}
%where $x_{ik}^{(n)}$ is the amount of resource $k\in \mathcal{K}$ belonging to player $n \in \mathcal{N}$ that is allocated  to application $i \in \mathcal{M}$. 



The optimization problem is: %given in Equation~\eqref{eq:opt_single}
\begin{subequations}\label{eq:opt_single}
	\begin{align}
	\max_{{X}_{SO}^{(n)}}\quad& u_n({X}_{SO}^{(n)}) \label{eq:objsingle}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall i \in \mathcal{M}_n, \label{eq:singlefirst} \displaybreak[0]\\
	& x_{ik}^{(n)} \leq r^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecond} \displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}. \label{eq:singlethird} \displaybreak[2]
	\end{align}
\end{subequations}
The goal of this single objective optimization problem is for every domain  to  maximize its utility by allocating available resources only to its own applications. %The first constraint \eqref{eq:singlefirst} indicates that the allocated resources to all the users $i \in \mathcal{M}_n$ cannot be more than the capacity. The second constraint \eqref{eq:singlesecond} indicates that the allocated resources cannot be more than the required resources, while the final constraint \eqref{eq:singlethird} indicates that the allocation cannot be negative.  
\par Next, we present the resource allocation problem for different domains that share their resources with each other. In the resource sharing case,  each domain aims to  maximize sum of utilities obtained by a) allocating resources to its native applications i.e., $u_n({X}_{i \in \mathcal{M}_n}^{(n)})$ where ${X}_{i \in \mathcal{M}_n}^{(n)}$ represents the allocation decision at domain $n$ for applications $i \in \mathcal{M}_n$, and b) allocating resources to  applications of other domains i.e.,  $u_j^n({X}_{i \in \mathcal{M}_j}^{(n)}),\; \forall j\in \mathcal{N}\backslash n$, where ${X}_{i \in \mathcal{M}_j}^{(n)}$ represents the allocation of resources to applications $i \in \mathcal{M}_j, \; \forall j \in \mathcal{N}\backslash n$  at domain $n$. This leads to: 
% in Equation~\eqref{eq:opt_higher}.  
\begin{subequations}\label{eq:opt_higher}
	\begin{align}
	\max_{\mathcal{X}}\quad&  \bigg(u_n({X}_{i \in \mathcal{M}_n}^{(n)})+ \sum_{j \in \mathcal{N}\backslash n}  u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})\bigg) \quad \forall n \in \mathcal{N} \label{eq:obj}\\%\{u_1(\mathcal{A}),u_2(\mathcal{A}),\cdots,u_N(\mathcal{A})\} \label{eq:obj}\\%U(A)\label{eq:obj}\\
	\text{s.t.}\quad & \sum_{i \in \mathcal{M}} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall n \in \mathcal{N},  \label{eq:obj1} \displaybreak[0]\\
	& \sum_{n \in \mathcal{N}}x_{ik}^{(n)} \leq r^{}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K},  \label{eq:obj2}\displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}. \label{eq:obj3} \displaybreak[2]
	\end{align}
\end{subequations}
%\begin{itemize}
% so that each enclaves first facilitates its own users and then assign the remaining resource to the users of other enclaves. $w_n +w'_{n}=1$  where $w_n > w'_{n}$. E.g., $w_n=0.8$ and $w'_{n}=0.2$ would mean that each enclave has an incentive to first satisfy its own users (higher utility) and then share the excess resources for other users $j \in \mathcal{N}\backslash n $
%	\item 
The first constraint in both optimization problems, \eqref{eq:opt_single}  and \eqref{eq:opt_higher}, indicates that the allocated resources cannot be more than the capacity. The second constraint  in \eqref{eq:singlesecond} and \eqref{eq:obj2} indicates, that the allocated resources should not be more than the required resources.  The last constraint, \eqref{eq:singlethird} and \eqref{eq:obj3},  indicates that allocation decision cannot be negative. 

The utility $u_n({X}_{i \in \mathcal{M}_n}^{(n)})$ given in \eqref{eq:obj}, that each player receives, is a payment that all users $i \in \mathcal{M}_n$  who use the resources pay the player. %Users of other domains $j \in \mathcal{N}\backslash n $ that use resources of domain $n$  will be charged at a rate that player $j$ would have charged the user $i \in \mathcal{M}_j$, had the request been fulfilled by player $j$. Hence, 
 $u^{n}_j({X}_{i \in \mathcal{M}_j}^{(n)})$ is the utility that domain $n$ receives for sharing its resources with domain $j$. %There are different ways to capture this profit. However, for now, we can say that it would be equivalent to whatever domain $j$ would have earned had it satisfied the requests itself (however it can't as it does not have resources, so it borrows resources from domain $n$ and assigns all the profit it gains from the users to player $n$). 
 %We also assume that th
%\vspace{-0.02in}
\subsection{Assumptions}\label{sec:assumption}
 In our model, we assume that  utilities are  concave injective functions  for which the inverse of first derivative exists, such as $(1-e^{-x})$. While our centralized NBS framework requires only concave injective utility function, the existence of first derivative's inverse is required for the distributed NBS (details in Section \ref{sec:nbs}).  
 We also assume that  resources required by different applications are more than the capacity of domains. Hence, all resources are fully utilized at the optimal solution.   The single objective optimization problem in \eqref{eq:opt_single} is feasible for all the players $n \in \mathcal{N}$. Furthermore, we assume that  there exists solutions that are better than the disagreement point for all the players. 
% that retain the concavity and $1-1$ property after taking the first derivative as well. 
%	\item  $w_n$ is the weight assigned to the utility of player $n$. $\zeta_n$ is the weight assigned to the utility $u^{n}_j(\mathcal{X})$. 
%\end{itemize}
%The optimization problem in Equation~\eqref{eq:opt_higher} is a modified scalarized MOO problem \cite{cho2017survey}. 
\begin{comment}
Before we get into the details of solving the problem, we present an example to understand this
\begin{example}
Let's say we have two different data centers owned by service provider $A$ and $B$ respectively ($A$ and $B$ are game players). Resources available at domain $A$ and $B$ are represented by  $C^{A}$ and $C^{B}$ respectively.  Users in sets $\mathcal{M}_{A}$ and $\mathcal{M}_{B}$ ask for resources and pay a certain price (profit for data centers)  $u_A(\mathcal{X})$ and $u_B(\mathcal{X})$. However, let's say $A$ has scarce resources while $B$ has excess resources. So by forming a coalition, users in $\mathcal{M}_s \subset\mathcal{M}_{A}$ that can't be satisfied by $A$ will be provided resources by $B$ without the users realizing who are providing the resources (since the coalition will make everything appear as one to the user). The profit that $B$ will earn for providing its resources will be equivalent to the profit $A$ would have earned (as $A$ has agreed upon a certain contract with its users $\mathcal{M}_{A}$) had it satisfied the user's request itself. So for $B$, it will earn utility $u_B(X)$ for satisfying its own users plus $u_A^B(X^{\mathcal{M}_s})$ (slight abuse of notation where $X^{\mathcal{M}_s}$ represents the allocation decision for users ${\mathcal{M}_s}$ in domain $B$) for satisfying the users $\mathcal{M}_s \subset\mathcal{M}_{A}$. So this added utility $u_A^B(X^{\mathcal{M}_s})$ is the pay-off for $B$ to share resources. This coalition clearly helps both. $A$ increases its customer satisfaction (as per the contract $A$ had agreed to provide resources to all the users $\mathcal{M}_{A}$), while $B$ earns extra using its excess resources. So it is a stable coalition.
\end{example}

\begin{example}[Utility Example]
For any two players \{1,2\},  $u_1 (\mathcal{X})$ will be given by 
\begin{equation}
u_1(\mathcal{X})=\sum_{i \in \mathcal{M}_1}\bigg(\prod_{k=1}^{{K}}\frac{1}{1+e^{-m(x_{ik}^{(1)}-R^{(1)}_{req,ik})}}\bigg)
\end{equation}
$u_2 (\mathcal{X})$ will be given by 
\begin{equation}
u_2(\mathcal{X})=\sum_{i \in \mathcal{M}_2}\bigg(\prod_{k=1}^{|\mathcal{K}|}(1-e^{-(\frac{1}{R^{(2)}_{req,ik}})x_{ik}^{(2)}})\bigg)
\end{equation}
 $u_2^{\mathcal{X}} (\mathcal{X})$ will be given by 
 \begin{equation}
 u_2^{1}(\mathcal{X})=\sum_{i \in \mathcal{M}_2}\bigg(\prod_{k=1}^{|\mathcal{K}|}(1-e^{-(\frac{1}{R^{(2)}_{req,ik}})x_{ik}^{(1)}})\bigg)
 \end{equation}
  $u_1^{\mathcal{X}} (\mathcal{X})$ will be given by 
  \begin{equation}
  u_1^{2}(\mathcal{X})=\sum_{i \in \mathcal{M}_1}\bigg(\prod_{k=1}^{{K}}\frac{1}{1+e^{-m(x_{ik}^{(2)}-R^{(1)}_{req,ik})}}\bigg)
  \end{equation}
\end{example}
\end{comment}


%\subsection{Choice of Utility Function for Resource Allocation Problem}
%The resource allocation problem can be represented using a \emph{monotone non-decreasing utility function}. This is because in the systems that we consider, such as a cloud service provider or a cellular communication system etc.,  the more the resources provided, the higher is the gain or utility for the service provider. It is highly unlikely that the utility of any service provider will decrease with increase in the amount of resources allocated.  


%satisfying user requests increases the gain or utility for the service provider.  increases with increase in the amount of resources allocated to the user. It is highly unlikely for any r
\begin{comment}
\subsection{Game Theoretic Solution}

We first define the characteristic function $v$ for our game that can solve  problem in~\eqref{eq:opt_higher} 
\begin{align} \label{eq:payoff_function}
v(\mathcal{N})=\sum_{\substack{\text{$n \in \mathcal{N}$} \\ \text{$C_{k}= \sum_{n \in \mathcal{N}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in \mathcal{N}$}\\ \text{$\sum_{j \in \mathcal{N}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}$}}}\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in \mathcal{N},j\neq n} u^{n}_j(\mathcal{X})\bigg)
\end{align}
\begin{remark}
	The characteristic function in Equation~\eqref{eq:payoff_function} is for the grand coalition $\mathcal{N}$. For any $S \subseteq \mathcal{N}$, the characteristic function will be 
\end{remark}
\begin{align} \label{eq:payoff_s_function}
v({S})=\sum_{\substack{\text{$n \in {S}$} \\ \text{$C_{k}= \sum_{n \in {S}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {S}$}\\ \text{$\sum_{j \in {S}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S}$}}} \bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in S,j\neq n} u^{n}_j(\mathcal{X})\bigg)
\end{align}
\begin{theorem}
%	A Cooperative game $(\mathcal{N}, v)$ of $\mathcal{N}$ players and $v$ payoff function that can be used to solve the multi-objective optimization problem given in \eqref{eq:opt_higher}, is canonical\footnote{for monotonically non-decreasing utilities/pay-off function} with Transferable utility
Resource allocation and sharing problem (with multiple objectives) in aforementioned settings can be modeled as a canonical cooperative game with TU. 
\end{theorem}
\begin{proof}
To prove this, we need to show that the characteristic function of resource sharing and allocation problem satisfies the following two conditions
%	For a game to be canonical, we need to prove that the game  is superadditive and the payoff function is of characteristic form. 
	\begin{itemize}
		\item \textbf{Characteristic form of payoff:} As the utility function in a resource sharing and allocation problem  only relies on the domains that are part of the coalition, the game or payoff function is of characteristic form
		\item \textbf{Superadditivity:} Super-additivity for TU games requires $v(S_1 \cup S_2 )\geq v(S_1)+V(S_2) \; \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, s.t. S_1\cap S_2 =\emptyset$ i.e. we have to prove that the pay-off or utility for a domain in the coalition is as good as domain working alone or in a smaller coalition. Due to monotonicity property of the utility functions used,  for all  players/domains $n \in \mathcal{N}$,  $u_n(X_n^{NC})\leq u_n(X_n^{C})$ as $X_n^{NC}\subset {X_n^{C}}$ \footnote{because $X_n^{C}$ can contain much more elements due to the increase in $C$ in the coalition} where $X_n^{C}$ and $X_n^{NC}$ are the allocation decisions in  a cooperative game  and independent setting respectively for domain $n$. 
	\end{itemize}
\end{proof}
\begin{lemma}\label{lemma:MOOGame}
A canonical cooperative game $(\mathcal{N}, v)$ with TU can be used to obtain the Pareto-optimal solutions for the multi-objective optimization problem given in \eqref{eq:opt_higher}
\end{lemma}

%Given that the game is canonical, we are going to explore potential solution approaches for such a game. We start with the \emph{Core} \cite{han2012game}. 

To prove Lemma \ref{lemma:MOOGame}, we must show that the core is non-empty for  our canonical game. To do this, we first show that our game is convex. 

\begin{definition}[Convex Games]
	A coalition game is said to be convex if and only if for every player $n \in \mathcal{N}$, the marginal contribution of the player is non-decreasing W.R.T set inclusion. Mathematically, for $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash \{n\}$ 
	\begin{equation}\label{eq:convexgames}
	v(S_1 \cup \{n\})-v(S_1) \leq v(S_2 \cup \{n\})-v(S_2)
	\end{equation} 
\end{definition}
\begin{theorem}
	Our canonical game is convex
\end{theorem}
\begin{proof}
Let us consider two coalition $S_1$ and $S_2$, where $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash\{j\}$ where $j \in \mathcal{N}$. Then we first calculate $v(S_2 \cup \{j\})-v(S_1 \cup \{j\})$
\begin{align}\label{eq:convexityProof}
& \sum_{\substack{\text{$n \in {S_2}$},\; \text{$C_{k}= \sum_{n \in {S_2}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}$}\\ \text{$\sum_{j \in {S_2}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {S_2}, k\neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) - \nonumber \\
& \Bigg(\sum_{\substack{\text{$n \in {S_1}$},\; \text{$C_{k}= \sum_{n \in {S_1}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {S_1}$} \\ \text{$\sum_{j \in {S_1}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_1}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {S_1}, k \neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_1)}(\mathcal{X}) + \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\nonumber \Bigg)\\ 
&= \sum_{\substack{\text{$n \in {S_2}\backslash S_1$}, \text{$C_{k}= \sum_{n \in {S_2}\backslash S_1}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}\backslash S_1$} \\ \text{$\sum_{j \in {S_2 \backslash S_1}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2 \backslash S_1}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {\{S_2 \backslash S_1\}}, k \neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) \nonumber \\
&   + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) - w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X}) \nonumber \\
& = v(S_2)- v(S_1)+ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})  \nonumber \\
& \geq v(S_2)- v(S_1)
\end{align}
	where the last inequality follows from the fact that $ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\geq 0$ (monotonicity of the utility)
\end{proof}
\end{comment}

%Related to the core, there are certain questions that we must answer
\begin{comment}
\begin{enumerate}
	\item Is the core non-empty?
	\item If the core is non-empty and consists of different pay-off allocations, how do we choose any particular pay-off allocation vector? 
\end{enumerate}
Below we attempt to answer these questions



\begin{definition}[Balanced Collection] Let $\Omega$ be a collection of different coalitions. $\Omega$ is considered to be a \emph{balanced collection} if we can find non-negative weights $w_S$ for each $S \in \Omega$ such that for every player $n$ 
	\begin{align}\label{eq:balancedcollection}
	\sum_{S \in \Omega, S \ni n}w_S =1 
	\end{align}
\end{definition}

\begin{definition}[Balanced Game] A game is called balanced if for every balanced collection $\Omega$, the payoff vector $\mathbf{x}$ will be in $V_{\mathcal{N}}$ if $\mathbf{x}_S \in V_S\; \forall S \in \Omega$ 
	%Let $\Omega$ be a collection of different coalitions. $\Omega$ is considered to be a \emph{balanced collection} if we can find non-negative weights $w_S$ for each $S \in \Omega$ such that for every player $n$ 
\end{definition}
\begin{theorem}[Bondareva-Shapley Theorem]\label{thm:BST}
	The core of a game is non-empty if and only if the game is balanced
\end{theorem}


\begin{theorem}
The core for canonical game with our characteristic function(in Equation~\eqref{eq:payoff_function}) is non-empty
\end{theorem}

\begin{proof}
From the definition of characteristic functions for TU games (see \cite{han2012game} for details), $v: 2^{\mathcal{N}}$ \textrightarrow $\mathbb{R}$ with $v(\emptyset)=\emptyset$. This means that the total number of coalitions possible for $\mathcal{N}$ players is $2^{|\mathcal{N}|}-1$ (we ignore the empty set). For $\Omega$, the non-negative weights $w_S$ which satisfy the condition for  balanced collection in Equation~\eqref{eq:balancedcollection} are given by $\frac{1}{2^{|\mathcal{N}|-1}}$. Hence $\Omega$ is a balanced collection. We also know that $v(S)\subseteq v(\mathcal{N})$ as $v(\mathcal{N})$ is defined over a larger feasible set due to increased amount of available resources. Leveraging the monotonicity property of the utility functions used, we know that any payoff vector  $\mathbf{x}$ will be in $V_{\mathcal{N}}$ if $\mathbf{x}_S$\footnote{$\mathbf{x}_S$ is the projection of $\mathbf{x}$ onto the vector space $\mathbb{R}^{|S|}$} $\in V_S\; \forall S \in \Omega$. Hence our canonical game with characteristic function $v$ in Equation~\eqref{eq:payoff_function} is balanced and its core is non-empty (from Theorem \ref{thm:BST})

\end{proof}
\end{comment}


%For our problem, does the Shapley value lie in the core? To do so we first define \emph{convex games}
\begin{comment}
\begin{theorem}
	The core of any convex game $(\mathcal{N},v)$ is non-empty and large. 
\end{theorem}
\begin{proof}
	Available in \cite{sharkey1982cooperative}
\end{proof}
While the existence of core i.e., core being non-empty, guarantees the grand coalition is stable, finding a suitable allocation from the core is challenging particularly when the core is large (our game). Furthermore, as mentioned earlier, fairness is also a shortcoming of core based solutions.  Shapley value can be  used to obtain a fair allocation, however, we first need to show that the Shapley value lies in the core to guarantee that the Shapley value based allocation is stable for the grand coalition. 
\begin{theorem}
	The Shapley value in Equation~\eqref{eq:shapleyvalue} lies in the core of our canonical game
\end{theorem}
\begin{proof}
	Since our canonical game is convex, the Shapley value lies in the core \cite{han2012game} (see \cite{roger1991game} for details)
\end{proof}
We summarize this in the remark below. 
\begin{remark}
If a TU game $(\mathcal{N}, v)$ is convex, then the core is non-empty and the Shapley Value lies in the core \cite{garg2013novel}.	
\end{remark}
Calculation of Shapley value given in Equation~\eqref{eq:shapleyvalue} is challenging \cite{han2012game}. Since our game is convex, calculating its Shapley value is slightly easier as given below. 

%Now that we have proved that the game is convex, we divert our attention to the calculation of Shapley value for a convex game. 


\subsubsection{Shapley Value for a Convex Game}
Let $\pi$ denote the permutation of players in our game.  Then for any permutation $p$ from the total possible permutations $|\mathcal{N}|!$, one can obtain the initial segments of ordering by \cite{garg2013novel}
\begin{equation}\label{eq:initialsegment}
O_{\pi, r}=\{ n \in \mathcal{N} : \pi(n) \leq r \}, \; r \in \{1, \cdots, N\}
\end{equation}
where $O_{\pi, 0}=\{\}$ and $O_{\pi, |\mathcal{N}|} =\mathcal{N}$. $\pi(n)$ refers to the position of the player $n$ in the permutation $\pi$. The core of any particular ordering $\pi$ can be obtained by solving  equations
\begin{equation}
\label{eq:x_i_pi_sol}
x_n^{\pi}(O_{\pi, r}) = v(O_{\pi, r}), \; r \in \{ 1, \cdots, N\}
\end{equation}
The solution to  above Equations~\eqref{eq:x_i_pi_sol} will result in a payoff vector $x^{\pi}$ where the elements of the vector are given by 
\begin{equation}
\label{eq:vectorelements}
x_n^{\pi}=v(O_{\pi, \pi(n)})- v(O_{\pi, \pi(n)-1}), \quad \forall n \in \mathcal{N} 
\end{equation}
The payoff vectors $x^{\pi}$ represent the extreme points of the core in convex games \cite{garg2013novel}. So if $\prod$ represents the set of all possible permutations of $\mathcal{N}$, the Shapley value of any player $n$ can be calculated as 
\begin{equation}
\label{eq:shapleyconvex}
\phi_n=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} x_n^{\pi}
\end{equation}
\begin{comment}
So for our coalition game $(\mathcal{N},v)$, the Shapley value is 
\begin{align}
\label{eq:ourshapleyconvex}
\phi_n&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} \bigg( \sum_{\substack{\text{$n \in {O_{\pi, \pi(n)}}$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)}}$} \\ \text{$$}\text{$\sum_{j \in {O_{\pi, \pi(n)}}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in O_{\pi, \pi(n)}$}}}\bigg(w_n u_n^{(\pi)}(\mathcal{A})+ w'_{n}\sum_{j \in {O_{\pi, \pi(n)}}, j \neq  n} u^{n,(\pi)}_j(\mathcal{A})\bigg)- \nonumber \\
&\Bigg(\sum_{\substack{\text{$n \in {O_{\pi, \pi(n)-1}}$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)-1}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)-1}}$}}}\bigg(w_n u^{(\pi)}_n(\mathcal{A})+ w'_{n}\sum_{j \in {O_{\pi, \pi(n)-1}}, j \neq n} u^{n,(\pi)}_j(\mathcal{A})\bigg)\Bigg) \nonumber \\
&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} \bigg( \sum_{\substack{\text{$n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1} }$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}$} \\ \text{$\sum_{j \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}$} }}\bigg(w_n u^{(\pi)}_n(\mathcal{A})+  \nonumber \\ 
& w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{n,(\pi)}_j(\mathcal{A}) +  w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{j,(\pi)}_n(\mathcal{A})  \bigg)\bigg) \nonumber \\
&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod}\bigg(w_nu^{(\pi)}_n(\mathcal{A})+ w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{n,(\pi)}_j(\mathcal{A}) +w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{j,(\pi)}_n(\mathcal{A}) \bigg) 
\end{align}
where Equation~\eqref{eq:ourshapleyconvex} provides the Shapley value for our convex game. It is evident that our Shapley value depends on the utility of the player $n$, the utility  player $n$ achieves by allocating resources to players in $j \in O_{\pi, \pi(n)}, j \neq n $ and the utility player $j \neq n, j \in O_{\pi, \pi(n)}$ achieves by allocating resources to player $n$  in every possible permutation. 

\begin{comment}
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $tt$ 
		\State \textbf{Output}: The optimal hit probabilities
		\State \textbf{Step $1$:}  $t \leftarrow$0, $\boldsymbol{\lambda^{(t)}\leftarrow\lambda_0}$, $\boldsymbol{\mu^{(t)}\leftarrow\mu_0}$
		\While{Equation \eqref{eq:gradient1} $\neq$ 0}%$\partial L(\boldsymbol{h,\lambda,\mu})/\partial \lambda_{l} \neq0$ $\&\& $ $\partial L(\boldsymbol{h,\lambda,\mu})/\partial \mu_{ip} \neq0$}
		\State \textbf{Step $2$}:$\boldsymbol{h_{il}^{(p)}[t]} \leftarrow \frac{w_i\beta^{|p|-l}}{\lambda_{l}[t-1]\Bigg(\prod_{\substack{q \neq p,\\ q:l\in\{1,\cdots,|q|\}}}(1-h_{il}^{(q)}[t-1])\Bigg)+\mu_{ip}[t-1]}. $ %Algorithm 2($\boldsymbol{\lambda^{(t)},\mu^{(t)}}$) %\Comment{The node id and file content to Algorithm \ref{algo:alg1} for calculating the price function using~(\ref{eq:gradient2}) }
		\State \textbf{Step $3$:} Update $\lambda$ and $\mu$ using  \eqref{eq:update},  t $\leftarrow t+1$
		%	\State \textbf{Step $4$}: $\boldsymbol \tau_{\chi} \longleftarrow \text{Convex}(\text{slave},\boldsymbol u_{\chi})$ \Comment{Solve the slave optimization problem for $\boldsymbol \tau_{\chi}$  }
		%	\State \textbf{Step $5$}: $(\boldsymbol b_{\chi}, \boldsymbol{\delta_{\chi}}, \text{obj}_{\chi})  \longleftarrow \text{Rounding}(\boldsymbol u_{\chi},\boldsymbol \tau_{\chi})$ \Comment{Round the values of $\boldsymbol u_{\chi}$, remap $\boldsymbol u_{\chi}, \boldsymbol \tau_{\chi}$ to $\boldsymbol{b}_{\chi}$ and $ \boldsymbol{\delta}_{\chi}$ and obtain the new objective function value  }
		\EndWhile
	\end{algorithmic}
	\caption{Iterative Distributed Algorithm}
	\label{algo:alg}
\end{algorithm}
\end{comment}
\begin{comment}
\begin{remark}
	Shapley value calculation for our convex game requires solving at least $2^{N}-1$ optimization problems
\end{remark}
Algorithm \ref{algo:alg1} provides an overview of our proposed approach. We obtain $R, C$ and the utility of all players as $\mathbf{u}$. We initialize each player's utility value ($\mathbf{u}(R,\mathcal{X})$), Shapley value ($\boldsymbol{\phi} $) and resource allocation decision $\mathcal{X}$ to $0$. Then we calculate the Shapley value for the players and assign it to $\mathbf{u}(R,\mathcal{X})$. Finally to obtain $\mathcal{X}$, we take the inverse function of $\mathbf{u}$. As we are using monotone utilities, we know that the inverse of the utilities exist.

\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0, $ \boldsymbol{\phi} \leftarrow$0,  
		\State \textbf{Step $1$:}  Calculate Shapley Value $\phi_n$ using Equation \eqref{eq:shapleyconvex} $\forall n \in \mathcal{N}$
		\State \textbf{Step $2$:} $ \mathbf{u}(R,\mathcal{X}) \leftarrow \boldsymbol{\phi}$
		\State \textbf{Step $3$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{Shapley Value based Resource Allocation}
	\label{algo:alg1}
\end{algorithm}
%It is worth mentioning here that the Shapley value will only provide us the utility each player is going to receive that lies in the core (as a result of cooperation). The allocation decision can be obtained by taking the inverse of utilities.  \par 
\subsubsection{Reducing the Computational Complexity}
As mentioned earlier, that the calculation of Shapley value for our convex game requires at solving at least $2^{N}-1$ optimization problems that is computationally expensive. To reduce the complexity, we propose a computationally efficient approach in Algorithm 2 that requires solving $2N$ optimization problems i.e. $\mathcal{O}(N)$.  The input into the algorithm consists of available resources/capacities, user requirements and the utilities of all game players. The output of the algorithm is $\mathcal{X}$. In Step 1, the utility values of the players, the allocation decision,  and two vectors $\boldsymbol{O_1}$ and $\boldsymbol{O_2}$. In Step 2, every player's utility is calculated without any resource sharing i.e. single optimization and the values are stored in the vector $\boldsymbol{O_1}$. Then $C, R$ are updated and we move to Step 4, where we calculated the utilities $u_j^n$'s for all the players with updated $C, R$ and store them in $\boldsymbol{O_2}$. 

\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0, $ \boldsymbol{\phi} \leftarrow$0,  $ \boldsymbol{O_1} \leftarrow$0, $ \boldsymbol{O_2} \leftarrow$0, 
		\State \textbf{Step $2$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_1^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single}}
		\EndFor
		\State \textbf{Step $3$:} Update $C$ and $R$ based on Step 2
		\State \textbf{Step $4$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_2^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single_j}}
		\State Update $C$ and $R$
		\EndFor
		\State \textbf{Step $5$:} $u_n(R,\mathcal{X})\leftarrow O_1^n+O_2^n$ $\forall n \in \mathcal{N}$ 
		\State \textbf{Step $6$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{$\mathcal{O}$($N$) algorithm for obtaining Core's allocation}
	\label{algo:alg2}
\end{algorithm}
\begin{subequations}\label{eq:opt_single_j}
	\begin{align}
	\max_{\mathcal{X}}\quad& \sum_{j\neq n}u_j^n(\mathcal{X}) \quad  \forall n \in \mathcal{N} \label{eq:objsinglej}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall i \in \mathcal{M}\backslash\mathcal{M}_n, \label{eq:singlefirstj} \displaybreak[0]\\
	& x_{ik}^{(n)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecondj} \displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlethirdj} \displaybreak[2]
	\end{align}
\end{subequations}
\begin{theorem}
	The solution obtained from Algorithm \ref{algo:alg2} lies in the \emph{core}
\end{theorem}
\begin{proof}
	To prove the theorem, we need to show that the utilities obtained in Step $5$ of Algorithm \ref{algo:alg2}; a) are individually rational; b) are group rational and c) no players  have the incentive to leave the grand coalition and form another another coalition $S \subset \mathcal{N}$. 
	\paragraph{Individual Rationality} For each player $n \in \mathcal{N}$, the solution $O_1^n$ obtained by solving the optimization problem in Equation \eqref{eq:opt_single} is the utility a player will obtain by working alone i.e. it is $v\{n\}$. The value $O_2^n$ in Step 4 is either zero or positive but cannot be negative due to the nature of utility used i.e. 
	\begin{align}
u_n(R,\mathcal{X})&=O_1^n+O_2^n \quad \forall n \in \mathcal{N} \nonumber \\
u_n(R,\mathcal{X})&\geq O_1^n \quad \forall n \in \mathcal{N}\nonumber 
	\end{align}
	
	
	 Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is individually rational.
	\paragraph{Group Rationality} The value of the grand coalition $v\{\mathcal{N}\}$ as per Equation \eqref{eq:payoff_function} is the sum of utilities $u_n$'s and $u_j^n$'s. Steps 2, 4 and 5 of Algorithm \ref{algo:alg2} obtain the sum of the utilities as well. Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is group rational rational. 
	\par Furthermore, due to super-additivity of the game and monotonic non-decreasing nature of the utilities, no players have the incentive to form a smaller coalition. Hence Algorithm \ref{algo:alg2} provides a solution from the core.  
\end{proof}
\end{comment}
%\vspace{-0.1in}

==> arxiv version/arxiv version/04-exp-results.tex <==




We evaluate the performance of the proposed NBS framework for resource sharing and allocation across several  settings  in Table \ref{tab:settings} where the communication cost between ESPs $1$ and $3$ is higher than the cost between ESP $1$ and $2$, and ESP $2$ and $3$. Each ESP has three different  resources, i.e., storage, communication and computation. The model can be extended to include other  resources/parameters. %We present the results in four different settings as given in Table \ref{tab:settings}. 
We study the proposed framework using both synthetic and real-world data traces \cite{shen2015statistical,kohne2014federatedcloudsim,kohne2016evaluation}. 
For the study with synthetic and real-world data traces,  request matrices and capacity vectors, $\forall n \in \mathcal{N}$ are randomly generated for each setting. % within a pre-specified range\footnote{The larger the number of applications in our simulation settings, the larger is the range for random number generation.}. 
To show the advantage of resource sharing for both synthetic and   data trace,  we set large resource capacities at certain ESPs so that they can improve their utilities by sharing  available resources with other ESPs for meeting the demand of  latter ESPs. 
% ESPs so that they can improve their utilities by  shar the available resources with other CSPs and assist them in meeting demand.   

% While our framework can work with any concave and injective utility function for which the inverse of first derivative exists, the utilities assigned to players in simulation for illustrative purpose are %\vspace{-0.1in}
%\begin{align}\label{eq:utilityPlayers}
%u_n(\mathcal{X})=\sum_{i\in \mathcal{M}_n}\sum_{k=1}^{K}\big(1-e^{-{x_{ik}^{(n)}}}\big),\quad  \forall n \in \mathcal{N}.
%\end{align}
\begin{figure}[h!]
	%	\centering
	\includegraphics[width=0.53\textwidth]{figures/dist2}%withNBS_mod3}
	%	\vspace{-0.1in}
	\caption{Comparison of centralized and distributed algorithms.}
	\protect\label{fig:dist}
	%	\vspace{-0.2in}
\end{figure}


Simulations were run in \texttt{Matlab R2019a} on a \texttt{Core-i7} processor with \texttt{16 GB RAM}. To solve the optimization problems in \eqref{eq:opt_single} and \eqref{eq:objmain2}, we use the \texttt{OPTI-toolbox}\cite{currie2012opti}. %Below, we provide detailed experimental results.
 We  evaluate our proposed algorithms from the perspective of  service providers that are interested in maximizing their utilities and  evaluate the impact of our framework on the applications.	%\vspace{-0.2in} 
 We define  application \emph{request satisfaction} (RS)  as the ratio of  allocated  resources to   requested resources. %, i.e., $x_{n,k}^{j}/r_{n,k}^{j}$. % We define RS as the percentage to which the requests of different applications are satisfied.
% The RS for a single application is $x_{ik}^{(n)}/r_{ik}^{(n)}$. 
 Mathematically, average RS for an ESP $n$ in the resource sharing case  is defined as: %\vspace{-0.1in}
 \begin{align}\label{eq:requestsatisfaction}
 \centering 
 RS_{n}= \frac{\sum_{j \in \mathcal{M}_n}\sum_{k \in \mathcal{K}}\big(\frac{\sum_{m \in \mathcal{{N}}}x_{m,k}^{j}}{r_{n,k}^{j}}\big)}{M_nK} \times 100, %\bigg(\big(100-\frac{(r_{ik}^{(n)}-x_{ik}^{(n)})}{r_{ik}^{(n)}}\big)\times 100\bigg)}{M_nK} 
\end{align} 
The utility  and communication cost functions used in simulation are given in \eqref{eq:utility}.

\begin{align}\label{eq:utility}
\centering
u^j(x_{n,k}^j) & = 1-e^{-(x_{n,k}^j-r_{n,k}^j+\delta)}, \nonumber \\
D^j(x_{n,k}^j) &= \frac{x_{n,k}^j}{w},
\end{align}
Here $\delta$ is set to $1$ and weight $w$ is randomly chosen.

 \begin{comment}
Furthermore, the utility each CSP earned by satisfying requests for resources by application $j$ in the simulations is given in \eqref{eq:util}. 

 \begin{align}\label{eq:util}
\centering 
u_n^j(x_{n,k}^j+\sum_{m \in \mathcal{{N}}\backslash n}x_{m,k}^j)= 1-e^{-(x_{n,k}^j+\sum_{m \in \mathcal{{N}}\backslash n}x_{m,k}^j-r_{n,k}^j +\delta t)}
\end{align} 
where $\delta_t$ was set to be $1$ and the communication cost $C_n^l(\boldsymbol{.})$ was  a weighted linear function of the resource allocated at the remote CSP. 
\end{comment}


\begin{table}[]
	\centering
	\caption{Simulation network settings.}
	\begin{tabular}{|l|l|}
		\hline
		\textbf{Setting}   & \textbf{Parameters} \\ \hline
		\textbf{1} & $N=3, M_n=3,\forall n \in \mathcal{N}, K=3$                    \\ \hline
		\textbf{2} & $N=3, M_n=20,\forall n \in \mathcal{N}, K=3$                    \\ \hline
		\textbf{3 (data traces)} & $N=3, M_n=20,\forall n \in \mathcal{N}, K=3$                    \\ \hline
		%	\textbf{3} & $N=3, M_n=100,\forall n \in \mathcal{N}$                    \\ \hline
		%	\textbf{4} & $N=6, M_n=3,\forall n \in \mathcal{N}$                   \\ \hline
	\end{tabular}
	\vspace{-0.2in}
	\label{tab:settings}
\end{table}
%\begin{comment}

%\end{comment}
\begin{figure*}

	%	\centering
	\includegraphics[width=1.02\textwidth]{figures/three3}%withNBS_mod3}
	%	\vspace{-0.1in}
	\caption{Utility, average request satisfaction and average resource utilization for Setting $1$ when ESPs are working alone and using our proposed NBS framework.}
	\protect\label{fig:withNBS1}
%\vspace{0.15in}
\end{figure*}
\begin{figure*}
	%	\centering
	\includegraphics[width=1.02\textwidth]{figures/three20}%withNBS_mod3}
	%	\vspace{-0.1in}
	\caption{Utility, average request satisfaction and average resource utilization for Setting $2$ when ESPs are working alone and using our proposed NBS framework.}
	\protect\label{fig:withNBS2}
	%	\vspace{0.1in}
\end{figure*}
\subsection{Simulations results for synthetic data}
%The efficacy of our distributed algorithm is evaluated using simulations for a $3$ ESP - $3$ application setting  as shown in Figure \ref{fig:dist}.
\subsubsection{{Evaluation of the distributed algorithm}}
%\textbf{\red{[To be added]}}
To validate our results related to strong duality and our proposed distributed algorithm, we obtain the solution for Setting $1$ in Table \ref{tab:settings} using both the central and distributed algorithm as shown in Figure \ref{fig:dist}. It is evident that both the algorithms converge to the same solution, hence the duality gap is zero and our proposed distributed algorithm converges to the global optimal. 

\subsubsection{Utility, resource utilization, request satisfaction and fairness}

To highlight the efficacy of our framework, we compare its performance with a setting where ESPs  work alone (i.e., no resource sharing among ESPs). 
  In particular, we compare ESP utility, the average resource utilization (averaged across all $k$ resources) and the average request satisfaction (averaged across requests of all ESPs applications) in Figures \ref{fig:withNBS1} and \ref{fig:withNBS2} for $3$ and $20$ applications per ESP, respectively. 
%\paragraph{ESP Utility}
%In both Figures \ref{fig:withNBS1} and \ref{fig:withNBS2},  it is evident that the utility of all CSPs improves with resource sharing. 
When ESP $1$  works alone, it has a resource deficit (evident from $100\%$ average resource utilization and  average request satisfaction of less than 60\%  and 80\% in Figures \ref{fig:withNBS1} and \ref{fig:withNBS2}, respectively) whereas ESPs $2$ and $3$ have  resource surpluses as indicated by less than $100\%$ resource utilization and $100\%$ request satisfaction. The resource deficit results in a lower utility and request satisfaction for ESP $1$. 

%When working alone, CSP $1$ has  lower utility due to resource deficit resulting in a lower application satisfaction. 
%is penalized with a negative utility (customer dissatisfaction) due to its resource deficit, hence it has a lower utility.
 On the other hand,  both ESPs $2$ and $3$   achieve  higher utilities by satisfying all their applications when working alone. However, by using our resource sharing framework, the utilities of all ESPs improve as the framework provides optimal resource sharing.  %Utilities of ESPs $2$ and $3$ improve as they  share their resources with ESP $1$, whereas ESP $1$'s utility improves due to improved request satisfaction. 
 For the case with  three applications,  average request satisfaction improves from $86.11\%$ (working alone) to $94.5\%$ (resource sharing) whereas it improves from  $90.9\%$ to $99\%$ for the $20$ application case. It is worth noting  that request satisfaction for native applications of ESPs $2$ and $3$ reduce as these ESPs allocate their resources to applications of ESP $1$ for a higher utility. 
Furthermore,   resource utilizations also increase for the ESPs with resource surpluses as they share their resources with the ESP with a resource deficit. To measure the degree of fairness of the proposed sharing framework, we calculate  \emph{Jain}'s index\footnote{$\frac{1}{|N|}\leq$Jain's index$\leq 1$ where $1$ is the highest value of fairness.} \cite{jain1999throughput,jain1984aquantitative} that is $0.95$ and $0.99$ for the cases with $3$ and $20$ applications. % indicating that our framework has a higher notion of fairness as it is based on NBS. 
Especially for scenarios with a large number of applications, these results reveal  that our framework enables  fair sharing and allocation of resources among ESPs, as one would expect from the product-based fairness as offered by the NBS. 
%\vspace{-0.2in}
\subsection{Results for the data traces}
We use trace files from \emph{fastStorage}, \emph{Rnd} \cite{shen2015statistical}, and \emph{materna} \cite{kohne2014federatedcloudsim,kohne2016evaluation}. 
%The trace files from \cite{shen2015statistical} have two different traces, i.e., \emph{fastStorage} and \emph{Rnd} whereas the trace files from \emph{materna} \cite{kohne2014federatedcloudsim,kohne2016evaluation} contain three datasets of different numbers of VMs.
 We simulate a setting with three different ESPs and randomly extract the normalized resource request information related to the number of CPU cores, the amount of CPU and memory (RAM) for 20 different resource requests  from  \emph{fastStorage}, \emph{Rnd} and \emph{materna} dataset. Since the datasets do not provide the capacities of these service providers, we assign capacities in such a way that fastStorage serves as the ESP with resource deficit while the other two have resource surplus. Figure \ref{fig:withNBS6} shows ESP utilities,  request satisfaction and resource utilization based on  the  data traces. It is evident that ESP utilities  improve  and resource utilizations  increase to satisfy more applications by use of the proposed NBS framework. The average request satisfaction also increases from $83.3\%$ to $92.05\%$ whereas the Jain index is  $0.98$. 
\begin{figure*}
	%	\centering
	\includegraphics[width=1.00\textwidth]{figures/tr1}%withNBS_mod3}
	%	\vspace{-0.1in}
	\caption{Utility, average request satisfaction and average resource utilization for Setting $3$ when ESPs are working alone and using our proposed NBS framework.}
	\protect\label{fig:withNBS6}
	%	\vspace{-0.1in}
\end{figure*}
\begin{comment}
\begin{figure}
%	\centering
	\includegraphics[width=0.4\textwidth]{figures/three20tr.eps}%withNBS_mod3}
	\vspace{-0.1in}
	\caption{Utility of CSPs with trace files.}

		\vspace{-0.2in}
\end{figure}

\begin{figure}
	%\centering
	\subfloat[Utility function\label{fig:withNBS3}]{\includegraphics[width=0.255\textwidth]{figures/three20tr_1.eps}}
	%	\qquad
	\hspace{-0.2in}
	\subfloat[Resource utilization \label{fig:withNBS4}]{\includegraphics[width=0.255\textwidth]{figures/three20tr2_1.eps}}
	\caption{Utility and resource utilization for the trace files (Setting $3$) using our proposed framework. }%
	%\label{fig:example}%
	\protect\label{fig:withNBS6}
	\vspace{-0.25in}
\end{figure}

\end{comment}

\begin{table*}[]
	\centering
	\caption{Comparison of our NBS based resource sharing and allocation framework with other NBS based solutions.}
	\begin{tabular}{|c|p{1.0cm}|p{2.0cm}|c|p{5.5cm}|}
		\hline
		\multirow{2}{*}{\textbf{Reference}} & \multirow{2}{*}{\textbf{Objective}} & \multirow{2}{*}{\textbf{Resource Sharing}} & \multicolumn{2}{c|}{\textbf{Distributed Algorithm}}             \\ \cline{4-5} 
		&                                     &                                            & \textbf{Proposed?}      & \multicolumn{1}{c|}{\textbf{Technique}} \\ \hline
		\multicolumn{1}{|l|}{\cite{yaiche2000game}}              & \multicolumn{1}{l|}{Fair Bandwidth allocation}               & \multicolumn{1}{c|}{$\times$}                      & \multicolumn{1}{c|}{$\checkmark$} & Gradient Projection                                   \\ \hline		
		
		\multicolumn{1}{|l|}{\cite{xu2012general}}              & \multicolumn{1}{l|}{Fairness}               & \multicolumn{1}{c|}{$\times$}                      & \multicolumn{1}{c|}{$\checkmark$} & Dual decomposition and sub-gradient method are used. %The authors consider generic concave utility.                                      
		\\ \hline
		
		\multicolumn{1}{|l|}{\cite{hassan2014virtual}}              & \multicolumn{1}{l|}{Cost and Resource Utilization}               & \multicolumn{1}{c|}{$\times$}                      & \multicolumn{1}{c|}{$\times$} & N/A                                     \\ \hline
		
		\multicolumn{1}{|l|}{\cite{he2013toward}}              & \multicolumn{1}{l|}{Cost and User Experience}               & \multicolumn{1}{c|}{$\times$}                      & \multicolumn{1}{c|}{$\times$} & N/A                                     \\ \hline
		
		\multicolumn{1}{|l|}{\cite{feng2012bargaining}}              & \multicolumn{1}{l|}{Resource utilization}               & \multicolumn{1}{c|}{$\times$}                      & \multicolumn{1}{c|}{$\times$} & N/A                                  \\ \hline		
		
		
		
		
		\multicolumn{1}{|l|}{\cite{guo2013cooperative}}              & \multicolumn{1}{l|}{Bandwidth allocation}               & \multicolumn{1}{c|}{$\times$}                      & \multicolumn{1}{c|}{$\checkmark$} & Gradient Projection                                   \\ \hline		
		
		\multicolumn{1}{|l|}{Our Approach}              & \multicolumn{1}{l|}{Service provider utility and user satisfaction}               & \multicolumn{1}{c|}{$\checkmark$}                      & \multicolumn{1}{c|}{$\checkmark$} & Gradient descent based algorithm that works for the class of utilities described in \ref{sec:assumption}.                                   \\ \hline			
		
	\end{tabular}
	\label{tab:comparison}
\end{table*}



==> arxiv version/arxiv version/05-conclusions.tex <==
The focus in this paper is to optimally utilize available resources for satisfying a larger number of edge applications and improving the utility of edge service providers. We have shown that although ESPs may have different utilities, they should share
resources to improve their utilities and enhance application request satisfaction. Resource sharing among ESPs has been formulated as a bargaining problem and a resource-sharing framework using Nash Bargaining Solution (NBS) has been proposed, which has also been shown to be beneficial for the ESPs. Since a centralized solution for obtaining the NBS may not always be desirable, the strong duality property has been proved, which has enabled us to develop a distributed algorithm for the NBS. Using synthetic and real-world  data traces, we have demonstrated the effectiveness of the proposed framework.  In particular, our results confirm that ESPs with resource
deficits and surpluses can improve their utilities as well as application satisfaction by sharing resources.




==> arxiv version/arxiv version/game-theory.tex <==
%\subsection{Game Theoretic Solution}
We first define the characteristic function $v$ for our game that can solve  problem in~\eqref{eq:opt_higher} 

\begin{figure*}[!t]
	\normalsize
\begin{align} \label{eq:payoff_function}
v(\mathcal{N})=\sum_{\substack{\text{$n \in \mathcal{N}$},\;\text{$C_{k}= \sum_{n \in \mathcal{N}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in \mathcal{N}$}\\ \text{$\sum_{j \in \mathcal{N}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}$}}}\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in \mathcal{N},j\neq n} u^{n}_j(\mathcal{X})\bigg)
\end{align}
	\hrulefill
	\vspace*{-4pt}
\end{figure*}



\begin{remark}
	The characteristic function in Equation~\eqref{eq:payoff_function} is for the grand coalition $\mathcal{N}$. For any $S \subseteq \mathcal{N}$, the characteristic function will be given by Equation~\eqref{eq:payoff_s_function}
\end{remark}


\begin{figure*}[!t]
	\normalsize
\begin{align} \label{eq:payoff_s_function}
v({S})=\sum_{\substack{\text{$n \in {S}$},\; \text{$C_{k}= \sum_{n \in {S}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {S}$}\\ \text{$\sum_{j \in {S}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S}$}}} \bigg(w_n u_n(\mathcal{X})+\zeta_{n}\sum_{j \in S,j\neq n} u^{n}_j(\mathcal{X})\bigg)
\end{align}
\hrulefill
\vspace*{-4pt}
\end{figure*}


\begin{theorem}
%	A Cooperative game $(\mathcal{N}, v)$ of $\mathcal{N}$ players and $v$ payoff function that can be used to solve the multi-objective optimization problem given in \eqref{eq:opt_higher}, is canonical\footnote{for monotonically non-decreasing utilities/pay-off function} with Transferable utility
Resource allocation and sharing problem (with multiple objectives) in aforementioned settings can be modeled as a canonical cooperative game with TU. 
\end{theorem}
\begin{proof}
To prove this, we need to show that the characteristic function of resource sharing and allocation problem satisfies the following two conditions
%	For a game to be canonical, we need to prove that the game  is superadditive and the payoff function is of characteristic form. 
	\begin{itemize}
		\item \textbf{Characteristic form of payoff:} As the utility function in a resource sharing and allocation problem  only relies on the domains that are part of the coalition, the game or payoff function is of characteristic form
		\item \textbf{Superadditivity:} Super-additivity for TU games requires $v(S_1 \cup S_2 )\geq v(S_1)+V(S_2) \; \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, s.t. S_1\cap S_2 =\emptyset$ i.e. we have to prove that the pay-off or utility for a domain in the coalition is as good as domain working alone or in a smaller coalition. Due to monotonicity property of the utility functions used,  for all  players/domains $n \in \mathcal{N}$,  $u_n(X_n^{NC})\leq u_n(X_n^{C})$ as $X_n^{NC}\subset {X_n^{C}}$ \footnote{because $X_n^{C}$ can contain much more elements due to the increase in $C$ in the coalition} where $X_n^{C}$ and $X_n^{NC}$ are the allocation decisions in  a cooperative game  and independent setting respectively for domain $n$. 
	\end{itemize}
\end{proof}
\begin{lemma}\label{lemma:MOOGame}
A canonical cooperative game $(\mathcal{N}, v)$ with TU can be used to obtain the Pareto-optimal solutions for the multi-objective optimization problem given in \eqref{eq:opt_higher}
\end{lemma}

%Given that the game is canonical, we are going to explore potential solution approaches for such a game. We start with the \emph{Core} \cite{han2012game}. 

To prove Lemma \ref{lemma:MOOGame}, we must show that the core is non-empty for  our canonical game. To do this, we first show that our game is convex. 

\begin{definition}[Convex Games]
	A coalition game is said to be convex if and only if for every player $n \in \mathcal{N}$, the marginal contribution of the player is non-decreasing W.R.T set inclusion. Mathematically, for $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash \{n\}$ 
	\begin{equation}\label{eq:convexgames}
	v(S_1 \cup \{n\})-v(S_1) \leq v(S_2 \cup \{n\})-v(S_2)
	\end{equation} 
\end{definition}
\begin{theorem}
	Our canonical game is convex
\end{theorem}
\begin{proof}
Let us consider two coalition $S_1$ and $S_2$, where $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash\{j\}$ where $j \in \mathcal{N}$. Then we first calculate $v(S_2 \cup \{j\})-v(S_1 \cup \{j\})$ in Equation \eqref{eq:convexityProof}. 

\begin{figure*}[!t]
	\normalsize
\begin{align}\label{eq:convexityProof}
& \sum_{\substack{\text{$n \in {S_2}$},\; \text{$C_{k}= \sum_{n \in {S_2}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}$}\\ \text{$\sum_{j \in {S_2}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {S_2}, k\neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) - \nonumber \\
& \Bigg(\sum_{\substack{\text{$n \in {S_1}$},\; \text{$C_{k}= \sum_{n \in {S_1}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {S_1}$} \\ \text{$\sum_{j \in {S_1}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_1}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {S_1}, k \neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_1)}(\mathcal{X}) + \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\nonumber \Bigg)\\ 
&= \sum_{\substack{\text{$n \in {S_2}\backslash S_1$}, \text{$C_{k}= \sum_{n \in {S_2}\backslash S_1}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}\backslash S_1$} \\ \text{$\sum_{j \in {S_2 \backslash S_1}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2 \backslash S_1}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {\{S_2 \backslash S_1\}}, k \neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) \nonumber \\
&   + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) - w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X}) \nonumber \\
& = v(S_2)- v(S_1)+ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})  \nonumber \\
& \geq v(S_2)- v(S_1)
\end{align}
	% Restore the current equation number.
	%%\setcounter{equation}{\value{MYtempeqncnt}}
	% The IEEE uses as a separator
	\hrulefill
	% The spacer can be tweaked to stop underfull vboxes.
	\vspace*{4pt}
\end{figure*}

\begin{comment}
	\begin{align}\label{eq:convexityProof}
	& \sum_{\substack{\text{$n \in {S_2}$} \\ \text{$R_{av,k}= \sum_{n \in {S_2}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}$}\\ \text{$\sum_{j \in {S_2}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2}$}}}\bigg(w_n u_n(\mathcal{A})+ w'_{n}\sum_{k \in {S_2}, k\neq n} u^{j}_k(\mathcal{A})\bigg) + w_j u_j ^{(S_2)}(\mathcal{A}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{A}) - \nonumber \\
	& \Bigg(\sum_{\substack{\text{$n \in {S_1}$} \\ \text{$R_{av,k}= \sum_{n \in {S_1}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {S_1}$} \\ \text{$\sum_{j \in {S_1}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_1}$}}}\bigg(w_n u_n(\mathcal{A})+ w'_{n}\sum_{k \in {S_1}, k \neq n} u^{j}_k(\mathcal{A})\bigg) + w_j u_j ^{(S_1)}(\mathcal{A}) + \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{A})\nonumber \Bigg)\\ 
	&= \sum_{\substack{\text{$n \in {S_2}\backslash S_1$} \\ \text{$R_{av,k}= \sum_{n \in {S_2}\backslash S_1}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}\backslash S_1$} \\ \text{$\sum_{j \in {S_2 \backslash S_1}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2 \backslash S_1}$}}}\bigg(w_n u_n(\mathcal{A})+ w'_{n}\sum_{k \in {\{S_2 \backslash S_1\}}, k \neq n} u^{j}_k(\mathcal{A})\bigg) + w_j u_j ^{(S_2)}(\mathcal{A}) \nonumber \\
	&   + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{A}) - w_j u_j ^{(S_1)}(\mathcal{A}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{A}) \nonumber \\
	& = v(S_2)- v(S_1)+ w_j u_j ^{(S_2)}(\mathcal{A}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{A}) -  w_j u_j ^{(S_1)}(\mathcal{A}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{A})  \nonumber \\
	& \geq v(S_2)- v(S_1)
	\end{align}
	\end{comment}

The last inequality in Equation \eqref{eq:convexityProof} follows from the fact that $ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\geq 0$ (monotonicity of the utility)
\end{proof}


%Related to the core, there are certain questions that we must answer
\begin{comment}
\begin{enumerate}
	\item Is the core non-empty?
	\item If the core is non-empty and consists of different pay-off allocations, how do we choose any particular pay-off allocation vector? 
\end{enumerate}
Below we attempt to answer these questions



\begin{definition}[Balanced Collection] Let $\Omega$ be a collection of different coalitions. $\Omega$ is considered to be a \emph{balanced collection} if we can find non-negative weights $w_S$ for each $S \in \Omega$ such that for every player $n$ 
	\begin{align}\label{eq:balancedcollection}
	\sum_{S \in \Omega, S \ni n}w_S =1 
	\end{align}
\end{definition}

\begin{definition}[Balanced Game] A game is called balanced if for every balanced collection $\Omega$, the payoff vector $\mathbf{x}$ will be in $V_{\mathcal{N}}$ if $\mathbf{x}_S \in V_S\; \forall S \in \Omega$ 
	%Let $\Omega$ be a collection of different coalitions. $\Omega$ is considered to be a \emph{balanced collection} if we can find non-negative weights $w_S$ for each $S \in \Omega$ such that for every player $n$ 
\end{definition}
\begin{theorem}[Bondareva-Shapley Theorem]\label{thm:BST}
	The core of a game is non-empty if and only if the game is balanced
\end{theorem}


\begin{theorem}
The core for canonical game with our characteristic function(in Equation~\eqref{eq:payoff_function}) is non-empty
\end{theorem}

\begin{proof}
From the definition of characteristic functions for TU games (see \cite{han2012game} for details), $v: 2^{\mathcal{N}}$ \textrightarrow $\mathbb{R}$ with $v(\emptyset)=\emptyset$. This means that the total number of coalitions possible for $\mathcal{N}$ players is $2^{|\mathcal{N}|}-1$ (we ignore the empty set). For $\Omega$, the non-negative weights $w_S$ which satisfy the condition for  balanced collection in Equation~\eqref{eq:balancedcollection} are given by $\frac{1}{2^{|\mathcal{N}|-1}}$. Hence $\Omega$ is a balanced collection. We also know that $v(S)\subseteq v(\mathcal{N})$ as $v(\mathcal{N})$ is defined over a larger feasible set due to increased amount of available resources. Leveraging the monotonicity property of the utility functions used, we know that any payoff vector  $\mathbf{x}$ will be in $V_{\mathcal{N}}$ if $\mathbf{x}_S$\footnote{$\mathbf{x}_S$ is the projection of $\mathbf{x}$ onto the vector space $\mathbb{R}^{|S|}$} $\in V_S\; \forall S \in \Omega$. Hence our canonical game with characteristic function $v$ in Equation~\eqref{eq:payoff_function} is balanced and its core is non-empty (from Theorem \ref{thm:BST})

\end{proof}
\end{comment}


%For our problem, does the Shapley value lie in the core? To do so we first define \emph{convex games}

\begin{theorem}
	The core of any convex game $(\mathcal{N},v)$ is non-empty and large. 
\end{theorem}
\begin{proof}
	Available in \cite{sharkey1982cooperative}
\end{proof}
While the existence of core i.e., core being non-empty, guarantees the grand coalition is stable, finding a suitable allocation from the core is challenging particularly when the core is large (our game). Furthermore, as mentioned earlier, fairness is also a shortcoming of core based solutions.  Shapley value can be  used to obtain a fair allocation, however, we first need to show that the Shapley value lies in the core to guarantee that the Shapley value based allocation is stable for the grand coalition. 
\begin{theorem}
	The Shapley value in Equation~\eqref{eq:shapleyvalue} lies in the core of our canonical game
\end{theorem}
\begin{proof}
	Since our canonical game is convex, the Shapley value lies in the core \cite{han2012game} (see \cite{roger1991game} for details)
\end{proof}
We summarize this in the remark below. 
\begin{remark}
If a TU game $(\mathcal{N}, v)$ is convex, then the core is non-empty and the Shapley Value lies in the core \cite{garg2013novel}.	
\end{remark}
Calculation of Shapley value given in Equation~\eqref{eq:shapleyvalue} is challenging \cite{han2012game}. Since our game is convex, calculating its Shapley value is slightly easier as given below. 

%Now that we have proved that the game is convex, we divert our attention to the calculation of Shapley value for a convex game. 


\subsubsection{Shapley Value for a Convex Game}
Let $\pi$ denote the permutation of players in our game.  Then for any permutation $p$ from the total possible permutations $|\mathcal{N}|!$, one can obtain the initial segments of ordering by \cite{garg2013novel}
\begin{equation}\label{eq:initialsegment}
O_{\pi, r}=\{ n \in \mathcal{N} : \pi(n) \leq r \}, \; r \in \{1, \cdots, N\}
\end{equation}
where $O_{\pi, 0}=\{\}$ and $O_{\pi, |\mathcal{N}|} =\mathcal{N}$. $\pi(n)$ refers to the position of the player $n$ in the permutation $\pi$. The core of any particular ordering $\pi$ can be obtained by solving  equations
\begin{equation}
\label{eq:x_i_pi_sol}
x_n^{\pi}(O_{\pi, r}) = v(O_{\pi, r}), \; r \in \{ 1, \cdots, N\}
\end{equation}
The solution to  above Equations~\eqref{eq:x_i_pi_sol} will result in a payoff vector $x^{\pi}$ where the elements of the vector are given by 
\begin{equation}
\label{eq:vectorelements}
x_n^{\pi}=v(O_{\pi, \pi(n)})- v(O_{\pi, \pi(n)-1}), \quad \forall n \in \mathcal{N} 
\end{equation}
The payoff vectors $x^{\pi}$ represent the extreme points of the core in convex games \cite{garg2013novel}. So if $\prod$ represents the set of all possible permutations of $\mathcal{N}$, the Shapley value of any player $n$ can be calculated as 
\begin{equation}
\label{eq:shapleyconvex}
\phi_n=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} x_n^{\pi}
\end{equation}
\begin{comment}
So for our coalition game $(\mathcal{N},v)$, the Shapley value is 
\begin{align}
\label{eq:ourshapleyconvex}
\phi_n&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} \bigg( \sum_{\substack{\text{$n \in {O_{\pi, \pi(n)}}$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)}}$} \\ \text{$$}\text{$\sum_{j \in {O_{\pi, \pi(n)}}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in O_{\pi, \pi(n)}$}}}\bigg(w_n u_n^{(\pi)}(\mathcal{A})+ w'_{n}\sum_{j \in {O_{\pi, \pi(n)}}, j \neq  n} u^{n,(\pi)}_j(\mathcal{A})\bigg)- \nonumber \\
&\Bigg(\sum_{\substack{\text{$n \in {O_{\pi, \pi(n)-1}}$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)-1}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)-1}}$}}}\bigg(w_n u^{(\pi)}_n(\mathcal{A})+ w'_{n}\sum_{j \in {O_{\pi, \pi(n)-1}}, j \neq n} u^{n,(\pi)}_j(\mathcal{A})\bigg)\Bigg) \nonumber \\
&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} \bigg( \sum_{\substack{\text{$n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1} }$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}$} \\ \text{$\sum_{j \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}$} }}\bigg(w_n u^{(\pi)}_n(\mathcal{A})+  \nonumber \\ 
& w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{n,(\pi)}_j(\mathcal{A}) +  w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{j,(\pi)}_n(\mathcal{A})  \bigg)\bigg) \nonumber \\
&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod}\bigg(w_nu^{(\pi)}_n(\mathcal{A})+ w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{n,(\pi)}_j(\mathcal{A}) +w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{j,(\pi)}_n(\mathcal{A}) \bigg) 
\end{align}
where Equation~\eqref{eq:ourshapleyconvex} provides the Shapley value for our convex game. It is evident that our Shapley value depends on the utility of the player $n$, the utility  player $n$ achieves by allocating resources to players in $j \in O_{\pi, \pi(n)}, j \neq n $ and the utility player $j \neq n, j \in O_{\pi, \pi(n)}$ achieves by allocating resources to player $n$  in every possible permutation. 

\begin{comment}
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $tt$ 
		\State \textbf{Output}: The optimal hit probabilities
		\State \textbf{Step $1$:}  $t \leftarrow$0, $\boldsymbol{\lambda^{(t)}\leftarrow\lambda_0}$, $\boldsymbol{\mu^{(t)}\leftarrow\mu_0}$
		\While{Equation \eqref{eq:gradient1} $\neq$ 0}%$\partial L(\boldsymbol{h,\lambda,\mu})/\partial \lambda_{l} \neq0$ $\&\& $ $\partial L(\boldsymbol{h,\lambda,\mu})/\partial \mu_{ip} \neq0$}
		\State \textbf{Step $2$}:$\boldsymbol{h_{il}^{(p)}[t]} \leftarrow \frac{w_i\beta^{|p|-l}}{\lambda_{l}[t-1]\Bigg(\prod_{\substack{q \neq p,\\ q:l\in\{1,\cdots,|q|\}}}(1-h_{il}^{(q)}[t-1])\Bigg)+\mu_{ip}[t-1]}. $ %Algorithm 2($\boldsymbol{\lambda^{(t)},\mu^{(t)}}$) %\Comment{The node id and file content to Algorithm \ref{algo:alg1} for calculating the price function using~(\ref{eq:gradient2}) }
		\State \textbf{Step $3$:} Update $\lambda$ and $\mu$ using  \eqref{eq:update},  t $\leftarrow t+1$
		%	\State \textbf{Step $4$}: $\boldsymbol \tau_{\chi} \longleftarrow \text{Convex}(\text{slave},\boldsymbol u_{\chi})$ \Comment{Solve the slave optimization problem for $\boldsymbol \tau_{\chi}$  }
		%	\State \textbf{Step $5$}: $(\boldsymbol b_{\chi}, \boldsymbol{\delta_{\chi}}, \text{obj}_{\chi})  \longleftarrow \text{Rounding}(\boldsymbol u_{\chi},\boldsymbol \tau_{\chi})$ \Comment{Round the values of $\boldsymbol u_{\chi}$, remap $\boldsymbol u_{\chi}, \boldsymbol \tau_{\chi}$ to $\boldsymbol{b}_{\chi}$ and $ \boldsymbol{\delta}_{\chi}$ and obtain the new objective function value  }
		\EndWhile
	\end{algorithmic}
	\caption{Iterative Distributed Algorithm}
	\label{algo:alg}
\end{algorithm}
\end{comment}
\begin{remark}\label{rem:shap}
	Shapley value calculation for our convex game requires solving at least $2^{N}-1$ optimization problems
\end{remark}
Algorithm \ref{algo:alg1} provides an overview of our proposed approach. We obtain $R, C$ and the utility of all players as $\mathbf{u}$. We initialize each player's utility value ($\mathbf{u}(R,\mathcal{X})$), Shapley value ($\boldsymbol{\phi} $) and resource allocation decision $\mathcal{X}$ to $0$. Then we calculate the Shapley value for the players and assign it to $\mathbf{u}(R,\mathcal{X})$. Finally to obtain $\mathcal{X}$, we take the inverse function of $\mathbf{u}$. As we are using monotone utilities, we know that the inverse of the utilities exist.
\par A fundamental issue with Shapley value is its complexity. As mentioned in Remark \ref{rem:shap}, Shapley value calculation requires solving a  large number of optimization problems that is not suitable for a game with larger number of players. Therefore, reducing the complexity of obtaining an allocation from the core is always favorable. 
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0, $ \boldsymbol{\phi} \leftarrow$0,  
		\State \textbf{Step $1$:}  Calculate Shapley Value $\phi_n$ using Equation \eqref{eq:shapleyconvex} $\forall n \in \mathcal{N}$
	    \State \textbf{Step $2$:} $ \mathbf{u}(R,\mathcal{X}) \leftarrow \boldsymbol{\phi}$
	    \State \textbf{Step $3$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
		\end{algorithmic}
	\caption{Shapley Value based Resource Allocation}
	\label{algo:alg1}
\end{algorithm}
%It is worth mentioning here that the Shapley value will only provide us the utility each player is going to receive that lies in the core (as a result of cooperation). The allocation decision can be obtained by taking the inverse of utilities.  \par 
\subsection{Reducing the Computational Complexity}
%As mentioned earlier, that the calculation of Shapley value for our convex game requires at solving at least $2^{N}-1$ optimization problems that is computationally expensive. 
To reduce the complexity, we propose a computationally efficient approach in Algorithm 2 that requires solving $2N$ optimization problems i.e. $\mathcal{O}(N)$.  The input into the algorithm consists of available resources/capacities, user requirements and the utilities of all game players. The output of the algorithm is $\mathcal{X}$. In Step 1, the utility values of the players, the allocation decision,  and two vectors $\boldsymbol{O_1}$ and $\boldsymbol{O_2}$. In Step 2, every player's utility is calculated without any resource sharing i.e. single optimization and the values are stored in the vector $\boldsymbol{O_1}$. Then $C, R$ are updated and we move to Step 4, where we calculated the utilities $u_j^n$'s for all the players with updated $C, R$ and store them in $\boldsymbol{O_2}$. 

\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0,   $ \boldsymbol{O_1} \leftarrow$0, $ \boldsymbol{O_2} \leftarrow$0, 
		\State \textbf{Step $2$:}
		 \For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_1^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single}}
		\EndFor
		\State \textbf{Step $3$:} Update $R, C$ based on Step 2
		\State \textbf{Step $4$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_2^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single_j} with updated C and R}
		\State Update C and R
		\EndFor
		\State \textbf{Step $5$:} $u_n(R,\mathcal{X})\leftarrow O_1^n+O_2^n$ $\forall n \in \mathcal{N}$ 
		\State \textbf{Step $6$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{$\mathcal{O}$($N$) algorithm for obtaining Core's allocation}
	\label{algo:alg2}
\end{algorithm}
\begin{subequations}\label{eq:opt_single_j}
	\begin{align}
	\max_{\mathcal{X}}\quad& \sum_{j\neq n}u_j^n(\mathcal{X}) \quad  \forall n \in \mathcal{N} \label{eq:objsinglej}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall i \in \mathcal{M}\backslash\mathcal{M}_n, \label{eq:singlefirstj} \displaybreak[0]\\
	& x_{ik}^{(n)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecondj} \displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlethirdj} \displaybreak[2]
	\end{align}
\end{subequations}
\begin{theorem}
	The solution obtained from Algorithm \ref{algo:alg2} lies in the \emph{core}
\end{theorem}
\begin{proof}
	To prove the theorem, we need to show that the utilities obtained in Step $5$ of Algorithm \ref{algo:alg2}; a) are individually rational; b) are group rational and c) no players  have the incentive to leave the grand coalition and form another another coalition $S \subset \mathcal{N}$. 
	\paragraph{Individual Rationality} For each player $n \in \mathcal{N}$, the solution $O_1^n$ obtained by solving the optimization problem in Equation \eqref{eq:opt_single} is the utility a player will obtain by working alone i.e. it is $v\{n\}$. The value $O_2^n$ in Step 4 is either zero or positive but cannot be negative due to the nature of utility used i.e. 
	\begin{align}
	u_n(R,\mathcal{X})&=O_1^n+O_2^n \quad \forall n \in \mathcal{N} \nonumber \\
	u_n(R,\mathcal{X})&\geq O_1^n \quad \forall n \in \mathcal{N}\nonumber 
	\end{align}
	
	
	Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is individually rational.
	\paragraph{Group Rationality} The value of the grand coalition $v\{\mathcal{N}\}$ as per Equation \eqref{eq:payoff_function} is the sum of utilities $u_n$'s and $u_j^n$'s. Steps 2, 4 and 5 of Algorithm \ref{algo:alg2} obtain the sum of the utilities as well. Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is group rational rational. 
	\par Furthermore, due to super-additivity of the game and monotonic non-decreasing nature of the utilities, no players have the incentive to form a smaller coalition. Hence Algorithm \ref{algo:alg2} provides a solution from the core.  
\end{proof}

==> arxiv version/arxiv version/nbs.tex <==
We first present an introduction to NBS and then discuss our proposed NBS based resource sharing framework. 
\subsection{Primer on Nash Bargaining Solution (NBS)}\label{sec:prelim}
\input{preli}

\subsection{Proposed Framework}
As mentioned earlier, NBS is  a Pareto optimal and fair solution in settings that involve different players (ESPs in our case) where each player has an objective to optimize. Therefore, it can be used to solve our MOO problem in \eqref{eq:opt_higher} as we have different ESPs  that need to optimize their objectives and improve their utilities over what they would receive  working alone. 
 We first specify the disagreement point for our bargaining problem. If the ESPs  cannot come to an agreement, they can all start working alone.  Hence the disagreement point  is the solution to the SOO problem given in \eqref{eq:opt_single} for all ESPs. Let us denote the solution to the SOO problem by $d_n^0, \forall\; n \in \mathcal{N}$.   In the cooperative setting\footnote{Service providers share resources among each other.}, the utility (represented by $s_n$ in \eqref{eq:nashProbNplayer})  for an ESP $n \in \mathcal{N}$  is given by: 
 \begin{align}
%\big(\sum_{j \in \mathcal{M}_n}u_n^j(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^j+\mathbf{x}_n^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^l+\nonumber \\
%\mathbf{x}_n^l)-D_n^l(\mathbf{x}_n^l)\big)\big) \nonumber
%&\sum_{j \in \mathcal{M}_n}\Big(u_n^j(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^j+\mathbf{x}_n^j)- u_n^j(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^j) \Big)+ \nonumber \displaybreak[0]\\
%&\Big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^l+\mathbf{x}_n^l)-u_n^l(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^l)-\nonumber\\ &D_n^l(\mathbf{x}_n^l)\Big)
U= &\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)- u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big) \nonumber \displaybreak[0] \\
&\hspace*{-0.2in}+\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)- \displaybreak[1]\nonumber\\
&\hspace*{-0.1in} D^l({x}_{n,k}^l)\big)\Big). \nonumber 
 \end{align} 
  Below, we  present the centralized NBS algorithm. % and then propose a distributed algorithm for NBS. %\vspace{-0.2in}
 \subsubsection{Centralized NBS}
 We first present the optimization problem to obtain NBS for our $N-$ESP bargaining game  \cite{harsanyi1963simplified} and then present its equivalent problem \cite{yaiche2000game} that is computationally efficient to solve. 
 %Therefore,  we state the following theorem.  %Using this information, the optimization problem for NBS in \eqref{eq:nashProbNplayer} can be rewritten as 
 \begin{theorem} The NBS  for the MOO optimization problem in \eqref{eq:opt_higher} can be  obtained by solving the following optimization problem:% in \eqref{eq:nashProbNplayermod}.
 \begin{subequations}\label{eq:nashProbNplayermod}
 	\begin{align}
  	\max_{\mathbf{X}}\;& \prod_{n=1}^{N}\hspace*{-0.05in}\bigg(\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)-u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big)  \nonumber \\
  	&+\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)\nonumber\\
  	&- D^l({x}_{n,k}^l)\big)\Big)-d_n^0
  	\bigg),\label{eq:objmain} \\
 	\text{s.t.}\quad & Constraints \; in \; \eqref{eq:obj1}-\eqref{eq:obj4}, \nonumber \\
 %	&\sum_{j \in \mathcal{M}_n}\Big(u_n^j(\sum_{m \in \overline{\mathcal{N}}}\mathbf{x}_m^j+\mathbf{x}_n^j)- u_n^j(\sum_{m \in \overline{\mathcal{N}}}\mathbf{x}_m^j) \Big)+ \nonumber \\
 	&\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)-u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big)  \nonumber \\
 	&+\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)\nonumber\\
 	&- D^l({x}_{n,k}^l)\big)\Big)> d_n^0, \quad \forall \; n \in \mathcal{N}.\label{eq:disagreemt}
 	\end{align}
 \end{subequations}
 \end{theorem}%\vspace{-0.2in}
\begin{proof}
The feasible set for the above optimization problem is convex and compact, since all constraints are convex and intersection of convex sets is a convex set. Furthermore, based on our assumptions, there exist solutions (allocation and sharing decisions) that  provide better utility than the disagreement point $d_n^0, \forall\; n \in \mathcal{N}$. Hence, the solution of the optimization problem in \eqref{eq:nashProbNplayermod} is the NBS.
\end{proof}%\vspace{-0.1in}
However, solving \eqref{eq:nashProbNplayermod} is computationally complex and the problem is not always convex.  Therefore, there is a need for an efficient method to obtain the NBS. %\vspace{-0.1in}
%\subsection{Complexity Reduction}
Toward this goal,  we transform the problem \eqref{eq:nashProbNplayermod} into an equivalent problem as proposed in \cite{yaiche2000game}. %first need to transform our problem as stated in the following theorem. 

\begin{comment}
\begin{theorem}[Problem transformation\cite{yaiche2000game}]
	\label{thm:transformation}
	Suppose for every player $n \in \mathcal{N}$, $s_n \in \mathcal{S}$ is injective function in the feasible set $\mathcal{F}$ (satisfying all the constraints). Under the assumptions of NBS, let us consider the following
	\begin{align}
	\label{eq:nashProbN}
	\max_{s_1,\cdots,s_N}\;\prod_{n=1}^{N}(s_n-d_n),\; s.t.\;  s_n \in \mathcal{F},\; \forall n \in \mathcal{N}
	\end{align}\vspace{-0.15in}
		\begin{align}
	\label{eq:nashProbN2}
	\max_{s_1,\cdots,s_N}\;\sum_{n=1}^{N}\ln(s_n-d_n),\; s.t.\;  s_n \in \mathcal{F},\; \forall n \in \mathcal{N}
	\end{align}
	\begin{enumerate}
		\item Equation \eqref{eq:nashProbN} has a unique solution  and the bargaining solution is just a single point, where as Equation \eqref{eq:nashProbN2} is a convex optimization problem with a unique solution.
		\item The optimization problems in Equations \eqref{eq:nashProbN} and \eqref{eq:nashProbN2} are equivalent. Hence, the  unique solution of Equation \eqref{eq:nashProbN2} is the NBS.
		%\item The unique solution of Equation \eqref{eq:nashProbN2} is the NBS.
	\end{enumerate}
\end{theorem}
The above transformation reduces the complexity and always guarantees an NBS \cite{khan2009cooperative}. 
\end{comment}


\begin{corollary}%[\cite{weiser1994scheduling,stefanescu1984arbitrated}]
The NBS for \eqref{eq:opt_higher} is obtained by solving the following optimization problem:
%	\begin{align}\label{eq:objmain1} 
%\max_{\mathcal{X}}\quad& \prod_{n=1}^{N}\bigg(u_n(\mathcal{X})+ \big(\sum_{j \in \mathcal{N},j\neq n}  u^{n}_j(\mathcal{X})\big)-d_n^0\bigg), \; s.t. \; \mathcal{X} \in  \mathcal{F}
%\end{align}
%	\begin{align}\label{eq:objmain2} 
%\max_{\mathcal{X}}\quad& \sum_{n=1}^{N}\bigg(u_n(\mathcal{X})+ \big(\sum_{j \in \mathcal{N},j\neq n}  u^{n}_j(\mathcal{X})\big)-d_n^0(\mathcal{X})\bigg), \; s.t. \; \mathcal{X} \in  \mathcal{F}
%\end{align}
%\begin{subequations}\label{eq:objmain2} 
	\begin{align}\label{eq:objmain2} 
	\max_{\mathbf{X}}\;& \sum_{n=1}^{N}\ln\bigg(\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)- \nonumber \\
	&u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big) +\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)\nonumber\\
	&-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)- D^l({x}_{n,k}^l)\big)\Big)-d_n^0
	\bigg),\\
	\text{s.t.}\quad &  Constraints \; in \; \eqref{eq:obj1}-\eqref{eq:obj4}, \; \eqref{eq:disagreemt}. \nonumber 
	\end{align}
\end{corollary}
%\vspace{-0.2in}
\begin{proof}
	ESP utilities are concave and  bounded above. Furthermore, the feasible set along with the set of achievable utilities ($\mathcal{S}$) is convex and compact (due to the nature of  utilities and constraints). %Hence, the NBS with higher complexity  is guaranteed to exist. 
	Utilities of ESPs are also injective functions of the allocation decision. Hence \eqref{eq:objmain2} is equivalent to \eqref{eq:nashProbNplayermod} \cite{yaiche2000game}. Since   the logarithm of any positive real number is concave\cite{boyd2004convex},  \eqref{eq:objmain2} is a convex optimization problem with a unique solution, which is the NBS. %Hence using Theorem \ref{thm:transformation}, the result follows. 
\end{proof}
%\vspace{-0.1in}
The centralized Algorithm \ref{algo:centralnbs} provides the allocation decision using NBS. %Traditionally, each ESP receives a pay-off equal to the utility it achieves by solving \eqref{eq:objmain2}. However, due to the nature of utility we suggested to use for reducing resource fragmentation, an  ESP may over-estimate its payoff achieved by allocating resources to an application\footnote{The utility earned by ESP $n$ for allocating resources to application $j$ considers the resources allocated at other ESPs as well, i.e., $u_n^j(\mathbf{x}_n^j+\sum_{m \in \mathcal{{N}}\backslash n}\mathbf{x}_{m}^j)$. Hence, even if  a ESP $n$ allocates no resources to application $j$ (while other ESPs do), ESP $n$ will be assigned a payoff based on the resources allocated by other ESPs.}. Hence, the utility needs to be divided among different ESPs using the rule specified in \eqref{eq:payoffrule} where $P_n^j$ is the payoff ESP $n$ receives for allocating resources to application $j$ and $P_T^j$ is the total payoff obtained from allocating resources to application $j$. 
%\begin{equation}
%\label{eq:payoffrule}
%P_n^j= \frac{\mathbf{x}_n^j}{\sum_{m \in \mathcal{{N}}}\mathbf{x}_m^j}\times P_T^j
%\end{equation}
%the utility achieved by each ESP in \eqref{eq:objmain2} is the payoff that the ESP wou

\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}:  $C, R$, and vector of utility functions of all ESPs $\boldsymbol{u}$ %  and $\mathcal{X}_0$ %$\forall \boldsymbol{\nu_0$, $\mu_0}\in\mathcal{R}$ and $\boldsymbol h_0$ 
		\State \textbf{Output}: The optimal resource allocation $\mathbf{X}$ and payoffs of all ESPs
		\State \textbf{Step $1$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {d_n^0} \leftarrow$ \texttt{Objective function at optimal point in Equation \eqref{eq:opt_single}}
		\EndFor
		\State \textbf{Step $2$:} $\mathbf{X} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:objmain2}} %$\forall n \in \mathcal{{N}}$
	%	\State \textbf{Step $3$:} $P_n^j\leftarrow$ \texttt{Payoff received by ESP} $\forall n \in \mathcal{{N}}, j \in \mathcal{{M}}$\texttt{ using \eqref{eq:payoffrule}}
	\end{algorithmic}
	\caption{Centralized Algorithm for NBS}
	\label{algo:centralnbs}
\end{algorithm}


\begin{comment}
\begin{theorem}\label{thm:centralsolution}
	The solution to the optimization problem in \eqref{eq:objmain2}, provided that the inverse of the first derivative of $u_{n}^j(x_{n,k}^j)$ and $f_n^l=(u_{n}^l(x_{n,k}^l)-C_n^l(x_{n,k}^l))$ exist, is given by 
	\begin{equation}
	\label{eq:solcentral}
	x_{n,k}^{*j}=    u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j,\zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j}), \quad \quad \quad \forall j \in \mathcal{M},
%	x_{n,k}^{*j}=    u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j,\zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j},r_{k}^j), \quad \quad \quad \forall j \in \mathcal{M},%   \left\{\begin{matrix}
%  u_n^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)}), \quad \quad \quad \forall i \in \mathcal{M}_n\\
 % u_{jn}^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)}), \quad \forall i \in \mathcal{M}\backslash\mathcal{M}_n 	
%	\end{matrix}\right.
	%U_n^{'-1}(\alpha_k^{(n)}, \beta_{ik})
	\end{equation}
		\begin{equation}
	\label{eq:solcentral2}
	x_{n,k}^{*l}=    f_n^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Lambda_{n,k}^{l}), \quad  \forall l \in \{\mathcal{M}\backslash\mathcal{{M}}_n\},%   \left\{\begin{matrix}
	%  u_n^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)}), \quad \quad \quad \forall i \in \mathcal{M}_n\\
	% u_{jn}^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)}), \quad \forall i \in \mathcal{M}\backslash\mathcal{M}_n 	
	%	\end{matrix}\right.
	%U_n^{'-1}(\alpha_k^{(n)}, \beta_{ik})
	\end{equation}
	where   $u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j,\zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j})$ and $f_n^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Lambda_{n,k}^{l})$ are  %and $u_{jn}^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)})$ are
	 the inverse of the first derivative of $u_{n}^j$ and $(u_{n}^l(x_{n,k}^l)-C_n^l(x_{n,k}^l))$, respectively. %and $u_j^n$ respectively. 
	$\alpha_{n,k}$,  $\beta_{k}^j$, $\zeta_{n}$, and $\gamma_{n,k}^{j}$ are the \emph{Lagrange} multipliers and $\Lambda_{n,k}^{j}=\bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\mathbf{x}_n^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg)$. 
	
	% $\Lambda_{n,k}^{j}=\prod_{t\in \{\mathcal{N}\backslash n\}}\bigg(\sum_{j \in \mathcal{M}_n}u_t^j(\mathbf{x}_t^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_t\}} u_t^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_t^0\bigg)$.
	
	%$\Lambda_{n,k}^{j}=\bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\mathbf{x}_n^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg)$. 
	
	
	
	%$\Lambda_{n,k}^{j}=\bigg(\sum_{j \in \mathcal{M}_n}\big(u_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}} \frac{\sum_{n \in \mathcal{{N}}}x_{n,k}^{j}}{r_{k}^{j}}\big)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg)$.
\end{theorem}
\begin{proof}
	

	
	

	
	The Lagrangian function  for \eqref{eq:objmain2} is given in \eqref{eq:lagrangian} on the next page.  %$\boldsymbol{\alpha}$, $\boldsymbol{\beta},$  $\boldsymbol{\zeta}$ and $\boldsymbol{\gamma}$ are vector of Lagrangian multipliers. The first term in the Lagrangian function represents the improvement in the utility of a player sharing and allocating its resources (compared to only allocating its resources to its own applications). The second term is the profit the player will be making by charging each unit of its available resources with $\alpha_k$. The third term is the penalty for violating the positive allocation constraint. The fourth term is the profit a game player earns by allocating resources to applications for satisfying the applications demands $r_{ik}$ at a price of $\beta_{ik}$, while the last term is the incentive for the system to not degrade the performance of any player below the disagreement point. 	
	Since the Lagrangian function consists of differentiable and continuous functions, we can use gradients to obtain the optimal allocation decision and Lagrangian multipliers. %To obtain the maximum of Lagrangian function with respect to (w.r.t.) the allocation decision ${x_{ik}^{(n)}}$, we calculate the gradient of \eqref{eq:lagrangian} w.r.t. ${x_{ik}^{(n)}}$ and set it to zero as the first derivative diminishes at the maxima. 
	Depending on the application $j$, we have two cases: 
	\begin{enumerate}
		\item \textbf{$j \in \mathcal{M}_n$:}$\frac{\partial \mathcal{L}}{\partial x_{n,k}^{j}}=0$
			\begin{align}
		\label{eq:gradLagObj}
	%	 \Big(u_n^{'j}(x_{n,k}^{j})+\frac{1}{r_{k}^j}\Big)(1+\Lambda_{n,k}^{j}\zeta_{n})-\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j-\nonumber \\
	%	 \gamma_{n,k}^{j})=0,\nonumber \\
u_n^{'j}(x_{n,k}^{j})(1+\Lambda_{n,k}^{j}\zeta_{n})-\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j-\gamma_{n,k}^{j})=0,\nonumber \\	
	%	 \implies u_n^{'j}(x_{n,k}^{j})=\frac{\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Lambda_{n,k}^{j}\zeta_{n}}-\frac{1}{r_{k}^j}, \nonumber \\
		  \implies u_n^{'j}(x_{n,k}^{j})=\frac{\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Lambda_{n,k}^{j}\zeta_{n}}, \nonumber \\
		%& \nonumber \\
	%	\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j},r_{k}^j).
				\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j}).
		\end{align}
		%	Where the last step follows from the fact that  utility function used is $1-1$, so its derivative is also $1-1$ and its inverse $U_n^{'-1}(\alpha_k, \beta_{ik})$ can easily be computed.
	\item \textbf{$l \in \{\mathcal{M}\backslash\mathcal{M}_n\}$:} $\frac{\partial \mathcal{L}}{\partial x_{n,k}^{l}}=0$
		\begin{align}
	\label{eq:gradLagObjcase2}
	 f^{'l}_n(x_{n,k}^{l})(1+\Lambda_{n,k}^{l}\zeta_{n})-\Lambda_{n,k}^{l}(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})=0,\nonumber \\ 
	\implies  f^{'l}_n(x_{n,k}^{l})=\frac{\Lambda_{n,k}^{l}(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})}{1+\Lambda_{n,k}^{l}\zeta_{n}}, \nonumber \\
	%& \nonumber \\
	\implies \quad x_{n,k}^{*l}= f_{n}^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Lambda_{n,k}^{l}).
	\end{align}
	\end{enumerate}
\end{proof}

In cases where $u_n^{'-j}(\boldsymbol{.})$  and $f_{n}^{'-l}(\boldsymbol{.}) $ do not exist, one should use alternate methods such as {gradient based iterative equation}\cite{tychogiorgos2013non}: % in \eqref{eq:gradientbasediterative} can be used \cite{tychogiorgos2013non}.

\begin{align}
\label{eq:gradientbasediterative}
x_{n,k}^{j}(t+1)=x_{n,k}^{j}(t)+\epsilon_{n,k}^{j}\frac{\partial \mathcal{L}}{\partial x_{n,k}^{j}}
\end{align}
where $\epsilon_{n,k}^{j}$ is a positive step size. 
%Algorithm \ref{algo:centralnbs} shows our centralized algorithm that provides the NBS for \eqref{eq:opt_higher}. 

\end{comment}

	\begin{figure*}[!t]
	\normalsize
	\begin{align}
	\label{eq:lagrangian}
	\mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta, \zeta,\gamma,\pi})&= 
	\sum_{n=1}^{N}\ln\bigg(\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)- u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big)+\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-\nonumber\\
	&\hspace*{-1.3in}\quad u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)- D^l({x}_{n,k}^l)\big)\Big)-d^0_n\bigg) +   \quad \sum_{\substack{n \in \mathcal{N},\\j \in \mathcal{M},\\k \in \mathcal{K}}}\gamma_{n,k}^{j}x_{n,k}^{j} +\sum_{\substack{n \in \mathcal{N},\\k \in \mathcal{K}}}\alpha_{n,k} (C_{n,k}-\sum_{j \in \mathcal{M}}x_{n,k}^{j}) +\sum_{\substack{j \in \mathcal{M},\\k \in \mathcal{K}}}\beta_{k}^j (r_{k}^{j}-\sum_{n \in \mathcal{N}}x_{n,k}^{j}) + \sum_{n \in \mathcal{N}} \zeta_{n}  \nonumber \\
	& \hspace*{-1.3in}\quad \bigg(\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u_n^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)- u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big)+ \quad \Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)-\nonumber\\
	&\hspace*{-1.3in}\quad  D^l({x}_{n,k}^l)\big)\Big)-d_n^0
	\bigg)+\sum_{\substack{n\in \mathcal{{N}},\\l\in \overline{\mathcal{M}},\\k\in\mathcal{K}}}\pi_{n,k}^l \Big(u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-
	u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)-  D^l({x}_{n,k}^l)\Big).
	\end{align}
	\hrulefill
\end{figure*}
\section{Distributed algorithm for NBS}\label{sec:dist}
While resource allocation and sharing  using a central algorithm is feasible, it is desirable to develop low overhead distributed algorithms. %A distributed algorithm will eliminate the need for the coalition (central) controller discussed in Section \ref{sec:sysmodel} and domains can exchange information among each other.   %modern communication networks may require the ability to develop distributed algorithms without significant messaging overhead. 
To obtain a distributed algorithm,  we rely on \emph{Duality Theory} and use the \emph{Lagrangian} function   in \eqref{eq:lagrangian}. 
The dual optimization problem is given by %\vspace{-0.2in}
\begin{align}\label{eq:dualopt}
\min_{\boldsymbol{\alpha},\boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}} D(\boldsymbol{\alpha},\boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi})&= \mathcal{L}\big(\mathbf{X}^{*}(\boldsymbol{\alpha,\beta},\boldsymbol{\zeta,\gamma,\pi}),\nonumber \\& \boldsymbol{\alpha,\beta,\zeta,\gamma,\pi} \big), \nonumber \\
\; s.t. \; \boldsymbol{\alpha},\boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}\geq 0.
\end{align}
%whereas \vspace{-0.2in} 
%where \vspace{-0.12in}
\begin{align}\label{eq:supLag}
\mathbf{X}^{*}(\boldsymbol{\alpha,\beta},\boldsymbol{\zeta,\gamma,\pi})= \arg \max_{\mathbf{X}} \mathcal{L}(\mathbf{X},\boldsymbol{\alpha,\beta},\boldsymbol{\zeta,\gamma,\pi} ).
\end{align}
The dual problem can be solved iteratively using gradient descent (since the dual problem is a minimization problem) as below:
\begin{align}\label{eq:iterativeDual}
\alpha_{n,k}[t+1] &=  \alpha_{n,k}[t]- \phi_{n,k} \frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \alpha_{n,k}}, \nonumber \displaybreak[0] \\
\beta_{k}^j[t+1] &=  \beta_{k}^j[t]- \eta_{k}^j \frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \beta_{k}^j}, \nonumber \\
\zeta_{n}[t+1] &=  \zeta_{n}[t]- \omega_{n} \frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \zeta_{n}}, \nonumber \displaybreak[0]\\
\gamma_{n,k}^{j}[t+1] &=  \gamma_{n,k}^{j}[t]- \theta_{n,k}^{j} \frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \gamma_{n,k}^{j}},\nonumber \\
\pi_{n,k}^{l}[t+1]&=\pi_{n,k}^{l}[t]-\psi_{n,k}^l \frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \pi_{n,k}^{l}},
\end{align}
where $\phi_{n,k}$, $\eta_{k}^j$,  $\omega_{n}$, $\theta_{n,k}^{j}$ and $\psi_{n,k}^l$ are positive step sizes. Furthermore, the gradients in \eqref{eq:iterativeDual} are given below.%\vspace{-0.2in}
\begin{comment}
	\begin{figure*}[!t]
	\normalsize
	\begin{align}
	\label{eq:lagrangian2}
	\mathcal{L}(\mathbf{X}_n, \boldsymbol{\alpha}, \boldsymbol{\beta, \zeta,\gamma})&= %\sum_{n=1}^{N}\ln\bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\mathbf{x}_n^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg) +  \quad \sum_{n \in \mathcal{N}}\sum_{j \in \mathcal{M}}\sum_{k \in \mathcal{K}}\gamma_{n,k}^{j}x_{n,k}^{j} +\nonumber \\
	\prod_{n=1}^{N}\bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\mathbf{x}_n^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg) +  \quad \sum_{n \in \mathcal{N}}\sum_{j \in \mathcal{M}}\sum_{k \in \mathcal{K}}\gamma_{n,k}^{j}x_{n,k}^{j} +\nonumber \\
	& \quad\sum_{n \in \mathcal{N}}\sum_{k \in \mathcal{K}}\alpha_{n,k} (C_{n,k}-\sum_{j \in \mathcal{M}}x_{n,k}^{j}) + \sum_{j \in \mathcal{M}}\sum_{k \in \mathcal{K}}\beta_{k}^j (r_{k}^{j}-\sum_{n \in \mathcal{N}}x_{n,k}^{j}) + \sum_{n \in \mathcal{N}} \zeta_{n} \bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\mathbf{x}_n^j)+ \nonumber \\
	&  \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-  C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg).
	%	\mathcal{L}(\mathbf{X}_n, \boldsymbol{\alpha}, \boldsymbol{\beta, \zeta,\gamma})&= \sum_{n=1}^{N}\ln\bigg(\sum_{j \in \mathcal{M}_n}\big(u_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}} \frac{x_{n,k}^{j}}{r_{k}^{j}}\big)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg) +  \quad \sum_{n \in \mathcal{N}}\sum_{j \in \mathcal{M}}\sum_{k \in \mathcal{K}}\gamma_{n,k}^{j}x_{n,k}^{j} +\nonumber \\
	%	& \quad\sum_{n \in \mathcal{N}}\sum_{k \in \mathcal{K}}\alpha_{n,k} (C_{n,k}-\sum_{j \in \mathcal{M}}x_{n,k}^{j}) + \sum_{j \in \mathcal{M}}\sum_{k \in \mathcal{K}}\beta_{k}^j (r_{k}^{j}-\sum_{n \in \mathcal{N}}x_{n,k}^{j}) + \sum_{n \in \mathcal{N}} \zeta_{n} \bigg(\sum_{j \in \mathcal{M}_n}\big(u_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}} \frac{x_{n,k}^{j}}{r_{k}^{j}}\big)+ \nonumber \\
	%	&  \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-  C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg).
	\end{align}
	\hrulefill
	%	\vspace*{-5pt}
	%	\vspace{-0.15in}
\end{figure*}	
\end{comment}
\begin{align}\label{eq:gradforLagrangieMultipliers}
\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta}, \boldsymbol{\zeta,\gamma,\pi}) }{\partial  \alpha_{n,k}}&= (C_{n,k}-\sum_{j \in \mathcal{M}}x_{n,k}^{j}),\nonumber \\
\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta}, \boldsymbol{\zeta,\gamma,\pi}) }{\partial  \beta_{k}^j} &= (r_{k}^{j}-\sum_{n \in \mathcal{N}}x_{n,k}^{j}),\nonumber \\
\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \zeta_{n}} &=\bigg(\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)-  \nonumber \\
&\hspace*{-1.2in}u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big)+\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-\nonumber\\
&\hspace*{-1.2in}u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)- D^l({x}_{n,k}^l)\big)\Big)-d_n^0
\bigg)
, \nonumber \\
\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \gamma_{n,k}^{j}} &= x_{n,k}^{j},\nonumber\\
\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \pi_{n,k}^{l}} &=\Big(u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-\nonumber \\
&\hspace*{-1.2in}
u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)-  D^l({x}_{n,k}^l)\Big).
\end{align}
%%Since the primal problem is convex, the convergence of the primal-dual algorithm that consists of \eqref{eq:supLag} and \eqref{eq:iterativeDual} is guaranteed \cite{panigrahy2017and} i.e., it will converge to the unique global optimal with zero-duality gap. Algorithm \eqref{algo:primal-dual-alg} shows our primal-dual algorithm. 
Unless certain  conditions such as Slater's constraint qualification  are satisfied, \emph{strong duality}\footnote{Strong duality implies that there is no duality gap between the primal and dual problem.} is not guaranteed to hold for our primal and dual problems \cite{boyd2004convex}. However,  we rely on the following theorems to show that strong duality holds.
\begin{theorem}[Sufficient Condition\cite{tychogiorgos2013non}]\label{thm:georgesufficient}
	If the price based function $\mathbf{X}^*(\boldsymbol{\alpha,\beta},\boldsymbol{\zeta,\gamma,\pi})$ is continuous at one or more of the optimal Lagrange multipliers,  the iterative algorithm consisting of  \eqref{eq:supLag} and \eqref{eq:iterativeDual} will converge to the global optimal solution. 
\end{theorem}
\begin{theorem}[Necessary Condition\cite{tychogiorgos2013non}]\label{thm:georgenecessary}
	The condition in Theorem \ref{thm:georgesufficient} is also necessary if at least one of the constraints in \eqref{eq:objmain2} is active (binding) at the optimal solution. % and eliminate the need for a central controller. The domain controllers can exchange  information about capacities, and  requirements and obtain the NBS.  
\end{theorem}
\begin{lemma}\label{lem:constraintsactive}
	At the optimal solution, the optimal Lagrange multiplier vector corresponding to the capacity constraint is non-zero, i.e., $\boldsymbol{\alpha_k^{*}}>0$. 
\end{lemma}
\begin{proof}
	At the optimal point, all  resources are fully utilized,  i.e., capacity constraints are active. From \emph{complementary slackness}\cite{boyd2004convex}, we know that %\vspace{-0.08in}
	\begin{align}\label{eq:compslackness}
	\alpha^*_{n,k}\bigg(\sum_{j\in \mathcal{M}} x_{n,k}^{*j}- C_{n,k}\bigg)=0, \forall n \in \mathcal{N}. 
	\end{align}
	Since $\sum_{j\in \mathcal{M}} x_{n,k}^{*j}= C_{n,k}$, i.e., the constraint is active, which implies that $\boldsymbol{\alpha_k^{*}} >0$.
\end{proof}
%\vspace{-0.12in}
\begin{theorem}\label{thm:duality}
For any concave injective utility function for which the inverse of the first derivative exists, the iterative distributed algorithm consisting of  \eqref{eq:supLag} and \eqref{eq:iterativeDual}  converges to the global optimal solution.% i.e., strong duality holds.% for our resource sharing and allocation problem if we use a concave, injective utility function for which the inverse of  first derivative exists. 
\end{theorem}
%\begin{proof}
%	See Appendix \ref{sec:FirstAppendix} for the proof
%	\end{proof}
\begin{proof}
	We show that the price function obtained by $\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi})}{\partial x_{n,k}^{j}}=0$ is continuous at one or more of the optimal Lagrange multipliers for \eqref{eq:lagrangian}.  
	
	Let  $u^{'-j}(\boldsymbol{.})$ %(\alpha_{n,k}, \beta_{k}^j,\zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j})$ 
	and $f^{'-l}(\boldsymbol{.})$ %%(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Lambda_{n,k}^{l})$ 
	represent   %and $u_{jn}^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)})$ are
	the inverses of the first derivative of $u^j$ and $\big(u^l(\sum_{m\in\overline{\mathcal{N}}} x_{m,k}^l+x_{n,k}^l)-u^l(\sum_{m\in\overline{\mathcal{N}}} x_{m,k}^l) -D^l(x_{n,k}^l)\big)$, respectively. %and $u_j^n$ respectively. 
	$\alpha_{n,k}$,  $\beta_{k}^j$, $\zeta_{n}$,  $\gamma_{n,k}^{j}$ and $\pi_{n,k}^l$ are the \emph{Lagrange} multipliers whereas:   
	\begin{align}
	\Delta_{n}&=\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)- u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big)+ \nonumber \\
	&\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)- \nonumber\\
	&D^l({x}_{n,k}^l)\big)\Big)-d_n^0
	%\sum_{j \in \mathcal{M}_n}\Big(u_n^j(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^j+\mathbf{x}_n^j)- u_n^j(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^j) \Big)+ \nonumber \\
	%&\Big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^l+\mathbf{x}_n^l)-u_n^l(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^l)-\nonumber\\ &D_n^l(\mathbf{x}_n^l)\Big)-d_n^0, \nonumber 
	\end{align}
	We consider two different cases
% There are two different cases that we evaluate in the following: %To simplify the proof, we only consider the case  in which $i \in \mathcal{M}_n$ below. The proof for the case when $i \in \mathcal{M}\backslash\mathcal{M}_n$ is similar. 
	%\begin{enumerate}
	%	\item 
%	\vspace{-0.12in}
	
	\subsubsection{	\textbf{$j \in \mathcal{M}_n$:}$\frac{\partial \mathcal{L}}{\partial x_{n,k}^{j}}=0$}
%	\vspace{-0.05in}
		\begin{align}
		\label{eq:gradLagObj22}
		&u^{'j}(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+x_{n,k}^{j})(1+\Delta_{n}^{}\zeta_{n})-\Delta_{n}^{}(\alpha_{n,k}+\nonumber \\
		&\beta_{k}^j-\gamma_{n,k}^{j})=0,\nonumber \\	
		&\implies u^{'j}(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+x_{n,k}^{j})=\frac{\Delta_{n}^{}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n}^{}\zeta_{n}}, \nonumber \\
		& x_{n,k}^{j}=u^{'-j}\Bigg(\frac{\Delta_{n}^{}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n}^{}\zeta_{n}}\Bigg)-\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j. %\nonumber \\
		%& \nonumber \\
		%	\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j},r_{k}^j).
		%	&\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Delta_{n,k}^{j}).
		%\vspace{-0.12in}
		\end{align}
		 We prove that \eqref{eq:gradLagObj22} is continuous at the optimal point by showing that the numerator $\Delta_{n}^{}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})$ and denominator $1+\Delta_{n}^{}\zeta_{n} $ are positive\footnote{Positive numerator and denominator are required if $u^{'-j}$ is $\log$. For other cases, it will suffice to prove that the denominator is non-zero. }. 	At the optimal point, the denominator $(1+\Delta_{n}^{*}\zeta^*_{n})$ is positive as $\Delta_{n}^{*}>0$ (from Section \ref{sec:assumption}) and $\zeta^*_{n}=0$ (from complementary slackness).	Similarly, in the numerator, %$\Delta_{n,k}^j$ (from Section \ref{sec:assumption}) and $e^{(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j-\bar{r}_{n,k}^j)}$ are positive.
		 $(\alpha^*_{n,k}+\beta_{k}^{*j}-\gamma_{n,k}^{*j})>0$, as  $\alpha_{n,k}^{*}>0$ (from Lemma \ref{lem:constraintsactive}) and  $\alpha_{n,k}^{*}+\beta_{k}^{*j}> \gamma_{n,k}^{*j}$ (from \emph{sensitivity analysis} \cite{boyd2004convex}). Hence, \eqref{eq:gradLagObj22} is continuous at the optimal point.
		  \begin{comment}
		 As an example, we set
		 	For sake of the proof, we set \\ $u_n^j=1-e^{-(x_{n,k}^j+\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j-r_{n,k}^j+\delta t)}$ where $\bar{r}_{k}^j=r_{k}^j+\delta t$. %However, the results hold for any concave injective utility function for which the inverse of the first derivative exists.  
		 	\eqref{eq:gradLagObj22} can then be rewritten as:
		 \begin{align}\label{eq:proof1}
		 e^{-(x_{n,k}^j+\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j-\bar{r}_{k}^j)}= \frac{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n,k}^{j}\zeta_{n}},\quad\nonumber \\
		 e^{x_{n,k}^j}= \frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{k}^j)}},\quad\quad\nonumber \\
		 x_{n,k}^j=\ln\bigg(\frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{k}^j)}}\bigg).
		 \end{align} 
		 where \eqref{eq:proof1} is continuous at the optimal point. 
		  
		
		
		 For \eqref{eq:gradLagObj22} to be continuous at the optimal point,
		
		 we need 
		%\vspace{-0.1in}
		For sake of the proof, we set \\ $u_n^j=1-e^{-(x_{n,k}^j+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-r_{n,k}^j+\delta t)}$ where $\bar{r}_{k}^j=r_{k}^j+\delta t$. However, the results hold for any concave injective utility function for which the inverse of the first derivative exists.  \eqref{eq:gradLagObj22} can then be rewritten as:
		\begin{align}\label{eq:proof1}
		 e^{-(x_{n,k}^j+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{k}^j)}= \frac{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n,k}^{j}\zeta_{n}},\quad\nonumber \\
		e^{x_{n,k}^j}= \frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{k}^j)}},\quad\quad\nonumber \\
		x_{n,k}^j=\ln\bigg(\frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{k}^j)}}\bigg).
		\end{align} 
		%We know that $\Lambda_{ik}^{(n)>0$, 
		For continuity, we need both the numerator and denominator inside the $\ln(\boldsymbol{.})$ function of \eqref{eq:proof1} to be positive.  
		At the optimal point, the numerator $(1+\Delta_{n,k}^{*j}\zeta^*_{n})$ is positive as $\Delta_{n,k}^{*j}>0$ (from Section \ref{sec:assumption}) and $\zeta^*_{n}=0$ (from complementary slackness).	Similarly, in the denominator, $\Delta_{n,k}^j$ (from Section \ref{sec:assumption}) and $e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}$ are positive. $(\alpha^*_{n,k}+\beta_{k}^{*j}-\gamma_{n,k}^{*j})>0$, as  $\alpha_{n,k}^{*}>0$ (from Lemma \ref{lem:constraintsactive}) and  $\alpha_{n,k}^{*}+\beta_{k}^{*j}> \gamma_{n,k}^{*j}$ (from \emph{sensitivity analysis} \cite{boyd2004convex}). %Furthermore, the denominator $(r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}^*+\beta_{k}^{*j}- \gamma_{n,k}^{*j})-1>0)$ based on our assumptions in Section \ref{sec:assumption}.
		Hence, the price based function in \eqref{eq:proof1} is continuous in at least one optimal Lagrange multiplier vector. 
		\end{comment}
\\		
		%	Where the last step follows from the fact that  utility function used is $1-1$, so its derivative is also $1-1$ and its inverse $U_n^{'-1}(\alpha_k, \beta_{ik})$ can easily be computed.
		%\item 
		\subsubsection{\textbf{$l \in \{\mathcal{M}\backslash\mathcal{M}_n\}$:} $\frac{\partial \mathcal{L}}{\partial x_{n,k}^{l}}=0$}
		\begin{align}
		\label{eq:gradLagObjcase22}
		&f^{'l}(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+x_{n,k}^{l})(1+\Delta_{n}^{}\zeta_{n}+\Delta_{n}^{}\pi_{n,k}^l)-\Delta_{n}^{}(\alpha_{n,k}+\nonumber \\
		&\beta_{k}^l-\gamma_{n,k}^{l})=0,\nonumber \\
		&\implies  f^{'l}(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+x_{n,k}^{l})=\frac{\Delta_{n}^{}(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})}{1+\Delta_{n}^{}\zeta_{n}+\Delta_{n}^{}\pi_{n,k}^j}. \nonumber \\
		&  x_{n,k}^{l}=f^{'-l}\Bigg(\frac{\Delta_{n}^{}(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})}{1+\Delta_{n}^{}\zeta_{n}+\Delta_{n}^{}\pi_{n,k}^l}\Bigg)-\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l. \nonumber \\
		\end{align}
%	\end{enumerate}
\begin{comment}
	As done earlier, we set  $u_n^l=1-e^{-(x_{n,k}^l+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^l-\bar{r}_{k}^l)}$, \\ and $C_n^l=x_{n,k}^l/w_k^l$, where $w_k^l$ is a positive weighting factor to capture  the communication cost. Then $ f^{'l}_n(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^l+x_{n,k}^{l})$ can be rewritten as 
	\begin{align}
	\label{eq:fnl}
	 f^{'l}_n(\boldsymbol{.})= e^{-(x_{n,k}^l+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^l-\bar{r}_{k}^l)}-\frac{1}{w_k^l}
	\end{align}
Plugging \eqref{eq:fnl} in \eqref{eq:gradLagObj22} and solving for $x_{n,k}^l$, we obtain
	\begin{align}
	\label{eq:fnl2}
	x_{n,k}^l=\ln \Bigg(\frac{w_k^l(1+\Delta_{n,k}^{l}\zeta_{n})e^{-(\sum_{m \in \mathcal{N}\backslash n}x_{m,k}^l-\bar{r}_{k}^l)}}{w_k^l\Delta_{n,k}^l(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})+1+\Delta_{n,k}^{l}\zeta_{n}}\Bigg).
	\end{align}
	\end{comment}
	The continuity at optimal point can be established using arguments similar  to that for  $j \in \mathcal{{M}}_n$ case. The proof of zero-duality gap follows from Theorem \ref{thm:georgesufficient}.  Hence, strong duality holds and our proposed distributed algorithm converges to the NBS. 
\end{proof}

\begin{comment}
\begin{proof}
	We show that the price function obtained by $\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma})}{\partial x_{n,k}^{j}}=0$ is continuous at one or more of the optimal Lagrange multipliers for \eqref{eq:lagrangian2}. Let $\Delta_{n,k}^{j}=\prod_{t\in \{\mathcal{N}\backslash n\}}\bigg(\sum_{j \in \mathcal{M}_t}u_t^j(\mathbf{x}_t^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_t\}} u_t^l(\mathbf{x}_t^l)-C_n^l(\mathbf{x}_t^l)\big)-d_t^0\bigg)$. %To simplify the proof, we only consider the case  in which $i \in \mathcal{M}_n$ below. The proof for the case when $i \in \mathcal{M}\backslash\mathcal{M}_n$ is similar. 
	
	
		\begin{enumerate}
		\item \textbf{$j \in \mathcal{M}_n$:}$\frac{\partial \mathcal{L}}{\partial x_{n,k}^{j}}=0$
		\begin{align}
		\label{eq:gradLagObj22}
		%	 \Big(u_n^{'j}(x_{n,k}^{j})+\frac{1}{r_{k}^j}\Big)(1+\Lambda_{n,k}^{j}\zeta_{n})-\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j-\nonumber \\
		%	 \gamma_{n,k}^{j})=0,\nonumber \\
		u_n^{'j}(x_{n,k}^{j})(\Delta_{n,k}^{j}+\zeta_{n})-(\alpha_{n,k}+\beta_{k}^j-\gamma_{n,k}^{j})=0,\nonumber \\	
		%	 \implies u_n^{'j}(x_{n,k}^{j})=\frac{\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Lambda_{n,k}^{j}\zeta_{n}}-\frac{1}{r_{k}^j}, \nonumber \\
		\implies u_n^{'j}(x_{n,k}^{j})=\frac{(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{\Delta_{n,k}^{j}+\zeta_{n}}, \nonumber \\
		%& \nonumber \\
		%	\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j},r_{k}^j).
		\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Delta_{n,k}^{j}).
		\end{align}
		%	Where the last step follows from the fact that  utility function used is $1-1$, so its derivative is also $1-1$ and its inverse $U_n^{'-1}(\alpha_k, \beta_{ik})$ can easily be computed.
		\item \textbf{$l \in \{\mathcal{M}\backslash\mathcal{M}_n\}$:} $\frac{\partial \mathcal{L}}{\partial x_{n,k}^{l}}=0$
		\begin{align}
		\label{eq:gradLagObjcase22}
		f^{'l}_n(x_{n,k}^{l})(\Delta_{n,k}^{l}+\zeta_{n})-(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})=0,\nonumber \\ 
		\implies  f^{'l}_n(x_{n,k}^{l})=\frac{(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})}{\Delta_{n,k}^{l}+\zeta_{n}}, \nonumber \\
		%& \nonumber \\
		\implies \quad x_{n,k}^{*l}= f_{n}^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Delta_{n,k}^{l}).
		\end{align}
	\end{enumerate}
	
	

	\begin{align}
\label{eq:gradLagObj2}
u_n^{'j}(x_{n,k}^{j})(1+\Lambda_{n,k}^{j}\zeta_{n})-\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})=0,\nonumber \\
\implies u_n^{'j}(x_{n,k}^{j})=\frac{\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Lambda_{n,k}^{j}\zeta_{n}}, \nonumber \\
%& \nonumber \\
\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j}).
\end{align}	
	\end{comment}
%		\begin{align}
%	\label{eq:gradLagObj2}
%	 u'_n(x_{ik}^{(n)})(1+\Lambda_{ik}^{(n)}\zeta^{(n)})-\Lambda_{ik}^{(n)}(\alpha_k^{(n)}+\beta_{ik}- \gamma_{ik}^{(n)})=0,\nonumber \\
%\implies u'_n(x_{ik}^{(n)})=\frac{\Lambda_{ik}^{(n)}(\alpha_k^{(n)}+\beta_{ik}-\gamma_{ik}^{(n)})}{1+\Lambda_{ik}^{(n)}\zeta^{(n)}}. % \nonumber \\
%& \nonumber \\
%\implies \quad x_{ik}^{*(n)}= U_n^{'-1}(\alpha_k^{(n)}, \beta_{ik}, \zeta^{(n)},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)})
%	\end{align}
%	\vspace{-0.12in}
\begin{comment}	
To simplify the proof, we only consider the case  in which $j \in \mathcal{M}_n$ below. The proof for the case when $i \in \mathcal{M}\backslash\mathcal{M}_n$ is similar. For illustrative purpose, we use $\bigg(1-e^{-{x_{n,k}^{j}}}\bigg)$ % $\ln(x_{n,k}^{j})$ 
as the utility. However, the results hold true for any concave injective utility function for which  inverse of the first derivative exists.  \eqref{eq:gradLagObj} is rewritten as:
%such as $\log (x_{ik}^{(n)})$ on $\mathbb{R}_{++}$, \eqref{eq:gradLagObj2} is rewritten as
\begin{align}\label{eq:priceLog}
e^{-{x_{n,k}^{j}}}&=\frac{(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{\Delta_{n,k}^{j}+\zeta_{n}},\nonumber \\
%e^{-{x_{n,k}^{j}}}&=\frac{r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})-(1+\Lambda_{n,k}^{j}\zeta_{n})}{r_k^j(1+\Lambda_{n,k}^{j}\zeta_{n})},\nonumber \\
\implies x_{n,k}^{j}&=\ln\bigg(\frac{\Delta_{n,k}^{j}+\zeta_{n}}{(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}\bigg).
%\implies x_{n,k}^{j}&=\ln\bigg(\frac{r_k^j(1+\Lambda_{n,k}^{j}\zeta_{n})}{r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})-(1+\Lambda_{n,k}^{j}\zeta_{n})}\bigg).
%\frac{1}{x_{ik}^{(n)}}=\frac{\alpha_k^{(n)}+\beta_{ik}}{1+\zeta^{(n)}} \implies {x_{ik}^{(n)}}= \frac{1+\zeta^{(n)}}{\alpha_k^{(n)}+\beta_{ik}}%{x_{ik}^{(n)}}=
\end{align} 
%We know that $\Lambda_{ik}^{(n)>0$, 
%For continuity, we need both the numerator and denominator inside the $\ln(\boldsymbol{.})$ function of \eqref{eq:priceLog} to be positive.  
At the optimal point, the numerator $(\Delta_{n,k}^{*j}+\zeta^*_{n})$ is positive as $\Delta_{n,k}^{*j}>0$ (from Section \ref{sec:assumption}) and $\zeta^*_{n}=0$ (from complementary slackness). %Hence, \eqref{eq:priceLog} can be rewritten as 
%\begin{align}\label{eq:priceLog2}
 %x_{n,k}^{*j}&=\ln\bigg(\frac{r_k^j}{r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}^*+\beta_{k}^{*j}- \gamma_{n,k}^{*j})-1}\bigg).
%\end{align} 
Similarly, $(\alpha^*_{n,k}+\beta_{k}^{*j}-\gamma_{n,k}^{*j})>0$, as  $\alpha_{n,k}^{*}>0$ (from Lemma \ref{lem:constraintsactive}) and  $\alpha_{n,k}^{*}+\beta_{k}^{*j}> \gamma_{n,k}^{*j}$ (from \emph{sensitivity analysis} \cite{boyd2004convex}). %Furthermore, the denominator $(r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}^*+\beta_{k}^{*j}- \gamma_{n,k}^{*j})-1>0)$ based on our assumptions in Section \ref{sec:assumption}.
Hence, the price based function in \eqref{eq:priceLog} is continuous in at least one optimal Lagrange multiplier vector. The proof follows from Theorem \ref{thm:georgesufficient}. 
\end{proof}
\end{comment}
For calculating $x_{n,k}^{j}$ at time $t$, we use $\Delta_{n}^{}$ calculated at $t-1$. 
Algorithm \ref{algo:primal-dual-alg} is a distributed algorithm that provides the global optimal solution to \eqref{eq:nashProbNplayermod}.
\paragraph{Protocol for Distributed Execution}
All ESPs first broadcast information regarding resource requests from their native applications. Then any randomly chosen ESP starts allocating resources as specified in Step $2$ of Algorithm \ref{algo:primal-dual-alg} and updates the corresponding Lagrangian multipliers. This ESP then  passes on the information about its allocation  and updated request matrix to the next ESP (that has not yet allocated resources in the current round\footnote{A single round consists of all the ESPs executing Step $2$ of Algorithm \ref{algo:primal-dual-alg} once.}) that repeats the  same procedure until all the ESPs allocate their resources.    This process continues until the first order conditions given in \cite{ktlagrangian} are met. 
%ESPs need to exchange information related to requests and  allocation decision. Al 
%\paragraph{Convergence Properties of the Algorithm}
%The convergence of our proposed algorithm depends on a number of factors such as the requests, capacities, and utilities used along with the step size for gradient descent. In particular, the step size must be carefully chosen as a very small step size can slow  the convergence rate, whereas a large step size will result in divergence. 

 
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $\forall\; \boldsymbol{\alpha_0,\; \beta_0,\zeta_0,\gamma_0,\pi_0}$, $C, R$, vector of utility function of all ESPs $\boldsymbol{u}$  and $\mathbf{X}_0$ %$\forall \boldsymbol{\nu_0$, $\mu_0}\in\mathcal{R}$ and $\boldsymbol h_0$ 
		\State \textbf{Output}: The optimal resource allocation $\mathbf{X} $ and payoffs of all ESPs
		\State \textbf{Step $0$:}  $t=0$, $\boldsymbol \alpha[t]\leftarrow\boldsymbol \alpha_0$, $\boldsymbol\beta[t]\leftarrow\boldsymbol\beta_0$, $\boldsymbol\zeta[t]\leftarrow\boldsymbol\zeta_0$, $\boldsymbol\gamma[t]\leftarrow\boldsymbol\gamma_0$,$\boldsymbol\pi[t]\leftarrow\boldsymbol\pi_0$$, \mathbf{X}[t]\leftarrow \mathbf{X}_0$
			\State \textbf{Step $1$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {d_n^0} \leftarrow$ \texttt{Objective function at optimal point in Equation \eqref{eq:opt_single}}
		\EndFor
		\State \textbf{Step 2: $t\geq 1$} 
		\While{{First order conditions\cite{ktlagrangian}$\neq$true }}%{Equation \eqref{eq:gradforLagrangieMultipliers} $\neq$ 0}
		\State Compute $ x_{n,k}^{j}[t+1]$ for $j\in\mathcal{M},$ $k\in\mathcal{K}$ and $n\in\mathcal{N}$ through \eqref{eq:gradLagObj22} and \eqref{eq:gradLagObjcase22};
		\State Compute $\boldsymbol\alpha[t+1]$, $\boldsymbol\beta[t+1]$, $\boldsymbol\zeta[t+1]$,  $\boldsymbol\gamma[t+1]$ and $\boldsymbol\pi[t+1]$ through~(\ref{eq:iterativeDual}) given $\mathbf{X}[t+1],$ $\boldsymbol\alpha[t]$,  $\boldsymbol \beta[t]$, $\boldsymbol \zeta[t]$,  $\boldsymbol\gamma[t]$ and $\boldsymbol\pi[t]$%for $l\in V,$ $i\in\mathcal{D}$ and $p\in\mathcal{P}^i$
		\EndWhile
	%	\State \textbf{Step 2:} $P_n^j\leftarrow$ \texttt{Payoff received by ESP} $\forall n \in \mathcal{{N}}, j \in \mathcal{{M}}$\texttt{ using \eqref{eq:payoffrule}} 
	\end{algorithmic}
	\caption{Distributed Algorithm for NBS}
	\label{algo:primal-dual-alg}
\end{algorithm}

 


==> arxiv version/arxiv version/preli.tex <==
\begin{comment}
In this section, we present an overview of  Multi-Objective Optimization (MOO), bargaining theory  and Nash Bargaining Solution (NBS). %\vspace{-0.1in}
\subsection{Multi-Objective Optimization}
 For $m$ inequality constraints and $p$ equality constraints, the MOO problem is to identify a vector $\boldsymbol{x}^*=[x_1^*,x_2^*,\cdots ,x_t^*]^T$ that maximizes a vector function
	\begin{equation}\label{eq:vectorobjective}
	\centering 
	\bar{f}(\boldsymbol{x})=[f_1(\boldsymbol{x}),f_2(\boldsymbol{x}),\cdots,f_N(\boldsymbol{x})]^T
	\end{equation}
	subject to 
	\begin{align}\label{eq:constraints}
	\centering 
	& g_i(\boldsymbol{x})\geq 0, \; i=1,2,\cdots,m, \\
	&h_i(\boldsymbol{x})=0\;\; i=1,2,\cdots,p, \nonumber
	\end{align}
	where $N$ is the total number of objectives,  $\boldsymbol{x}=[x_1,x_2,\cdots ,x_t]^T$ is a vector of $t$ decision variables and the feasible set is denoted by $F$.
The fundamental difference from  single objective optimization (SOO)  is that MOO involves a vector of objective functions rather than a single objective function. This indicates that the solution is not a single point but a \emph{frontier} of solutions known as \emph{Pareto frontier} or \emph{Pareto boundary} (see \cite{cho2017survey} for details). Some basic definitions related to MOO are: 
\begin{definition}{Strongly Pareto non-dominated solution\cite{cho2017survey}:}
%	\small
	A feasible solution $x$ is strongly Pareto non-dominated if there is no $y\in F$ such that $f_n(y)\geq f_n(x)$ $\forall n=1,2,\cdots,N$ and $f_n(y)>f_n(x)$ for at least one $n$\footnote{This means that there is no other feasible solution that can improve an objective without worsening at least one other objective.}.
\end{definition}
\begin{definition}{Weakly Pareto non-dominated solution\cite{cho2017survey}:}
%	\small
	A feasible solution $x$ is weakly Pareto non-dominated if there is no $y\in F$ such that $f_n(y)>f_n(x)$ $\forall n=1,2,\cdots,N.$
\end{definition}





\begin{definition}{Pareto Optimality\cite{cho2017survey}:}
	For any maximization problem,  $\boldsymbol{x}^*$ is $Pareto\; optimal$ if the following holds for every $\boldsymbol{x} \in F$
	\begin{align}\label{eq:paretoptimality}
	\bar{f}(\boldsymbol{x}^*)\geq\bar{f}(\boldsymbol{x}) 
	\end{align}
	where $\bar{f}(\boldsymbol{x})=[f_1(\boldsymbol{x}),f_2(\boldsymbol{x}),\cdots,f_k(\boldsymbol{x})]^T$ and  
	$\bar{f}(\boldsymbol{x}^*)=[f_1(\boldsymbol{x}^*),f_2(\boldsymbol{x}^*),\cdots,f_k(\boldsymbol{x}^*)]^T$.
\end{definition}

\subsection{Bargaining Theory}
%In any trade or sharing of resources among different entities, where the entities may have conflicting interests, reaching an agreement and deciding the terms of agreement is a challenge. 
In a \emph{bargaining situation}, two or more  players (service providers) can benefit by reaching an agreement. However,  players can have conflicting interests regarding the terms of the agreement. \emph{Bargaining theory} deals with studying such bargaining situations arising in a number of problems. In resource allocation  problem,  resource providers are interested in maximizing their utility (pay-off)  by satisfying the requests of different applications. 
%\par  The four main challenging issues surrounding bargaining theory are efficiency, selection of an outcome, coordination of strategies to obtain an outcome and the enforcement of agreement (see \cite{han2012game} for details). 
%\begin{enumerate}
%	\item \textbf{Efficiency:} A bargaining problem can have  a number of outcomes. Therefore, it is important to identify solutions that are beneficial for all players involved in the bargaining problem. 
%	\item \textbf{Distribution:} Once the solutions are identified, the next step is to select an outcome from the set of solutions. 
%	\item \textbf{Coordination of Strategy:} Following the selection of an outcome, the next step is to identify the joint strategy to obtain that solution. 
%	\item \textbf{ Enforcement of Agreement:}  The terms of agreement are identified for enforcing the chosen strategy. 
%\end{enumerate}
%Two important components of bargaining theory are the bargaining process and  bargaining outcome. Bargaining process deals with the procedure and steps a bargainer must take to reach an agreement over a chosen bargaining outcome. Bargaining outcome is obtained following the bargaining process. 
Below we discuss one of  the most widely used bargaining solutions, i.e., \emph{Nash Bargaining Solution} as it guarantees the Pareto optimality \cite{khan2009cooperative}. 
\end{comment}
%\subsection{Nash Bargaining Solution (NBS)}
%Nash, \cite{nash1950bargaining}, abstracted the bargaining process and only dealt with bargaining outcome using an axiomatic approach. 
We use a two-player game as a toy example to introduce NBS.  Consider two players $1,$ and  $2$ that need to reach an agreement (e.g., resource allocation decision) in an outcome space $\mathcal{A}\subseteq \mathbb{R}^2$ \cite{han2012game}. Both players have a utility given by $u_1$ and $u_2$ over the space $\mathcal{A} \cup \{D\}$ where $D$ specifies a \emph{disagreement outcome} for players in the event of a disagreement, i.e., when  two players cannot reach an agreement. Let $\mathcal{S}$ be the set of all possible utilities that both  players can achieve: %\vspace{-0.1in}

\begin{align}
\label{eq:possibleut}
\mathcal{S}= \{(u_1(a_1),u_2(a_2)) | (a_1,a_2) \in \mathcal{A} \}
\end{align}

We also define $d=(d_1, d_2)$, where $d_1=u_1(D)$ and $d_2=u_2(D)$, as the payoff each player receives at the disagreement point. We define the bargaining problem  as the pair $(\mathcal{S},d)$ where $\mathcal{S} \subset \mathbb{R}^2$ and $d \in \mathcal{S}$ such that 
\begin{itemize}
	\item $\mathcal{S}$ is a convex and compact set;
	\item There exists $s \in \mathcal{S}$ such that $s > d$.
\end{itemize}
In NBS, the goal is to obtain a function $f(\mathcal{S},d)$ that provides  a unique outcome in $ \mathcal{S}$ for every bargaining problem $(\mathcal{S},d)$. Nash studied the possible outcomes (agreements) that players can reach whereas the agreements, along with the Pareto optimality, must also  satisfy the following set of  axioms (also called \emph{fairness} axioms) \cite{han2012game}:
\begin{enumerate}
%	\item \textbf{Pareto Optimality}
	\item \textbf{Symmetry:}  The bargaining solution will not discriminate among  players if players are indistinguishable, i.e., players have identical utilities. 
	\item \textbf{Invariance to equivalent utility representation:} If a bargaining problem  $(\mathcal{S},d)$ is transformed into another bargaining problem  $(\mathcal{S}',d')$ where $s_i'=\gamma_is_i+\zeta_i$ and $d_i'=\gamma_id_i+\zeta_i$, $\gamma_i >0$, then $f( \mathcal{S}',d')=\gamma_if(\mathcal{S},d)+\zeta_i$
	\item \textbf{Independence of irrelevant alternatives:} For any two bargaining problems  $(\mathcal{S},d)$ and  $(\mathcal{S}',d)$ where $\mathcal{S}'\subseteq \mathcal{S}$, if $f(\mathcal{S},d) \in \mathcal{S}'$, then $f(\mathcal{S}',d)=f(\mathcal{S},d)$. %This means that if any bargaining problem in any region $\mathcal{S}$ results in an outcome $f(\mathcal{S},d)$, which lies in $\mathcal{S}'\subseteq \mathcal{S}$, then any hypothetical bargaining problem in $\mathcal{S}'$ will also result in the same solution. 
\end{enumerate}
\cite{nash1950bargaining} shows that there is a unique bargaining solution that satisfies above axioms. We present it in the following theorem. 
\begin{theorem}{\cite{han2012game}}
	There exists a unique solution satisfying the aforementioned axioms and this solution is the pair of utilities $(s_1^*,s_2^*) \in \mathcal{S}$ that solves the following optimization problem:
	\begin{align}
	\label{eq:nashProb}
	\max_{s_1,s_2}\;(s_1-d_1)(s_2-d_2),\; s.t. (s_1,s_2)\in \mathcal{S}, \; (s_1,s_2)\geq (d_1,d_2).
	\end{align}\
\end{theorem}
The solution of \eqref{eq:nashProb} is the NBS. % Nash in \cite{nash1950bargaining} derived the NBS for only two players. However, it has been extended to 
The above framework can be extended to $N$ players  by allowing $\mathcal{S}$ to be an $N$-dimensional space \cite{harsanyi1963simplified}. For this case, the bargaining problem $(\mathcal{S},d)$, with $d=(d_1,d_2,\cdots, d_N)$ as the disagreement point, becomes the unique solution of the optimization problem below.
%\vspace{-0.1in}
	\begin{align}\vspace{-0.1in}
\label{eq:nashProbNplayer}
\max_{s_1,\cdots,s_N}&\;\prod_{n=1}^{N}(s_n-d_n),\; \nonumber \\
s.t.\quad  &(s_1,\cdots,s_N)\in \mathcal{S}, \nonumber \\
& (s_1,\cdots,s_N)\geq (d_1,\cdots, d_N).
\end{align}
Solving \eqref{eq:nashProb} is easier compared to the $N-$player bargaining problem in \eqref{eq:nashProbNplayer}\cite{han2012game}. %Different optimization techniques such as the bisection method can be used to obtain the NBS for an $N-$player bargaining problem. 
In this paper, we transform our problem into an equivalent convex problem that is comparatively easier to solve.  
 
\begin{remark}
  As each player in an  $N$-player bargaining game has a particular objective to optimize, the resulting problem is multi-objective,  where the goal is to obtain a Pareto optimal solution. NBS is a fair and Pareto optimal solution for such MOO problems, provided that the fairness axioms are satisfied.  % as it takes the objective of every game player into account. 
\end{remark}%\vspace{-0.25in}

\begin{comment}
\subsection{Cooperative Game Theory}
Cooperative game theory is the set of analytical tools that assists in understanding the behavior of rational players in a cooperative setting \cite{han2012game}. Players can have agreements among themselves that affects the strategies as well as obtained utilities of the players. Cooperative games are primarily of two types: bargaining theory and coalition games. Bargaining theory deals with the bargaining process that arise among the players while joining an agreement while coalition games deals with the formation of the coalitions among cooperating players. Formally

\begin{definition}{Coalition Games \cite{han2012game}:}
Any coalition game can be represented by the pair $(\mathcal{N},v)$ where $\mathcal{N}$ is the set of players that play the game, while $v$ is the mapping function that determines the utilities or payoffs the players in $\mathcal{N}$ receive. 
\end{definition}

\begin{definition}{Characteristic form Coalition Games: \cite{han2012game}:}
	Any coalition game is said to be of \emph{characteristic} form where the value of coalition $S \subseteq \mathcal{N}$ depends only on the members of coalition. 
\end{definition}

\begin{definition}{Transferable Utility (TU):}
If the total utility of any coalition can be divided in any manner among the game players, then the game has a \emph{transferable} utility. 
\end{definition}

\begin{definition}{Characteristic function:}
The characteristic function for any coalitional game with TU is a mapping $v: 2^{\mathcal{N}} \mapsto \mathbb{R}$ with $v(\emptyset)=0$
\end{definition}

\begin{definition}{Superadditivity of TU games:}
A canonical game with TU is said to be superadditive if the following property is satisfied. 
\begin{equation}\label{eq:superadditivity}
v(S_1 \cup S_2 )\geq v(S_1)+V(S_2) \; \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, s.t. S_1\cap S_2 =\emptyset
\end{equation}
i.e., formation of large coalitions is always desired and the players do not lose any utility by joining the coalition. 
\end{definition}

\subsubsection{Canonical Game}
A coalition game is canonical if 
\begin{itemize}
	\item It is in characteristic form
	\item It is superadditive
\end{itemize}
The \emph{core} and Shapley value are widely used concepts for dealing with Canonical games as discussed below. 
\subsection{Core}
Before we present details of core, we first define some terms \cite{han2012game}

\begin{definition}[Group Rational]
	A payoff vector $\textbf{x}\in \mathbb{R}^\mathcal{N}$ for dividing $v(\mathcal{N})$ is group-rational if $\sum_{n \in \mathcal{N}}x_n=v(\mathcal{N})$.
\end{definition}

\begin{definition}[Individual Rational]
	A payoff vector $\textbf{x}\in \mathbb{R}^\mathcal{N}$ is individually-rational if every player can obtain a benefit no less than acting alone, i.e., $x_n \geq v(\{n\}), \forall n\in \mathcal{N}$.
\end{definition}

\begin{definition}[Imputation]
	A payoff vector that is both individual and group rational is known as an imputation. 
\end{definition}


Based on the above definitions, we can now define the core of a TU canonical coalition game

\begin{definition}[Core]
	For any TU canonical game $(\mathcal{N},v)$, the core is the set of imputations in which no coalition $S\subset\mathcal{N}$ has any incentive to reject the proposed payoff allocation and deviate from the grand coalition to form a coalition $S$ instead. This can be mathematically expressed as 
	\begin{align}\label{eq:coreTU}
	\mathcal{C}_{TU}=\bigg \{ \mathbf{x}: \sum_{n \in \mathcal{N}}x_n=v(\mathcal{N}) \; and \; \sum_{i \in S} x_i \geq v(S)\; \forall\; S\subseteq \mathcal{N}\bigg\}
	\end{align}
\end{definition}
\begin{remark}
	Any payoff allocation from the core is Pareto-optimal as evident from definition of the core. Furthermore, the grand coalition formed is stable
\end{remark}
However, the core is not always guaranteed to exist. Even if the core exists, it might be too large so finding a suitable allocation from the core is not easy. Furthermore, as seen from the definition, the allocation from the core might not always be fair to all the players. 
\subsection{Shapley Value}
 %Now that we have the answer to the question about non-emptiness of the core, we divert our attention to the selection of any pay-off allocation from the core. As evident, the core for our problem is quite large. Therefore, selecting a suitable core allocation can be difficult \cite{han2012game}. 
 \emph{Shapley value} \cite{shapley1988value} can be used to address the aforementioned  shortcomings of the core. For the characteristic function $v$ (the characteristic function is also called the game \cite{han2012game}), Shapley proposed an allocation $\phi_n(v)$ that satisfies the following axioms \cite{la2004game}:
 \begin{enumerate}
 	\item \emph{Efficiency Axiom}: $\sum_{n \in \mathcal{N}}\phi_n(v)=v(\mathcal{N})$. This axiom in essence is the group rationality.
 	\item \emph{Symmetry Axiom}: If any two players $m$ and $n$ are such that $v(S \cup \{n\})=v(S \cup \{m\})$, then for every coalition $S\backslash(m,n)$, $\phi_n(v)=\phi_m(v)$. This axiom indicates that if any two players/domains have similar contributions in a coalition then their assigned payoffs must be same as well.
 	\item \emph{Dummy Axion}: If any player $n$ is such that $v(S)=v(S \cup \{n\})$, then for every coalition $S\backslash n$, $\phi_n (v)=0$. Dummy axiom indicates that players that do not contribute to the value of coalition will not get any payoff. 
 	\item \emph{Additivity Axion}: If $j$ and $k$ are any two games, then $\phi(j+k)=\phi(j)+\phi(k)$. This axiom indicates that $\phi$ is a unique mapping over the space of the coalitional games.
 \end{enumerate}
 Based on the above axioms, Shapley  showed that there exists a unique function $\phi$ defined on all games that satisfies the aforementioned axioms \cite{la2004game}. The function is given by
 
 \begin{equation}\label{eq:shapleyvalue}
 \phi_n(v)=\sum_{S\subseteq \mathcal{N}\backslash n}\frac{|S|! (|\mathcal{N}|-|S|-1)!}{|\mathcal{N}|!}\bigg[ v(S \cup \{n\}) -v(S) \bigg]
 \end{equation} 
\end{comment}

==> arxiv version/arxiv version/proof1.tex <==
\begin{proof}
	We show that the price function obtained by $\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma})}{\partial x_{n,k}^{j}}=0$ is continuous at one or more of the optimal Lagrange multipliers for \eqref{eq:lagrangian}. 
	
	Let both $u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j,\zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j})$ and $f_n^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Lambda_{n,k}^{l})$ are  %and $u_{jn}^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)})$ are
	the inverses of the first derivative of $u_{n}^j$ and $(u_{n}^l(x_{n,k}^l)-C_n^l(x_{n,k}^l))$, respectively. %and $u_j^n$ respectively. 
	$\alpha_{n,k}$,  $\beta_{k}^j$, $\zeta_{n}$, and $\gamma_{n,k}^{j}$ are the \emph{Lagrange} multipliers whereas   $\Delta_{n,k}^{j}=\bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j+{x}_{n,k}^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^l+{x}_{n,k}^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg)$. There are two different cases that we evaluate in the following: %To simplify the proof, we only consider the case  in which $i \in \mathcal{M}_n$ below. The proof for the case when $i \in \mathcal{M}\backslash\mathcal{M}_n$ is similar. 
	\begin{enumerate}
	\item \textbf{$j \in \mathcal{M}_n$:}$\frac{\partial \mathcal{L}}{\partial x_{n,k}^{j}}=0$
	\begin{align}
	\label{eq:gradLagObj22}
%	\frac{u_n^{'j}(\mathbf{x}_n^j+\sum_{t\in \mathcal{{N}}\backslash n}\mathbf{x}_t^j)+\sum_{t \in \mathcal{{N}}\backslash n}}{\Delta_{n,k}^j}, \nonumber \\
	%	 \Big(u_n^{'j}(x_{n,k}^{j})+\frac{1}{r_{k}^j}\Big)(1+\Lambda_{n,k}^{j}\zeta_{n})-\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j-\nonumber \\
	%	 \gamma_{n,k}^{j})=0,\nonumber \\
	&u_n^{'j}(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j+x_{n,k}^{j})(1+\Delta_{n,k}^{j}\zeta_{n})-\Delta_{n,k}^{j}(\alpha_{n,k}+\nonumber \\
	&\beta_{k}^j-\gamma_{n,k}^{j})=0,\nonumber \\	
	%	 \implies u_n^{'j}(x_{n,k}^{j})=\frac{\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Lambda_{n,k}^{j}\zeta_{n}}-\frac{1}{r_{k}^j}, \nonumber \\
	& u_n^{'j}(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j+x_{n,k}^{j})=\frac{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n,k}^{j}\zeta_{n}}, \nonumber \\
	%& \nonumber \\
	%	\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j},r_{k}^j).
%	&\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Delta_{n,k}^{j}).
	\end{align}
For sake of the proof, we set  $u_j^n=1-e^{-(x_{n,k}^j+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j+-r_{n,k}^j+\delta t)}$ where $\bar{r}_{n,k}^j=r_{n,k}^j+\delta t$. However, the theory hold for any concave injective utility function for which the inverse of the first derivative exists.  Then \eqref{eq:gradLagObj22} becomes:
	\begin{align}\label{eq:proof1}
	& e^{-(x_{n,k}^j+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}= \frac{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n,k}^{j}\zeta_{n}},\hspace{0.2in} \nonumber \\
		e^{x_{n,k}^j}&= \frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}},\nonumber \\
		x_{n,k}^j&=\ln\bigg(\frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}}\bigg).
	\end{align} 
%We know that $\Lambda_{ik}^{(n)>0$, 
	 For continuity, we need both the numerator and denominator inside the $\ln(\boldsymbol{.})$ function of \eqref{eq:proof1} to be positive.  
At the optimal point, the numerator $(1+\Delta_{n,k}^{*j}\zeta^*_{n})$ is positive as $\Delta_{n,k}^{*j}>0$ (from Section \ref{sec:assumption}) and $\zeta^*_{n}=0$ (from complementary slackness).	Similarly, in the denominator, $\Delta_{n,k}^j$ (from Section \ref{sec:assumption}) and $e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}$ are positive. $(\alpha^*_{n,k}+\beta_{k}^{*j}-\gamma_{n,k}^{*j})>0$, as  $\alpha_{n,k}^{*}>0$ (from Lemma \ref{lem:constraintsactive}) and  $\alpha_{n,k}^{*}+\beta_{k}^{*j}> \gamma_{n,k}^{*j}$ (from \emph{sensitivity analysis} \cite{boyd2004convex}). %Furthermore, the denominator $(r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}^*+\beta_{k}^{*j}- \gamma_{n,k}^{*j})-1>0)$ based on our assumptions in Section \ref{sec:assumption}.
Hence, the price based function in \eqref{eq:proof1} is continuous in at least one optimal Lagrange multiplier vector. The proof follows from Theorem \ref{thm:georgesufficient}. 
	
	
	%	Where the last step follows from the fact that  utility function used is $1-1$, so its derivative is also $1-1$ and its inverse $U_n^{'-1}(\alpha_k, \beta_{ik})$ can easily be computed.
	\item \textbf{$l \in \{\mathcal{M}\backslash\mathcal{M}_n\}$:} $\frac{\partial \mathcal{L}}{\partial x_{n,k}^{l}}=0$
	\begin{align}
	\label{eq:gradLagObjcase22}
	f^{'l}_n(x_{n,k}^{l})(1+\Delta_{n,k}^{l}\zeta_{n})-\Delta_{n,k}^{l}(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})=0,\nonumber \\ 
	\implies  f^{'l}_n(x_{n,k}^{l})=\frac{(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})}{1+\Delta_{n,k}^{l}\zeta_{n}}, \nonumber \\
	%& \nonumber \\
	\implies \quad x_{n,k}^{*l}= f_{n}^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Delta_{n,k}^{l}).
	\end{align}
\end{enumerate}


\end{proof}

==> arxiv version/arxiv version/related.tex <==
\subsection{Resource allocation in Edge Computing}
Jiao et al. \cite{jiao2018social} propose an auction-based resource allocation scheme for edge service providers that provide resources for blockchains. The proposed mechanism maximizes the social welfare and guarantees truthfulness, computational efficiency and individual rationality. He et al. \cite{he2018s} analyze the optimal provisioning of shareable and non-shareable edge resources to different applications.    %It is shown that the problem is NP-hard in general and they  propose a constant factor algorithm as well as different heuristics. 
Plachy et al. \cite{plachy2016dynamic} consider the mobility problem in mobile edge clouds and propose a novel algorithm for  selecting communication path and VM placement. The proposed approach relies on predicting user movement that helps in VM placement and accordingly selecting the communication path. Nishio et al. \cite{nishio2013service} propose a resource sharing architecture for mobile clouds that relies on service-oriented utility functions and is closest to our work. However, they primarily consider service latency and rely on a centralized framework whereas we present a distributed framework that requires a specific utility function that can be used to model different metrics such as latency, delay, and numerous other objectives. In \cite{zafari2020let}, we modeled resource sharing among mobile edge clouds as a cooperative game. However, the MOO problem in \cite{zafari2020let} is non-convex  that is hard to solve compared to the convex problem solved here. Furthermore, the cooperative game based framework lacks the fairness guaranteed by NBS. % and is closest to our work. 
 Furthermore, in contrast with \cite{jiao2018social,plachy2016dynamic} and \cite{he2018s} that primarily consider resource allocation, our proposed framework deals with resource sharing among ESPs with different objectives. 

\subsection{NBS based Resource Allocation}
Yaiche et al. \cite{yaiche2000game} use NBS to allocate bandwidth for elastic services in  high speed networks. 
Xu et al. \cite{xu2012general} consider the fairness criteria when allocating resources to different cloud users and make use of the  NBS to guarantee fairness. Using dual composition and sub-gradient method, the authors also develop a distributed algorithm. Hassan et al.  \cite{hassan2014virtual} propose an NBS-based model for cost-effective and dynamic VM allocation with multimedia traffic, and show that it can reduce the cost of running different servers along with maximizing resource utilization and satisfying the QoS requirements. He et al. \cite{he2013toward}   study the optimal deployment of content in a cloud assisted video distribution system. 
Feng et al. \cite{feng2012bargaining} use NBS  for Virtual Machine (VM) migration to maximize the resource utilization in a video streaming data center. 
\par 
In contrast with  \cite{yaiche2000game, feng2012bargaining, guo2013cooperative,he2013toward,hassan2014virtual},  to the best of our knowledge, our  framework is first of its kind that uses NBS for  resource sharing among ESPs  with different utilities (objective functions). We show that resource sharing can improve  utilities  of ESPs and enhance application satisfaction. 
Furthermore, for a particular class of utilities, we have proved that distributed algorithm exists for obtaining NBS for the resource sharing and allocation problem. Table \ref{tab:comparison} summarizes some other solutions proposed in the literature  that use NBS for resource allocation in different systems.   Other distributed algorithms proposed in literature either rely on dual decomposition \cite{xu2012general} or gradient projection \cite{yaiche2000game,guo2013cooperative}. However, most of the functions are not dual decomposable and gradient projection is a computationally expensive approach \cite{bertsekas1997nonlinear}, whereas gradient descent is widely used particularly  in machine and deep learning.   
 












==> arxiv version/game-theory.tex <==
%\subsection{Game Theoretic Solution}
We first define the characteristic function $v$ for our game that can solve  problem in~\eqref{eq:opt_higher} 

\begin{figure*}[!t]
	\normalsize
\begin{align} \label{eq:payoff_function}
v(\mathcal{N})=\sum_{\substack{\text{$n \in \mathcal{N}$},\;\text{$C_{k}= \sum_{n \in \mathcal{N}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in \mathcal{N}$}\\ \text{$\sum_{j \in \mathcal{N}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}$}}}\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in \mathcal{N},j\neq n} u^{n}_j(\mathcal{X})\bigg)
\end{align}
	\hrulefill
	\vspace*{-4pt}
\end{figure*}



\begin{remark}
	The characteristic function in Equation~\eqref{eq:payoff_function} is for the grand coalition $\mathcal{N}$. For any $S \subseteq \mathcal{N}$, the characteristic function will be given by Equation~\eqref{eq:payoff_s_function}
\end{remark}


\begin{figure*}[!t]
	\normalsize
\begin{align} \label{eq:payoff_s_function}
v({S})=\sum_{\substack{\text{$n \in {S}$},\; \text{$C_{k}= \sum_{n \in {S}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {S}$}\\ \text{$\sum_{j \in {S}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S}$}}} \bigg(w_n u_n(\mathcal{X})+\zeta_{n}\sum_{j \in S,j\neq n} u^{n}_j(\mathcal{X})\bigg)
\end{align}
\hrulefill
\vspace*{-4pt}
\end{figure*}


\begin{theorem}
%	A Cooperative game $(\mathcal{N}, v)$ of $\mathcal{N}$ players and $v$ payoff function that can be used to solve the multi-objective optimization problem given in \eqref{eq:opt_higher}, is canonical\footnote{for monotonically non-decreasing utilities/pay-off function} with Transferable utility
Resource allocation and sharing problem (with multiple objectives) in aforementioned settings can be modeled as a canonical cooperative game with TU. 
\end{theorem}
\begin{proof}
To prove this, we need to show that the characteristic function of resource sharing and allocation problem satisfies the following two conditions
%	For a game to be canonical, we need to prove that the game  is superadditive and the payoff function is of characteristic form. 
	\begin{itemize}
		\item \textbf{Characteristic form of payoff:} As the utility function in a resource sharing and allocation problem  only relies on the domains that are part of the coalition, the game or payoff function is of characteristic form
		\item \textbf{Superadditivity:} Super-additivity for TU games requires $v(S_1 \cup S_2 )\geq v(S_1)+V(S_2) \; \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, s.t. S_1\cap S_2 =\emptyset$ i.e. we have to prove that the pay-off or utility for a domain in the coalition is as good as domain working alone or in a smaller coalition. Due to monotonicity property of the utility functions used,  for all  players/domains $n \in \mathcal{N}$,  $u_n(X_n^{NC})\leq u_n(X_n^{C})$ as $X_n^{NC}\subset {X_n^{C}}$ \footnote{because $X_n^{C}$ can contain much more elements due to the increase in $C$ in the coalition} where $X_n^{C}$ and $X_n^{NC}$ are the allocation decisions in  a cooperative game  and independent setting respectively for domain $n$. 
	\end{itemize}
\end{proof}
\begin{lemma}\label{lemma:MOOGame}
A canonical cooperative game $(\mathcal{N}, v)$ with TU can be used to obtain the Pareto-optimal solutions for the multi-objective optimization problem given in \eqref{eq:opt_higher}
\end{lemma}

%Given that the game is canonical, we are going to explore potential solution approaches for such a game. We start with the \emph{Core} \cite{han2012game}. 

To prove Lemma \ref{lemma:MOOGame}, we must show that the core is non-empty for  our canonical game. To do this, we first show that our game is convex. 

\begin{definition}[Convex Games]
	A coalition game is said to be convex if and only if for every player $n \in \mathcal{N}$, the marginal contribution of the player is non-decreasing W.R.T set inclusion. Mathematically, for $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash \{n\}$ 
	\begin{equation}\label{eq:convexgames}
	v(S_1 \cup \{n\})-v(S_1) \leq v(S_2 \cup \{n\})-v(S_2)
	\end{equation} 
\end{definition}
\begin{theorem}
	Our canonical game is convex
\end{theorem}
\begin{proof}
Let us consider two coalition $S_1$ and $S_2$, where $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash\{j\}$ where $j \in \mathcal{N}$. Then we first calculate $v(S_2 \cup \{j\})-v(S_1 \cup \{j\})$ in Equation \eqref{eq:convexityProof}. 

\begin{figure*}[!t]
	\normalsize
\begin{align}\label{eq:convexityProof}
& \sum_{\substack{\text{$n \in {S_2}$},\; \text{$C_{k}= \sum_{n \in {S_2}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}$}\\ \text{$\sum_{j \in {S_2}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {S_2}, k\neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) - \nonumber \\
& \Bigg(\sum_{\substack{\text{$n \in {S_1}$},\; \text{$C_{k}= \sum_{n \in {S_1}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {S_1}$} \\ \text{$\sum_{j \in {S_1}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_1}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {S_1}, k \neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_1)}(\mathcal{X}) + \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\nonumber \Bigg)\\ 
&= \sum_{\substack{\text{$n \in {S_2}\backslash S_1$}, \text{$C_{k}= \sum_{n \in {S_2}\backslash S_1}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}\backslash S_1$} \\ \text{$\sum_{j \in {S_2 \backslash S_1}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2 \backslash S_1}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {\{S_2 \backslash S_1\}}, k \neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) \nonumber \\
&   + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) - w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X}) \nonumber \\
& = v(S_2)- v(S_1)+ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})  \nonumber \\
& \geq v(S_2)- v(S_1)
\end{align}
	% Restore the current equation number.
	%%\setcounter{equation}{\value{MYtempeqncnt}}
	% The IEEE uses as a separator
	\hrulefill
	% The spacer can be tweaked to stop underfull vboxes.
	\vspace*{4pt}
\end{figure*}

\begin{comment}
	\begin{align}\label{eq:convexityProof}
	& \sum_{\substack{\text{$n \in {S_2}$} \\ \text{$R_{av,k}= \sum_{n \in {S_2}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}$}\\ \text{$\sum_{j \in {S_2}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2}$}}}\bigg(w_n u_n(\mathcal{A})+ w'_{n}\sum_{k \in {S_2}, k\neq n} u^{j}_k(\mathcal{A})\bigg) + w_j u_j ^{(S_2)}(\mathcal{A}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{A}) - \nonumber \\
	& \Bigg(\sum_{\substack{\text{$n \in {S_1}$} \\ \text{$R_{av,k}= \sum_{n \in {S_1}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {S_1}$} \\ \text{$\sum_{j \in {S_1}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_1}$}}}\bigg(w_n u_n(\mathcal{A})+ w'_{n}\sum_{k \in {S_1}, k \neq n} u^{j}_k(\mathcal{A})\bigg) + w_j u_j ^{(S_1)}(\mathcal{A}) + \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{A})\nonumber \Bigg)\\ 
	&= \sum_{\substack{\text{$n \in {S_2}\backslash S_1$} \\ \text{$R_{av,k}= \sum_{n \in {S_2}\backslash S_1}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}\backslash S_1$} \\ \text{$\sum_{j \in {S_2 \backslash S_1}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2 \backslash S_1}$}}}\bigg(w_n u_n(\mathcal{A})+ w'_{n}\sum_{k \in {\{S_2 \backslash S_1\}}, k \neq n} u^{j}_k(\mathcal{A})\bigg) + w_j u_j ^{(S_2)}(\mathcal{A}) \nonumber \\
	&   + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{A}) - w_j u_j ^{(S_1)}(\mathcal{A}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{A}) \nonumber \\
	& = v(S_2)- v(S_1)+ w_j u_j ^{(S_2)}(\mathcal{A}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{A}) -  w_j u_j ^{(S_1)}(\mathcal{A}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{A})  \nonumber \\
	& \geq v(S_2)- v(S_1)
	\end{align}
	\end{comment}

The last inequality in Equation \eqref{eq:convexityProof} follows from the fact that $ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\geq 0$ (monotonicity of the utility)
\end{proof}


%Related to the core, there are certain questions that we must answer
\begin{comment}
\begin{enumerate}
	\item Is the core non-empty?
	\item If the core is non-empty and consists of different pay-off allocations, how do we choose any particular pay-off allocation vector? 
\end{enumerate}
Below we attempt to answer these questions



\begin{definition}[Balanced Collection] Let $\Omega$ be a collection of different coalitions. $\Omega$ is considered to be a \emph{balanced collection} if we can find non-negative weights $w_S$ for each $S \in \Omega$ such that for every player $n$ 
	\begin{align}\label{eq:balancedcollection}
	\sum_{S \in \Omega, S \ni n}w_S =1 
	\end{align}
\end{definition}

\begin{definition}[Balanced Game] A game is called balanced if for every balanced collection $\Omega$, the payoff vector $\mathbf{x}$ will be in $V_{\mathcal{N}}$ if $\mathbf{x}_S \in V_S\; \forall S \in \Omega$ 
	%Let $\Omega$ be a collection of different coalitions. $\Omega$ is considered to be a \emph{balanced collection} if we can find non-negative weights $w_S$ for each $S \in \Omega$ such that for every player $n$ 
\end{definition}
\begin{theorem}[Bondareva-Shapley Theorem]\label{thm:BST}
	The core of a game is non-empty if and only if the game is balanced
\end{theorem}


\begin{theorem}
The core for canonical game with our characteristic function(in Equation~\eqref{eq:payoff_function}) is non-empty
\end{theorem}

\begin{proof}
From the definition of characteristic functions for TU games (see \cite{han2012game} for details), $v: 2^{\mathcal{N}}$ \textrightarrow $\mathbb{R}$ with $v(\emptyset)=\emptyset$. This means that the total number of coalitions possible for $\mathcal{N}$ players is $2^{|\mathcal{N}|}-1$ (we ignore the empty set). For $\Omega$, the non-negative weights $w_S$ which satisfy the condition for  balanced collection in Equation~\eqref{eq:balancedcollection} are given by $\frac{1}{2^{|\mathcal{N}|-1}}$. Hence $\Omega$ is a balanced collection. We also know that $v(S)\subseteq v(\mathcal{N})$ as $v(\mathcal{N})$ is defined over a larger feasible set due to increased amount of available resources. Leveraging the monotonicity property of the utility functions used, we know that any payoff vector  $\mathbf{x}$ will be in $V_{\mathcal{N}}$ if $\mathbf{x}_S$\footnote{$\mathbf{x}_S$ is the projection of $\mathbf{x}$ onto the vector space $\mathbb{R}^{|S|}$} $\in V_S\; \forall S \in \Omega$. Hence our canonical game with characteristic function $v$ in Equation~\eqref{eq:payoff_function} is balanced and its core is non-empty (from Theorem \ref{thm:BST})

\end{proof}
\end{comment}


%For our problem, does the Shapley value lie in the core? To do so we first define \emph{convex games}

\begin{theorem}
	The core of any convex game $(\mathcal{N},v)$ is non-empty and large. 
\end{theorem}
\begin{proof}
	Available in \cite{sharkey1982cooperative}
\end{proof}
While the existence of core i.e., core being non-empty, guarantees the grand coalition is stable, finding a suitable allocation from the core is challenging particularly when the core is large (our game). Furthermore, as mentioned earlier, fairness is also a shortcoming of core based solutions.  Shapley value can be  used to obtain a fair allocation, however, we first need to show that the Shapley value lies in the core to guarantee that the Shapley value based allocation is stable for the grand coalition. 
\begin{theorem}
	The Shapley value in Equation~\eqref{eq:shapleyvalue} lies in the core of our canonical game
\end{theorem}
\begin{proof}
	Since our canonical game is convex, the Shapley value lies in the core \cite{han2012game} (see \cite{roger1991game} for details)
\end{proof}
We summarize this in the remark below. 
\begin{remark}
If a TU game $(\mathcal{N}, v)$ is convex, then the core is non-empty and the Shapley Value lies in the core \cite{garg2013novel}.	
\end{remark}
Calculation of Shapley value given in Equation~\eqref{eq:shapleyvalue} is challenging \cite{han2012game}. Since our game is convex, calculating its Shapley value is slightly easier as given below. 

%Now that we have proved that the game is convex, we divert our attention to the calculation of Shapley value for a convex game. 


\subsubsection{Shapley Value for a Convex Game}
Let $\pi$ denote the permutation of players in our game.  Then for any permutation $p$ from the total possible permutations $|\mathcal{N}|!$, one can obtain the initial segments of ordering by \cite{garg2013novel}
\begin{equation}\label{eq:initialsegment}
O_{\pi, r}=\{ n \in \mathcal{N} : \pi(n) \leq r \}, \; r \in \{1, \cdots, N\}
\end{equation}
where $O_{\pi, 0}=\{\}$ and $O_{\pi, |\mathcal{N}|} =\mathcal{N}$. $\pi(n)$ refers to the position of the player $n$ in the permutation $\pi$. The core of any particular ordering $\pi$ can be obtained by solving  equations
\begin{equation}
\label{eq:x_i_pi_sol}
x_n^{\pi}(O_{\pi, r}) = v(O_{\pi, r}), \; r \in \{ 1, \cdots, N\}
\end{equation}
The solution to  above Equations~\eqref{eq:x_i_pi_sol} will result in a payoff vector $x^{\pi}$ where the elements of the vector are given by 
\begin{equation}
\label{eq:vectorelements}
x_n^{\pi}=v(O_{\pi, \pi(n)})- v(O_{\pi, \pi(n)-1}), \quad \forall n \in \mathcal{N} 
\end{equation}
The payoff vectors $x^{\pi}$ represent the extreme points of the core in convex games \cite{garg2013novel}. So if $\prod$ represents the set of all possible permutations of $\mathcal{N}$, the Shapley value of any player $n$ can be calculated as 
\begin{equation}
\label{eq:shapleyconvex}
\phi_n=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} x_n^{\pi}
\end{equation}
\begin{comment}
So for our coalition game $(\mathcal{N},v)$, the Shapley value is 
\begin{align}
\label{eq:ourshapleyconvex}
\phi_n&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} \bigg( \sum_{\substack{\text{$n \in {O_{\pi, \pi(n)}}$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)}}$} \\ \text{$$}\text{$\sum_{j \in {O_{\pi, \pi(n)}}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in O_{\pi, \pi(n)}$}}}\bigg(w_n u_n^{(\pi)}(\mathcal{A})+ w'_{n}\sum_{j \in {O_{\pi, \pi(n)}}, j \neq  n} u^{n,(\pi)}_j(\mathcal{A})\bigg)- \nonumber \\
&\Bigg(\sum_{\substack{\text{$n \in {O_{\pi, \pi(n)-1}}$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)-1}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)-1}}$}}}\bigg(w_n u^{(\pi)}_n(\mathcal{A})+ w'_{n}\sum_{j \in {O_{\pi, \pi(n)-1}}, j \neq n} u^{n,(\pi)}_j(\mathcal{A})\bigg)\Bigg) \nonumber \\
&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} \bigg( \sum_{\substack{\text{$n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1} }$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}$} \\ \text{$\sum_{j \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}$} }}\bigg(w_n u^{(\pi)}_n(\mathcal{A})+  \nonumber \\ 
& w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{n,(\pi)}_j(\mathcal{A}) +  w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{j,(\pi)}_n(\mathcal{A})  \bigg)\bigg) \nonumber \\
&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod}\bigg(w_nu^{(\pi)}_n(\mathcal{A})+ w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{n,(\pi)}_j(\mathcal{A}) +w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{j,(\pi)}_n(\mathcal{A}) \bigg) 
\end{align}
where Equation~\eqref{eq:ourshapleyconvex} provides the Shapley value for our convex game. It is evident that our Shapley value depends on the utility of the player $n$, the utility  player $n$ achieves by allocating resources to players in $j \in O_{\pi, \pi(n)}, j \neq n $ and the utility player $j \neq n, j \in O_{\pi, \pi(n)}$ achieves by allocating resources to player $n$  in every possible permutation. 

\begin{comment}
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $tt$ 
		\State \textbf{Output}: The optimal hit probabilities
		\State \textbf{Step $1$:}  $t \leftarrow$0, $\boldsymbol{\lambda^{(t)}\leftarrow\lambda_0}$, $\boldsymbol{\mu^{(t)}\leftarrow\mu_0}$
		\While{Equation \eqref{eq:gradient1} $\neq$ 0}%$\partial L(\boldsymbol{h,\lambda,\mu})/\partial \lambda_{l} \neq0$ $\&\& $ $\partial L(\boldsymbol{h,\lambda,\mu})/\partial \mu_{ip} \neq0$}
		\State \textbf{Step $2$}:$\boldsymbol{h_{il}^{(p)}[t]} \leftarrow \frac{w_i\beta^{|p|-l}}{\lambda_{l}[t-1]\Bigg(\prod_{\substack{q \neq p,\\ q:l\in\{1,\cdots,|q|\}}}(1-h_{il}^{(q)}[t-1])\Bigg)+\mu_{ip}[t-1]}. $ %Algorithm 2($\boldsymbol{\lambda^{(t)},\mu^{(t)}}$) %\Comment{The node id and file content to Algorithm \ref{algo:alg1} for calculating the price function using~(\ref{eq:gradient2}) }
		\State \textbf{Step $3$:} Update $\lambda$ and $\mu$ using  \eqref{eq:update},  t $\leftarrow t+1$
		%	\State \textbf{Step $4$}: $\boldsymbol \tau_{\chi} \longleftarrow \text{Convex}(\text{slave},\boldsymbol u_{\chi})$ \Comment{Solve the slave optimization problem for $\boldsymbol \tau_{\chi}$  }
		%	\State \textbf{Step $5$}: $(\boldsymbol b_{\chi}, \boldsymbol{\delta_{\chi}}, \text{obj}_{\chi})  \longleftarrow \text{Rounding}(\boldsymbol u_{\chi},\boldsymbol \tau_{\chi})$ \Comment{Round the values of $\boldsymbol u_{\chi}$, remap $\boldsymbol u_{\chi}, \boldsymbol \tau_{\chi}$ to $\boldsymbol{b}_{\chi}$ and $ \boldsymbol{\delta}_{\chi}$ and obtain the new objective function value  }
		\EndWhile
	\end{algorithmic}
	\caption{Iterative Distributed Algorithm}
	\label{algo:alg}
\end{algorithm}
\end{comment}
\begin{remark}\label{rem:shap}
	Shapley value calculation for our convex game requires solving at least $2^{N}-1$ optimization problems
\end{remark}
Algorithm \ref{algo:alg1} provides an overview of our proposed approach. We obtain $R, C$ and the utility of all players as $\mathbf{u}$. We initialize each player's utility value ($\mathbf{u}(R,\mathcal{X})$), Shapley value ($\boldsymbol{\phi} $) and resource allocation decision $\mathcal{X}$ to $0$. Then we calculate the Shapley value for the players and assign it to $\mathbf{u}(R,\mathcal{X})$. Finally to obtain $\mathcal{X}$, we take the inverse function of $\mathbf{u}$. As we are using monotone utilities, we know that the inverse of the utilities exist.
\par A fundamental issue with Shapley value is its complexity. As mentioned in Remark \ref{rem:shap}, Shapley value calculation requires solving a  large number of optimization problems that is not suitable for a game with larger number of players. Therefore, reducing the complexity of obtaining an allocation from the core is always favorable. 
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0, $ \boldsymbol{\phi} \leftarrow$0,  
		\State \textbf{Step $1$:}  Calculate Shapley Value $\phi_n$ using Equation \eqref{eq:shapleyconvex} $\forall n \in \mathcal{N}$
	    \State \textbf{Step $2$:} $ \mathbf{u}(R,\mathcal{X}) \leftarrow \boldsymbol{\phi}$
	    \State \textbf{Step $3$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
		\end{algorithmic}
	\caption{Shapley Value based Resource Allocation}
	\label{algo:alg1}
\end{algorithm}
%It is worth mentioning here that the Shapley value will only provide us the utility each player is going to receive that lies in the core (as a result of cooperation). The allocation decision can be obtained by taking the inverse of utilities.  \par 
\subsection{Reducing the Computational Complexity}
%As mentioned earlier, that the calculation of Shapley value for our convex game requires at solving at least $2^{N}-1$ optimization problems that is computationally expensive. 
To reduce the complexity, we propose a computationally efficient approach in Algorithm 2 that requires solving $2N$ optimization problems i.e. $\mathcal{O}(N)$.  The input into the algorithm consists of available resources/capacities, user requirements and the utilities of all game players. The output of the algorithm is $\mathcal{X}$. In Step 1, the utility values of the players, the allocation decision,  and two vectors $\boldsymbol{O_1}$ and $\boldsymbol{O_2}$. In Step 2, every player's utility is calculated without any resource sharing i.e. single optimization and the values are stored in the vector $\boldsymbol{O_1}$. Then $C, R$ are updated and we move to Step 4, where we calculated the utilities $u_j^n$'s for all the players with updated $C, R$ and store them in $\boldsymbol{O_2}$. 

\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0,   $ \boldsymbol{O_1} \leftarrow$0, $ \boldsymbol{O_2} \leftarrow$0, 
		\State \textbf{Step $2$:}
		 \For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_1^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single}}
		\EndFor
		\State \textbf{Step $3$:} Update $R, C$ based on Step 2
		\State \textbf{Step $4$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_2^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single_j} with updated C and R}
		\State Update C and R
		\EndFor
		\State \textbf{Step $5$:} $u_n(R,\mathcal{X})\leftarrow O_1^n+O_2^n$ $\forall n \in \mathcal{N}$ 
		\State \textbf{Step $6$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{$\mathcal{O}$($N$) algorithm for obtaining Core's allocation}
	\label{algo:alg2}
\end{algorithm}
\begin{subequations}\label{eq:opt_single_j}
	\begin{align}
	\max_{\mathcal{X}}\quad& \sum_{j\neq n}u_j^n(\mathcal{X}) \quad  \forall n \in \mathcal{N} \label{eq:objsinglej}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall i \in \mathcal{M}\backslash\mathcal{M}_n, \label{eq:singlefirstj} \displaybreak[0]\\
	& x_{ik}^{(n)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecondj} \displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlethirdj} \displaybreak[2]
	\end{align}
\end{subequations}
\begin{theorem}
	The solution obtained from Algorithm \ref{algo:alg2} lies in the \emph{core}
\end{theorem}
\begin{proof}
	To prove the theorem, we need to show that the utilities obtained in Step $5$ of Algorithm \ref{algo:alg2}; a) are individually rational; b) are group rational and c) no players  have the incentive to leave the grand coalition and form another another coalition $S \subset \mathcal{N}$. 
	\paragraph{Individual Rationality} For each player $n \in \mathcal{N}$, the solution $O_1^n$ obtained by solving the optimization problem in Equation \eqref{eq:opt_single} is the utility a player will obtain by working alone i.e. it is $v\{n\}$. The value $O_2^n$ in Step 4 is either zero or positive but cannot be negative due to the nature of utility used i.e. 
	\begin{align}
	u_n(R,\mathcal{X})&=O_1^n+O_2^n \quad \forall n \in \mathcal{N} \nonumber \\
	u_n(R,\mathcal{X})&\geq O_1^n \quad \forall n \in \mathcal{N}\nonumber 
	\end{align}
	
	
	Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is individually rational.
	\paragraph{Group Rationality} The value of the grand coalition $v\{\mathcal{N}\}$ as per Equation \eqref{eq:payoff_function} is the sum of utilities $u_n$'s and $u_j^n$'s. Steps 2, 4 and 5 of Algorithm \ref{algo:alg2} obtain the sum of the utilities as well. Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is group rational rational. 
	\par Furthermore, due to super-additivity of the game and monotonic non-decreasing nature of the utilities, no players have the incentive to form a smaller coalition. Hence Algorithm \ref{algo:alg2} provides a solution from the core.  
\end{proof}

==> arxiv version/nbs.tex <==
We first present an introduction to NBS and then discuss our proposed NBS based resource sharing framework. 
\subsection{Primer on Nash Bargaining Solution (NBS)}\label{sec:prelim}
\input{preli}

\subsection{Proposed Framework}
As mentioned earlier, NBS is  a Pareto optimal and fair solution in settings that involve different players (ESPs in our case) where each player has an objective to optimize. Therefore, it can be used to solve our MOO problem in \eqref{eq:opt_higher} as we have different ESPs  that need to optimize their objectives and improve their utilities over what they would receive  working alone. 
 We first specify the disagreement point for our bargaining problem. If the ESPs  cannot come to an agreement, they can all start working alone.  Hence the disagreement point  is the solution to the SOO problem given in \eqref{eq:opt_single} for all ESPs. Let us denote the solution to the SOO problem by $d_n^0, \forall\; n \in \mathcal{N}$.   In the cooperative setting\footnote{Service providers share resources among each other.}, the utility (represented by $s_n$ in \eqref{eq:nashProbNplayer})  for an ESP $n \in \mathcal{N}$  is given by: 
 \begin{align}
%\big(\sum_{j \in \mathcal{M}_n}u_n^j(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^j+\mathbf{x}_n^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^l+\nonumber \\
%\mathbf{x}_n^l)-D_n^l(\mathbf{x}_n^l)\big)\big) \nonumber
%&\sum_{j \in \mathcal{M}_n}\Big(u_n^j(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^j+\mathbf{x}_n^j)- u_n^j(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^j) \Big)+ \nonumber \displaybreak[0]\\
%&\Big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^l+\mathbf{x}_n^l)-u_n^l(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^l)-\nonumber\\ &D_n^l(\mathbf{x}_n^l)\Big)
U= &\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)- u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big) \nonumber \displaybreak[0] \\
&\hspace*{-0.2in}+\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)- \displaybreak[1]\nonumber\\
&\hspace*{-0.1in} D^l({x}_{n,k}^l)\big)\Big). \nonumber 
 \end{align} 
  Below, we  present the centralized NBS algorithm. % and then propose a distributed algorithm for NBS. %\vspace{-0.2in}
 \subsubsection{Centralized NBS}
 We first present the optimization problem to obtain NBS for our $N-$ESP bargaining game  \cite{harsanyi1963simplified} and then present its equivalent problem \cite{yaiche2000game} that is computationally efficient to solve. 
 %Therefore,  we state the following theorem.  %Using this information, the optimization problem for NBS in \eqref{eq:nashProbNplayer} can be rewritten as 
 \begin{theorem} The NBS  for the MOO optimization problem in \eqref{eq:opt_higher} can be  obtained by solving the following optimization problem:% in \eqref{eq:nashProbNplayermod}.
 \begin{subequations}\label{eq:nashProbNplayermod}
 	\begin{align}
  	\max_{\mathbf{X}}\;& \prod_{n=1}^{N}\hspace*{-0.05in}\bigg(\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)-u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big)  \nonumber \\
  	&+\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)\nonumber\\
  	&- D^l({x}_{n,k}^l)\big)\Big)-d_n^0
  	\bigg),\label{eq:objmain} \\
 	\text{s.t.}\quad & Constraints \; in \; \eqref{eq:obj1}-\eqref{eq:obj4}, \nonumber \\
 %	&\sum_{j \in \mathcal{M}_n}\Big(u_n^j(\sum_{m \in \overline{\mathcal{N}}}\mathbf{x}_m^j+\mathbf{x}_n^j)- u_n^j(\sum_{m \in \overline{\mathcal{N}}}\mathbf{x}_m^j) \Big)+ \nonumber \\
 	&\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)-u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big)  \nonumber \\
 	&+\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)\nonumber\\
 	&- D^l({x}_{n,k}^l)\big)\Big)> d_n^0, \quad \forall \; n \in \mathcal{N}.\label{eq:disagreemt}
 	\end{align}
 \end{subequations}
 \end{theorem}%\vspace{-0.2in}
\begin{proof}
The feasible set for the above optimization problem is convex and compact, since all constraints are convex and intersection of convex sets is a convex set. Furthermore, based on our assumptions, there exist solutions (allocation and sharing decisions) that  provide better utility than the disagreement point $d_n^0, \forall\; n \in \mathcal{N}$. Hence, the solution of the optimization problem in \eqref{eq:nashProbNplayermod} is the NBS.
\end{proof}%\vspace{-0.1in}
However, solving \eqref{eq:nashProbNplayermod} is computationally complex and the problem is not always convex.  Therefore, there is a need for an efficient method to obtain the NBS. %\vspace{-0.1in}
%\subsection{Complexity Reduction}
Toward this goal,  we transform the problem \eqref{eq:nashProbNplayermod} into an equivalent problem as proposed in \cite{yaiche2000game}. %first need to transform our problem as stated in the following theorem. 

\begin{comment}
\begin{theorem}[Problem transformation\cite{yaiche2000game}]
	\label{thm:transformation}
	Suppose for every player $n \in \mathcal{N}$, $s_n \in \mathcal{S}$ is injective function in the feasible set $\mathcal{F}$ (satisfying all the constraints). Under the assumptions of NBS, let us consider the following
	\begin{align}
	\label{eq:nashProbN}
	\max_{s_1,\cdots,s_N}\;\prod_{n=1}^{N}(s_n-d_n),\; s.t.\;  s_n \in \mathcal{F},\; \forall n \in \mathcal{N}
	\end{align}\vspace{-0.15in}
		\begin{align}
	\label{eq:nashProbN2}
	\max_{s_1,\cdots,s_N}\;\sum_{n=1}^{N}\ln(s_n-d_n),\; s.t.\;  s_n \in \mathcal{F},\; \forall n \in \mathcal{N}
	\end{align}
	\begin{enumerate}
		\item Equation \eqref{eq:nashProbN} has a unique solution  and the bargaining solution is just a single point, where as Equation \eqref{eq:nashProbN2} is a convex optimization problem with a unique solution.
		\item The optimization problems in Equations \eqref{eq:nashProbN} and \eqref{eq:nashProbN2} are equivalent. Hence, the  unique solution of Equation \eqref{eq:nashProbN2} is the NBS.
		%\item The unique solution of Equation \eqref{eq:nashProbN2} is the NBS.
	\end{enumerate}
\end{theorem}
The above transformation reduces the complexity and always guarantees an NBS \cite{khan2009cooperative}. 
\end{comment}


\begin{corollary}%[\cite{weiser1994scheduling,stefanescu1984arbitrated}]
The NBS for \eqref{eq:opt_higher} is obtained by solving the following optimization problem:
%	\begin{align}\label{eq:objmain1} 
%\max_{\mathcal{X}}\quad& \prod_{n=1}^{N}\bigg(u_n(\mathcal{X})+ \big(\sum_{j \in \mathcal{N},j\neq n}  u^{n}_j(\mathcal{X})\big)-d_n^0\bigg), \; s.t. \; \mathcal{X} \in  \mathcal{F}
%\end{align}
%	\begin{align}\label{eq:objmain2} 
%\max_{\mathcal{X}}\quad& \sum_{n=1}^{N}\bigg(u_n(\mathcal{X})+ \big(\sum_{j \in \mathcal{N},j\neq n}  u^{n}_j(\mathcal{X})\big)-d_n^0(\mathcal{X})\bigg), \; s.t. \; \mathcal{X} \in  \mathcal{F}
%\end{align}
%\begin{subequations}\label{eq:objmain2} 
	\begin{align}\label{eq:objmain2} 
	\max_{\mathbf{X}}\;& \sum_{n=1}^{N}\ln\bigg(\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)- \nonumber \\
	&u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big) +\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)\nonumber\\
	&-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)- D^l({x}_{n,k}^l)\big)\Big)-d_n^0
	\bigg),\\
	\text{s.t.}\quad &  Constraints \; in \; \eqref{eq:obj1}-\eqref{eq:obj4}, \; \eqref{eq:disagreemt}. \nonumber 
	\end{align}
\end{corollary}
%\vspace{-0.2in}
\begin{proof}
	ESP utilities are concave and  bounded above. Furthermore, the feasible set along with the set of achievable utilities ($\mathcal{S}$) is convex and compact (due to the nature of  utilities and constraints). %Hence, the NBS with higher complexity  is guaranteed to exist. 
	Utilities of ESPs are also injective functions of the allocation decision. Hence \eqref{eq:objmain2} is equivalent to \eqref{eq:nashProbNplayermod} \cite{yaiche2000game}. Since   the logarithm of any positive real number is concave\cite{boyd2004convex},  \eqref{eq:objmain2} is a convex optimization problem with a unique solution, which is the NBS. %Hence using Theorem \ref{thm:transformation}, the result follows. 
\end{proof}
%\vspace{-0.1in}
The centralized Algorithm \ref{algo:centralnbs} provides the allocation decision using NBS. %Traditionally, each ESP receives a pay-off equal to the utility it achieves by solving \eqref{eq:objmain2}. However, due to the nature of utility we suggested to use for reducing resource fragmentation, an  ESP may over-estimate its payoff achieved by allocating resources to an application\footnote{The utility earned by ESP $n$ for allocating resources to application $j$ considers the resources allocated at other ESPs as well, i.e., $u_n^j(\mathbf{x}_n^j+\sum_{m \in \mathcal{{N}}\backslash n}\mathbf{x}_{m}^j)$. Hence, even if  a ESP $n$ allocates no resources to application $j$ (while other ESPs do), ESP $n$ will be assigned a payoff based on the resources allocated by other ESPs.}. Hence, the utility needs to be divided among different ESPs using the rule specified in \eqref{eq:payoffrule} where $P_n^j$ is the payoff ESP $n$ receives for allocating resources to application $j$ and $P_T^j$ is the total payoff obtained from allocating resources to application $j$. 
%\begin{equation}
%\label{eq:payoffrule}
%P_n^j= \frac{\mathbf{x}_n^j}{\sum_{m \in \mathcal{{N}}}\mathbf{x}_m^j}\times P_T^j
%\end{equation}
%the utility achieved by each ESP in \eqref{eq:objmain2} is the payoff that the ESP wou

\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}:  $C, R$, and vector of utility functions of all ESPs $\boldsymbol{u}$ %  and $\mathcal{X}_0$ %$\forall \boldsymbol{\nu_0$, $\mu_0}\in\mathcal{R}$ and $\boldsymbol h_0$ 
		\State \textbf{Output}: The optimal resource allocation $\mathbf{X}$ and payoffs of all ESPs
		\State \textbf{Step $1$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {d_n^0} \leftarrow$ \texttt{Objective function at optimal point in Equation \eqref{eq:opt_single}}
		\EndFor
		\State \textbf{Step $2$:} $\mathbf{X} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:objmain2}} %$\forall n \in \mathcal{{N}}$
	%	\State \textbf{Step $3$:} $P_n^j\leftarrow$ \texttt{Payoff received by ESP} $\forall n \in \mathcal{{N}}, j \in \mathcal{{M}}$\texttt{ using \eqref{eq:payoffrule}}
	\end{algorithmic}
	\caption{Centralized Algorithm for NBS}
	\label{algo:centralnbs}
\end{algorithm}


\begin{comment}
\begin{theorem}\label{thm:centralsolution}
	The solution to the optimization problem in \eqref{eq:objmain2}, provided that the inverse of the first derivative of $u_{n}^j(x_{n,k}^j)$ and $f_n^l=(u_{n}^l(x_{n,k}^l)-C_n^l(x_{n,k}^l))$ exist, is given by 
	\begin{equation}
	\label{eq:solcentral}
	x_{n,k}^{*j}=    u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j,\zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j}), \quad \quad \quad \forall j \in \mathcal{M},
%	x_{n,k}^{*j}=    u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j,\zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j},r_{k}^j), \quad \quad \quad \forall j \in \mathcal{M},%   \left\{\begin{matrix}
%  u_n^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)}), \quad \quad \quad \forall i \in \mathcal{M}_n\\
 % u_{jn}^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)}), \quad \forall i \in \mathcal{M}\backslash\mathcal{M}_n 	
%	\end{matrix}\right.
	%U_n^{'-1}(\alpha_k^{(n)}, \beta_{ik})
	\end{equation}
		\begin{equation}
	\label{eq:solcentral2}
	x_{n,k}^{*l}=    f_n^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Lambda_{n,k}^{l}), \quad  \forall l \in \{\mathcal{M}\backslash\mathcal{{M}}_n\},%   \left\{\begin{matrix}
	%  u_n^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)}), \quad \quad \quad \forall i \in \mathcal{M}_n\\
	% u_{jn}^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)}), \quad \forall i \in \mathcal{M}\backslash\mathcal{M}_n 	
	%	\end{matrix}\right.
	%U_n^{'-1}(\alpha_k^{(n)}, \beta_{ik})
	\end{equation}
	where   $u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j,\zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j})$ and $f_n^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Lambda_{n,k}^{l})$ are  %and $u_{jn}^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)})$ are
	 the inverse of the first derivative of $u_{n}^j$ and $(u_{n}^l(x_{n,k}^l)-C_n^l(x_{n,k}^l))$, respectively. %and $u_j^n$ respectively. 
	$\alpha_{n,k}$,  $\beta_{k}^j$, $\zeta_{n}$, and $\gamma_{n,k}^{j}$ are the \emph{Lagrange} multipliers and $\Lambda_{n,k}^{j}=\bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\mathbf{x}_n^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg)$. 
	
	% $\Lambda_{n,k}^{j}=\prod_{t\in \{\mathcal{N}\backslash n\}}\bigg(\sum_{j \in \mathcal{M}_n}u_t^j(\mathbf{x}_t^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_t\}} u_t^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_t^0\bigg)$.
	
	%$\Lambda_{n,k}^{j}=\bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\mathbf{x}_n^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg)$. 
	
	
	
	%$\Lambda_{n,k}^{j}=\bigg(\sum_{j \in \mathcal{M}_n}\big(u_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}} \frac{\sum_{n \in \mathcal{{N}}}x_{n,k}^{j}}{r_{k}^{j}}\big)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg)$.
\end{theorem}
\begin{proof}
	

	
	

	
	The Lagrangian function  for \eqref{eq:objmain2} is given in \eqref{eq:lagrangian} on the next page.  %$\boldsymbol{\alpha}$, $\boldsymbol{\beta},$  $\boldsymbol{\zeta}$ and $\boldsymbol{\gamma}$ are vector of Lagrangian multipliers. The first term in the Lagrangian function represents the improvement in the utility of a player sharing and allocating its resources (compared to only allocating its resources to its own applications). The second term is the profit the player will be making by charging each unit of its available resources with $\alpha_k$. The third term is the penalty for violating the positive allocation constraint. The fourth term is the profit a game player earns by allocating resources to applications for satisfying the applications demands $r_{ik}$ at a price of $\beta_{ik}$, while the last term is the incentive for the system to not degrade the performance of any player below the disagreement point. 	
	Since the Lagrangian function consists of differentiable and continuous functions, we can use gradients to obtain the optimal allocation decision and Lagrangian multipliers. %To obtain the maximum of Lagrangian function with respect to (w.r.t.) the allocation decision ${x_{ik}^{(n)}}$, we calculate the gradient of \eqref{eq:lagrangian} w.r.t. ${x_{ik}^{(n)}}$ and set it to zero as the first derivative diminishes at the maxima. 
	Depending on the application $j$, we have two cases: 
	\begin{enumerate}
		\item \textbf{$j \in \mathcal{M}_n$:}$\frac{\partial \mathcal{L}}{\partial x_{n,k}^{j}}=0$
			\begin{align}
		\label{eq:gradLagObj}
	%	 \Big(u_n^{'j}(x_{n,k}^{j})+\frac{1}{r_{k}^j}\Big)(1+\Lambda_{n,k}^{j}\zeta_{n})-\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j-\nonumber \\
	%	 \gamma_{n,k}^{j})=0,\nonumber \\
u_n^{'j}(x_{n,k}^{j})(1+\Lambda_{n,k}^{j}\zeta_{n})-\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j-\gamma_{n,k}^{j})=0,\nonumber \\	
	%	 \implies u_n^{'j}(x_{n,k}^{j})=\frac{\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Lambda_{n,k}^{j}\zeta_{n}}-\frac{1}{r_{k}^j}, \nonumber \\
		  \implies u_n^{'j}(x_{n,k}^{j})=\frac{\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Lambda_{n,k}^{j}\zeta_{n}}, \nonumber \\
		%& \nonumber \\
	%	\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j},r_{k}^j).
				\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j}).
		\end{align}
		%	Where the last step follows from the fact that  utility function used is $1-1$, so its derivative is also $1-1$ and its inverse $U_n^{'-1}(\alpha_k, \beta_{ik})$ can easily be computed.
	\item \textbf{$l \in \{\mathcal{M}\backslash\mathcal{M}_n\}$:} $\frac{\partial \mathcal{L}}{\partial x_{n,k}^{l}}=0$
		\begin{align}
	\label{eq:gradLagObjcase2}
	 f^{'l}_n(x_{n,k}^{l})(1+\Lambda_{n,k}^{l}\zeta_{n})-\Lambda_{n,k}^{l}(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})=0,\nonumber \\ 
	\implies  f^{'l}_n(x_{n,k}^{l})=\frac{\Lambda_{n,k}^{l}(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})}{1+\Lambda_{n,k}^{l}\zeta_{n}}, \nonumber \\
	%& \nonumber \\
	\implies \quad x_{n,k}^{*l}= f_{n}^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Lambda_{n,k}^{l}).
	\end{align}
	\end{enumerate}
\end{proof}

In cases where $u_n^{'-j}(\boldsymbol{.})$  and $f_{n}^{'-l}(\boldsymbol{.}) $ do not exist, one should use alternate methods such as {gradient based iterative equation}\cite{tychogiorgos2013non}: % in \eqref{eq:gradientbasediterative} can be used \cite{tychogiorgos2013non}.

\begin{align}
\label{eq:gradientbasediterative}
x_{n,k}^{j}(t+1)=x_{n,k}^{j}(t)+\epsilon_{n,k}^{j}\frac{\partial \mathcal{L}}{\partial x_{n,k}^{j}}
\end{align}
where $\epsilon_{n,k}^{j}$ is a positive step size. 
%Algorithm \ref{algo:centralnbs} shows our centralized algorithm that provides the NBS for \eqref{eq:opt_higher}. 

\end{comment}

	\begin{figure*}[!t]
	\normalsize
	\begin{align}
	\label{eq:lagrangian}
	\mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta, \zeta,\gamma,\pi})&= 
	\sum_{n=1}^{N}\ln\bigg(\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)- u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big)+\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-\nonumber\\
	&\hspace*{-1.3in}\quad u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)- D^l({x}_{n,k}^l)\big)\Big)-d^0_n\bigg) +   \quad \sum_{\substack{n \in \mathcal{N},\\j \in \mathcal{M},\\k \in \mathcal{K}}}\gamma_{n,k}^{j}x_{n,k}^{j} +\sum_{\substack{n \in \mathcal{N},\\k \in \mathcal{K}}}\alpha_{n,k} (C_{n,k}-\sum_{j \in \mathcal{M}}x_{n,k}^{j}) +\sum_{\substack{j \in \mathcal{M},\\k \in \mathcal{K}}}\beta_{k}^j (r_{k}^{j}-\sum_{n \in \mathcal{N}}x_{n,k}^{j}) + \sum_{n \in \mathcal{N}} \zeta_{n}  \nonumber \\
	& \hspace*{-1.3in}\quad \bigg(\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u_n^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)- u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big)+ \quad \Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)-\nonumber\\
	&\hspace*{-1.3in}\quad  D^l({x}_{n,k}^l)\big)\Big)-d_n^0
	\bigg)+\sum_{\substack{n\in \mathcal{{N}},\\l\in \overline{\mathcal{M}},\\k\in\mathcal{K}}}\pi_{n,k}^l \Big(u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-
	u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)-  D^l({x}_{n,k}^l)\Big).
	\end{align}
	\hrulefill
\end{figure*}
\section{Distributed algorithm for NBS}\label{sec:dist}
While resource allocation and sharing  using a central algorithm is feasible, it is desirable to develop low overhead distributed algorithms. %A distributed algorithm will eliminate the need for the coalition (central) controller discussed in Section \ref{sec:sysmodel} and domains can exchange information among each other.   %modern communication networks may require the ability to develop distributed algorithms without significant messaging overhead. 
To obtain a distributed algorithm,  we rely on \emph{Duality Theory} and use the \emph{Lagrangian} function   in \eqref{eq:lagrangian}. 
The dual optimization problem is given by %\vspace{-0.2in}
\begin{align}\label{eq:dualopt}
\min_{\boldsymbol{\alpha},\boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}} D(\boldsymbol{\alpha},\boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi})&= \mathcal{L}\big(\mathbf{X}^{*}(\boldsymbol{\alpha,\beta},\boldsymbol{\zeta,\gamma,\pi}),\nonumber \\& \boldsymbol{\alpha,\beta,\zeta,\gamma,\pi} \big), \nonumber \\
\; s.t. \; \boldsymbol{\alpha},\boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}\geq 0.
\end{align}
%whereas \vspace{-0.2in} 
%where \vspace{-0.12in}
\begin{align}\label{eq:supLag}
\mathbf{X}^{*}(\boldsymbol{\alpha,\beta},\boldsymbol{\zeta,\gamma,\pi})= \arg \max_{\mathbf{X}} \mathcal{L}(\mathbf{X},\boldsymbol{\alpha,\beta},\boldsymbol{\zeta,\gamma,\pi} ).
\end{align}
The dual problem can be solved iteratively using gradient descent (since the dual problem is a minimization problem) as below:
\begin{align}\label{eq:iterativeDual}
\alpha_{n,k}[t+1] &=  \alpha_{n,k}[t]- \phi_{n,k} \frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \alpha_{n,k}}, \nonumber \displaybreak[0] \\
\beta_{k}^j[t+1] &=  \beta_{k}^j[t]- \eta_{k}^j \frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \beta_{k}^j}, \nonumber \\
\zeta_{n}[t+1] &=  \zeta_{n}[t]- \omega_{n} \frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \zeta_{n}}, \nonumber \displaybreak[0]\\
\gamma_{n,k}^{j}[t+1] &=  \gamma_{n,k}^{j}[t]- \theta_{n,k}^{j} \frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \gamma_{n,k}^{j}},\nonumber \\
\pi_{n,k}^{l}[t+1]&=\pi_{n,k}^{l}[t]-\psi_{n,k}^l \frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \pi_{n,k}^{l}},
\end{align}
where $\phi_{n,k}$, $\eta_{k}^j$,  $\omega_{n}$, $\theta_{n,k}^{j}$ and $\psi_{n,k}^l$ are positive step sizes. Furthermore, the gradients in \eqref{eq:iterativeDual} are given below.%\vspace{-0.2in}
\begin{comment}
	\begin{figure*}[!t]
	\normalsize
	\begin{align}
	\label{eq:lagrangian2}
	\mathcal{L}(\mathbf{X}_n, \boldsymbol{\alpha}, \boldsymbol{\beta, \zeta,\gamma})&= %\sum_{n=1}^{N}\ln\bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\mathbf{x}_n^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg) +  \quad \sum_{n \in \mathcal{N}}\sum_{j \in \mathcal{M}}\sum_{k \in \mathcal{K}}\gamma_{n,k}^{j}x_{n,k}^{j} +\nonumber \\
	\prod_{n=1}^{N}\bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\mathbf{x}_n^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg) +  \quad \sum_{n \in \mathcal{N}}\sum_{j \in \mathcal{M}}\sum_{k \in \mathcal{K}}\gamma_{n,k}^{j}x_{n,k}^{j} +\nonumber \\
	& \quad\sum_{n \in \mathcal{N}}\sum_{k \in \mathcal{K}}\alpha_{n,k} (C_{n,k}-\sum_{j \in \mathcal{M}}x_{n,k}^{j}) + \sum_{j \in \mathcal{M}}\sum_{k \in \mathcal{K}}\beta_{k}^j (r_{k}^{j}-\sum_{n \in \mathcal{N}}x_{n,k}^{j}) + \sum_{n \in \mathcal{N}} \zeta_{n} \bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\mathbf{x}_n^j)+ \nonumber \\
	&  \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-  C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg).
	%	\mathcal{L}(\mathbf{X}_n, \boldsymbol{\alpha}, \boldsymbol{\beta, \zeta,\gamma})&= \sum_{n=1}^{N}\ln\bigg(\sum_{j \in \mathcal{M}_n}\big(u_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}} \frac{x_{n,k}^{j}}{r_{k}^{j}}\big)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg) +  \quad \sum_{n \in \mathcal{N}}\sum_{j \in \mathcal{M}}\sum_{k \in \mathcal{K}}\gamma_{n,k}^{j}x_{n,k}^{j} +\nonumber \\
	%	& \quad\sum_{n \in \mathcal{N}}\sum_{k \in \mathcal{K}}\alpha_{n,k} (C_{n,k}-\sum_{j \in \mathcal{M}}x_{n,k}^{j}) + \sum_{j \in \mathcal{M}}\sum_{k \in \mathcal{K}}\beta_{k}^j (r_{k}^{j}-\sum_{n \in \mathcal{N}}x_{n,k}^{j}) + \sum_{n \in \mathcal{N}} \zeta_{n} \bigg(\sum_{j \in \mathcal{M}_n}\big(u_n^j(\mathbf{x}_n^j)+\sum_{k \in \mathcal{K}} \frac{x_{n,k}^{j}}{r_{k}^{j}}\big)+ \nonumber \\
	%	&  \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\mathbf{x}_n^l)-  C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg).
	\end{align}
	\hrulefill
	%	\vspace*{-5pt}
	%	\vspace{-0.15in}
\end{figure*}	
\end{comment}
\begin{align}\label{eq:gradforLagrangieMultipliers}
\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta}, \boldsymbol{\zeta,\gamma,\pi}) }{\partial  \alpha_{n,k}}&= (C_{n,k}-\sum_{j \in \mathcal{M}}x_{n,k}^{j}),\nonumber \\
\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta}, \boldsymbol{\zeta,\gamma,\pi}) }{\partial  \beta_{k}^j} &= (r_{k}^{j}-\sum_{n \in \mathcal{N}}x_{n,k}^{j}),\nonumber \\
\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \zeta_{n}} &=\bigg(\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)-  \nonumber \\
&\hspace*{-1.2in}u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big)+\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-\nonumber\\
&\hspace*{-1.2in}u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)- D^l({x}_{n,k}^l)\big)\Big)-d_n^0
\bigg)
, \nonumber \\
\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \gamma_{n,k}^{j}} &= x_{n,k}^{j},\nonumber\\
\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi}) }{\partial  \pi_{n,k}^{l}} &=\Big(u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-\nonumber \\
&\hspace*{-1.2in}
u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)-  D^l({x}_{n,k}^l)\Big).
\end{align}
%%Since the primal problem is convex, the convergence of the primal-dual algorithm that consists of \eqref{eq:supLag} and \eqref{eq:iterativeDual} is guaranteed \cite{panigrahy2017and} i.e., it will converge to the unique global optimal with zero-duality gap. Algorithm \eqref{algo:primal-dual-alg} shows our primal-dual algorithm. 
Unless certain  conditions such as Slater's constraint qualification  are satisfied, \emph{strong duality}\footnote{Strong duality implies that there is no duality gap between the primal and dual problem.} is not guaranteed to hold for our primal and dual problems \cite{boyd2004convex}. However,  we rely on the following theorems to show that strong duality holds.
\begin{theorem}[Sufficient Condition\cite{tychogiorgos2013non}]\label{thm:georgesufficient}
	If the price based function $\mathbf{X}^*(\boldsymbol{\alpha,\beta},\boldsymbol{\zeta,\gamma,\pi})$ is continuous at one or more of the optimal Lagrange multipliers,  the iterative algorithm consisting of  \eqref{eq:supLag} and \eqref{eq:iterativeDual} will converge to the global optimal solution. 
\end{theorem}
\begin{theorem}[Necessary Condition\cite{tychogiorgos2013non}]\label{thm:georgenecessary}
	The condition in Theorem \ref{thm:georgesufficient} is also necessary if at least one of the constraints in \eqref{eq:objmain2} is active (binding) at the optimal solution. % and eliminate the need for a central controller. The domain controllers can exchange  information about capacities, and  requirements and obtain the NBS.  
\end{theorem}
\begin{lemma}\label{lem:constraintsactive}
	At the optimal solution, the optimal Lagrange multiplier vector corresponding to the capacity constraint is non-zero, i.e., $\boldsymbol{\alpha_k^{*}}>0$. 
\end{lemma}
\begin{proof}
	At the optimal point, all  resources are fully utilized,  i.e., capacity constraints are active. From \emph{complementary slackness}\cite{boyd2004convex}, we know that %\vspace{-0.08in}
	\begin{align}\label{eq:compslackness}
	\alpha^*_{n,k}\bigg(\sum_{j\in \mathcal{M}} x_{n,k}^{*j}- C_{n,k}\bigg)=0, \forall n \in \mathcal{N}. 
	\end{align}
	Since $\sum_{j\in \mathcal{M}} x_{n,k}^{*j}= C_{n,k}$, i.e., the constraint is active, which implies that $\boldsymbol{\alpha_k^{*}} >0$.
\end{proof}
%\vspace{-0.12in}
\begin{theorem}\label{thm:duality}
For any concave injective utility function for which the inverse of the first derivative exists, the iterative distributed algorithm consisting of  \eqref{eq:supLag} and \eqref{eq:iterativeDual}  converges to the global optimal solution.% i.e., strong duality holds.% for our resource sharing and allocation problem if we use a concave, injective utility function for which the inverse of  first derivative exists. 
\end{theorem}
%\begin{proof}
%	See Appendix \ref{sec:FirstAppendix} for the proof
%	\end{proof}
\begin{proof}
	We show that the price function obtained by $\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma,\pi})}{\partial x_{n,k}^{j}}=0$ is continuous at one or more of the optimal Lagrange multipliers for \eqref{eq:lagrangian}.  
	
	Let  $u^{'-j}(\boldsymbol{.})$ %(\alpha_{n,k}, \beta_{k}^j,\zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j})$ 
	and $f^{'-l}(\boldsymbol{.})$ %%(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Lambda_{n,k}^{l})$ 
	represent   %and $u_{jn}^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)})$ are
	the inverses of the first derivative of $u^j$ and $\big(u^l(\sum_{m\in\overline{\mathcal{N}}} x_{m,k}^l+x_{n,k}^l)-u^l(\sum_{m\in\overline{\mathcal{N}}} x_{m,k}^l) -D^l(x_{n,k}^l)\big)$, respectively. %and $u_j^n$ respectively. 
	$\alpha_{n,k}$,  $\beta_{k}^j$, $\zeta_{n}$,  $\gamma_{n,k}^{j}$ and $\pi_{n,k}^l$ are the \emph{Lagrange} multipliers whereas:   
	\begin{align}
	\Delta_{n}&=\sum_{\substack{j \in \mathcal{M}_n,\\k \in \mathcal{K}}}\Big(u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+{x}_{n,k}^j)- u^j(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j) \Big)+ \nonumber \\
	&\Big(\sum_{\substack{l \in \overline{\mathcal{M}},\\k \in \mathcal{K}}}\big( u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+{x}_{n,k}^l)-u^l(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l)- \nonumber\\
	&D^l({x}_{n,k}^l)\big)\Big)-d_n^0
	%\sum_{j \in \mathcal{M}_n}\Big(u_n^j(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^j+\mathbf{x}_n^j)- u_n^j(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^j) \Big)+ \nonumber \\
	%&\Big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^l+\mathbf{x}_n^l)-u_n^l(\sum_{m \in \mathcal{N}\backslash n}\mathbf{x}_m^l)-\nonumber\\ &D_n^l(\mathbf{x}_n^l)\Big)-d_n^0, \nonumber 
	\end{align}
	We consider two different cases
% There are two different cases that we evaluate in the following: %To simplify the proof, we only consider the case  in which $i \in \mathcal{M}_n$ below. The proof for the case when $i \in \mathcal{M}\backslash\mathcal{M}_n$ is similar. 
	%\begin{enumerate}
	%	\item 
%	\vspace{-0.12in}
	
	\subsubsection{	\textbf{$j \in \mathcal{M}_n$:}$\frac{\partial \mathcal{L}}{\partial x_{n,k}^{j}}=0$}
%	\vspace{-0.05in}
		\begin{align}
		\label{eq:gradLagObj22}
		&u^{'j}(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+x_{n,k}^{j})(1+\Delta_{n}^{}\zeta_{n})-\Delta_{n}^{}(\alpha_{n,k}+\nonumber \\
		&\beta_{k}^j-\gamma_{n,k}^{j})=0,\nonumber \\	
		&\implies u^{'j}(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j+x_{n,k}^{j})=\frac{\Delta_{n}^{}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n}^{}\zeta_{n}}, \nonumber \\
		& x_{n,k}^{j}=u^{'-j}\Bigg(\frac{\Delta_{n}^{}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n}^{}\zeta_{n}}\Bigg)-\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j. %\nonumber \\
		%& \nonumber \\
		%	\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j},r_{k}^j).
		%	&\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Delta_{n,k}^{j}).
		%\vspace{-0.12in}
		\end{align}
		 We prove that \eqref{eq:gradLagObj22} is continuous at the optimal point by showing that the numerator $\Delta_{n}^{}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})$ and denominator $1+\Delta_{n}^{}\zeta_{n} $ are positive\footnote{Positive numerator and denominator are required if $u^{'-j}$ is $\log$. For other cases, it will suffice to prove that the denominator is non-zero. }. 	At the optimal point, the denominator $(1+\Delta_{n}^{*}\zeta^*_{n})$ is positive as $\Delta_{n}^{*}>0$ (from Section \ref{sec:assumption}) and $\zeta^*_{n}=0$ (from complementary slackness).	Similarly, in the numerator, %$\Delta_{n,k}^j$ (from Section \ref{sec:assumption}) and $e^{(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j-\bar{r}_{n,k}^j)}$ are positive.
		 $(\alpha^*_{n,k}+\beta_{k}^{*j}-\gamma_{n,k}^{*j})>0$, as  $\alpha_{n,k}^{*}>0$ (from Lemma \ref{lem:constraintsactive}) and  $\alpha_{n,k}^{*}+\beta_{k}^{*j}> \gamma_{n,k}^{*j}$ (from \emph{sensitivity analysis} \cite{boyd2004convex}). Hence, \eqref{eq:gradLagObj22} is continuous at the optimal point.
		  \begin{comment}
		 As an example, we set
		 	For sake of the proof, we set \\ $u_n^j=1-e^{-(x_{n,k}^j+\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j-r_{n,k}^j+\delta t)}$ where $\bar{r}_{k}^j=r_{k}^j+\delta t$. %However, the results hold for any concave injective utility function for which the inverse of the first derivative exists.  
		 	\eqref{eq:gradLagObj22} can then be rewritten as:
		 \begin{align}\label{eq:proof1}
		 e^{-(x_{n,k}^j+\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^j-\bar{r}_{k}^j)}= \frac{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n,k}^{j}\zeta_{n}},\quad\nonumber \\
		 e^{x_{n,k}^j}= \frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{k}^j)}},\quad\quad\nonumber \\
		 x_{n,k}^j=\ln\bigg(\frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{k}^j)}}\bigg).
		 \end{align} 
		 where \eqref{eq:proof1} is continuous at the optimal point. 
		  
		
		
		 For \eqref{eq:gradLagObj22} to be continuous at the optimal point,
		
		 we need 
		%\vspace{-0.1in}
		For sake of the proof, we set \\ $u_n^j=1-e^{-(x_{n,k}^j+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-r_{n,k}^j+\delta t)}$ where $\bar{r}_{k}^j=r_{k}^j+\delta t$. However, the results hold for any concave injective utility function for which the inverse of the first derivative exists.  \eqref{eq:gradLagObj22} can then be rewritten as:
		\begin{align}\label{eq:proof1}
		 e^{-(x_{n,k}^j+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{k}^j)}= \frac{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n,k}^{j}\zeta_{n}},\quad\nonumber \\
		e^{x_{n,k}^j}= \frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{k}^j)}},\quad\quad\nonumber \\
		x_{n,k}^j=\ln\bigg(\frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{k}^j)}}\bigg).
		\end{align} 
		%We know that $\Lambda_{ik}^{(n)>0$, 
		For continuity, we need both the numerator and denominator inside the $\ln(\boldsymbol{.})$ function of \eqref{eq:proof1} to be positive.  
		At the optimal point, the numerator $(1+\Delta_{n,k}^{*j}\zeta^*_{n})$ is positive as $\Delta_{n,k}^{*j}>0$ (from Section \ref{sec:assumption}) and $\zeta^*_{n}=0$ (from complementary slackness).	Similarly, in the denominator, $\Delta_{n,k}^j$ (from Section \ref{sec:assumption}) and $e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}$ are positive. $(\alpha^*_{n,k}+\beta_{k}^{*j}-\gamma_{n,k}^{*j})>0$, as  $\alpha_{n,k}^{*}>0$ (from Lemma \ref{lem:constraintsactive}) and  $\alpha_{n,k}^{*}+\beta_{k}^{*j}> \gamma_{n,k}^{*j}$ (from \emph{sensitivity analysis} \cite{boyd2004convex}). %Furthermore, the denominator $(r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}^*+\beta_{k}^{*j}- \gamma_{n,k}^{*j})-1>0)$ based on our assumptions in Section \ref{sec:assumption}.
		Hence, the price based function in \eqref{eq:proof1} is continuous in at least one optimal Lagrange multiplier vector. 
		\end{comment}
\\		
		%	Where the last step follows from the fact that  utility function used is $1-1$, so its derivative is also $1-1$ and its inverse $U_n^{'-1}(\alpha_k, \beta_{ik})$ can easily be computed.
		%\item 
		\subsubsection{\textbf{$l \in \{\mathcal{M}\backslash\mathcal{M}_n\}$:} $\frac{\partial \mathcal{L}}{\partial x_{n,k}^{l}}=0$}
		\begin{align}
		\label{eq:gradLagObjcase22}
		&f^{'l}(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+x_{n,k}^{l})(1+\Delta_{n}^{}\zeta_{n}+\Delta_{n}^{}\pi_{n,k}^l)-\Delta_{n}^{}(\alpha_{n,k}+\nonumber \\
		&\beta_{k}^l-\gamma_{n,k}^{l})=0,\nonumber \\
		&\implies  f^{'l}(\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l+x_{n,k}^{l})=\frac{\Delta_{n}^{}(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})}{1+\Delta_{n}^{}\zeta_{n}+\Delta_{n}^{}\pi_{n,k}^j}. \nonumber \\
		&  x_{n,k}^{l}=f^{'-l}\Bigg(\frac{\Delta_{n}^{}(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})}{1+\Delta_{n}^{}\zeta_{n}+\Delta_{n}^{}\pi_{n,k}^l}\Bigg)-\sum_{m \in \overline{\mathcal{N}}}{x}_{m,k}^l. \nonumber \\
		\end{align}
%	\end{enumerate}
\begin{comment}
	As done earlier, we set  $u_n^l=1-e^{-(x_{n,k}^l+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^l-\bar{r}_{k}^l)}$, \\ and $C_n^l=x_{n,k}^l/w_k^l$, where $w_k^l$ is a positive weighting factor to capture  the communication cost. Then $ f^{'l}_n(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^l+x_{n,k}^{l})$ can be rewritten as 
	\begin{align}
	\label{eq:fnl}
	 f^{'l}_n(\boldsymbol{.})= e^{-(x_{n,k}^l+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^l-\bar{r}_{k}^l)}-\frac{1}{w_k^l}
	\end{align}
Plugging \eqref{eq:fnl} in \eqref{eq:gradLagObj22} and solving for $x_{n,k}^l$, we obtain
	\begin{align}
	\label{eq:fnl2}
	x_{n,k}^l=\ln \Bigg(\frac{w_k^l(1+\Delta_{n,k}^{l}\zeta_{n})e^{-(\sum_{m \in \mathcal{N}\backslash n}x_{m,k}^l-\bar{r}_{k}^l)}}{w_k^l\Delta_{n,k}^l(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})+1+\Delta_{n,k}^{l}\zeta_{n}}\Bigg).
	\end{align}
	\end{comment}
	The continuity at optimal point can be established using arguments similar  to that for  $j \in \mathcal{{M}}_n$ case. The proof of zero-duality gap follows from Theorem \ref{thm:georgesufficient}.  Hence, strong duality holds and our proposed distributed algorithm converges to the NBS. 
\end{proof}

\begin{comment}
\begin{proof}
	We show that the price function obtained by $\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma})}{\partial x_{n,k}^{j}}=0$ is continuous at one or more of the optimal Lagrange multipliers for \eqref{eq:lagrangian2}. Let $\Delta_{n,k}^{j}=\prod_{t\in \{\mathcal{N}\backslash n\}}\bigg(\sum_{j \in \mathcal{M}_t}u_t^j(\mathbf{x}_t^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_t\}} u_t^l(\mathbf{x}_t^l)-C_n^l(\mathbf{x}_t^l)\big)-d_t^0\bigg)$. %To simplify the proof, we only consider the case  in which $i \in \mathcal{M}_n$ below. The proof for the case when $i \in \mathcal{M}\backslash\mathcal{M}_n$ is similar. 
	
	
		\begin{enumerate}
		\item \textbf{$j \in \mathcal{M}_n$:}$\frac{\partial \mathcal{L}}{\partial x_{n,k}^{j}}=0$
		\begin{align}
		\label{eq:gradLagObj22}
		%	 \Big(u_n^{'j}(x_{n,k}^{j})+\frac{1}{r_{k}^j}\Big)(1+\Lambda_{n,k}^{j}\zeta_{n})-\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j-\nonumber \\
		%	 \gamma_{n,k}^{j})=0,\nonumber \\
		u_n^{'j}(x_{n,k}^{j})(\Delta_{n,k}^{j}+\zeta_{n})-(\alpha_{n,k}+\beta_{k}^j-\gamma_{n,k}^{j})=0,\nonumber \\	
		%	 \implies u_n^{'j}(x_{n,k}^{j})=\frac{\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Lambda_{n,k}^{j}\zeta_{n}}-\frac{1}{r_{k}^j}, \nonumber \\
		\implies u_n^{'j}(x_{n,k}^{j})=\frac{(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{\Delta_{n,k}^{j}+\zeta_{n}}, \nonumber \\
		%& \nonumber \\
		%	\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j},r_{k}^j).
		\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Delta_{n,k}^{j}).
		\end{align}
		%	Where the last step follows from the fact that  utility function used is $1-1$, so its derivative is also $1-1$ and its inverse $U_n^{'-1}(\alpha_k, \beta_{ik})$ can easily be computed.
		\item \textbf{$l \in \{\mathcal{M}\backslash\mathcal{M}_n\}$:} $\frac{\partial \mathcal{L}}{\partial x_{n,k}^{l}}=0$
		\begin{align}
		\label{eq:gradLagObjcase22}
		f^{'l}_n(x_{n,k}^{l})(\Delta_{n,k}^{l}+\zeta_{n})-(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})=0,\nonumber \\ 
		\implies  f^{'l}_n(x_{n,k}^{l})=\frac{(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})}{\Delta_{n,k}^{l}+\zeta_{n}}, \nonumber \\
		%& \nonumber \\
		\implies \quad x_{n,k}^{*l}= f_{n}^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Delta_{n,k}^{l}).
		\end{align}
	\end{enumerate}
	
	

	\begin{align}
\label{eq:gradLagObj2}
u_n^{'j}(x_{n,k}^{j})(1+\Lambda_{n,k}^{j}\zeta_{n})-\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})=0,\nonumber \\
\implies u_n^{'j}(x_{n,k}^{j})=\frac{\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Lambda_{n,k}^{j}\zeta_{n}}, \nonumber \\
%& \nonumber \\
\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j}).
\end{align}	
	\end{comment}
%		\begin{align}
%	\label{eq:gradLagObj2}
%	 u'_n(x_{ik}^{(n)})(1+\Lambda_{ik}^{(n)}\zeta^{(n)})-\Lambda_{ik}^{(n)}(\alpha_k^{(n)}+\beta_{ik}- \gamma_{ik}^{(n)})=0,\nonumber \\
%\implies u'_n(x_{ik}^{(n)})=\frac{\Lambda_{ik}^{(n)}(\alpha_k^{(n)}+\beta_{ik}-\gamma_{ik}^{(n)})}{1+\Lambda_{ik}^{(n)}\zeta^{(n)}}. % \nonumber \\
%& \nonumber \\
%\implies \quad x_{ik}^{*(n)}= U_n^{'-1}(\alpha_k^{(n)}, \beta_{ik}, \zeta^{(n)},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)})
%	\end{align}
%	\vspace{-0.12in}
\begin{comment}	
To simplify the proof, we only consider the case  in which $j \in \mathcal{M}_n$ below. The proof for the case when $i \in \mathcal{M}\backslash\mathcal{M}_n$ is similar. For illustrative purpose, we use $\bigg(1-e^{-{x_{n,k}^{j}}}\bigg)$ % $\ln(x_{n,k}^{j})$ 
as the utility. However, the results hold true for any concave injective utility function for which  inverse of the first derivative exists.  \eqref{eq:gradLagObj} is rewritten as:
%such as $\log (x_{ik}^{(n)})$ on $\mathbb{R}_{++}$, \eqref{eq:gradLagObj2} is rewritten as
\begin{align}\label{eq:priceLog}
e^{-{x_{n,k}^{j}}}&=\frac{(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{\Delta_{n,k}^{j}+\zeta_{n}},\nonumber \\
%e^{-{x_{n,k}^{j}}}&=\frac{r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})-(1+\Lambda_{n,k}^{j}\zeta_{n})}{r_k^j(1+\Lambda_{n,k}^{j}\zeta_{n})},\nonumber \\
\implies x_{n,k}^{j}&=\ln\bigg(\frac{\Delta_{n,k}^{j}+\zeta_{n}}{(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}\bigg).
%\implies x_{n,k}^{j}&=\ln\bigg(\frac{r_k^j(1+\Lambda_{n,k}^{j}\zeta_{n})}{r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})-(1+\Lambda_{n,k}^{j}\zeta_{n})}\bigg).
%\frac{1}{x_{ik}^{(n)}}=\frac{\alpha_k^{(n)}+\beta_{ik}}{1+\zeta^{(n)}} \implies {x_{ik}^{(n)}}= \frac{1+\zeta^{(n)}}{\alpha_k^{(n)}+\beta_{ik}}%{x_{ik}^{(n)}}=
\end{align} 
%We know that $\Lambda_{ik}^{(n)>0$, 
%For continuity, we need both the numerator and denominator inside the $\ln(\boldsymbol{.})$ function of \eqref{eq:priceLog} to be positive.  
At the optimal point, the numerator $(\Delta_{n,k}^{*j}+\zeta^*_{n})$ is positive as $\Delta_{n,k}^{*j}>0$ (from Section \ref{sec:assumption}) and $\zeta^*_{n}=0$ (from complementary slackness). %Hence, \eqref{eq:priceLog} can be rewritten as 
%\begin{align}\label{eq:priceLog2}
 %x_{n,k}^{*j}&=\ln\bigg(\frac{r_k^j}{r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}^*+\beta_{k}^{*j}- \gamma_{n,k}^{*j})-1}\bigg).
%\end{align} 
Similarly, $(\alpha^*_{n,k}+\beta_{k}^{*j}-\gamma_{n,k}^{*j})>0$, as  $\alpha_{n,k}^{*}>0$ (from Lemma \ref{lem:constraintsactive}) and  $\alpha_{n,k}^{*}+\beta_{k}^{*j}> \gamma_{n,k}^{*j}$ (from \emph{sensitivity analysis} \cite{boyd2004convex}). %Furthermore, the denominator $(r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}^*+\beta_{k}^{*j}- \gamma_{n,k}^{*j})-1>0)$ based on our assumptions in Section \ref{sec:assumption}.
Hence, the price based function in \eqref{eq:priceLog} is continuous in at least one optimal Lagrange multiplier vector. The proof follows from Theorem \ref{thm:georgesufficient}. 
\end{proof}
\end{comment}
For calculating $x_{n,k}^{j}$ at time $t$, we use $\Delta_{n}^{}$ calculated at $t-1$. 
Algorithm \ref{algo:primal-dual-alg} is a distributed algorithm that provides the global optimal solution to \eqref{eq:nashProbNplayermod}.
\paragraph{Protocol for Distributed Execution}
All ESPs first broadcast information regarding resource requests from their native applications. Then any randomly chosen ESP starts allocating resources as specified in Step $2$ of Algorithm \ref{algo:primal-dual-alg} and updates the corresponding Lagrangian multipliers. This ESP then  passes on the information about its allocation  and updated request matrix to the next ESP (that has not yet allocated resources in the current round\footnote{A single round consists of all the ESPs executing Step $2$ of Algorithm \ref{algo:primal-dual-alg} once.}) that repeats the  same procedure until all the ESPs allocate their resources.    This process continues until the first order conditions given in \cite{ktlagrangian} are met. 
%ESPs need to exchange information related to requests and  allocation decision. Al 
%\paragraph{Convergence Properties of the Algorithm}
%The convergence of our proposed algorithm depends on a number of factors such as the requests, capacities, and utilities used along with the step size for gradient descent. In particular, the step size must be carefully chosen as a very small step size can slow  the convergence rate, whereas a large step size will result in divergence. 

 
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $\forall\; \boldsymbol{\alpha_0,\; \beta_0,\zeta_0,\gamma_0,\pi_0}$, $C, R$, vector of utility function of all ESPs $\boldsymbol{u}$  and $\mathbf{X}_0$ %$\forall \boldsymbol{\nu_0$, $\mu_0}\in\mathcal{R}$ and $\boldsymbol h_0$ 
		\State \textbf{Output}: The optimal resource allocation $\mathbf{X} $ and payoffs of all ESPs
		\State \textbf{Step $0$:}  $t=0$, $\boldsymbol \alpha[t]\leftarrow\boldsymbol \alpha_0$, $\boldsymbol\beta[t]\leftarrow\boldsymbol\beta_0$, $\boldsymbol\zeta[t]\leftarrow\boldsymbol\zeta_0$, $\boldsymbol\gamma[t]\leftarrow\boldsymbol\gamma_0$,$\boldsymbol\pi[t]\leftarrow\boldsymbol\pi_0$$, \mathbf{X}[t]\leftarrow \mathbf{X}_0$
			\State \textbf{Step $1$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {d_n^0} \leftarrow$ \texttt{Objective function at optimal point in Equation \eqref{eq:opt_single}}
		\EndFor
		\State \textbf{Step 2: $t\geq 1$} 
		\While{{First order conditions\cite{ktlagrangian}$\neq$true }}%{Equation \eqref{eq:gradforLagrangieMultipliers} $\neq$ 0}
		\State Compute $ x_{n,k}^{j}[t+1]$ for $j\in\mathcal{M},$ $k\in\mathcal{K}$ and $n\in\mathcal{N}$ through \eqref{eq:gradLagObj22} and \eqref{eq:gradLagObjcase22};
		\State Compute $\boldsymbol\alpha[t+1]$, $\boldsymbol\beta[t+1]$, $\boldsymbol\zeta[t+1]$,  $\boldsymbol\gamma[t+1]$ and $\boldsymbol\pi[t+1]$ through~(\ref{eq:iterativeDual}) given $\mathbf{X}[t+1],$ $\boldsymbol\alpha[t]$,  $\boldsymbol \beta[t]$, $\boldsymbol \zeta[t]$,  $\boldsymbol\gamma[t]$ and $\boldsymbol\pi[t]$%for $l\in V,$ $i\in\mathcal{D}$ and $p\in\mathcal{P}^i$
		\EndWhile
	%	\State \textbf{Step 2:} $P_n^j\leftarrow$ \texttt{Payoff received by ESP} $\forall n \in \mathcal{{N}}, j \in \mathcal{{M}}$\texttt{ using \eqref{eq:payoffrule}} 
	\end{algorithmic}
	\caption{Distributed Algorithm for NBS}
	\label{algo:primal-dual-alg}
\end{algorithm}

 


==> arxiv version/preli.tex <==
\begin{comment}
In this section, we present an overview of  Multi-Objective Optimization (MOO), bargaining theory  and Nash Bargaining Solution (NBS). %\vspace{-0.1in}
\subsection{Multi-Objective Optimization}
 For $m$ inequality constraints and $p$ equality constraints, the MOO problem is to identify a vector $\boldsymbol{x}^*=[x_1^*,x_2^*,\cdots ,x_t^*]^T$ that maximizes a vector function
	\begin{equation}\label{eq:vectorobjective}
	\centering 
	\bar{f}(\boldsymbol{x})=[f_1(\boldsymbol{x}),f_2(\boldsymbol{x}),\cdots,f_N(\boldsymbol{x})]^T
	\end{equation}
	subject to 
	\begin{align}\label{eq:constraints}
	\centering 
	& g_i(\boldsymbol{x})\geq 0, \; i=1,2,\cdots,m, \\
	&h_i(\boldsymbol{x})=0\;\; i=1,2,\cdots,p, \nonumber
	\end{align}
	where $N$ is the total number of objectives,  $\boldsymbol{x}=[x_1,x_2,\cdots ,x_t]^T$ is a vector of $t$ decision variables and the feasible set is denoted by $F$.
The fundamental difference from  single objective optimization (SOO)  is that MOO involves a vector of objective functions rather than a single objective function. This indicates that the solution is not a single point but a \emph{frontier} of solutions known as \emph{Pareto frontier} or \emph{Pareto boundary} (see \cite{cho2017survey} for details). Some basic definitions related to MOO are: 
\begin{definition}{Strongly Pareto non-dominated solution\cite{cho2017survey}:}
%	\small
	A feasible solution $x$ is strongly Pareto non-dominated if there is no $y\in F$ such that $f_n(y)\geq f_n(x)$ $\forall n=1,2,\cdots,N$ and $f_n(y)>f_n(x)$ for at least one $n$\footnote{This means that there is no other feasible solution that can improve an objective without worsening at least one other objective.}.
\end{definition}
\begin{definition}{Weakly Pareto non-dominated solution\cite{cho2017survey}:}
%	\small
	A feasible solution $x$ is weakly Pareto non-dominated if there is no $y\in F$ such that $f_n(y)>f_n(x)$ $\forall n=1,2,\cdots,N.$
\end{definition}





\begin{definition}{Pareto Optimality\cite{cho2017survey}:}
	For any maximization problem,  $\boldsymbol{x}^*$ is $Pareto\; optimal$ if the following holds for every $\boldsymbol{x} \in F$
	\begin{align}\label{eq:paretoptimality}
	\bar{f}(\boldsymbol{x}^*)\geq\bar{f}(\boldsymbol{x}) 
	\end{align}
	where $\bar{f}(\boldsymbol{x})=[f_1(\boldsymbol{x}),f_2(\boldsymbol{x}),\cdots,f_k(\boldsymbol{x})]^T$ and  
	$\bar{f}(\boldsymbol{x}^*)=[f_1(\boldsymbol{x}^*),f_2(\boldsymbol{x}^*),\cdots,f_k(\boldsymbol{x}^*)]^T$.
\end{definition}

\subsection{Bargaining Theory}
%In any trade or sharing of resources among different entities, where the entities may have conflicting interests, reaching an agreement and deciding the terms of agreement is a challenge. 
In a \emph{bargaining situation}, two or more  players (service providers) can benefit by reaching an agreement. However,  players can have conflicting interests regarding the terms of the agreement. \emph{Bargaining theory} deals with studying such bargaining situations arising in a number of problems. In resource allocation  problem,  resource providers are interested in maximizing their utility (pay-off)  by satisfying the requests of different applications. 
%\par  The four main challenging issues surrounding bargaining theory are efficiency, selection of an outcome, coordination of strategies to obtain an outcome and the enforcement of agreement (see \cite{han2012game} for details). 
%\begin{enumerate}
%	\item \textbf{Efficiency:} A bargaining problem can have  a number of outcomes. Therefore, it is important to identify solutions that are beneficial for all players involved in the bargaining problem. 
%	\item \textbf{Distribution:} Once the solutions are identified, the next step is to select an outcome from the set of solutions. 
%	\item \textbf{Coordination of Strategy:} Following the selection of an outcome, the next step is to identify the joint strategy to obtain that solution. 
%	\item \textbf{ Enforcement of Agreement:}  The terms of agreement are identified for enforcing the chosen strategy. 
%\end{enumerate}
%Two important components of bargaining theory are the bargaining process and  bargaining outcome. Bargaining process deals with the procedure and steps a bargainer must take to reach an agreement over a chosen bargaining outcome. Bargaining outcome is obtained following the bargaining process. 
Below we discuss one of  the most widely used bargaining solutions, i.e., \emph{Nash Bargaining Solution} as it guarantees the Pareto optimality \cite{khan2009cooperative}. 
\end{comment}
%\subsection{Nash Bargaining Solution (NBS)}
%Nash, \cite{nash1950bargaining}, abstracted the bargaining process and only dealt with bargaining outcome using an axiomatic approach. 
We use a two-player game as a toy example to introduce NBS.  Consider two players $1,$ and  $2$ that need to reach an agreement (e.g., resource allocation decision) in an outcome space $\mathcal{A}\subseteq \mathbb{R}^2$ \cite{han2012game}. Both players have a utility given by $u_1$ and $u_2$ over the space $\mathcal{A} \cup \{D\}$ where $D$ specifies a \emph{disagreement outcome} for players in the event of a disagreement, i.e., when  two players cannot reach an agreement. Let $\mathcal{S}$ be the set of all possible utilities that both  players can achieve: %\vspace{-0.1in}

\begin{align}
\label{eq:possibleut}
\mathcal{S}= \{(u_1(a_1),u_2(a_2)) | (a_1,a_2) \in \mathcal{A} \}
\end{align}

We also define $d=(d_1, d_2)$, where $d_1=u_1(D)$ and $d_2=u_2(D)$, as the payoff each player receives at the disagreement point. We define the bargaining problem  as the pair $(\mathcal{S},d)$ where $\mathcal{S} \subset \mathbb{R}^2$ and $d \in \mathcal{S}$ such that 
\begin{itemize}
	\item $\mathcal{S}$ is a convex and compact set;
	\item There exists $s \in \mathcal{S}$ such that $s > d$.
\end{itemize}
In NBS, the goal is to obtain a function $f(\mathcal{S},d)$ that provides  a unique outcome in $ \mathcal{S}$ for every bargaining problem $(\mathcal{S},d)$. Nash studied the possible outcomes (agreements) that players can reach whereas the agreements, along with the Pareto optimality, must also  satisfy the following set of  axioms (also called \emph{fairness} axioms) \cite{han2012game}:
\begin{enumerate}
%	\item \textbf{Pareto Optimality}
	\item \textbf{Symmetry:}  The bargaining solution will not discriminate among  players if players are indistinguishable, i.e., players have identical utilities. 
	\item \textbf{Invariance to equivalent utility representation:} If a bargaining problem  $(\mathcal{S},d)$ is transformed into another bargaining problem  $(\mathcal{S}',d')$ where $s_i'=\gamma_is_i+\zeta_i$ and $d_i'=\gamma_id_i+\zeta_i$, $\gamma_i >0$, then $f( \mathcal{S}',d')=\gamma_if(\mathcal{S},d)+\zeta_i$
	\item \textbf{Independence of irrelevant alternatives:} For any two bargaining problems  $(\mathcal{S},d)$ and  $(\mathcal{S}',d)$ where $\mathcal{S}'\subseteq \mathcal{S}$, if $f(\mathcal{S},d) \in \mathcal{S}'$, then $f(\mathcal{S}',d)=f(\mathcal{S},d)$. %This means that if any bargaining problem in any region $\mathcal{S}$ results in an outcome $f(\mathcal{S},d)$, which lies in $\mathcal{S}'\subseteq \mathcal{S}$, then any hypothetical bargaining problem in $\mathcal{S}'$ will also result in the same solution. 
\end{enumerate}
\cite{nash1950bargaining} shows that there is a unique bargaining solution that satisfies above axioms. We present it in the following theorem. 
\begin{theorem}{\cite{han2012game}}
	There exists a unique solution satisfying the aforementioned axioms and this solution is the pair of utilities $(s_1^*,s_2^*) \in \mathcal{S}$ that solves the following optimization problem:
	\begin{align}
	\label{eq:nashProb}
	\max_{s_1,s_2}\;(s_1-d_1)(s_2-d_2),\; s.t. (s_1,s_2)\in \mathcal{S}, \; (s_1,s_2)\geq (d_1,d_2).
	\end{align}\
\end{theorem}
The solution of \eqref{eq:nashProb} is the NBS. % Nash in \cite{nash1950bargaining} derived the NBS for only two players. However, it has been extended to 
The above framework can be extended to $N$ players  by allowing $\mathcal{S}$ to be an $N$-dimensional space \cite{harsanyi1963simplified}. For this case, the bargaining problem $(\mathcal{S},d)$, with $d=(d_1,d_2,\cdots, d_N)$ as the disagreement point, becomes the unique solution of the optimization problem below.
%\vspace{-0.1in}
	\begin{align}\vspace{-0.1in}
\label{eq:nashProbNplayer}
\max_{s_1,\cdots,s_N}&\;\prod_{n=1}^{N}(s_n-d_n),\; \nonumber \\
s.t.\quad  &(s_1,\cdots,s_N)\in \mathcal{S}, \nonumber \\
& (s_1,\cdots,s_N)\geq (d_1,\cdots, d_N).
\end{align}
Solving \eqref{eq:nashProb} is easier compared to the $N-$player bargaining problem in \eqref{eq:nashProbNplayer}\cite{han2012game}. %Different optimization techniques such as the bisection method can be used to obtain the NBS for an $N-$player bargaining problem. 
In this paper, we transform our problem into an equivalent convex problem that is comparatively easier to solve.  
 
\begin{remark}
  As each player in an  $N$-player bargaining game has a particular objective to optimize, the resulting problem is multi-objective,  where the goal is to obtain a Pareto optimal solution. NBS is a fair and Pareto optimal solution for such MOO problems, provided that the fairness axioms are satisfied.  % as it takes the objective of every game player into account. 
\end{remark}%\vspace{-0.25in}

\begin{comment}
\subsection{Cooperative Game Theory}
Cooperative game theory is the set of analytical tools that assists in understanding the behavior of rational players in a cooperative setting \cite{han2012game}. Players can have agreements among themselves that affects the strategies as well as obtained utilities of the players. Cooperative games are primarily of two types: bargaining theory and coalition games. Bargaining theory deals with the bargaining process that arise among the players while joining an agreement while coalition games deals with the formation of the coalitions among cooperating players. Formally

\begin{definition}{Coalition Games \cite{han2012game}:}
Any coalition game can be represented by the pair $(\mathcal{N},v)$ where $\mathcal{N}$ is the set of players that play the game, while $v$ is the mapping function that determines the utilities or payoffs the players in $\mathcal{N}$ receive. 
\end{definition}

\begin{definition}{Characteristic form Coalition Games: \cite{han2012game}:}
	Any coalition game is said to be of \emph{characteristic} form where the value of coalition $S \subseteq \mathcal{N}$ depends only on the members of coalition. 
\end{definition}

\begin{definition}{Transferable Utility (TU):}
If the total utility of any coalition can be divided in any manner among the game players, then the game has a \emph{transferable} utility. 
\end{definition}

\begin{definition}{Characteristic function:}
The characteristic function for any coalitional game with TU is a mapping $v: 2^{\mathcal{N}} \mapsto \mathbb{R}$ with $v(\emptyset)=0$
\end{definition}

\begin{definition}{Superadditivity of TU games:}
A canonical game with TU is said to be superadditive if the following property is satisfied. 
\begin{equation}\label{eq:superadditivity}
v(S_1 \cup S_2 )\geq v(S_1)+V(S_2) \; \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, s.t. S_1\cap S_2 =\emptyset
\end{equation}
i.e., formation of large coalitions is always desired and the players do not lose any utility by joining the coalition. 
\end{definition}

\subsubsection{Canonical Game}
A coalition game is canonical if 
\begin{itemize}
	\item It is in characteristic form
	\item It is superadditive
\end{itemize}
The \emph{core} and Shapley value are widely used concepts for dealing with Canonical games as discussed below. 
\subsection{Core}
Before we present details of core, we first define some terms \cite{han2012game}

\begin{definition}[Group Rational]
	A payoff vector $\textbf{x}\in \mathbb{R}^\mathcal{N}$ for dividing $v(\mathcal{N})$ is group-rational if $\sum_{n \in \mathcal{N}}x_n=v(\mathcal{N})$.
\end{definition}

\begin{definition}[Individual Rational]
	A payoff vector $\textbf{x}\in \mathbb{R}^\mathcal{N}$ is individually-rational if every player can obtain a benefit no less than acting alone, i.e., $x_n \geq v(\{n\}), \forall n\in \mathcal{N}$.
\end{definition}

\begin{definition}[Imputation]
	A payoff vector that is both individual and group rational is known as an imputation. 
\end{definition}


Based on the above definitions, we can now define the core of a TU canonical coalition game

\begin{definition}[Core]
	For any TU canonical game $(\mathcal{N},v)$, the core is the set of imputations in which no coalition $S\subset\mathcal{N}$ has any incentive to reject the proposed payoff allocation and deviate from the grand coalition to form a coalition $S$ instead. This can be mathematically expressed as 
	\begin{align}\label{eq:coreTU}
	\mathcal{C}_{TU}=\bigg \{ \mathbf{x}: \sum_{n \in \mathcal{N}}x_n=v(\mathcal{N}) \; and \; \sum_{i \in S} x_i \geq v(S)\; \forall\; S\subseteq \mathcal{N}\bigg\}
	\end{align}
\end{definition}
\begin{remark}
	Any payoff allocation from the core is Pareto-optimal as evident from definition of the core. Furthermore, the grand coalition formed is stable
\end{remark}
However, the core is not always guaranteed to exist. Even if the core exists, it might be too large so finding a suitable allocation from the core is not easy. Furthermore, as seen from the definition, the allocation from the core might not always be fair to all the players. 
\subsection{Shapley Value}
 %Now that we have the answer to the question about non-emptiness of the core, we divert our attention to the selection of any pay-off allocation from the core. As evident, the core for our problem is quite large. Therefore, selecting a suitable core allocation can be difficult \cite{han2012game}. 
 \emph{Shapley value} \cite{shapley1988value} can be used to address the aforementioned  shortcomings of the core. For the characteristic function $v$ (the characteristic function is also called the game \cite{han2012game}), Shapley proposed an allocation $\phi_n(v)$ that satisfies the following axioms \cite{la2004game}:
 \begin{enumerate}
 	\item \emph{Efficiency Axiom}: $\sum_{n \in \mathcal{N}}\phi_n(v)=v(\mathcal{N})$. This axiom in essence is the group rationality.
 	\item \emph{Symmetry Axiom}: If any two players $m$ and $n$ are such that $v(S \cup \{n\})=v(S \cup \{m\})$, then for every coalition $S\backslash(m,n)$, $\phi_n(v)=\phi_m(v)$. This axiom indicates that if any two players/domains have similar contributions in a coalition then their assigned payoffs must be same as well.
 	\item \emph{Dummy Axion}: If any player $n$ is such that $v(S)=v(S \cup \{n\})$, then for every coalition $S\backslash n$, $\phi_n (v)=0$. Dummy axiom indicates that players that do not contribute to the value of coalition will not get any payoff. 
 	\item \emph{Additivity Axion}: If $j$ and $k$ are any two games, then $\phi(j+k)=\phi(j)+\phi(k)$. This axiom indicates that $\phi$ is a unique mapping over the space of the coalitional games.
 \end{enumerate}
 Based on the above axioms, Shapley  showed that there exists a unique function $\phi$ defined on all games that satisfies the aforementioned axioms \cite{la2004game}. The function is given by
 
 \begin{equation}\label{eq:shapleyvalue}
 \phi_n(v)=\sum_{S\subseteq \mathcal{N}\backslash n}\frac{|S|! (|\mathcal{N}|-|S|-1)!}{|\mathcal{N}|!}\bigg[ v(S \cup \{n\}) -v(S) \bigg]
 \end{equation} 
\end{comment}

==> arxiv version/proof1.tex <==
\begin{proof}
	We show that the price function obtained by $\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma})}{\partial x_{n,k}^{j}}=0$ is continuous at one or more of the optimal Lagrange multipliers for \eqref{eq:lagrangian}. 
	
	Let both $u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j,\zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j})$ and $f_n^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Lambda_{n,k}^{l})$ are  %and $u_{jn}^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)})$ are
	the inverses of the first derivative of $u_{n}^j$ and $(u_{n}^l(x_{n,k}^l)-C_n^l(x_{n,k}^l))$, respectively. %and $u_j^n$ respectively. 
	$\alpha_{n,k}$,  $\beta_{k}^j$, $\zeta_{n}$, and $\gamma_{n,k}^{j}$ are the \emph{Lagrange} multipliers whereas   $\Delta_{n,k}^{j}=\bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j+{x}_{n,k}^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^l+{x}_{n,k}^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg)$. There are two different cases that we evaluate in the following: %To simplify the proof, we only consider the case  in which $i \in \mathcal{M}_n$ below. The proof for the case when $i \in \mathcal{M}\backslash\mathcal{M}_n$ is similar. 
	\begin{enumerate}
	\item \textbf{$j \in \mathcal{M}_n$:}$\frac{\partial \mathcal{L}}{\partial x_{n,k}^{j}}=0$
	\begin{align}
	\label{eq:gradLagObj22}
%	\frac{u_n^{'j}(\mathbf{x}_n^j+\sum_{t\in \mathcal{{N}}\backslash n}\mathbf{x}_t^j)+\sum_{t \in \mathcal{{N}}\backslash n}}{\Delta_{n,k}^j}, \nonumber \\
	%	 \Big(u_n^{'j}(x_{n,k}^{j})+\frac{1}{r_{k}^j}\Big)(1+\Lambda_{n,k}^{j}\zeta_{n})-\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j-\nonumber \\
	%	 \gamma_{n,k}^{j})=0,\nonumber \\
	&u_n^{'j}(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j+x_{n,k}^{j})(1+\Delta_{n,k}^{j}\zeta_{n})-\Delta_{n,k}^{j}(\alpha_{n,k}+\nonumber \\
	&\beta_{k}^j-\gamma_{n,k}^{j})=0,\nonumber \\	
	%	 \implies u_n^{'j}(x_{n,k}^{j})=\frac{\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Lambda_{n,k}^{j}\zeta_{n}}-\frac{1}{r_{k}^j}, \nonumber \\
	& u_n^{'j}(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j+x_{n,k}^{j})=\frac{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n,k}^{j}\zeta_{n}}, \nonumber \\
	%& \nonumber \\
	%	\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j},r_{k}^j).
%	&\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Delta_{n,k}^{j}).
	\end{align}
For sake of the proof, we set  $u_j^n=1-e^{-(x_{n,k}^j+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j+-r_{n,k}^j+\delta t)}$ where $\bar{r}_{n,k}^j=r_{n,k}^j+\delta t$. However, the theory hold for any concave injective utility function for which the inverse of the first derivative exists.  Then \eqref{eq:gradLagObj22} becomes:
	\begin{align}\label{eq:proof1}
	& e^{-(x_{n,k}^j+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}= \frac{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n,k}^{j}\zeta_{n}},\hspace{0.2in} \nonumber \\
		e^{x_{n,k}^j}&= \frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}},\nonumber \\
		x_{n,k}^j&=\ln\bigg(\frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}}\bigg).
	\end{align} 
%We know that $\Lambda_{ik}^{(n)>0$, 
	 For continuity, we need both the numerator and denominator inside the $\ln(\boldsymbol{.})$ function of \eqref{eq:proof1} to be positive.  
At the optimal point, the numerator $(1+\Delta_{n,k}^{*j}\zeta^*_{n})$ is positive as $\Delta_{n,k}^{*j}>0$ (from Section \ref{sec:assumption}) and $\zeta^*_{n}=0$ (from complementary slackness).	Similarly, in the denominator, $\Delta_{n,k}^j$ (from Section \ref{sec:assumption}) and $e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}$ are positive. $(\alpha^*_{n,k}+\beta_{k}^{*j}-\gamma_{n,k}^{*j})>0$, as  $\alpha_{n,k}^{*}>0$ (from Lemma \ref{lem:constraintsactive}) and  $\alpha_{n,k}^{*}+\beta_{k}^{*j}> \gamma_{n,k}^{*j}$ (from \emph{sensitivity analysis} \cite{boyd2004convex}). %Furthermore, the denominator $(r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}^*+\beta_{k}^{*j}- \gamma_{n,k}^{*j})-1>0)$ based on our assumptions in Section \ref{sec:assumption}.
Hence, the price based function in \eqref{eq:proof1} is continuous in at least one optimal Lagrange multiplier vector. The proof follows from Theorem \ref{thm:georgesufficient}. 
	
	
	%	Where the last step follows from the fact that  utility function used is $1-1$, so its derivative is also $1-1$ and its inverse $U_n^{'-1}(\alpha_k, \beta_{ik})$ can easily be computed.
	\item \textbf{$l \in \{\mathcal{M}\backslash\mathcal{M}_n\}$:} $\frac{\partial \mathcal{L}}{\partial x_{n,k}^{l}}=0$
	\begin{align}
	\label{eq:gradLagObjcase22}
	f^{'l}_n(x_{n,k}^{l})(1+\Delta_{n,k}^{l}\zeta_{n})-\Delta_{n,k}^{l}(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})=0,\nonumber \\ 
	\implies  f^{'l}_n(x_{n,k}^{l})=\frac{(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})}{1+\Delta_{n,k}^{l}\zeta_{n}}, \nonumber \\
	%& \nonumber \\
	\implies \quad x_{n,k}^{*l}= f_{n}^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Delta_{n,k}^{l}).
	\end{align}
\end{enumerate}


\end{proof}

==> arxiv version/related.tex <==
\subsection{Resource allocation in Edge Computing}
Jiao et al. \cite{jiao2018social} propose an auction-based resource allocation scheme for edge service providers that provide resources for blockchains. The proposed mechanism maximizes the social welfare and guarantees truthfulness, computational efficiency and individual rationality. He et al. \cite{he2018s} analyze the optimal provisioning of shareable and non-shareable edge resources to different applications.    %It is shown that the problem is NP-hard in general and they  propose a constant factor algorithm as well as different heuristics. 
Plachy et al. \cite{plachy2016dynamic} consider the mobility problem in mobile edge clouds and propose a novel algorithm for  selecting communication path and VM placement. The proposed approach relies on predicting user movement that helps in VM placement and accordingly selecting the communication path. Nishio et al. \cite{nishio2013service} propose a resource sharing architecture for mobile clouds that relies on service-oriented utility functions and is closest to our work. However, they primarily consider service latency and rely on a centralized framework whereas we present a distributed framework that requires a specific utility function that can be used to model different metrics such as latency, delay, and numerous other objectives. In \cite{zafari2020let}, we modeled resource sharing among mobile edge clouds as a cooperative game. However, the MOO problem in \cite{zafari2020let} is non-convex  that is hard to solve compared to the convex problem solved here. Furthermore, the cooperative game based framework lacks the fairness guaranteed by NBS. % and is closest to our work. 
 Furthermore, in contrast with \cite{jiao2018social,plachy2016dynamic} and \cite{he2018s} that primarily consider resource allocation, our proposed framework deals with resource sharing among ESPs with different objectives. 

\subsection{NBS based Resource Allocation}
Yaiche et al. \cite{yaiche2000game} use NBS to allocate bandwidth for elastic services in  high speed networks. 
Xu et al. \cite{xu2012general} consider the fairness criteria when allocating resources to different cloud users and make use of the  NBS to guarantee fairness. Using dual composition and sub-gradient method, the authors also develop a distributed algorithm. Hassan et al.  \cite{hassan2014virtual} propose an NBS-based model for cost-effective and dynamic VM allocation with multimedia traffic, and show that it can reduce the cost of running different servers along with maximizing resource utilization and satisfying the QoS requirements. He et al. \cite{he2013toward}   study the optimal deployment of content in a cloud assisted video distribution system. 
Feng et al. \cite{feng2012bargaining} use NBS  for Virtual Machine (VM) migration to maximize the resource utilization in a video streaming data center. 
\par 
In contrast with  \cite{yaiche2000game, feng2012bargaining, guo2013cooperative,he2013toward,hassan2014virtual},  to the best of our knowledge, our  framework is first of its kind that uses NBS for  resource sharing among ESPs  with different utilities (objective functions). We show that resource sharing can improve  utilities  of ESPs and enhance application satisfaction. 
Furthermore, for a particular class of utilities, we have proved that distributed algorithm exists for obtaining NBS for the resource sharing and allocation problem. Table \ref{tab:comparison} summarizes some other solutions proposed in the literature  that use NBS for resource allocation in different systems.   Other distributed algorithms proposed in literature either rely on dual decomposition \cite{xu2012general} or gradient projection \cite{yaiche2000game,guo2013cooperative}. However, most of the functions are not dual decomposable and gradient projection is a computationally expensive approach \cite{bertsekas1997nonlinear}, whereas gradient descent is widely used particularly  in machine and deep learning.   
 












==> game-theory.tex <==
%\subsection{Game Theoretic Solution}
We first define the characteristic function $v$ for our game that can solve  problem in~\eqref{eq:opt_higher} 

\begin{figure*}[!t]
	\normalsize
\begin{align} \label{eq:payoff_function}
v(\mathcal{N})=\sum_{\substack{\text{$n \in \mathcal{N}$},\;\text{$C_{k}= \sum_{n \in \mathcal{N}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in \mathcal{N}$}\\ \text{$\sum_{j \in \mathcal{N}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in \mathcal{N}$}}}\bigg(w_n u_n(\mathcal{X})+ \zeta_{n}\sum_{j \in \mathcal{N},j\neq n} u^{n}_j(\mathcal{X})\bigg)
\end{align}
	\hrulefill
	\vspace*{-4pt}
\end{figure*}



\begin{remark}
	The characteristic function in Equation~\eqref{eq:payoff_function} is for the grand coalition $\mathcal{N}$. For any $S \subseteq \mathcal{N}$, the characteristic function will be given by Equation~\eqref{eq:payoff_s_function}
\end{remark}


\begin{figure*}[!t]
	\normalsize
\begin{align} \label{eq:payoff_s_function}
v({S})=\sum_{\substack{\text{$n \in {S}$},\; \text{$C_{k}= \sum_{n \in {S}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {S}$}\\ \text{$\sum_{j \in {S}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \; \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S}$}}} \bigg(w_n u_n(\mathcal{X})+\zeta_{n}\sum_{j \in S,j\neq n} u^{n}_j(\mathcal{X})\bigg)
\end{align}
\hrulefill
\vspace*{-4pt}
\end{figure*}


\begin{theorem}
%	A Cooperative game $(\mathcal{N}, v)$ of $\mathcal{N}$ players and $v$ payoff function that can be used to solve the multi-objective optimization problem given in \eqref{eq:opt_higher}, is canonical\footnote{for monotonically non-decreasing utilities/pay-off function} with Transferable utility
Resource allocation and sharing problem (with multiple objectives) in aforementioned settings can be modeled as a canonical cooperative game with TU. 
\end{theorem}
\begin{proof}
To prove this, we need to show that the characteristic function of resource sharing and allocation problem satisfies the following two conditions
%	For a game to be canonical, we need to prove that the game  is superadditive and the payoff function is of characteristic form. 
	\begin{itemize}
		\item \textbf{Characteristic form of payoff:} As the utility function in a resource sharing and allocation problem  only relies on the domains that are part of the coalition, the game or payoff function is of characteristic form
		\item \textbf{Superadditivity:} Super-additivity for TU games requires $v(S_1 \cup S_2 )\geq v(S_1)+V(S_2) \; \forall S_1 \subset \mathcal{N}, S_2 \subset \mathcal{N}, s.t. S_1\cap S_2 =\emptyset$ i.e. we have to prove that the pay-off or utility for a domain in the coalition is as good as domain working alone or in a smaller coalition. Due to monotonicity property of the utility functions used,  for all  players/domains $n \in \mathcal{N}$,  $u_n(X_n^{NC})\leq u_n(X_n^{C})$ as $X_n^{NC}\subset {X_n^{C}}$ \footnote{because $X_n^{C}$ can contain much more elements due to the increase in $C$ in the coalition} where $X_n^{C}$ and $X_n^{NC}$ are the allocation decisions in  a cooperative game  and independent setting respectively for domain $n$. 
	\end{itemize}
\end{proof}
\begin{lemma}\label{lemma:MOOGame}
A canonical cooperative game $(\mathcal{N}, v)$ with TU can be used to obtain the Pareto-optimal solutions for the multi-objective optimization problem given in \eqref{eq:opt_higher}
\end{lemma}

%Given that the game is canonical, we are going to explore potential solution approaches for such a game. We start with the \emph{Core} \cite{han2012game}. 

To prove Lemma \ref{lemma:MOOGame}, we must show that the core is non-empty for  our canonical game. To do this, we first show that our game is convex. 

\begin{definition}[Convex Games]
	A coalition game is said to be convex if and only if for every player $n \in \mathcal{N}$, the marginal contribution of the player is non-decreasing W.R.T set inclusion. Mathematically, for $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash \{n\}$ 
	\begin{equation}\label{eq:convexgames}
	v(S_1 \cup \{n\})-v(S_1) \leq v(S_2 \cup \{n\})-v(S_2)
	\end{equation} 
\end{definition}
\begin{theorem}
	Our canonical game is convex
\end{theorem}
\begin{proof}
Let us consider two coalition $S_1$ and $S_2$, where $S_1\subseteq S_2 \subseteq \mathcal{N}\backslash\{j\}$ where $j \in \mathcal{N}$. Then we first calculate $v(S_2 \cup \{j\})-v(S_1 \cup \{j\})$ in Equation \eqref{eq:convexityProof}. 

\begin{figure*}[!t]
	\normalsize
\begin{align}\label{eq:convexityProof}
& \sum_{\substack{\text{$n \in {S_2}$},\; \text{$C_{k}= \sum_{n \in {S_2}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}$}\\ \text{$\sum_{j \in {S_2}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {S_2}, k\neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) - \nonumber \\
& \Bigg(\sum_{\substack{\text{$n \in {S_1}$},\; \text{$C_{k}= \sum_{n \in {S_1}}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {S_1}$} \\ \text{$\sum_{j \in {S_1}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_1}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {S_1}, k \neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_1)}(\mathcal{X}) + \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\nonumber \Bigg)\\ 
&= \sum_{\substack{\text{$n \in {S_2}\backslash S_1$}, \text{$C_{k}= \sum_{n \in {S_2}\backslash S_1}C_{k}^{(n)} $} \\ \text{$\sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}\backslash S_1$} \\ \text{$\sum_{j \in {S_2 \backslash S_1}}x_{ik}^{(j)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2 \backslash S_1}$}}}\bigg(w_n u_n(\mathcal{X})+ w'_{n}\sum_{k \in {\{S_2 \backslash S_1\}}, k \neq n} u^{j}_k(\mathcal{X})\bigg) + w_j u_j ^{(S_2)}(\mathcal{X}) \nonumber \\
&   + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) - w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X}) \nonumber \\
& = v(S_2)- v(S_1)+ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})  \nonumber \\
& \geq v(S_2)- v(S_1)
\end{align}
	% Restore the current equation number.
	%%\setcounter{equation}{\value{MYtempeqncnt}}
	% The IEEE uses as a separator
	\hrulefill
	% The spacer can be tweaked to stop underfull vboxes.
	\vspace*{4pt}
\end{figure*}

\begin{comment}
	\begin{align}\label{eq:convexityProof}
	& \sum_{\substack{\text{$n \in {S_2}$} \\ \text{$R_{av,k}= \sum_{n \in {S_2}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}$}\\ \text{$\sum_{j \in {S_2}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2}$}}}\bigg(w_n u_n(\mathcal{A})+ w'_{n}\sum_{k \in {S_2}, k\neq n} u^{j}_k(\mathcal{A})\bigg) + w_j u_j ^{(S_2)}(\mathcal{A}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{A}) - \nonumber \\
	& \Bigg(\sum_{\substack{\text{$n \in {S_1}$} \\ \text{$R_{av,k}= \sum_{n \in {S_1}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {S_1}$} \\ \text{$\sum_{j \in {S_1}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_1}$}}}\bigg(w_n u_n(\mathcal{A})+ w'_{n}\sum_{k \in {S_1}, k \neq n} u^{j}_k(\mathcal{A})\bigg) + w_j u_j ^{(S_1)}(\mathcal{A}) + \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{A})\nonumber \Bigg)\\ 
	&= \sum_{\substack{\text{$n \in {S_2}\backslash S_1$} \\ \text{$R_{av,k}= \sum_{n \in {S_2}\backslash S_1}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K},\; \forall n \in {S_2}\backslash S_1$} \\ \text{$\sum_{j \in {S_2 \backslash S_1}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \quad \forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in {S_2 \backslash S_1}$}}}\bigg(w_n u_n(\mathcal{A})+ w'_{n}\sum_{k \in {\{S_2 \backslash S_1\}}, k \neq n} u^{j}_k(\mathcal{A})\bigg) + w_j u_j ^{(S_2)}(\mathcal{A}) \nonumber \\
	&   + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{A}) - w_j u_j ^{(S_1)}(\mathcal{A}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{A}) \nonumber \\
	& = v(S_2)- v(S_1)+ w_j u_j ^{(S_2)}(\mathcal{A}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{A}) -  w_j u_j ^{(S_1)}(\mathcal{A}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{A})  \nonumber \\
	& \geq v(S_2)- v(S_1)
	\end{align}
	\end{comment}

The last inequality in Equation \eqref{eq:convexityProof} follows from the fact that $ w_j u_j ^{(S_2)}(\mathcal{X}) + \zeta_j\sum_{l \in S_2, l \neq j} u^{j}_{l}(\mathcal{X}) -  w_j u_j ^{(S_1)}(\mathcal{X}) - \zeta_j\sum_{l \in S_1, l \neq j} u^{j}_{l}(\mathcal{X})\geq 0$ (monotonicity of the utility)
\end{proof}


%Related to the core, there are certain questions that we must answer
\begin{comment}
\begin{enumerate}
	\item Is the core non-empty?
	\item If the core is non-empty and consists of different pay-off allocations, how do we choose any particular pay-off allocation vector? 
\end{enumerate}
Below we attempt to answer these questions



\begin{definition}[Balanced Collection] Let $\Omega$ be a collection of different coalitions. $\Omega$ is considered to be a \emph{balanced collection} if we can find non-negative weights $w_S$ for each $S \in \Omega$ such that for every player $n$ 
	\begin{align}\label{eq:balancedcollection}
	\sum_{S \in \Omega, S \ni n}w_S =1 
	\end{align}
\end{definition}

\begin{definition}[Balanced Game] A game is called balanced if for every balanced collection $\Omega$, the payoff vector $\mathbf{x}$ will be in $V_{\mathcal{N}}$ if $\mathbf{x}_S \in V_S\; \forall S \in \Omega$ 
	%Let $\Omega$ be a collection of different coalitions. $\Omega$ is considered to be a \emph{balanced collection} if we can find non-negative weights $w_S$ for each $S \in \Omega$ such that for every player $n$ 
\end{definition}
\begin{theorem}[Bondareva-Shapley Theorem]\label{thm:BST}
	The core of a game is non-empty if and only if the game is balanced
\end{theorem}


\begin{theorem}
The core for canonical game with our characteristic function(in Equation~\eqref{eq:payoff_function}) is non-empty
\end{theorem}

\begin{proof}
From the definition of characteristic functions for TU games (see \cite{han2012game} for details), $v: 2^{\mathcal{N}}$ \textrightarrow $\mathbb{R}$ with $v(\emptyset)=\emptyset$. This means that the total number of coalitions possible for $\mathcal{N}$ players is $2^{|\mathcal{N}|}-1$ (we ignore the empty set). For $\Omega$, the non-negative weights $w_S$ which satisfy the condition for  balanced collection in Equation~\eqref{eq:balancedcollection} are given by $\frac{1}{2^{|\mathcal{N}|-1}}$. Hence $\Omega$ is a balanced collection. We also know that $v(S)\subseteq v(\mathcal{N})$ as $v(\mathcal{N})$ is defined over a larger feasible set due to increased amount of available resources. Leveraging the monotonicity property of the utility functions used, we know that any payoff vector  $\mathbf{x}$ will be in $V_{\mathcal{N}}$ if $\mathbf{x}_S$\footnote{$\mathbf{x}_S$ is the projection of $\mathbf{x}$ onto the vector space $\mathbb{R}^{|S|}$} $\in V_S\; \forall S \in \Omega$. Hence our canonical game with characteristic function $v$ in Equation~\eqref{eq:payoff_function} is balanced and its core is non-empty (from Theorem \ref{thm:BST})

\end{proof}
\end{comment}


%For our problem, does the Shapley value lie in the core? To do so we first define \emph{convex games}

\begin{theorem}
	The core of any convex game $(\mathcal{N},v)$ is non-empty and large. 
\end{theorem}
\begin{proof}
	Available in \cite{sharkey1982cooperative}
\end{proof}
While the existence of core i.e., core being non-empty, guarantees the grand coalition is stable, finding a suitable allocation from the core is challenging particularly when the core is large (our game). Furthermore, as mentioned earlier, fairness is also a shortcoming of core based solutions.  Shapley value can be  used to obtain a fair allocation, however, we first need to show that the Shapley value lies in the core to guarantee that the Shapley value based allocation is stable for the grand coalition. 
\begin{theorem}
	The Shapley value in Equation~\eqref{eq:shapleyvalue} lies in the core of our canonical game
\end{theorem}
\begin{proof}
	Since our canonical game is convex, the Shapley value lies in the core \cite{han2012game} (see \cite{roger1991game} for details)
\end{proof}
We summarize this in the remark below. 
\begin{remark}
If a TU game $(\mathcal{N}, v)$ is convex, then the core is non-empty and the Shapley Value lies in the core \cite{garg2013novel}.	
\end{remark}
Calculation of Shapley value given in Equation~\eqref{eq:shapleyvalue} is challenging \cite{han2012game}. Since our game is convex, calculating its Shapley value is slightly easier as given below. 

%Now that we have proved that the game is convex, we divert our attention to the calculation of Shapley value for a convex game. 


\subsubsection{Shapley Value for a Convex Game}
Let $\pi$ denote the permutation of players in our game.  Then for any permutation $p$ from the total possible permutations $|\mathcal{N}|!$, one can obtain the initial segments of ordering by \cite{garg2013novel}
\begin{equation}\label{eq:initialsegment}
O_{\pi, r}=\{ n \in \mathcal{N} : \pi(n) \leq r \}, \; r \in \{1, \cdots, N\}
\end{equation}
where $O_{\pi, 0}=\{\}$ and $O_{\pi, |\mathcal{N}|} =\mathcal{N}$. $\pi(n)$ refers to the position of the player $n$ in the permutation $\pi$. The core of any particular ordering $\pi$ can be obtained by solving  equations
\begin{equation}
\label{eq:x_i_pi_sol}
x_n^{\pi}(O_{\pi, r}) = v(O_{\pi, r}), \; r \in \{ 1, \cdots, N\}
\end{equation}
The solution to  above Equations~\eqref{eq:x_i_pi_sol} will result in a payoff vector $x^{\pi}$ where the elements of the vector are given by 
\begin{equation}
\label{eq:vectorelements}
x_n^{\pi}=v(O_{\pi, \pi(n)})- v(O_{\pi, \pi(n)-1}), \quad \forall n \in \mathcal{N} 
\end{equation}
The payoff vectors $x^{\pi}$ represent the extreme points of the core in convex games \cite{garg2013novel}. So if $\prod$ represents the set of all possible permutations of $\mathcal{N}$, the Shapley value of any player $n$ can be calculated as 
\begin{equation}
\label{eq:shapleyconvex}
\phi_n=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} x_n^{\pi}
\end{equation}
\begin{comment}
So for our coalition game $(\mathcal{N},v)$, the Shapley value is 
\begin{align}
\label{eq:ourshapleyconvex}
\phi_n&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} \bigg( \sum_{\substack{\text{$n \in {O_{\pi, \pi(n)}}$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)}}$} \\ \text{$$}\text{$\sum_{j \in {O_{\pi, \pi(n)}}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in O_{\pi, \pi(n)}$}}}\bigg(w_n u_n^{(\pi)}(\mathcal{A})+ w'_{n}\sum_{j \in {O_{\pi, \pi(n)}}, j \neq  n} u^{n,(\pi)}_j(\mathcal{A})\bigg)- \nonumber \\
&\Bigg(\sum_{\substack{\text{$n \in {O_{\pi, \pi(n)-1}}$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)-1}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \; \forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)-1}}$}}}\bigg(w_n u^{(\pi)}_n(\mathcal{A})+ w'_{n}\sum_{j \in {O_{\pi, \pi(n)-1}}, j \neq n} u^{n,(\pi)}_j(\mathcal{A})\bigg)\Bigg) \nonumber \\
&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod} \bigg( \sum_{\substack{\text{$n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1} }$} \\ \text{$R_{av,k}= \sum_{n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}}R_{av,k}^{(n)} $} \\ \text{$\sum_{i} a_{ik}^{(n)}\leq R_{av,k}^{(n)} \;\forall k \in \mathcal{K}, \; \forall n \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}$} \\ \text{$\sum_{j \in {O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}}}a_{ik}^{(j)} \leq R^{(n)}_{req,ik} \;\forall\; i\in \mathcal{M}, k \in \mathcal{K}, n \in O_{\pi, \pi(n)}\backslash O_{\pi, \pi(n)-1}$} }}\bigg(w_n u^{(\pi)}_n(\mathcal{A})+  \nonumber \\ 
& w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{n,(\pi)}_j(\mathcal{A}) +  w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{j,(\pi)}_n(\mathcal{A})  \bigg)\bigg) \nonumber \\
&=\frac{1}{|\mathcal{N}|!}\sum_{\pi \in \prod}\bigg(w_nu^{(\pi)}_n(\mathcal{A})+ w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{n,(\pi)}_j(\mathcal{A}) +w'_{n}\sum_{j \in \{{O_{\pi, \pi(n)}} \}, j \neq n} u^{j,(\pi)}_n(\mathcal{A}) \bigg) 
\end{align}
where Equation~\eqref{eq:ourshapleyconvex} provides the Shapley value for our convex game. It is evident that our Shapley value depends on the utility of the player $n$, the utility  player $n$ achieves by allocating resources to players in $j \in O_{\pi, \pi(n)}, j \neq n $ and the utility player $j \neq n, j \in O_{\pi, \pi(n)}$ achieves by allocating resources to player $n$  in every possible permutation. 

\begin{comment}
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $tt$ 
		\State \textbf{Output}: The optimal hit probabilities
		\State \textbf{Step $1$:}  $t \leftarrow$0, $\boldsymbol{\lambda^{(t)}\leftarrow\lambda_0}$, $\boldsymbol{\mu^{(t)}\leftarrow\mu_0}$
		\While{Equation \eqref{eq:gradient1} $\neq$ 0}%$\partial L(\boldsymbol{h,\lambda,\mu})/\partial \lambda_{l} \neq0$ $\&\& $ $\partial L(\boldsymbol{h,\lambda,\mu})/\partial \mu_{ip} \neq0$}
		\State \textbf{Step $2$}:$\boldsymbol{h_{il}^{(p)}[t]} \leftarrow \frac{w_i\beta^{|p|-l}}{\lambda_{l}[t-1]\Bigg(\prod_{\substack{q \neq p,\\ q:l\in\{1,\cdots,|q|\}}}(1-h_{il}^{(q)}[t-1])\Bigg)+\mu_{ip}[t-1]}. $ %Algorithm 2($\boldsymbol{\lambda^{(t)},\mu^{(t)}}$) %\Comment{The node id and file content to Algorithm \ref{algo:alg1} for calculating the price function using~(\ref{eq:gradient2}) }
		\State \textbf{Step $3$:} Update $\lambda$ and $\mu$ using  \eqref{eq:update},  t $\leftarrow t+1$
		%	\State \textbf{Step $4$}: $\boldsymbol \tau_{\chi} \longleftarrow \text{Convex}(\text{slave},\boldsymbol u_{\chi})$ \Comment{Solve the slave optimization problem for $\boldsymbol \tau_{\chi}$  }
		%	\State \textbf{Step $5$}: $(\boldsymbol b_{\chi}, \boldsymbol{\delta_{\chi}}, \text{obj}_{\chi})  \longleftarrow \text{Rounding}(\boldsymbol u_{\chi},\boldsymbol \tau_{\chi})$ \Comment{Round the values of $\boldsymbol u_{\chi}$, remap $\boldsymbol u_{\chi}, \boldsymbol \tau_{\chi}$ to $\boldsymbol{b}_{\chi}$ and $ \boldsymbol{\delta}_{\chi}$ and obtain the new objective function value  }
		\EndWhile
	\end{algorithmic}
	\caption{Iterative Distributed Algorithm}
	\label{algo:alg}
\end{algorithm}
\end{comment}
\begin{remark}\label{rem:shap}
	Shapley value calculation for our convex game requires solving at least $2^{N}-1$ optimization problems
\end{remark}
Algorithm \ref{algo:alg1} provides an overview of our proposed approach. We obtain $R, C$ and the utility of all players as $\mathbf{u}$. We initialize each player's utility value ($\mathbf{u}(R,\mathcal{X})$), Shapley value ($\boldsymbol{\phi} $) and resource allocation decision $\mathcal{X}$ to $0$. Then we calculate the Shapley value for the players and assign it to $\mathbf{u}(R,\mathcal{X})$. Finally to obtain $\mathcal{X}$, we take the inverse function of $\mathbf{u}$. As we are using monotone utilities, we know that the inverse of the utilities exist.
\par A fundamental issue with Shapley value is its complexity. As mentioned in Remark \ref{rem:shap}, Shapley value calculation requires solving a  large number of optimization problems that is not suitable for a game with larger number of players. Therefore, reducing the complexity of obtaining an allocation from the core is always favorable. 
\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0, $ \boldsymbol{\phi} \leftarrow$0,  
		\State \textbf{Step $1$:}  Calculate Shapley Value $\phi_n$ using Equation \eqref{eq:shapleyconvex} $\forall n \in \mathcal{N}$
	    \State \textbf{Step $2$:} $ \mathbf{u}(R,\mathcal{X}) \leftarrow \boldsymbol{\phi}$
	    \State \textbf{Step $3$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
		\end{algorithmic}
	\caption{Shapley Value based Resource Allocation}
	\label{algo:alg1}
\end{algorithm}
%It is worth mentioning here that the Shapley value will only provide us the utility each player is going to receive that lies in the core (as a result of cooperation). The allocation decision can be obtained by taking the inverse of utilities.  \par 
\subsection{Reducing the Computational Complexity}
%As mentioned earlier, that the calculation of Shapley value for our convex game requires at solving at least $2^{N}-1$ optimization problems that is computationally expensive. 
To reduce the complexity, we propose a computationally efficient approach in Algorithm 2 that requires solving $2N$ optimization problems i.e. $\mathcal{O}(N)$.  The input into the algorithm consists of available resources/capacities, user requirements and the utilities of all game players. The output of the algorithm is $\mathcal{X}$. In Step 1, the utility values of the players, the allocation decision,  and two vectors $\boldsymbol{O_1}$ and $\boldsymbol{O_2}$. In Step 2, every player's utility is calculated without any resource sharing i.e. single optimization and the values are stored in the vector $\boldsymbol{O_1}$. Then $C, R$ are updated and we move to Step 4, where we calculated the utilities $u_j^n$'s for all the players with updated $C, R$ and store them in $\boldsymbol{O_2}$. 

\begin{algorithm}
	\begin{algorithmic}[]
		\State \textbf{Input}: $R, C,$ and vector of utility functions of all players $\mathbf{u}$ 
		\State \textbf{Output}: $\mathcal{X}$
		\State \textbf{Step $1$:}  $ \mathbf{u}(R,\mathcal{X}) \leftarrow$0,  $ \mathcal{X} \leftarrow$0,   $ \boldsymbol{O_1} \leftarrow$0, $ \boldsymbol{O_2} \leftarrow$0, 
		\State \textbf{Step $2$:}
		 \For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_1^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single}}
		\EndFor
		\State \textbf{Step $3$:} Update $R, C$ based on Step 2
		\State \textbf{Step $4$:}
		\For{\texttt{$n \in \mathcal{N}$}}
		\State $ {O_2^n} \leftarrow$ \texttt{Solution of the optimization problem in Equation \eqref{eq:opt_single_j} with updated C and R}
		\State Update C and R
		\EndFor
		\State \textbf{Step $5$:} $u_n(R,\mathcal{X})\leftarrow O_1^n+O_2^n$ $\forall n \in \mathcal{N}$ 
		\State \textbf{Step $6$:} $\mathcal{X}\leftarrow \mathbf{u}^{-1}$
	\end{algorithmic}
	\caption{$\mathcal{O}$($N$) algorithm for obtaining Core's allocation}
	\label{algo:alg2}
\end{algorithm}
\begin{subequations}\label{eq:opt_single_j}
	\begin{align}
	\max_{\mathcal{X}}\quad& \sum_{j\neq n}u_j^n(\mathcal{X}) \quad  \forall n \in \mathcal{N} \label{eq:objsinglej}\\
	\text{s.t.}\quad & \sum_{i} x_{ik}^{(n)}\leq C_{k}^{(n)} \quad \forall k \in \mathcal{K}, \quad \forall i \in \mathcal{M}\backslash\mathcal{M}_n, \label{eq:singlefirstj} \displaybreak[0]\\
	& x_{ik}^{(n)} \leq R^{(n)}_{ik} \quad \forall\; i\in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlesecondj} \displaybreak[1]\\
	&  x_{ik}^{(n)} \geq 0 \quad \forall\; i\in \mathcal{M}\backslash\mathcal{M}_n, k \in \mathcal{K}, \label{eq:singlethirdj} \displaybreak[2]
	\end{align}
\end{subequations}
\begin{theorem}
	The solution obtained from Algorithm \ref{algo:alg2} lies in the \emph{core}
\end{theorem}
\begin{proof}
	To prove the theorem, we need to show that the utilities obtained in Step $5$ of Algorithm \ref{algo:alg2}; a) are individually rational; b) are group rational and c) no players  have the incentive to leave the grand coalition and form another another coalition $S \subset \mathcal{N}$. 
	\paragraph{Individual Rationality} For each player $n \in \mathcal{N}$, the solution $O_1^n$ obtained by solving the optimization problem in Equation \eqref{eq:opt_single} is the utility a player will obtain by working alone i.e. it is $v\{n\}$. The value $O_2^n$ in Step 4 is either zero or positive but cannot be negative due to the nature of utility used i.e. 
	\begin{align}
	u_n(R,\mathcal{X})&=O_1^n+O_2^n \quad \forall n \in \mathcal{N} \nonumber \\
	u_n(R,\mathcal{X})&\geq O_1^n \quad \forall n \in \mathcal{N}\nonumber 
	\end{align}
	
	
	Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is individually rational.
	\paragraph{Group Rationality} The value of the grand coalition $v\{\mathcal{N}\}$ as per Equation \eqref{eq:payoff_function} is the sum of utilities $u_n$'s and $u_j^n$'s. Steps 2, 4 and 5 of Algorithm \ref{algo:alg2} obtain the sum of the utilities as well. Hence the solution obtained as a result of Algorithm \ref{algo:alg2} is group rational rational. 
	\par Furthermore, due to super-additivity of the game and monotonic non-decreasing nature of the utilities, no players have the incentive to form a smaller coalition. Hence Algorithm \ref{algo:alg2} provides a solution from the core.  
\end{proof}

==> proof1.tex <==
\begin{proof}
	We show that the price function obtained by $\frac{\partial \mathcal{L}(\mathbf{X}, \boldsymbol{\alpha}, \boldsymbol{\beta},\boldsymbol{\zeta,\gamma})}{\partial x_{n,k}^{j}}=0$ is continuous at one or more of the optimal Lagrange multipliers for \eqref{eq:lagrangian}. 
	
	Let both $u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j,\zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j})$ and $f_n^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Lambda_{n,k}^{l})$ are  %and $u_{jn}^{'-1}(\alpha_k^{(n)}, \beta_{ik},\zeta^{n},\gamma_{ik}^{(n)},\Lambda_{ik}^{(n)})$ are
	the inverses of the first derivative of $u_{n}^j$ and $(u_{n}^l(x_{n,k}^l)-C_n^l(x_{n,k}^l))$, respectively. %and $u_j^n$ respectively. 
	$\alpha_{n,k}$,  $\beta_{k}^j$, $\zeta_{n}$, and $\gamma_{n,k}^{j}$ are the \emph{Lagrange} multipliers whereas   $\Delta_{n,k}^{j}=\bigg(\sum_{j \in \mathcal{M}_n}u_n^j(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j+{x}_{n,k}^j)+ \big(\sum_{l \in \{\mathcal{M}\backslash \mathcal{M}_n\}} u_n^l(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^l+{x}_{n,k}^l)-C_n^l(\mathbf{x}_n^l)\big)-d_n^0\bigg)$. There are two different cases that we evaluate in the following: %To simplify the proof, we only consider the case  in which $i \in \mathcal{M}_n$ below. The proof for the case when $i \in \mathcal{M}\backslash\mathcal{M}_n$ is similar. 
	\begin{enumerate}
	\item \textbf{$j \in \mathcal{M}_n$:}$\frac{\partial \mathcal{L}}{\partial x_{n,k}^{j}}=0$
	\begin{align}
	\label{eq:gradLagObj22}
%	\frac{u_n^{'j}(\mathbf{x}_n^j+\sum_{t\in \mathcal{{N}}\backslash n}\mathbf{x}_t^j)+\sum_{t \in \mathcal{{N}}\backslash n}}{\Delta_{n,k}^j}, \nonumber \\
	%	 \Big(u_n^{'j}(x_{n,k}^{j})+\frac{1}{r_{k}^j}\Big)(1+\Lambda_{n,k}^{j}\zeta_{n})-\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j-\nonumber \\
	%	 \gamma_{n,k}^{j})=0,\nonumber \\
	&u_n^{'j}(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j+x_{n,k}^{j})(1+\Delta_{n,k}^{j}\zeta_{n})-\Delta_{n,k}^{j}(\alpha_{n,k}+\nonumber \\
	&\beta_{k}^j-\gamma_{n,k}^{j})=0,\nonumber \\	
	%	 \implies u_n^{'j}(x_{n,k}^{j})=\frac{\Lambda_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Lambda_{n,k}^{j}\zeta_{n}}-\frac{1}{r_{k}^j}, \nonumber \\
	& u_n^{'j}(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j+x_{n,k}^{j})=\frac{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n,k}^{j}\zeta_{n}}, \nonumber \\
	%& \nonumber \\
	%	\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Lambda_{n,k}^{j},r_{k}^j).
%	&\implies \quad x_{n,k}^{*j}= u_n^{'-j}(\alpha_{n,k}, \beta_{k}^j, \zeta_{n},\gamma_{n,k}^{j},\Delta_{n,k}^{j}).
	\end{align}
For sake of the proof, we set  $u_j^n=1-e^{-(x_{n,k}^j+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j+-r_{n,k}^j+\delta t)}$ where $\bar{r}_{n,k}^j=r_{n,k}^j+\delta t$. However, the theory hold for any concave injective utility function for which the inverse of the first derivative exists.  Then \eqref{eq:gradLagObj22} becomes:
	\begin{align}\label{eq:proof1}
	& e^{-(x_{n,k}^j+\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}= \frac{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})}{1+\Delta_{n,k}^{j}\zeta_{n}},\hspace{0.2in} \nonumber \\
		e^{x_{n,k}^j}&= \frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}},\nonumber \\
		x_{n,k}^j&=\ln\bigg(\frac{1+\Delta_{n,k}^{j}\zeta_{n}}{\Delta_{n,k}^{j}(\alpha_{n,k}+\beta_{k}^j- \gamma_{n,k}^{j})	e^{\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}}\bigg).
	\end{align} 
%We know that $\Lambda_{ik}^{(n)>0$, 
	 For continuity, we need both the numerator and denominator inside the $\ln(\boldsymbol{.})$ function of \eqref{eq:proof1} to be positive.  
At the optimal point, the numerator $(1+\Delta_{n,k}^{*j}\zeta^*_{n})$ is positive as $\Delta_{n,k}^{*j}>0$ (from Section \ref{sec:assumption}) and $\zeta^*_{n}=0$ (from complementary slackness).	Similarly, in the denominator, $\Delta_{n,k}^j$ (from Section \ref{sec:assumption}) and $e^{(\sum_{m \in \mathcal{N}\backslash n}{x}_{m,k}^j-\bar{r}_{n,k}^j)}$ are positive. $(\alpha^*_{n,k}+\beta_{k}^{*j}-\gamma_{n,k}^{*j})>0$, as  $\alpha_{n,k}^{*}>0$ (from Lemma \ref{lem:constraintsactive}) and  $\alpha_{n,k}^{*}+\beta_{k}^{*j}> \gamma_{n,k}^{*j}$ (from \emph{sensitivity analysis} \cite{boyd2004convex}). %Furthermore, the denominator $(r_k^j\Lambda_{n,k}^{j}(\alpha_{n,k}^*+\beta_{k}^{*j}- \gamma_{n,k}^{*j})-1>0)$ based on our assumptions in Section \ref{sec:assumption}.
Hence, the price based function in \eqref{eq:proof1} is continuous in at least one optimal Lagrange multiplier vector. The proof follows from Theorem \ref{thm:georgesufficient}. 
	
	
	%	Where the last step follows from the fact that  utility function used is $1-1$, so its derivative is also $1-1$ and its inverse $U_n^{'-1}(\alpha_k, \beta_{ik})$ can easily be computed.
	\item \textbf{$l \in \{\mathcal{M}\backslash\mathcal{M}_n\}$:} $\frac{\partial \mathcal{L}}{\partial x_{n,k}^{l}}=0$
	\begin{align}
	\label{eq:gradLagObjcase22}
	f^{'l}_n(x_{n,k}^{l})(1+\Delta_{n,k}^{l}\zeta_{n})-\Delta_{n,k}^{l}(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})=0,\nonumber \\ 
	\implies  f^{'l}_n(x_{n,k}^{l})=\frac{(\alpha_{n,k}+\beta_{k}^l-\gamma_{n,k}^{l})}{1+\Delta_{n,k}^{l}\zeta_{n}}, \nonumber \\
	%& \nonumber \\
	\implies \quad x_{n,k}^{*l}= f_{n}^{'-l}(\alpha_{n,k}, \beta_{k}^l,\zeta_{n},\gamma_{n,k}^{l},\Delta_{n,k}^{l}).
	\end{align}
\end{enumerate}


\end{proof}
